Temporal Reasoning Through Automatic Translation of tock-CSP into Timed Automata

In this work, we consider translating tock-CSP into Timed Automata for UPPAAL to facilitate using UPPAAL in reasoning about temporal specifications of tock-CSP models. The process algebra tock-CSP provides textual notations for modelling discrete-time behaviours, with the support of tools for automatic verification. Similarly, automatic verification of Timed Automata (TA) with a graphical notation is supported by the UPPAAL real-time verification toolbox \uppaal. The two modelling approaches, TA and tock-CSP, differ in both modelling and verification approaches, temporal logic and refinement, respectively, as well as their provided facilities for automatic verification. For instance, liveness requirements are difficult to specify with the constructs of tock-CSP, but they are easy to specify and verify in UPPAAL. To take advantage of temporal logic, we translate tock-CSP into TA for \uppaal; we have developed a translation technique and its supporting tool. We provide rules for translating tock-CSP into a network of small TAs for capturing the compositional structure of tock-CSP that is not available in TA. For validation, we start with an experimental approach based on finite approximations to trace sets. Then, we explore mathematical proof to establish the correctness of the rules for covering infinite traces.

==> EgGenPar/EgGen.tex <==

\begin{example} %{A translation of an Automatic Door System (ADS)} \\
\label{ads}
This example illustrates a translation of an Automatic Door System (ADS) that opens a door, and then after at least one-time unit, the system closes the door in synchronisation with a lighting controller, which turns-off the light after closing the door.  A tock-CSP specification of the system is as follows.


% A \verb|tock-CSP| process for modelling ADS is: \\
% \vspace{0.3cm}
%Consider a  model of ADS as \verb!tock-CSP! process:\\

\begin{lstlisting}
Controller = open -> tock -> close -> Controller

Lighting = close -> offLight -> Lighting

ADS = Controller [|{close}|] Lighting

\end{lstlisting}

% \verb!(open -> tock -> close -> SKIP)[|{close}|](close -> offLight -> SKIP)!
 
% \[ADS = (open -> tock -> close -> SKIP) [|{close}|] (close -> offLight -> SKIP) \]

\end{example}



ADS system has two components. A controller \verb!Controller! that opens and closes the system after one unit time. In \verb!tock-CSP! the process \verb!SKIP! indicates a termination of a process using the event \verb!tick!. The lighting controller \lstinline{Lighting} turns-off the light after closing the door. The two components synchronise on the event \lstinline{close}, which enables the lighting controller to turns-off the light. 



%Translation moved to overview
% % \vspace{0.3cm}

%  \begin{figure} %[H]
% \subfigure{\includegraphics [width=0.7\textwidth, height=0.3\textwidth]{EgGenParGray/taGenPar0_0.png}}
% \subfigure{\includegraphics [width=0.27\textwidth]{EgGenParGray/taPrefix00_1.png}}
% \subfigure{\includegraphics [width=0.3\textwidth]{EgGenParGray/taPrefix00_2.png}}
% \subfigure{\includegraphics [width=0.5\textwidth]{EgGenParGray/taPrefix00_3.png}}
% \subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/SyncTA.png}}
% \subfigure{\includegraphics [width=0.5\textwidth]{EgGenParGray/taPrefix01_2.png}}
% \subfigure{\includegraphics [width=0.3\textwidth]{EgGenParGray/taWait_n00_4.png}} 
% %   \hspace{-0.02\textwidth}
% \subfigure{\includegraphics [width=0.35\textwidth]{EgGenParGray/taPrefix01_3.png}}
% \hspace{0.3\textwidth}
% \subfigure{\includegraphics [width=0.3\textwidth]{EgGenParGray/taWait_n01_4.png}}
% \subfigure{\includegraphics [width=0.7\textwidth]{EgGenParGray/Env.png}}
% \caption{A list of TA for the translation of the process ADS}
% \label{ta_env}

% \end{figure}





% A translation of the process ADS produces a list of TA in Figure \ref{ta_env}. Details of the translated TA are as follows. Starting from the top-left corner, the first TA captures the translation of concurrency that starts the two processes \lstinline{Controller} and \lstinline{Lighting} concurrently in two possible orders, either \lstinline{Controller} then \lstinline{Lighting} or vice versa, and then also waits on state \lstinline{s5} for their termination actions in the two possible orders, either \lstinline{Controller} then \lstinline{Lighting} or vice versa, and then the whole system terminates with the action \lstinline{finishID0}.

% The second, third and fourth TA capture the translation of the process \lstinline{Controller}. The second TA captures the occurrence of the event \verb!open!. The third TA captures the occurrence of the events \verb!tock?! (with question mark) because the environment controls the progress of time because all processes synchronise with time.  The fourth TA captures the occurrence of the event \verb!close!, which needs to synchronise with a synchronisation controller, that is the fifth TA in the list of the TA.


% The sixth TA captures the event \verb!close! for the process  \lstinline{Lighting}, which also needs to synchronise with the synchronisation controller on the event \verb!close!. The seventh and ninth TA captures the occurrence of the events \verb!tick! for the termination of both \lstinline{Controller} then \lstinline{Lighting} processes, respectively. The eighth TA captures the event \verb!offLight!. Finally, the last TA is an environment TA that provides co-actions for all the translated events. Also, the environment TA serves the purpose of "closing" the overall system (in contrast to having an "open system") as required for the model checker.




==> all.tex <==





\section{Introduction}   %%%-----------------------------------------------------

Communicating Sequential Processes (CSP) is an established process algebra that provides a formal notation for both modelling and verification of concurrent systems \cite{R10, S10, H78}. The use of CSP for verification has been supported by several tools including powerful model-checkers \cite{TP14, R10, SL09}. 
% CSP and its modelling approaches have contributed to understanding the complexity of concurrent systems  \cite{S10}. 


%tockCSP------------------------------------------------------------------

Interest in using CSP has motivated the introduction of support for modelling \emph{discrete} time; \tockCSP{} provides an additional event $tock$ to record the progress of time. This enables using CSP for modelling time in discrete format suitable for formal verification. The notation of \tockCSP{} retains that of CSP, thus, automatic verification is supported by the existing tools of CSP. As a result, \tockCSP{} has been used in verifying real-time systems, such as security protocols \cite{NS00} and railways systems \cite{YF12}. Recently, \tockCSP{} has been used for capturing the semantics of RoboChart, a domain-specific language for modelling robotics applications \cite{MR16}. 

% Additionally, a recent extension of \tockCSP{} provides notations for specifying budgets and deadlines for effective modelling and verification of temporal specifications \cite{JP19}.



In this work, we introduce a technique for translating \tockCSP{} into TA that enables using \uppaal \cite{BD06} in verifying \tockCSP{} models. \uppaal \ is a tool-suite that allows the modelling of hybrid systems using a network of TAs and verifying the systems against temporal logic formulae.

%\uppaal is a tool-suite for modelling and verifying systems using TA and temporal logic. 

Both temporal logic and refinement are powerful approaches for model checking \cite{G08}.  The refinement approach models both the system and its specifications with the same notation \cite{R10, S10}, while the temporal logic enables asking whether a system captures the logical formula of the specification ($system \models formula$) \cite{CE86}. 

% Using both temporal logic and refinement have been supported with automatic verification tools, such as \uppaal \cite{BD06} and FDR \cite{TP14}, respectively.


Previously, Lowe has investigated the relationship between the refinement approach (in CSP) and the temporal logic approach \cite{G08}. The result shows that, in expressing temporal logic checks using refinement, it is necessary to use the infinite refusal testing model of CSP. The work highlights that capturing the expressive power of temporal logic in specifying the availability of an event (liveness specification) is not possible in the refinement model. Due to the difficulty of capturing refusal testing, automatic support becomes problematic. A previous old version of FDR supports refusal testing, but not its recent efficient version \cite{TP14}.

% . A desirable specification that ensures that a system performs something good.
% or something bad will never happen in the system. 


Additionally, Lowe's work \cite{G08} proves simple refinement checks cannot cope with three operators: $eventually$  ($\diamond p$: $p$ \textit{will hold in some subsequent state}),  $until$ ($p  \mathcal{U} q$: \textit{$p$ holds in every state until $q$ hold})  and $negation$  ($\neg ( \diamond p$): $p$ \textit{will never hold in the subsequent states}). These three operators express behaviour captured by infinite traces. Our translation work presented here will facilitate using the resources of temporal logic (and \uppaal) in checking specifications that are difficult to specify in \tockCSP{} models, as shown in Example \ref{ads}.  

% This will include liveness specifications, in addition to the three operators that cannot be specified in refinement models: eventually $(\diamond)$,  $ until (\mathcal{U}$) and  $negation (\neg) $, as illustrated in Example \ref{ads}.



\begin{example} %{A translation of an Automatic Door System (ADS)} \\
\label{ads}
An Automatic Door System (ADS) opens a door, and after at least one-time unit, closes the door in synchronisation with a lighting controller, which turns off the light. In \tockCSP{}, its description is as follows.


\begin{lstlisting}
       ADS = Controller [|{close}|] Lighting
Controller = open -> tock -> close -> Controller
  Lighting = close -> offLight -> Lighting
\end{lstlisting}

\end{example}

% \begin{lstlisting}
% Controller = open -> tock -> close -> Controller
% Lighting = open -> onLight -> close -> offLight -> Lighting
% ADS = Controller [|{open, close}|] Lighting
% \end{lstlisting}


% \begin{lstlisting}
% Controller = open -> tock -> close -> Controller
% Lighting = close -> offLight -> Lighting
% ADS = Controller [|{close}|] Lighting
% \end{lstlisting}



\hspace{-0.7cm}
The model ADS have two components, \lstinline{Controller} and \lstinline{Lighting}, which synchronise on the event \lstinline{close}; this enables \lstinline{Lighting} to turn off the light after closing the door. For instance, in  \tockCSP{}, there is no direct way of checking if the system eventually turns off the light when the environment is ready. However, temporal logic provides a direct construct for specifying liveness requirements. For example, in \uppaal, the requirement is specified as follow.

% \item \lstinline{A<> TA.offLight}  \\ 
    
\vspace{-0.25cm}
\begin{itemize}
    \item \lstinline{A<> offLight}  \\ 
        -- \textit{The system eventually turns off the light
        % \footnote{if the operating environment facilitates turning off the light.} 
        }
        
    % \item \lstinline{open --> onLight} \\
    %   - -  \textit{Door open until light on}
    % % - - \textit{Can the system always turns-off the light, if the environment permits.}
\end{itemize}

\noindent
\uppaal{} uses a subset of Timed Computational Tree Logic (TCTL) based on the notions of path and state \cite{BD06}.  A path formula describes a trace or path, whereas a state formula describes either a location or logical expression. There are five different forms of path formulae, categorised into three: liveness, reachability and safety. Liveness as either \lstinline{A<>q} \textit{(q is eventually satisfied)} or \lstinline{p --> q} \textit{(a state satisfying p leads to a state satisfying q)} \footnote{In the literature, $\diamond$ or $F$ are the commonly used symbols for expressing liveness.}.  The reachability formula is in the form of \lstinline{E<>q} \textit{(a state satisfying $q$ is reachable from the initial state)}. Safety is in the form of either \lstinline{A[]q}  \textit{(q holds in all reachable states)} or \lstinline{E[]q} \textit{(a path where q holds in all states on the path)}.






In verifying the correctness of the translation technique, we follow a series of steps.  First, we construct a systematic list of interesting \tockCSP{}  processes, which pair all the constructs of \tockCSP{} within the scope of this translation work. Second, we use the developed translation technique and its tool to translate the formulated processes into TA for \uppaal.  Third, we use another tool we developed in generating and comparing finite traces of the input \tockCSP{} models and the traces of the translated TA models, with the support of both FDR and \uppaal, respectively. This provides good evidence that the translated TA captures the behaviour of the input \tockCSP{} models.


To precisely describe the translation technique, we use Haskell \cite{H16}, a functional programming language, for expressing, implementing and evaluating the translation technique. The expressive power of Haskell help in providing formal descriptions of the translation technique as a list of translation rules, also suitable for a mathematical proof.


% To describe the translation technique is one of the challenging tasks we faced in this work,
% So, we take advantage of the concise construct of Haskell \cite{H16} in describing the technical part of the work. Haskell is a functional programming language, which we use for expressing, implementing and evaluating the translation technique. Both concise and expressive power of Haskell helps us in providing a precise description of the translation technique as a list of translation rules.




% Outline of the paper  ----------------------------------------------------------------------
The structure of the paper is as follows. Next, Section \ref{background} provides the backgrounds essential for understanding the translation technique.  In Section \ref{trans_rule}, we summarise the translation technique. We discuss an evaluation of the translation technique in Section \ref{evaluation}. In Section \ref{related_work}, we highlight relevant related works and also present a brief comparison with this work. Finally, in Section \ref{conclusion}, we highlight future work and also provide a conclusion for the paper.




%%  --------------------  BACKGROUND -----------------------
\section{Background}
\label{background}

This section discusses the required background for understanding the translation work. We begin by discussing the notations of \tockCSP{} and then discuss the target of the translation work, a network of suitable TA for \uppaal. 


%CSP and \verb!tock-CSP!
% \subsubsection{tock-CSP} 
% \noindent

An extension of CSP is \tockCSP{} that provides notations for modelling processes and their interactions, such as the basic processes: \lstinline{SKIP} and \lstinline{STOP}, for successful termination and deadlock, respectively. Also, there are operators such as \lstinline{prefix (->)} for describing an event that leads to a process. For example, the process \lstinline{move->SKIP} is a behaviour that moves and then terminates. 


% Furthermore, there are additional binary operators such as sequential composition (;), which combines two processes serially. For instance, \verb!P3 = P1;P2! behaves as process \verb!P1!, and then after successful termination of  \verb!P1!, \verb!P3! behaves as \verb!P2!.  For example, the process \verb!Ps = (move->SKIP);(turn->SKIP)!, specifies a system that moves, turns and then terminates, successfully.


There are binary operators such as sequential composition (;), which combines two processes serially. For instance, the process \texttt{P3 = P1;P2} behaves as process \texttt{P1}, and after successful termination of  \texttt{P1}, then \texttt{P3} behaves as \texttt{P2}. There are other binary operators for composing processes in different ways, such as concurrency, choice and interruption. Also, CSP has a special event $tau \ ( \tau ) $ for invisible actions that are internal to a system, specifically for internal communications, hidden from the operating environment. The collection of these operators provides a rich set of constructs for modelling untimed systems  \cite{R10, S10}. 
% , as detailed in . Comprehensive full details of CSP constructs, together with examples, are available in these books \cite{R10, S10}. 


% Toremove
For modelling time, \tockCSP{} has an event \verb!tock! \cite{R10} for modelling the progress of time. Each event \verb!tock! specifies a single unit of time. For example, the following process \texttt{Pt} specifies behaviour that \lstinline{moves}, after at least two time units, \lstinline{turns} and terminates.
\vspace{-0.3cm}
\[\texttt{Pt = move->tock->tock->turn->SKIP} \]  

% The addition of the special event \verb!tock! enables specifying temporal specification in a format that is suitable for formal analysis of timed system \cite{TP14}. 




% ToReturn
% Consequently, \tockCSP{} enriches the notations with adding a special event \verb!tock!, which records the progress of time \cite{R10}. Each event \verb!tock! specifies a single unit of time. For example,  a process \verb!Pt= move->tock->tock->turn->SKIP! specifies the behaviour of a system that moves, and then after at least two-time units, the system turns and then terminates. The addition of the special event \verb!tock! enables specifying temporal specification in a format that is suitable for formal analysis of timed system \cite{TP14}. 


%ToReturn
% In this work, we provide a translation technique that facilitates using the expressive power of temporal logic in verifying temporal specifications of real-time systems.  

For this work, we provide a BNF for the notation of \tockCSP{} we consider in developing this translation technique and its supporting tool. Part of the BNF is presented in Definition \ref{dfn_CSPproc} in Haskell. The complete BNF is available in an extended report \cite{extendedVersion}. 

% ToReturn with the previous paragraph
% The BNF forms the basic foundation of this translation work, and provides a good link for other related works and tools that are associated with \verb!tock-CSP!.

\begin{definition} \textbf{Data definition of \lstinline{CSPproc}} 
\label{dfn_CSPproc}


\begin{verbatim}
data CSPproc =   STOP | SKIP | Prefix Event CSPproc 
                | Seq CSPproc CSPproc 
                | GenPar CSPproc CSPproc [Event] 
                | Interleave CSPproc CSPproc 
                | ...
\end{verbatim}
\end{definition}

\noindent
For illustration, this part  of the BNF shows the constructs for \lstinline{STOP} (Deadlock), SKIP (successful termination), \lstinline{Prefix} (prefixing), \lstinline{Seq} (Sequential composition), and \lstinline{GenPar} (generalised parallel for concurrency) and \lstinline{Interleave} for describing processes that run concurrently without synchronisation. 


\subsubsection{Timed Automata for \uppaal} is graphical notations for modelling hybrid systems as a network of TA. Mathematically, TA is defined as a tuple $(L, l_0, C, A, E, I)$, where $L$ is a set of locations such that $l_0$  is the initial location, $C$ is a set of clocks, $A$ is a set of actions, $E$ is a set of edges that connects the locations $L$, and $I$ is an invariant associated to a location $l \in L$ in the form of $I:L \longrightarrow B(C)$. So, an edge $E$ is defined as $E \subseteq (L \times A \times B(C) \times 2^C \times L)$, which describes an edge from location $l \in L$ that is triggered by an action $a \in A$, guarded with a guard $B(C)$, and associated clock $C$  that is reset on following an edge $e \in E$ to a location $l \in L$ \cite{BD06, B11}. 

% Lastly, $I$ is a function that assigns an invariant to a location $I:L \longrightarrow B(C)$   \cite{BD06, B11}.


A system is modelled as a network of TAs that communicate over channel synchronisations or shared variables. A sending channel is decorated with an exclamation mark $(c!)$ while the corresponding receiving channel is decorated with a question mark $c?$. In describing a behaviour, a TA performs an action $c!$ to communicate with another TA that performs the corresponding co-action $c?$. There is also a broadcast channel for communication among multiple TAs, in the form of one-to-many communications (one sender with multiple receivers). 


% The TAs communicate over either a channel or a shared variable. A sending channel is decorated with an exclamation mark $(c!)$ while the corresponding receiving channel is decorated with a question mark $c?$. In describing a behaviour, a TA performs an action $c!$ to communicate with another TA that performs the corresponding co-action $c?$. There is also broadcast channel for communication among multiple TAs, in the form of one-to-many communication (one sender with multiple receivers). 

For expressing urgency, there are urgent channels and urgent location that do not allow delay. In addition, there is also a committed location; an urgent location that must participate in the next transition before any other transition. This committed location is useful in expressing atomicity, a compound action spanning multiple transitions that must be executed as a unit. Also, there are invariants for both specifying precise delay and enforcing progress \cite{BD06}. 



% For instance, a single broadcast channel $b!$ synchronises with multiple receiving channels $b?$.



%Env TA
Overall, \uppaal \ provides graphical notations for modelling a system as a network of TAs that model system's components that communicate with one another and the explicit operating environment. For example, the collection of TAs in Figure \ref{ta_ads} describes a system and its operating environment, which is explained in details in Section \ref{trans_rule}. Also, in specifying requirements, \uppaal \ has a subset of TCTL \cite{B09}  for specifying system properties that are verified automatically  \cite{LP07, LP97, BD06}.  


\section{An Overview of the Translation Technique}
\label{trans_rule}

Our translation technique takes an input \tockCSP{} model and produces a list of network TAs suitable for automatic verification in \uppaal{}. The occurrence of each \tockCSP{} event is captured in a small TA with an UPPALL's action,  which records an occurrence of the translated event, and the small TAs are composed into a network of TA that capture the behaviour of the input \tockCSP{} model.

% The action has the same name as the translated event. The technique composes these small TAs into a network of TA, which captures the behaviour of the input \tockCSP{} model. 


% Our translation technique produces a list of small TAs. The occurrence of each \tockCSP{} event is captured in a small TA with an UPPALL's action,  which records an occurrence of the translated event. The action has the same name as the translated event. The technique composes these small TAs into a network of TA, which captures the behaviour of the input \tockCSP{} model. 



%  \begin{figure}
 
%   \begin{subfigure}{\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=\linewidth, height=0.3\linewidth]{newEg/taGenPar0_0.png}
%   \caption{TA01}
% \end{subfigure}
%  \begin{subfigure}{.5\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=.8\linewidth, height=0.5\linewidth]{newEg/taPrefix00_1.png} 
%   \caption{TA02}
% \end{subfigure}
% \begin{subfigure}{.5\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=.8\linewidth, height=0.5\linewidth]{newEg/taPrefix00_2.png} 
%   \caption{TA03}
% \end{subfigure}

% \newline

% \begin{subfigure}{.6\textwidth}
%   \centering
%   % include third image
%   \includegraphics[width=\linewidth]{newEg/taPrefix00_3.png}
%   \caption{TA04}
% \end{subfigure}
% \begin{subfigure}{.4\textwidth}
%   \centering
%   % include fourth image
%   \includegraphics[width=.8\linewidth]{newEg/SyncTA.png}  
%   \caption{TA05}
% \end{subfigure}



% \newline

% \begin{subfigure}{.6\textwidth}
%   \centering
%   % include third image
%   \includegraphics[width=\linewidth]{newEg/taPrefix01_2.png} 
%   \caption{TA06}
% \end{subfigure}
% \begin{subfigure}{.4\textwidth}
%   \centering
%   % include fourth image
%   \includegraphics[width=.9\linewidth]{newEg/taPrefix01_3.png} 
%   \caption{TA07}
% \end{subfigure}

% \newline


% \begin{subfigure}{\textwidth}
%   \centering
%   \includegraphics[width=\linewidth, height=0.3\linewidth]{newEg/Env.png} 
%   \caption{TA08}
% \end{subfigure}

% \caption{A list of networked TA for the translation of the process ADS.}
% \label{ta_ads} 
% \end{figure}









%----------------------------------------- OLD
 \begin{figure} %[H]
\centering
\includegraphics [width=0.9\textwidth, height=0.4\textwidth]{EgGenParGray/taGenPar0_0.png}  \\
(a) TA00
 
\begin{tabular}{c c}
\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix00_1.png} &
\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix00_2.png} \\
 (b) TA01 &  (c) TA02 \\

\includegraphics [width=0.55\textwidth]{EgGenParGray/taPrefix00_3.png} &
\includegraphics [width=0.4\textwidth]{EgGenParGray/SyncTA.png} \\
(d) TA03 & (e) TA04 \\
\includegraphics [width=0.5\textwidth]{EgGenParGray/taPrefix01_2.png} &
\includegraphics  [width=0.4\textwidth]{EgGenParGray/taPrefix01_3.png}  \\
(f) TA05 &  (g) TA06 \\

%  \hspace{0.1\textwidth}
% \subfigure{\includegraphics [width=0.3\textwidth]{EgGenParGray/taWait_n01_4.png}}
\end{tabular}

% \includegraphics [width=0.9\textwidth]{EgGenParGray/Env.png}
\caption{A list of networked TA for the translation of the process ADS.}
\label{ta_ads}
\end{figure}


\begin{figure}
    \centering
\includegraphics [width=0.9\textwidth]{EgGenParGray/Env.png}
\caption{An environment TA for the translated behaviour of the process ADS.}
\label{ads_env}
\end{figure}


% %-----------------------------------------------
% \begin{figure}%
% \centering
%   \includegraphics[width=\linewidth, height=0.3\linewidth]{newEg/taGenPar0_0.png}
%   \caption{TA01}

% \subfigure[Sample1]{%
% % \label{fig:first}%
% \includegraphics[width=0.4\textwidth]{newEg/taPrefix00_1.png}}%
% \qquad
% \subfigure[Sample2]{%
% % \label{fig:second}%
% \includegraphics[width=0.4\textwidth]{newEg/taPrefix00_2.png}}%
% \subfigure[Sample1]{%
% % \label{fig:first}%
% \includegraphics[height=3cm]{newEg/taPrefix00_3.png}}%
% \qquad
% \subfigure[Sample2]{%
% % \label{fig:second}%
% \includegraphics[height=1cm]{newEg/SyncTA.png}}%

% \subfigure[Sample1]{%
% % \label{fig:first}%
% \includegraphics[height=3cm]{newEg/taPrefix01_2.png}}%
% \qquad
% \subfigure[Sample2]{%
% % \label{fig:second}%
% \includegraphics[height=1cm]{newEg/taPrefix01_2.png}}%
% \caption{sample}
% \end{figure}




% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{figure} %[H]
% \subfigure{\includegraphics [width=0.9\textwidth, height=0.4\textwidth]{EgGenParGray/taGenPar0_0.png}}

% \subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix00_1.png}}
%  \hspace{0.1\textwidth}
% \subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix00_2.png}}

% \subfigure{\includegraphics [width=0.55\textwidth]{EgGenParGray/taPrefix00_3.png}}
% \subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/SyncTA.png}}

% \subfigure{\includegraphics [width=0.55\textwidth]{EgGenParGray/taPrefix01_2.png}}
% \subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix01_3.png}}

%  \hspace{0.1\textwidth}
% % \subfigure{\includegraphics [width=0.3\textwidth]{EgGenParGray/taWait_n01_4.png}}
% \subfigure{\includegraphics [width=0.9\textwidth]{EgGenParGray/Env.png}}
% \caption{A list of networked TA for the translation of the process ADS.}
% \label{ta_ads}

% \end{figure}



\begin{example} A translation of the process ADS, from Example \ref{ads}, produces the network of small TA in Figure \ref{ta_ads}. 
\end{example}

\noindent
Details of the translated TA are as follows. Starting from the top, TA0 captures concurrency by starting the two concurrent automata corresponding to the processes \lstinline{Controller} and \lstinline{Lighting} in two possible orders, either \lstinline{Controller} then \lstinline{Lighting} or vice versa. Here we use the committed locations (\lstinline{s2}, \lstinline{s3} and \lstinline{s4}) to show that starting the concurrent processes is a compound action. Then TA0, waits on state \lstinline{s5} for the termination actions in the two possible orders, either \lstinline{Controller} terminates first then \lstinline{Lighting} or vice versa, thru locations \lstinline{s6} and \lstinline{s7}, respectively. For the termination, we did not use committed location because the processes can terminate at different time and TA0 synchronises the processes before the whole process terminates with the action \lstinline{finishID0}.


TA01, TA02 and TA03 capture the behaviour of the process \lstinline{Controller}. TA01 captures the occurrence of the event \lstinline{open}. TA02 captures the occurrence of the event \lstinline{tock?} (with a question mark) for synchronising with the environment in recording the progress of time. The fourth TA captures the occurrence of the event \lstinline{close} to synchronise with the synchronising controller TA04.

TA05 and TA06 capture the behaviour of the process \lstinline{Lighting}. TA05 captures the translation of \lstinline{close}, which also synchronises with the synchronisation controller (TA05). Then, TA06 captures the event  \lstinline{offLight}. Finally, Figure \ref{ads_env} is the environment TA that has co-actions for all the translated events. Also, the environment TA serves the purpose of `closing' the overall system as required for the model checker. In the environment TA, we use the variable \lstinline{start} to construct a guard \lstinline{start==0} that blocks the environment from restarting the system. This concludes the description of the list of TA for the process ADS.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Explanation of TA for ADS
% \paragraph{}


An alternative to using a list of small TAs is using a single large TA to capture the behaviour of the translated \tockCSP{} process. However, the main reason for using a list of small TAs is capturing the compositional structure of \tockCSP{}, which is not available in TA \cite{DH08}. For instance, it can be argued that a linear process constructed with a series of prefix operators can be translated into a linear TA. However, the compositional structure of \tockCSP{} is not suitable for this straightforward translation. For instance consider a case where the linear process is composed of an interrupting process, the behaviour is no longer linear because the process can be interrupted at any stable state, as shown in Example \ref{egPI}. A network of small TAs provides enough flexibility for composing TA in various ways to capture the behaviour of the original \tockCSP{} process. % , as explained below.  



In constructing the network of TA, we use additional \textbf{\textit{coordinating actions}} to link the small TA into a network TA for establishing the flow of the input \tockCSP{} process. For example, the channel \lstinline{startIDADS} links the environment TA (Figure \ref{ads_env}) with TA00, on performing the action \lstinline{startIDADS!} and  its co-action \lstinline{startIDADS?}.  Definition \ref{coordinating_action} describes the coordination action precisely.

% The definition of the coordinating action is in Definition \ref{coordinating_action}.

% %??Toreturn
% , respectively. Likewise, the channel \verb!startID00_1! connects the first TA with the second TA, on performing the actions \verb|startID00_1!| and its co-action \verb!startID00_1?!, respectively.  A precise definition of the coordinating actions is provided below in Definition \ref{coordinating_action}, together with the types of coordinating actions we use in developing the translation technique.




\begin{definition}

 \textbf{A Coordinating Action} is an \uppaal \ action that does not correspond to a \tockCSP{} event. There are six types of coordinating actions: \textbf{Flow actions} coordinate a link between two TAs for capturing the flow of their behaviour; 
\textbf{Terminating actions} record termination information, in addition to coordinating a link between two TAs;
\textbf{Synchronisation actions} coordinate a link between a TA that participate in a synchronisation action and a TA for controlling the synchronisation; 
\textbf{External choice actions} coordinate an external choice, such that choosing one of the TA that is part of the external choice blocks the other choices TAs; % that participate in the external choice;
\textbf{Interrupting actions} initiate an interrupting transition that enables a TA to interrupt another; and
\textbf{Exception actions} coordinate a link between a TA that raises an action for exception and a control TA that handles the action. 

\label{coordinating_action}
\end{definition}

% \vspace{-0.5cm}
\noindent
The names of each coordinated action are unique for ensuring the correct flow of the translated TA. In our implementation, the names of the flow actions are generated in the form \verb!startIDx!, where \verb!x! is either a natural number or the name of the input \tockCSP{} process.  We can see this in Example \ref{ads}; \verb!startID00_1! is the flow action that connects the first TA with the second TA.

Likewise, the names of the remaining coordinating actions follow the same pattern: \verb!keywordIDx!, where  \verb!keyword! is a designated word for each of the coordinating actions; \verb!finish! for a terminating action,  \verb!ext! for an external choice action, \verb!intrp! for an interrupting action, and \verb!excp! for an exception action. Similarly, we provide a special name of a synchronising action is in the form \verb!eventName___sync!: an event name appended with the keyword \verb!___sync! to differentiate a synchronising action from other actions \footnote{This is particularly important for analysis and is in the reserved keywords for the supporting tool.}.

% \footnote{This is particularly important for analysis and is going to be among the reserved keywords for the supporting tool.}.



We use termination actions for cases where a TA needs to communicate a successful termination for another TA to proceed. For instance, in translating sequential composition \lstinline{P1;P2} where the process \lstinline{P2} begins only after successful termination of the process \lstinline{P1}.  



For each translated \tockCSP{} specification, we provide an environment TA, like the TA in Figure \ref{ads_env}. The environment TA has corresponding co-actions for all the translated events of the input \tockCSP{} model, in addition to three coordinating actions that link the environment TA with the network of the translated TA. The first flow action links the environment with the first TA in the list of the translated TA (as illustrated in Figure \ref{ads_env} and TA00 in Figure \ref{ads}). This first flow action activates the behaviour of the translated TA. Second, a terminating action links back the terminating TA (like the action FinishID0 in TA00 in Figure \ref{ads}) to the environment TA to record a successful termination of a process (as shown in TA00 with the action FinishID0). Third, a flow action for \lstinline{tock} to record the progress of time. A precise definition of the structure of environment TA is in Definition \ref{dfn_envTA}.

%in Definition \ref{environment_TA}.



% \vspace{0.2cm}

\begin{definition} 
\label{dfn_envTA}
\textbf{An Environment TA} models an operating environment for \uppaal. In this work, the environment TA has one state and transitions for each co-action of all the events in the input \tockCSP{} process, in addition to three transitions: the first starting flow action, the final termination co-action, and the action \lstinline{tock} for indicating the progress of time.
\label{environment_TA}
\end{definition}


\noindent
In translating multi-synchronisation, we adopt a centralised approach developed in \cite{O05} and implemented using Java in \cite{F05}, which describes using a separate centralised controller for controlling multi-synchronisation events. Here, we use a separate TA with an \uppaal{} broadcast channel to communicate synchronising information among synchronising TA and a control TA.
% that control the synchronising action.

% In Example \ref{ads}, 

An example can be seen in Figure \ref{ads}, where we illustrate the strategy in translating the event \lstinline{close}, which synchronises the two processes \lstinline{Controller} and \lstinline{Lighting}. In Figure \ref{ta_ads}, TA04 captures the translation of \verb!close!, which synchronises TA03 and TA05. The synchronising TA (TA04) broadcasts the channel \verb!close___sync! to synchronise TA03 and TA05. 


Each synchronising TA has a guard for ensuring synchronisation with the correct number of TAs. The guard is a logical expression that adds variables from all the TAs synchronise on the synchronisation action. Each TA updates its variable from 0 to 1 to show its readiness for the synchronisation and waits for the synchronisation action. In Figure \ref{ta_ads}, the synchronising TA (TA04) has a guard expression \lstinline{(g_close00_3 + g_close01_2)==2}, which becomes true only when TA03 and TA05 update their synchronisation variables: \lstinline{g_close00_3} and \lstinline{g_close01_2}, from 0 to 1. Then, TA04 notifies the occurrence of the action \lstinline{close} and broadcasts the synchronising action \lstinline{close___sync!}. After the synchronisation, each TA reset its variable to zero and perform the remaining actions. A precise definition of synchronisation TA is in Definition \ref{dfn_syncTA}.



\begin{definition} \textbf{A synchronisation TA} coordinates synchronisation actions. Each synchronisation TA has an initial state and a committed state for each synchronisation action, such that each committed state is connected to the initial state with two transitions. The first transition from the initial state has a guard and an action. The guard is enabled only when all the processes are ready for synchronisation, which also enables the synchronising TA to perform the associated action that notifies the environment of its occurrence. In the second transition, the TA broadcasts the synchronisation action to all the processes that synchronise, which enable them to synchronise and proceed.
\label{dfn_syncTA}
\end{definition}


% \begin{definition} \textbf{A synchronisation TA} coordinates synchronisation actions. Each synchronisation TA has an initial state and a committed state for each synchronisation action, such that each committed state is connected to the initial state with two transitions. The first transition from the initial state has a guard and an action. The guard is enabled only when all the processes are ready for the synchronisation, which also enables the synchronising TA to perform the associated action that notifies the environment of its occurrence. In the second transition, the TA broadcasts the synchronisation action to all the processes that synchronise on the synchronisation action, which enable them synchronise and proceed.
% \label{dfn_syncTA}
% \end{definition}




% To ensure that the synchronisation TA synchronises with the required number of TA that participate in a synchronisation channel, we provide guards that block the broadcast channel until all the required TA are ready for the synchronisation. When the guard becomes ready, it enables the synchronising TA to broadcast the synchronisation action such that all the participating TA synchronise and progress with their behaviour, as well as the behaviour of the whole system.


%----------------------- External choice
In translating external choice, we provide additional transitions for capturing the behaviour of the chosen process in blocking the behaviour of the other processes. Initially, in the translated TA, all the initials \footnote{Initials are the first visible events of a process.} of the translated processes are available such that choosing one process blocks all the other choices.

% one of the processes blocks all the other choices.  

% choices with the provided additional actions for coordinating external choice, as define in Definition \ref{coordinating_action}.


\begin{figure}[t]
    \centering
    \begin{tabular}{c c}
    \includegraphics [width=0.45\textwidth]{EgExtChoice/taExtCh00.png} &
    \includegraphics [width=0.5\textwidth]{EgExtChoice/taPrefix00_1.png} \\
    
    (a) TA00  & (b) TA01 \\
    
    
    \includegraphics [width=0.5\textwidth]{EgExtChoice/taPrefix01_2.png} & 
    
     \includegraphics [width=0.3\textwidth]{EgExtChoice/taSTOP__00_2.png} \\
    
    % \vspace{-0.5cm}
    % \begin{tabular}{c}
    %  \includegraphics [width=0.3\textwidth]{EgExtChoice/taSTOP__00_2.png} \\
    % \includegraphics [width=0.3\textwidth]{EgExtChoice/taSTOP__01_3.png}
    % \end{tabular}
    
    \\
    TA02 & TA03  \\
    
    \includegraphics [width=0.3\textwidth]{EgExtChoice/taSTOP__01_3.png} & \\
    
    TA04 &   \\
    
    \end{tabular}
    

    \caption{A list of TA for the translated behaviour of the process Pe}
    % \\ \lstinline{Pe = (left->STOP)[](right->STOP)}
    \label{fig_ext_choice}
\end{figure}


% For example, a process \verb!Pe = P1[]P2!, that composes \verb!P1! and \verb!P2! with operator external choice; such that \verb!P1 = (right->STOP)! and \verb!P2 = (left->SKIP)!. The initials of \verb!P1! and \verb!P2! are \verb!right! and \verb!left!, respectively. The list of the translated TA is in Figure \ref{fig_ext_choice} The first TA in the list of TA for the translation of the process \verb!P1! has an additional transition for the added external choice action \verb!left_ext! (initials of \verb!P2!) that blocks \verb!P1!. Likewise the first TA of list of TA that capture the process \verb!P2! has an additional transition for the external choice choice event \verb!right_ext! (Initials of \verb!P1!) that blocks \verb!P2!. This enables a list of TA to capture the behaviour of external choice construct, such that a list of TA blocks another list of TA. Additional examples are also available in an extended technical report \cite{extendedVersion}.



%------------------------------------- Example external choice
% \begin{example}
%  An example of translating external choice is provided in Figure \ref{fig_ext_choice} for the process \lstinline{Pe = (left->STOP)[](right->STOP))}, which composes two processes \lstinline{(left->STOP)} and \lstinline{(right->STOP)} with the operator of external choice. 
% %  The process is translated into a list of TA.
% \end{example}


\begin{example} A translation of external choice is shown in Figure \ref{fig_ext_choice} for the process \lstinline{Pe = (left->STOP)[](right->STOP))}, which composes two processes \\\lstinline{left->STOP} and \lstinline{right->STOP} using the operator of external choice. 
\end{example}

\noindent
In Figure \ref{fig_ext_choice}, starting from the top-left, TA01 is a translation of the operator external choice. TA01 and TA03 capture the LHS process \lstinline{left->STOP}. TA02 and TA04 capture the RHS process \lstinline{right->STOP}.   TA01 has three transitions labelled with the flow actions: \lstinline{startIDp0_6?}, \lstinline{startID00_1!} and \lstinline{startId01_2!}. TA01 begins with the first flow action \lstinline{startIDpExtChoice?} to start the TAs (TA01 and TA02) for both the left and right process using  \lstinline{startID00_1!} and \lstinline{startId01_2!}, which make them available for choice.
% , to make both two processes available for a choice.
% The first TA is a translation of the operator external choice. The TA has 3 transitions, each label with a flow action, \lstinline{startIDp0_6} \lstinline{startID00_1} and \lstinline{startId01_2}. Initially, the behaviour of the TA synchronises on the first flow action \lstinline{startIDp0_6} and then immediately performs the two subsequent flow actions \lstinline{startID00_1} and \lstinline{startId01_2} that activates the translations of the LHS and RHS processes, \verb!(e1->SKIP)! and \verb!(e2->SKIP)! respectively. 


%ToUpdate ???????????????????????????

TA02 capture the translation of the event \lstinline{left}. Initially, the TA02 synchronises on the flow action \lstinline{startID00_1} and moves to location \lstinline{s2} where the TA has 3 possible transitions labelled with the actions: \lstinline{left_exch?}, \lstinline{right_exch!} and \lstinline{tock?}. With the co-action \lstinline{tock?}, the TA records the progress of time and remains on the same location \lstinline{s2}. With the co-action \lstinline{right_exch?}, the TA performs an external choice co-action for blocking the TA of the LHS process when the environment chooses the RHS process, and TA02 returns to its initial location \lstinline{s1}. Alternatively, TA02 performs the action \lstinline{left_exch!} when the environment chooses the LHS process, and TA02 progresses to location \lstinline{s3} to perform the chosen action \lstinline{left} that leads to location \lstinline{s5} and performs the flow action \lstinline{startID00_2}, which activates TA03 for the subsequent process \lstinline{STOP}. For the RHS process, TA02 captures the translation of the event \lstinline{right}, similar to the previous translation of event \lstinline{left}, which then activates TA04 for the process \lstinline{STOP}. Lastly, the omitted environment TA is similar to the environment TA in Figure \ref{ads_env}. This illustrates the translation of external choice.

% This describes the translation of the RHS process, and also completes the translation of the process \verb!Pe = (left->STOP)[](right->STOP)!.

% as shown in Figure \ref{fig_ext_choice}.
% into a list of TA in Figure \ref{fig_ext_choice}.

%ToReturn
% One might argue that a single TA can capture the translation of external choice operator.  However the problem is the compositional structure of \verb!tock-CSP!. In particular, if there is concurrency in either left or right process or both, a single TA can not handle both external choice and concurrency at the same time. This problem can be seen in translating a process like \verb!P = (e1->SKIP)[]((e2->SKIP)|||(e3-SKIP))!, where the RHS process have concurrent processes \verb!(e2->SKIP)! and \verb!(e3-SKIP))!

% \vspace{-0.15cm}
%----------------------- Interrupt
Similarly, in \tockCSP, a process can be interrupted by another process when it is composed with an interrupting operator (\verb!/\!). For capturing interrupting behaviour in TA, we provide additional transitions for expressing an interrupting action,  which enables a TA to interrupt another one. The translation of an interrupting process resembles the translation of an external choice as shown in the following example.





%-------------------------------------------
%ToReturn
% \begin{example} 
% An example of translating interrupt is provided in Figure \ref{fig_interrupt}, for the process \lstinline{Pi = (open->SKIP)/\(fire->close->SKIP)}. The RHS process \verb!(fire -> close -> SKIP)! can interrupt the behaviour \verb!(open -> SKIP)! at any stable state. In the translated behaviour of the LHS process, we provide additional interrupting actions (\lstinline{fire_intrpt}) that enables the translated behaviour of the RHS process to interrupt the LHS process. This additional interrupting actions are provided only for the initials of the RHS process (\verb!fire!). 
% \end{example}

\vspace{-0.3cm}
\begin{example} 
\label{egPI}
An example of translating interrupt is provided in Figure \ref{fig_interrupt}, for the translation of the process \lstinline{Pi = (open->STOP)/\(fire->close->STOP)}. 
\end{example}

\noindent
In the process \lstinline{Pi}, the RHS process \lstinline{(fire -> close -> STOP)} can interrupt the behaviour of \lstinline{(open->STOP)} at any stable state. In the translated behaviour of the LHS process, we provide additional interrupting actions (\lstinline{fire_intrpt}) that enable the translated behaviour of the RHS process to interrupt the behaviour of the LHS process. The interrupting actions are provided only for the initials of the RHS process (\lstinline{fire}). 





\begin{figure} [t]
    \centering
    \begin{tabular}{c c}
    
    \includegraphics [width=0.45\textwidth]{EgInterrupt/taIntrpt0_0.png} &
    
    \includegraphics [width=0.5\textwidth]{EgInterrupt/taPrefix00_1.png}  \\
    
    (a) TA00 &  (b) TA01  \\  
    
    \includegraphics [width=0.45\textwidth]{EgInterrupt/taSTOP__00_2.png} &
    
    \includegraphics [width=0.55\textwidth]{EgInterrupt/taPrefix01_2.png} \\
    
    (c) TA02  &   (d) TA03  \\
    
    \includegraphics [width=0.45\textwidth]{EgInterrupt/taPrefix01_3.png}  &
    
    \includegraphics [width=0.4\textwidth]{EgInterrupt/taSTOP__01_4.png} \\
    
    (e) TA04  & (f) TA05  \\
    \end{tabular}
    
    \caption{A list of TA for the translated behaviour of the process Pi.}
    % \\ \lstinline{Pi = (open->SKIP)/\\(fire->close->STOP)}}
    \label{fig_interrupt}
\end{figure}



In Figure \ref{fig_interrupt}, starting from the top-left, TA00 is a translation of the operator interrupt. TA01 and TA02 capture the translation of the LHS process \lstinline{open->STOP}. TA03, TA04 and TA05 capture the translation of the RHS process \lstinline{fire->close->STOP}. The environment TA is also omitted because it is also similar to the TA in Figure \ref{ads_env}.


% The first TA starts the TA for both processes using the flow actions \\

First, TA00 starts the first TAs (TA01 and TA03) of both processes using \lstinline{startID00_1!} and \lstinline{startID01_2!}, respectively. TA01 synchronises on the flow action \lstinline{startID00_1} and moves to location \lstinline{s2} where the TA has 3 possible transitions for the actions: \lstinline{tock?}, \lstinline{open!} and \lstinline{fire_intrpt?}. With the co-action \lstinline{tock?}, the TA records the progress of time and remains on the same location \lstinline{s2}. With the co-action \lstinline{fire_intrpt?}, the TA is interrupted by the RHS, and it returns to its initial location \lstinline{s1}. With the action \lstinline{open!}, the TA progresses to location \lstinline{s5} to perform the flow action \lstinline{startID00_2}, which activates TA02 for the subsequent process \lstinline{STOP}, where TA03 synchronises on the flow action \lstinline{startID00_2} and moves to location \lstinline{s2}, where it either performs the action \lstinline{tock?} to record the progress of time or is interrupted  through the co-action \lstinline{fire_intrpt?}, and returns to its initial location \lstinline{s1}. This completes the behaviour of the LHS process \lstinline{open->SKIP}.



TA03 captures the translation of the event \lstinline{fire}. TA03 begins with synchronising on the flow action \lstinline{startID01_2}, which progresses by interrupting the LHS process using the interrupting flow action \lstinline{fire_intrpt}, then \lstinline{fire}, and performs \lstinline{startID01_3} for activating TA04 which synchronises on the flow action and moves to location \lstinline{s2}, where it either performs the action \lstinline{tock?} for the progress of time and remains in the same location or performs the action \lstinline{close} and proceeds to location \lstinline{s5}, then performs the flow action \lstinline{startID01_4} for starting TA05 for the translation of \lstinline{STOP} (deadlock).


% Additional examples are available in the extended report \cite{extendedVersion}.

% For example, consider a process \lstinline{Pi = (open->SKIP)/\(fire->close->SKIP)}; the LHS process \verb!(open -> SKIP)! is interrupted by the process \verb!(fire -> close -> SKIP)!. In the translated behaviour of the LHS process, we provide additional transitions for the Interrupting actions that has the initials of the RHS process (\verb!fire!), which enables the behaviour of the RHS process to interrupt the behaviour of the LHS process, at any stable state of its behaviour. Additional examples are available in the extended report.


%??????????
% For example, given a process \verb!Pi = P1/\P2!, the process \verb|P1| can be interrupted by process \verb|P2|. Thus, in translating each event of process \verb|P1|, we provide additional transitions for the initials of the interrupting process \verb|P2|. The additional transitions enable the translated behaviour of process \verb|P2| to interrupt the translated behaviour of process \verb|P1| at any stable state of its behaviour.


We translate the event \lstinline{tock} into a corresponding action \lstinline{tock} for recording the progress of time in the translated TA using a broadcast channel that enables the environment TA to broadcast the progress of time for the TAs to synchronise using their coordination action. For instance, in Figure \ref{ta_ads}, the environment TA has a transition labelled with the action \lstinline{tock} guarded with the clock expression $ck \geq 1$, so that the action \lstinline{tock} happens every 1 time unit, and resets the clock $ck=0$ to zero on following the transition.







% Also, in \tockCSP, an event can be renamed or hidden from the operating environment. In translating renaming, we use a list of renamed events such that before translating each event, the technique checks if the event is renamed, and then translate the event appropriately with the corresponding new name. In the like manner, if an event is part of the hidden events, we use a list of hidden events such that technique uses a special name $itau$ for the hidden event. The event $itau$ has similar meaning to $tau$ for representing a hidden event in CSP. We differentiate the translated event $itau$ from $tau$, for the purpose of analysis.


% As described previously, in \verb!tock-CSP!, the event \verb!tock! records the progress of time. Thus, 

% We translate the event \verb!tock! into a corresponding action \verb!tock! for recording the progress of time in the translated TA using a broadcast channel that enables the translated TA to synchronise in recording the progress of time. The action \verb!tock! is broadcast by the environment TA, which causes all the processes to synchronise and record the progress of time using their corresponding co-actions \verb!tock?! (with a question mark). In particular, in Figure \ref{ta_ads} the last TA that models the environment, has a transition with an action \verb!tock! that is guarded with the expression $ck \leq 1$, so that the action \verb!tock! happens every 1 time unit, and resets the clock $ck=0$ to zero on following the transition.

% The translated action \verb!tock! is guarded with clock $clk<=1$ which trigger the action \verb!tock! and reset the clock $clk=0$.


% In translating non-determinism, TA has a non-determinism facility, using 


% Silent transitions enable a TA to take any of the silent transitions. 
We translate non-deterministic choice into silent transitions, such that the translated TA follows one of the silent transitions non-deterministically. Nevertheless, divergence is not part of the construct that we consider in this translation work because divergence is a sign of bad behaviour, which is going to be part of the future work. This completes an overview of the strategy we follow in developing the translation technique. A precise description of all the translation rules in Haskell is in the extended report of this work \cite{extendedVersion}.



% % %----------------------- Sample rule for translation of STOP
% % \subfile{a4_ruleStopNew}
% An example of the formalisation of the translation rules in Haskell is provided in Rule 1, which describes the translation of the construct  \verb!STOP!. All the remaining rules can be found in \cite{extendedVersion}. Rule \ref{rule_STOP} produces an output TA that is depicted in Figure \ref{STOP_map}, which has two locations and two transitions as defined in Rule \ref{rule_STOP}, Lines 7--9 and Lines 11--13, respectively. In Figure \ref{STOP_map}, we map the structure of the TA with the names used in the translation rule. The names are \lstinline{loc1, loc2, tran1, tran2, intrpt}. 




%----------------------------------------------

% % \vspace{1cm}
% \begin{figure}[t]
%     \centering

% \begin{tcolorbox} %[title=Title]
% \begin{trule} \textbf{Translation of STOP}
% \label{rule_STOP}
% \end{trule}
% \tcblower
% \begin{Verbatim}[numbers=left,numbersep=7pt]
% transTA STOP processName bid sid _ usedNames =
%   (([(TA idTA [] [] locs [] (Init loc1) trans)]), [] )
%   where 
%   idTA = "taSTOP__" ++ bid ++ show sid
   
%      --   Definition of locations in the TA  
%      -- = Location ID     Name  Label       LocType
%   loc1 = Location "id1"  "s0"  EmptyLabel  None
%   loc2 = Location "id2"  "s1"  EmptyLabel  None
%   locs = [loc1, loc2]

%      --    Definition of transitions in the TA 
%      --  = Transition Source   Target  [Label] [Edge]
%   tran1 = Transition loc1     loc2    [lab1]  []
%   tran2 = Transition loc2     loc2    [lab2]  []
%   intrp = transIntrpt intrptsInits loc1 loc2        
%   trans = [tran1, tran2] ++ intrp

%   --  Labels of the transitions in the TA
%   lab1 = Sync (VariableID 
%             (startEvent processName (bid ++ sid)) []) 
%              Ques
%   lab2 = Sync (VariableID "tock" []) Ques     

%   -- Get the initial events of an interrupting process
%   (_, _, _, _, _, intrptsInits, _, _) = usedNames

% \end{Verbatim}
% \end{tcolorbox}

%     % \includegraphics{}
%     % \caption{Caption}
%     % \label{fig:my_label}
% \end{figure}

% % %%% Previous description
% % %\pagebreak
% % \vspace{0.3cm}
% % \begin{trule} Translation of Deadlock
% % \begin{lstlisting}[mathescape, firstnumber=last]
% % transTA STOP processName _ startID _ _ =
% %    [ 
% % \end{lstlisting}
% % \begin{figure}[H]
% % \centering
% % \includegraphics [width=0.4\textwidth]{newImg/trule_stop.png}
% % \end{figure}
% % \begin{lstlisting}[mathescape, firstnumber=last]
% %    ]
% % where
% %  startEvent = startEvent processName startID
        
% % \end{lstlisting}
% % \label{trule_STOP}
% % \end{trule} 



% \begin{figure}
% \centering
% \includegraphics [width=0.5\textwidth]{figGray/stopMap.png}
%  \caption{A structure of an output TA for the translation of STOP from Rule 1.}
% \label{STOP_map}
% \end{figure}

%---------------------------------------------- OLD



%%%%%%%%%%%%%%%%%%%%%%% STOP
% \subsubsection{Translation of STOP}


% Here, we present a structure of the translation rule using one of the translation rule, which describes the translation of the construct  \verb!STOP!. We begin with presenting a rule for translating STOP and then follow with an example that illustrates using the rule in translating a \tockCSP{} process into TA.


%This section describes a translation of a constant process \lstinline{STOP}. The section begins with presenting a rule for translating STOP and then follows with an example that illustrates using the rule in translating a process.

%ToReturn
%?? You need to explain the fun transTA ?? \\


% A detailed description of Rule \ref{rule_STOP} is as follows. Each rule considers one construct. Line 1 identifies the definition of our translation function \lstinline{transTA} for \lstinline{STOP}, and it takes three extra parameters: \lstinline{processName}, \lstinline{bid} and \lstinline{sid}. The symbol underscore \footnote{In Haskell, the symbol underscore indicates a position of unused arguments. For conciseness, we use the underscore to omit unused arguments and provide only the required arguments for each translation rule.} represents unused arguments.
% % in the translation rule.


% Line 2 defines the output pairs, a list of output TA and a list of synchronising actions. The second element is empty ([]) in Rule 1 because there is no synchronising action in translating the construct \verb!STOP!. The first element describes the output TA, which has 6 parameters. First, \lstinline{idTA} is an identifier for the TA, which is defined subsequently in Line 4, as the concatenation of the keyword \lstinline{"taSTOP__"} with the 2nd and 3rd arguments of the function \lstinline{transTA}, that is \lstinline{bid} and \lstinline{sid} respectively. Additionally, still in Line 2, in the definition of the output TA, the 2nd, 3rd and 5th parameters are empty for the output TA. While the 4th parameter \lstinline{locs} is a list of locations for the output TA, as defined in Lines 7--9. The 6th parameter \lstinline{(Init loc1)} specifies \lstinline{loc1} as the initial location of the output TA. Last parameter \lstinline{trans} describes a list of transitions that connect the locations of the TA, as defined in line 12--13. Line 14 defines interrupting transitions that are generated with the function \lstinline{transIntrpt}, that is in the case where a process is composed with an interrupting process. Lines 17--20 define the labels of the transitions. Lastly, Line 23 extracts the initials of an interrupting process from the parameter \lstinline{usedNames}, which collects information such as the names of hidden events and renamed events.
% %and interrupting events.
% %, as described in Definition \ref{dfn_transTA}.



% The behaviour of the output TA begins with the first flow action (defined in Line 17). After that, the TA performs the action \lstinline{tock} (line 18), repeatedly, which allows the progress of time, unless there is an interrupt, which causes the TA to follow the interrupting transition, as defined in Line 14. 
% %ToReturn
% % An illustration of using this translation rule in translating a process is shown in Example \ref{ex_STOP}.




% %--------------------- EXAMPLE
% \vspace{-0.7cm}
% \begin{example} \label{ex_STOP}
% An example of translating a process \verb!STOP! that produces a list of TA, which contains two TAs as shown in Figure \ref{stop_ta1}. The LHS TA captures the translation of the construct $STOP$, in this case there is no interrupting transition because there is no interrupting process. A translation of interrupt has been provided separately. The RHS TA is an environment TA that we provide for translating each process, as described in Definition \ref{environment_TA}.


% % \begin{lstlisting}[mathescape, firstnumber=last]
% % transTA STOP "p0_1" 1 0 ([], [], [], [], [], [], [], ([],[])) =
% %         [ 
% % \end{lstlisting}


% \pagebreak

% \begin{lstlisting}[mathescape, firstnumber=last]
% transTA(STOP) = [
% \end{lstlisting}

% \begin{figure}[H]

% \includegraphics [width=0.5\textwidth]{figGray/taSTOP.png}
% \includegraphics [width=0.5\textwidth]{figGray/Env1_g.jpg}

% \caption{A list of TA for the translation of the construct STOP}
% \label{stop_ta1}
% \end{figure}


% \lstinline{  ]}
% \end{example}








%  ---------------------------------- EVALUATION 
\section{Evaluation}
\label{evaluation}

% To ensure that the translation work is correct, we have to prove soundness.
A sound translation ensures that properties of the source model are preserved in the translated models. This is determined by comparing the behaviours of the source model and the translated model \cite{T06, NN07, KM19, B81}. We follow this approach in comparing the behaviour of the input \tockCSP{} and the output TA, where we use two phases: experimental evaluation using trace semantics and mathematical proof using structural induction.



\subsection{Experimental Evaluation}
% In this work, we use traces to compare the behaviour of the input \tockCSP{} models and the traces of the translated TA models. We
In comparing the traces, we have developed an evaluation tool, which uses the translation tool to translate the \tockCSP{} model into TA, and then uses both FDR and \uppaal{} as black boxes in generating sets of finite traces. The structure of the evaluation tool is in Figure \ref{trace_analysis_system}, while the implementation of the tool is available in the repository \cite{extendedVersion}.


% In this work, we use traces to compare the behaviour of the input \tockCSP{} models and the traces of the translated TA models. We have developed an evaluation tool, which uses the translation tool to translate \tockCSP{} model into TA, and then uses both FDR and \uppaal \ as black boxes in generating sets of finite traces. The structure of the evaluation tool is shown in Figure \ref{trace_analysis_system}. 



In generating traces, like most model checkers, FDR produces only one trace (counterexample) at a time. So, based on the testing technique refinement \cite{NS08}, we have developed a trace-generation technique that repeatedly invokes FDR for generating traces until we get all the required trace set of the input \tockCSP{}. Similarly, based on another testing technique for temporal logic \cite{LP07}, we have developed another trace-generation  technique, which uses \uppaal{}  in generating finite discrete traces of the translated TA models. 

These two trace-generation techniques are components of our trace analysis tool (Figure \ref{trace_analysis_system}), which has two stages of analysing traces. In the first stage, we generate traces of the input \tockCSP{} and its corresponding translated TA, using both FDR and \uppaal, respectively. Then, we compare the generated traces, and if they do not match, we move to the second stage for further analysis. This is because FDR (refinement) can distinguish different permutations of events (traces). In contrast,  \uppaal{}  is not capable of detecting traces with different permutations because \uppaal{} uses a logical formula in generating traces \cite{LP07, BD06}. Thus, we use the power of FDR to complement \uppaal{} in generating and comparing traces of \tockCSP{} and TA.


\begin{figure}[t!] %[H]
    \centering
%    \includegraphics[width=0.7\textwidth]{C3_figs/traceAnalysis.png}
    \includegraphics[width=\textwidth, height=0.25\textheight]{fig/traceAnalysis.png}
    \caption{Structure of the trace analysis system}
    \label{trace_analysis_system}
\end{figure}



Basically, \uppaal{} checks if a system satisfies its requirement specifications (expressed in temporal logic), irrespective of the behaviour of the system. For example, \uppaal \ does not distinguish between the two traces $ \langle e1, e2, e3 \rangle$ and  $\langle e1, e3, e2 \rangle$, if both of them satisfy the requirement specification formula. The two traces contain the same three actions, but the action $e2$ and $e3$ occur in a different order. However, FDR is capable of detecting and generating both traces. Thus, in the second stage, we use \uppaal \ to check if all the traces of FDR are acceptable traces of the translated TA.
% , otherwise there are missing traces. 







% --------- short version begin
The developed tool helped us evaluate the translation technique by translating a list of systematically formulated \tockCSP{} processes that pair the constructs of \tockCSP{} in our BNF (Definition \ref{dfn_CSPproc}). The list contains 111 processes that are not more than five states in size. Archives of the processes and their traces are available in a repository of this work \cite{extendedVersion}.


%ToReturn
%An overview of the processess is in Table 

% We use this tool in evaluating the translation technique by translating a list of systematically formulated \tockCSP processes that pair the constructs of \tockCSP, within the scope of this translation work, which produces 111 processes of smaller sizes that are not more than five states in size. Archives of the processes and their traces are available in this repository \cite{extendedVersion}




%  Test cases ----------------------------------------
In addition, we test the translation technique with larger examples from the literature, such as an automated barrier to a car park \cite{S10}, a thermostat machine for monitoring ambient temperature \cite{S10}, an Automated Teller Machine (ATM)  \cite{R05}, a bookshop payment system \cite{S10}, and a railway crossing system \cite{R10}. An overview of these case studies is in Table \ref{table_caseStudies}, while the details, including the traces, are available in the repository of this work \cite{extendedVersion}. 

%ToReturn
% Traces are not included because the systems have infinite traces. This is due to the nature of \tockCSP models and other timed systems, they are reactive system with non-terminating processes that must allow time to progress \cite{R10}. Even a simple process such as $STOP$ have an infinite sequence of $tock$ as its traces.  Additional examples, together with details implementation of the trace generation techniques, are available in \cite{extendedVersion}.




% A reader may like to know the size of these test cases. However, all these test cases are reactive system, which means that they are non terminating process that has infinite traces. This is the nature of \tockCSP models and other time systems, they are non-terminating process that must allow time to progress \cite{R10}. Even the simple basic process such as $STOP$ have an infinite sequence of $tock$ as their traces.





% Case Studies        Average Timing    States    Transitions    Events    State/Transition
% ATM    FDR    0.0051    15    33    15    0.4545454545
%     UPPAAL    0.0084                
% AutoBarrier    FDR    0.0059    35    84    10    0.4166666667
%     UPPAAL    0.0134                
% PaymentSystem    FDR    0.0048    7    32    9    0.21875
%     UPPAAL    0.0011                
% Rail Crossing    FDR    0.0054    80    361    12    0.2216066482
%     UPPAAL    0.0072                
% Thermostat    FDR    0.0052    7    16    5    0.4375

%------------------------------------------------------
% However, 


% To Check??
% In these evaluations we consider traces of size up to ...

%ToReturn
% \begin{cmt}
% In these evaluations we consider traces of size up to ...
% \end{cmt}



Considering that the experimental approach with trace analysis is an approximation for establishing correctness with a finite set of traces. Covering infinite traces in proving correctness has to be using mathematical proof. 

% correctness for the complete set of traces (including infinite traces) has to be using mathematical proof. 
% This is achieved using structural induction.
% An account of our initial effort to produce a proof is provided next.



% Trace analysis is an approximation to establishing correctness with a finite set of traces. Proving correctness for the complete set of traces involves using mathematical proof to established that each construct of the input model is translated correctly. This is achieved using structural induction \cite{NN07}.  An account of our initial effort to produce a proof by structural induction is provided in the next section.

{ \renewcommand{\arraystretch}{1.2}
\begin{table}[t!]
    \centering
    \caption{An overview of the case studies}
    \label{table_caseStudies}
    \begin{tabular}{|r | c | c | c | c |}  \hline \hline
No. & System &    States  &    Transitions     &   Events     \\ \hline \hline


1 & Thermostat Machine      &      7    &   16            &   5       \\   \hline  \hline


2 & Bookshop Payment System &     7    &   32            &    9       \\   \hline \hline

3 & Simple ATM             &     15  &    33           &  15         \\ \hline \hline
 

4 & AutoBarrier system     &     35    &   84             &  10        \\  \hline \hline
 

5 & Rail Crossing System &     80    &   361            &   12       \\   \hline \hline

    \end{tabular} 
\end{table}
}
% \vspace{-5cm}


\subsection{An Initial Part of Mathematical Proof}
% \subsection{An Initial/Early/Preliminary Mathematical Proof}


%%-------------------------------Math proof
% \subfile{mathProof}

% ????? "You should say that the proof technique is structural induction over the syntax of your fragment of Tock-CSP, and your example is of the simplest base case."

%ToReturn
% This is an overview of our initial proof of the translation rules. We plan to use structural induction over the constructs of the input \tockCSP, within the scope of this translation work. 

Here, we illustrate part of the proof using a translation of the construct $STOP$, one of the base cases of the structural induction. Mathematically TA is defined as tuple \footnote{TA = $(L, l_0, C, A, E, I)$ where $L$ is a set of locations, $l_0$ is the initial location, $C$ is a set of clocks, $A$ is a set of actions, $E$ is a set of edge and $I$ is an invariant.}  (Section \ref{background}). Consider \lstinline{TA1} as the translation of the process \lstinline{STOP}, that is \lstinline{TA05} in Figure \ref{fig_interrupt}, then mathematically TA1 is express as follow.


% Our plan is to use mathematical induction in proving the translation rules.
% One of the base case is the translation of the construct $STOP$. The proof of the base case is as follow.



% \vspace{0.3cm}
% From Section \ref{background}, Mathematically, a TA is tuple, 

% % \[ TA = (L, l_0, C, A, E, I)  \]
% \begin{equation} \label{ta}
%     TA = (L, l_0, C, A, E, I)
% \end{equation}


\vspace{-0.7cm}
\begin{multline*}
TA1 =   ( \{s1, s2\}, s1,  \{ck\}, \{startID01\_4, tock\}, \\ 
        \{(s1, startID01\_4, \emptyset, \emptyset, s2), (s2, tock, ck\le1, ck, s2) \}, \{\} )
\end{multline*}


% \[ TA1 =   ( \{s0, s1\}, \ s0, \  \{ck\},  \ \{startID, tock\}, \  \{(s0, startID, , , s1), (s1, ck, tock, ck\le1, s1) \}, \ \{\} ) \]


% According to Alur \cite{AD94} and Bouyer \cite{B11}, in


% ?? Check path and trace again ??

%------------------------------------
% \noindent
% In TA, a path \cite{AD94, B11} is a sequence of consecutive transitions that begins from the initial state. There is only one path in TA1, as follows. 

% \begin{equation}
%  path =  \{ \langle (s0, startID, \emptyset, \emptyset, s1), (s1, tock, ck\le1, ck, s1) \rangle   \}   
% \end{equation}

% \noindent
% Also, a trace \cite{AD94, B11} (or word in the language of TA) is a sequence of actions in a given path. Therefore, a trace of TA1 is as follows.
%------------------------------------



\noindent
In the language of TA, a path \cite{AD94, B11} is a sequence of consecutive transitions that begins from the initial state; may possibly be an empty sequence. A trace \cite{AD94, B11} (or word) is a sequence of actions in a given path. In \lstinline{TA1}, there is only one infinite path; the first transition from location $s1$ to location $s2$ and the second transition from location  $s2$ and return to location $s2$, repeated infinitely ($s2$ to $s2$). The traces on the path are as follows.

% Similarly, according to Alur \cite{AD94} and Bouyer \cite{B12}, a trace (or word in the language of TA) is a sequence of action in a given path.

\vspace{-0.1cm}
\begin{equation}
traces'_{TA}(TA1) =  \{  \langle \rangle \}  \cup   \{ \langle startID01\_4 \rangle ^ \frown  \langle tock  \rangle ^ n \mid n \in N  \} 
\end{equation}

\vspace{0.1cm}

% \begin{equation}
% traces'_{TA}(TA1) =  \{  \langle \rangle,  \langle startID00 \rangle  \cat \langle tock \rangle^n  \} \ \ \ \ \ \ n = 0,1,2 \dots     
% \end{equation}

\noindent
The function $trace'_{TA}(TA)$ describes the traces of TA1 as follows. The first empty sequence happens at the initial state, before the first transition. The action \verb!startID00! happens on the first transition. The action \verb!tock! happens on the second transition, which is repeated infinitely for the infinite traces $\langle tock  \rangle ^ n $.

% % Thus, the function $traces'_{TA}(TA)$ starts from the initial location \lstinline{(l0)} of the first TA in the list of input TA, and traverse the network of TA to return a list of associated actions of the transitions on the path.



% % \[ traces_{TA}(TA) =  \{ [ \langle \rangle] ], \ [ \langle startID \rangle], \ [ \langle startID, tock^n \rangle]]  \} \]

% % \noindent
% % The function $traces'_{TA}(TA)$ starts from the initial location \lstinline{(l0)} of the first TA in the list of input TA, and traverse the network of TA to return a list of associated actions of the transitions on the path.

% %, as described in the definition of traces above.

% % For example, let \lstinline{TA1} be the first TA in Figure \ref{stop_ta1} then
% % \[ traceTA(TA1) =  \{ \langle startID, tock \rangle  \} \]


% %ToReturn
% % For example, in Figure \ref{stop_ta1}, starting from the left TA that has an initial location \lstinline{s0}, the first transition connects the two locations \lstinline{s0} and \lstinline{s1} with the action \lstinline{startID01}, and the trace becomes $ \{ \langle startID01 \rangle \}$. After that, the second transition from location \lstinline{s1} to itself \lstinline{s1} for the action \lstinline{tock}, and the trace becomes $ \{ \langle startID01, tock \rangle \}$. This second transition is repeated infinitely to create infinite series of the actions  $\lstinline{tock}^n$, and the trace becomes $ \{ \langle startID01,\ tock^n \rangle \}$.


Another function $trace_{TA}(TA)$ is similar to $traces'_{TA}(TA)$ but removes all the coordinating actions (Definition \ref{coordinating_action}) from the traces.
% % , which we use in this work.

% \vspace{-0.3cm}
% \begin{equation}
% traces_{TA}(TA1) =  traces'_{TA}(TA1) \backslash  CoordinatingActions
% \end{equation}

\vspace{-0.5cm}
\begin{equation}
traces_{TA}(TA) = \{ t \ \backslash  \ CoordinatingActions \mid t \in traces'_{TA}(TA)  \}
\end{equation}


% \noindent
% The function $trace'_{TA}(TA)$ takes a list of TA and returns set of traces without the coordinating actions. In Equation (3), we use the operator $\backslash$  for removing the coordinating actions from the set of traces. For instance, after removing the coordinating actions the traces of TA1 are as follows.

% % So, the function $trace'_{TA}(TA)$ takes a list of TA and returns set of traces without the coordinating actions. 

\noindent
Therefore, without the coordinating actions the traces of TA1 become.

 \vspace{-0.1cm}
\begin{equation}
traces_{TA}(TA1) = \{ \langle tock \rangle ^ n  \mid n \in N  \}
\end{equation}


% % \[ trace_{TA}(TA)  = traces(TA) \backslash CoordinatingActions   \]


% % This sections discusses the mathematical proofs  to setup a path for proving total correctness of the translation technique, which we developed in this work. The mathematical proof will establish that the traces of tock-CSP are similar to the traces of the translated TA in the following steps.

% % We plan to use Mathematical proof to establish that the traces of tock-CSP are similar to the traces of the translated TA in the following steps.

% %We plan to use this mathematical proof to establish that  

% \vspace{0.2cm}

% % \noindent
% % For this proof, our goal is establishing that the traces of \tockCSP models are the same as those of the translated TA models.
% %This is describe in the following steps.

% % \vspace{-0.5cm}
% % \begin{equation}
% %  traces_{tock-CSP}( \lstinline{tock-CSP}) \equiv traces_{TA}(transTA(\lstinline{tock-CSP}))    
% % \end{equation} 

% \noindent
\vspace{-0.2cm}
\begin{proof}
For this proof, our goal is to establish the traces of \tockCSP{} models are the same as those of the translated TA models. Here, \lstinline{transTA} is the translation function we have formalised (See Section \ref{trans_rule}) for translating \tockCSP{} models into TA models.  Thus, we need to establish that, for each valid \tockCSP{} process \lstinline{P}, within the scope of this work, as follows.
\end{proof}


 \vspace{-0.5cm}
\begin{equation}
traces_{tock-CSP}(P) = traces_{TA}(transTA(P)) 
\end{equation}

% \[ traces_{tock-CSP}(P) == traces_{TA}(transTA(P))   \]

% \vspace{0.2cm}
% In this case, for each translation rule we need to proof that the translated TA captures the behaviour of the translated construct of the \verb!tock-CSP!. Thus, starting with Rule \ref{rule_STOP} for the construct of a constant process \lstinline{STOP}:

\noindent
In this case, for each translation rule, we need to prove the translated TAs capture the behaviour of the corresponding input \tockCSP{} model. Thus, we use automatic proof, express in Haskell, starting from the translation of the basic process \lstinline{STOP}:

% first rule for translating the construct of a basic process

% \subsubsection{Proof for the Construct STOP $(Base \ case)$ }
% We start with the first rule (translation the construct of a basic process $STOP$; the first construct of the BNF (Section \ref{BNF_tockCSP}). For the proof by induction, we need to establish that: 
% % we are going to show that:



% \vspace{-0.5cm}
\begin{lstlisting}[numbers=left,numbersep=7pt, language=Haskell, breaklines=true, basicstyle=\ttfamily\small ]
         traces_tockCSP STOP = traces_TA (transTA STOP)
\end{lstlisting}     


% \begin{equation}
%      traces_{tock-CSP}(STOP) =  traces_{TA}(transTA(STOP)) 
% \end{equation}

\noindent
Thus, we need to show that
\begin{lstlisting}[numbers=left,numbersep=7pt, language=Haskell, breaklines=true, basicstyle=\ttfamily\small ]
  (traces_tockCSP n STOP = traces_TA n (transTA STOP)) 
    => (traces_tockCSP (n+1) STOP = traces_TA (n+1) (transTA STOP))
\end{lstlisting}

\noindent
This is illustrated as follows:
% -- Base case: STOP 
% We need to show that
\begin{lstlisting}[numbers=left,numbersep=7pt, language=Haskell, breaklines=true, basicstyle=\ttfamily\small, mathescape=true ]        
-- (traces_tockCSP n STOP = traces_TA n (transTA STOP)) 
--   => (traces_tockCSP (n+1) STOP = traces_TA (n+1) (transTA STOP))
proofTrans    STOP        n   =   
    traces_tockCSP (n+1) STOP
    :=: --{traces_tockCSP.stop, n<$\sim$n+1}
    [(replicate l "tock") | l <- [0..n+1]]
    :=: --{List comprehensions }
    [(replicate l "tock") | l <- [0..n]] ++ [replicate (n+1) "tock"]
    :=: --{traces_tockCSP.stop}
    (traces_tockCSP n STOP) ++ [replicate (n+1) "tock"]
    :=: --{Induction hypothesis} 
    nub ((traces_TA n (transTA STOP "ta" 0 0 0 [])) 
        ++ [replicate (n+1) "tock"])
    :=: --{transTA.stop, l$\sim$>r}
    nub (traces_TA n taSTOP
         ++ [replicate (n+1) "tock"])
    :=: --{tracesTA.n, l$\sim$>r, tas<$\sim$STOP}
    nub ([t \\ ["startID0_0"] | 
           t <- (traces'TA n taSTOP ) ] 
         ++ [replicate (n+1) "tock"] )
    :=: --{traces'TA.stop, l$\sim$>r}
    [t \\ flowActions taSTOP 
            |t <- ([("startID0_0"):s 
                |s <- [(replicate l "tock")|l <- [0..n] ] ] ) ] 
    ++ [replicate (n+1) "tock"]
    :=: --{Introducing the connection action}   
    [t \\ flowActions taSTOP 
        | t <- ([("startID0_0"):s
            |s <- [(replicate l "tock")|l <- [0..n] ] ])  ] 
    ++ [ t \\ ["startID0_0"] 
            | t <- [["startID0_0"] ++ (replicate (n+1) "tock")] ]
    :=: --{List comprehensions}
    [t \\ flowActions taSTOP 
            | t <- ([("startID0_0"):s
                |s <- [(replicate l "tock")|l <- [0..n+1] ] ] ) ]
    :=: --{traces'TA.stop, r$\sim$>l} 
    nub ([t \\ flowActions taSTOP   
           | t <- (traces'TA (n+1) taSTOP ) ] )
    :=: --{tracesTA.n, r$\sim$>l, n<$\sim$n+1, tas<$\sim$taSTOP}                           
    nub (traces_TA  (n+1)  taSTOP )
    :=: --{trans.stop, r->l}
    nub (traces_TA   (n+1)  (transTA STOP "ta" 0 0 0 []))
    :=: QED
        where 
           taSTOP = [([ "s0", "s1"], "s0",  ["ck"], ["startID0_0"], ["tock"], [("s0", "startID0_0", [], [], "s1"), ("s1", "tock", "ck<=1", "ck", "s1")], [] )] 
\end{lstlisting}


\begin{lstlisting}[numbers=left,numbersep=7pt, language=Haskell, breaklines=true, basicstyle=\ttfamily\small, numbers=none, mathescape=true] 
    $\therefore$  traces_tockCSP (n+1) STOP = traces_TA (n+1) (transTA STOP)
\end{lstlisting}

\noindent
Each step is evaluated automatically, which helped us prove that the traces of the translated TA for $STOP$ captures its traces correctly. 

% In this section, w
Here, we provide an overview of the proof by illustrating proof for the base case (STOP). Additional details of the proof are in the extended report \cite{extendedVersion}.


% In this section, we provide an overview of the proof by illustrating proof for the base case (STOP). Additional details of the proof are included in the extended report of this work \cite{extendedVersion}.

% In this section, we provide an overview of the proof with illustration of the proof for the base case (STOP). Additional details of the proof is included in the extended report of this work \cite{extendedVersion}.



%---------------------------------------------------------
% % In this case, we need to establish that, each construct of the tock-CSP has similar behaviour with the equivalent translated TA. This means that we have to use mathematical proof to establish the correctness of translating each construct, that is the list of the translation rules. Thus, starting with Rule \ref{rule_STOP} for the construct of a constant process \lstinline{STOP}:

% % \vspace{-0.3cm} 

% \begin{equation}
%      traces_{tock-CSP}(STOP)  = traces_{TA}(transTA(STOP)) 
% \end{equation}
% % \[ traces_{tock-CSP}(STOP) == traces_{TA}(transTA(STOP))   \]


% \vspace{0.3cm}
% \noindent
% For the LHS, in \tockCSP{} \cite{R10}, the traces of the constant process \lstinline{STOP} are:

% \begin{equation} \label{lhs}
%   traces_{tock-CSP}(STOP) = \{ \langle startID00 \rangle  ^ \frown \langle tock \rangle ^ n  \mid n \in N  \}
% \end{equation}



% % \begin{equation} \label{lhs}
% %   traces_{tock-CSP}(STOP) = \{ \langle startID00 \rangle  \cat \langle \mathit{tock}^n \rangle \mid n \in N  \}
  
% %   \{ \langle tock \rangle ^n \}   \ \ \ \ \ \ \ n = 0,1,2 \dots
% %  \end{equation}

% % \begin{equation}
% % traces_{tock-CSP}(STOP) = \{\langle\rangle, \langle tock ^n \rangle \}     
% % \end{equation}

% % \[ traces_{tock-CSP}(STOP) = \{\langle\rangle, \langle tock \rangle \}  \]

% % \vspace{0.3cm}
% % \noindent
% % For the RHS, the traces of the translated TA are as follows.
% % \[ traces_{TA}(transTA(STOP))  \] 
% %--------------------


% \vspace{0.2cm}
% \noindent
% For the RHS, Example \ref{ex_STOP} produces TA1 that captures the translation of construct $STOP$, then the traces of TA1 are as follows.
% % For the RHS, Example \ref{ex_STOP}, describes the translation of the construct $STOP$. Let TA1 be the first TA, which captures the translation of construct $STOP$, then the traces of TA1 are as follows.


% \begin{equation}
% traces'_{TA}(TA1) = \{  \langle \rangle \}  \cup   \{ \langle startID00 \rangle ^ \frown \langle tock  \rangle ^ n  \mid n \in N  \}
% \end{equation}



% % \begin{equation}
% % % \{ \langle \rangle, \ \langle startID00 \rangle \cat \langle tock \rangle ^n    \}     \ \ \ \ \ \ \ n = 0,1,2 \dots
% % \end{equation}
% % % \[ traceTA(TA1) =  \{ [<>], \ [<startID>], \ [<startID, tock>^n]]  \} \]


% % \[ traces_{TA} \{ \]

% % \begin{figure}[H]
% %     \centering
% %     \includegraphics[width=0.3\textwidth]{C4_figs/stopTrace.jpg}
% %     % \caption{Caption}
% %     % \label{fig:my_label}
% % \end{figure}

% % \Verb!                      } !


% \vspace{0.2cm} 
% \noindent
% After dropping the flow actions, the traces become:
% \vspace{-0.1cm}
% \begin{equation} \label{rhs}
% traces_{TA}(TA1) = \{ \langle \mathit{tock}^n \rangle \mid n \in N  \}
% \end{equation} 

% % \[  traceTA(TA1) =  \{ [\langle \rangle], [\langle tock \rangle ^n]]  \} \]



% \vspace{0.2cm}
% \noindent
% Therefore, from Equations (\ref{lhs}) and (\ref{rhs}), 
% \[ traces_{tock-CSP}(STOP) = traces_{TA}(transTA(STOP))  \]
% % \[ \ \ traces( \lstinline{tock-CSP}) == traces(transTA(\lstinline{tock-CSP}))  \]

% % \[ That \ is \ \ \{ [\langle \rangle], [\langle tock \rangle ^n]] \} == \{ [\langle \rangle], [\langle tock \rangle^n] \}  \]


% \noindent
% This proves that the traces of the translated TA for $STOP$ captures its traces correctly. Additional details of the mathematical proof is available in the extended report of this work \cite{extendedVersion}.

% We plan to follow the same pattern in completing the proof.

% We plan to proof all the remaining rules to establish the correctness of the translation rules that will cover infinite traces.

% This proves that the traces of the translated TA for the construct STOP captures its traces. We plan to proof all the remaining rules to establish the correctness of the translation rules that will cover infinite traces.







%% ----------------------------- RELATED WORK
\section{Related Work}
\label{related_work}


%Toreturn
% Several types of research explore using CSP in verifying temporal specifications, due to its potential capability of verifying real-time systems. 

Timed-CSP \cite{S10} is another popular extension of CSP that provides additional notations for capturing temporal specifications. Unlike \tockCSP, Timed-CSP records the progress of time with a series of positive real numbers, which facilitates reasoning in a format that is suitable for verifying real-time systems. However, the approach of Timed-CSP can not specify strict progress of time, neither deadline nor urgency. Additionally, traces of Timed-CSP become infinite, which is problematic for automatic analysis and verification \cite{R10}. Thus, there is no tool support for verifying Timed-CSP models. As a result of that, many researchers explore model transformations in supporting Timed-CSP with an automated verification tool. Timed-CSP has been translated into \tockCSP{} for using FDR in automatic verification \cite{O00}.

%ToReturn
%The work provides a link for utilising the facilities \tockCSP{} and its supporting tool FDR in verifying Timed-CSP model. 



%ToReturn
% Also, Timed-CSP has been translated into \uppaal \ to facilitate using the facilities of \uppaal \ in verifying Timed-CSP. 


Also, Timed-CSP has been translated into \uppaal. The work was initiated in \cite{DH08} and then subsequently improved in \cite{TS13}. Additionally, Timed-CSP has been translated into Constraint Logic Programming (CLP)  that facilitates reasoning with the support of the constraint solver CLP(R) \cite{DP06}.


However, there is less attention in applying the same transformation techniques in improving \tockCSP{}. An attempt for transforming TA into \tockCSP{} was proposed in \cite{K11}. Whereas in this work, we consider the opposite direction.
% of the proposed translation. 

%ToReturn
%translation \tockCSP{} into TA for \uppaal \ to be able to utilise the facilities of TA and \uppaal \ in verifying \tockCSP{} models.
 


%ToReturn -------------------------------------------
% Furthermore, another approach of reducing the complexity of refusal testing was provided in \cite{DR16}, which introduces a translation technique for using priority operator \cite{R10} to transform a question for refusal testing refinement into trace refinement. The technique is generalised to be applicable to the remaining three observational CSP models, namely acceptances, revivals, and finite linear observations \cite{R05}, all with the same motivation of reducing complexity and providing support for automatic verification for these four behavioural models. 

% However, their translation technique \cite{DR16} is limited to finite linear-time. While our translation work targets at using  Timed Computation Tree Logic (TCTL) that is powerful enough to cover branching time. Part of the future work will expand the comparison of our translation work with their approach of translating the refusal testing into trace models. 
%---------------------------------------------------


Apart from CSP and TA, model transformations have been used for improving various formal modelling notations. For instance, Circus has been translated into \lstinline{CSP||B} to use the tool ProB for automatic verification \cite{KJ17}. Additionally, the language B has been translated into TLA+ for automatic validation with TLC \cite{HL14}. Also, translating TLA+ to B has been investigated for automated validation of TLA+ with ProB \cite{HL12}, such that both B and TLA+ benefit from the resources of each other, specifically their supporting tools ProB and TLC, respectively, for automated verification. 


Model transformation is an established field, which has been used in addressing computational problems, for many decades, here we also consider model transformation, however, the novelty of this translation work is traced back to the early days of model translation works, such as the translation of the timed variants of LOTOS into TA \cite{CO95, HG98}. There is a recent systematic survey of model translation, which provides a rich collection of model transformations techniques and their supporting tools \cite{KM19}.

% A recent survey on model translation provides rich collections of model transformations techniques and their supporting tools \cite{KM19}.









\section{Conclusion}
\label{conclusion}

%-------------  CONCLUSION  --------------------------------------------------

In this work, we have presented a technique for translating \tockCSP{} into TA for \uppaal, which facilitates using temporal logic and automatic support with \uppaal \ in verifying \tockCSP{} models. This work provides an easier way of using TCTL in specifying liveness requirements that are difficult to specify and verify in \tockCSP{} with refinement models. Also, the result of this work sheds additional insight into the complex relationship between \tockCSP{} and TA, as well as the connection between the refinement model and temporal logic model. 


So far, we have used trace analysis in justifying the correctness of the translation work. In the future, first, we will complete the mathematical proof for the total correctness of the translation technique. Second, in this work, we cover the essential operators of \tockCSP{}. Next, we will expand the work to cover the remaining operators of \tockCSP{}, to help us translate extensive case studies. 
% to help us improve the the translation technique.
% of \tockCSP{} to \uppaal.  


Currently, we translate the event \lstinline{tock} into an action that is controlled by a timed clock in \uppaal.  A recommended next step is relating the notion of \lstinline{tock} to the notion of time in TA and getting rid of \lstinline{tock} as an action.  This additional extension will help us explore additional interesting facilities of \uppaal{} for verifying temporal specifications. Also, as part of the future work, a better understanding of relating \tockCSP{} to TA will help us explore using single TA instead of network TAs for more efficient verification.





==> ref.tex <==
@article{BS90,
abstract = {Although the theory of asynchronous circuits (fates back to the early 1950s, considerable progress has been made in this area in the past five years. This paper constitutes the first part of a two-part survey of the recent advances in this field. Part I of the survey presents a unified and concise overview of those aspects of the theory that (leaf with the behaviour of circuits under the assumption that delays in the circuit components and wires are unbounded. The historical development of the subject is presented, and some shortcomings of the earlier approaches are discussed. Ternary simulation is related to the binary analysis methods; the ternary approach is then used to correct the flaws in the earlier work. The question of realizability of sequential behaviors is then considered. It is shown that the class of realizable behaviors is rather severely restricted by the unbounded-delay assumption and that the use of bounded-delay models is more realistic. Part 11 of the survey will deal with bounded-delay models, MOS circuits, classical and delay-insensitive design methods, and complexity issues.},
author = {{J.A Brzozowski} and {C.J.H. Seger}},
journal = {Bull. Eur. Assoc. Theor. Comput. Sci. EATCS, Vol. 42(1990), No. October, p. 198-249},
title = {{Advances in asynchronous circuit theory. Part I : gate and unbounded inertial delay}},
year = {1990}
}

%[BRICS]
@inproceedings{BRICS,
  title={Brics-best practice in robotics},
  author={Bischoff, Rainer and Guhl, Tim and Prassler, Erwin and Nowak, Walter and Kraetzschmar, Gerhard and Bruyninckx, Herman and Soetens, Peter and Haegele, Martin and Pott, Andreas and Breedveld, Peter and others},
  booktitle={Robotics (ISR), 2010 41st International Symposium on and 2010 6th German Conference on Robotics (ROBOTIK)},
  pages={1--8},
  year={2010},
  organization={VDE}
}

%[Rosta]
@article{Rosta,
  title={The use of reuse for designing and manufacturing robots},
  author={Prassler, Erwin and Bruyninckx, Herman and Nilsson, Klas and Shakhimardanov, Azamat},
  journal={White Paper},
  year={2009}
}

%[OPros}
@inproceedings{OPros,
  title={An introduction to robot component model for opros (open platform for robotic services)},
  author={Song, Byoungyoul and Jung, Seungwoog and Jang, Choulsoo and Kim, Sunghoon},
  booktitle={Proceedings of the International Conference Simulation, Modeling Programming for Autonomous Robots Workshop},
  pages={592--603},
  year={2008}
}




%[orocos]
%http://www.orocos.org/
@misc{orocos,
keywords = {orocos},
mendeley-tags = {orocos},
title = {The orocos project, smarter control in robotics and automation 2018},
url ={http://www.orocos.org/ (Accessed: 18th September, 2018)},
journal={Orocos.org},
}


@article{B11,
  title={An introduction to timed automata},
  author={Bouyer, Patricia},
  journal={Actes {\'E}cole d’{\'e}t{\'e} ETR’05},
  pages={79--94},
  year={2011}
}


@phdthesis{Alur91,
author = {Alur, Rajeev},
file = {:home/abdul/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Alur - 1991 - TECHNIQUES FOR AUTOMATIC VERIFICATION OF REAL-TIME SYSTEMS.pdf:pdf},
keywords = {Alu91},
mendeley-tags = {Alu91},
title = {{TECHNIQUES FOR AUTOMATIC VERIFICATION OF REAL-TIME SYSTEMS}},
year = {1991}
}


@article{KK99,
author = {Katoen, J.P. and Katoen, J.P.},
journal = {Arbeitsberichte des},
keywords = {KK99},
mendeley-tags = {KK99},
number = {32},
pages = {1},
title = {{Concepts, algorithms, and tools for model checking}},
url = {http://scholar.google.com/scholar?hl=en{\&}btnG=Search{\&}q=intitle:Concepts,+Algorithms,+and+Tools+for+Model+Checking{\#}0},
volume = {2501},
year = {1999}
}
@article{KF07,
abstract = {Recently, Linear Temporal Logic (LTL) has been successfully applied to high-level task and motion planning problems for mobile robots. One of the main attributes of LTL is its close relationship with fragments of natural language. In this paper, we take the first steps toward building a natural language interface for LTL planning methods with mobile robots as the application domain. For this purpose, we built a structured English language which maps directly to a fragment of LTL.},
author = {Kress-Gazit, Hadas and Fainekos, Georgios E. and Pappas, George J.},
doi = {10.1109/IROS.2007.4398998},
isbn = {1424409128},
issn = {0169-1864},
journal = {IEEE Int. Conf. Intell. Robot. Syst.},
keywords = {KF07},
mendeley-tags = {KF07},
pages = {2717--2722},
title = {{From structured english to robot motion}},
year = {2007}
}
@misc{,
title = {{Frob A language for declarative robotic programming}}
}
@article{Vanthienen2013,
abstract = {Current state-of-the-art robot program development needs expert programmers. Moreover, most robot programs developed today are robot hardware and software specific, and therefore little reusable without modifications. This paper realizes easier robot (re-)programming, by software framework independent models that can be executed using different hard- and software platforms. First, the paper focuses on the formalization of the tasks to be fulfilled by a robot, more specifically constraint-based programming tasks using a Domain Specific Language (DSL). Second, it gives a reference implementation in Lua [1]. The presented DSL makes it easy to develop applications, yet is powerful to execute. It enables automatic model verification and code generation for different hard- and software platforms, diminishing code debugging efforts. Experimental validation shows the ease of creating an application and adapting it, the reduction of the amount of hand-written code, and the debugging aid offered through meaningful errors returned by model verification.},
author = {Vanthienen, Dominick and Klotzbuucher, Markus and {De Schutter}, Joris and {De Laet}, Tinne and Bruyninckx, Herman},
doi = {10.1109/IROS.2013.6696602},
isbn = {9781467363587},
issn = {21530858},
journal = {IEEE Int. Conf. Intell. Robot. Syst.},
pages = {1860--1866},
title = {{Rapid application development of constrained-based task modelling and execution using domain specific languages}},
year = {2013}
}
@book{HN14,
abstract = {Much of the technology that makes robots reli-able, human friendly, and adaptable for numerous applications has emerged from manufacturers of industrial robots. With an estimated installation base in 2014 of about 1:5 million units, some 171 000 new installations in that year and an annual turnover of the robotics industry estimated to be US{\$} 32 billion, industrial robots are by far the largest commercial application of robotics tech-nology today. The foundations for robot motion planning and control were initially developed with in-dustrial applications in mind. These applications deserve special attention in order to understand the origin of robotics science and to appreciate the many unsolved problems that still prevent the wider use of robots in today's agile manufac-turing environments. In this chapter, we present a brief history and descriptions of typical indus-trial robotics applications and at the same time we address current critical state-of-the-art techno-logical developments. We show how robots with different mechanisms fit different applications and how applications are further enabled by latest technologies, often adopted from technological fields outside manufacturing automation. We will first present a brief historical intro-duction to industrial robotics with a selection of contemporary application examples which at the same time refer to a critical key technology. Then, the basic principles that are used in industrial robotics and a review of programming methods 54.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {H{\"{a}}gele, Martin and Nilsson, Klas and Pires, J. Norberto and Bischoff, Rainer},
booktitle = {Springer Handb. Robot.},
doi = {10.1007/978-3-319-32552-1},
eprint = {arXiv:1011.1669v3},
isbn = {978-3-319-32550-7},
keywords = {HN14},
mendeley-tags = {HN14},
pmid = {25246403},
title = {{Industrial Robotics}},
year = {2016}
}
@article{N15,
author = {Nordmann, Arne},
isbn = {9781479969234},
keywords = {N15},
mendeley-tags = {N15},
number = {August},
pages = {5032--5039},
title = {{Modeling of Motion Primitive Architectures using Domain-Specific Languages}},
year = {2015}
}
@inproceedings{AH10,
abstract = {During the last two decades, software development has evolved continuously into an engineering discipline with systematic use of methods and tools to model and implement software. For example, object-oriented analysis and design is structuring software models according to real-life objects of the problem domain and their relations. However, the industrial robotics domain is still dominated by old-style, imperative robot programming languages, making software development difficult and expensive. For this reason, we introduce the object-oriented Robotics Application Programming Interface (Robotics API) for developing software for industrial robotic applications. The Robotics API offers an abstract, extensible domain model and provides common functionality, which can be easily used by application developers. The advantages of the Robotics API are illustrated with an application example.},
author = {Angerer, Andreas and Hoffmann, Alwin and Schierl, Andreas and Vistein, Michael and Reif, Wolfgang},
booktitle = {2010 IEEE/RSJ Int. Conf. Intell. Robot. Syst.},
doi = {10.1109/IROS.2010.5649098},
isbn = {978-1-4244-6674-0},
keywords = {AH10,application program interfaces,application programming interface,imperative robot programming languages,industrial robotics,industrial robots,object-oriented analysis,object-oriented design,object-oriented framework,object-oriented programming,robot programming,robotics API,software development,software engineering,software models},
mendeley-tags = {AH10},
title = {{The Robotics API: An object-oriented framework for modeling industrial robotics applications}},
year = {2010}
}
@article{M04,
abstract = {Cyberbotics Ltd. develops WebotsTM, a mobile robotics simulation software that provides you with a rapid prototyping environment for modelling, programming and simulating mobile robots. The provided robot libraries enable you to transfer your control programs to several commercially available real mobile robots. WebotsTM lets you define and modify a complete mobile robotics setup, even several different robots sharing the same environment. For each object, you can define a number of properties, such as shape, color, texture, mass, friction, etc. You can equip each robot with a large number of available sensors and actuators. You can program these robots using your favorite development environment, simulate them and optionally transfer the resulting programs onto your real robots. WebotsTM has been developed in collaboration with the Swiss Federal Institute of Technology in Lausanne, thoroughly tested, well documented and continuously maintained for over 7 years. It is now the main commercial product available from Cyberbotics Ltd.},
archivePrefix = {arXiv},
arxivId = {cs/0412052},
author = {Michel, O.},
doi = {10.1.1.86.1278},
eprint = {0412052},
isbn = {978-3-642-45345-8},
issn = {1729-8806},
journal = {Int. J. Adv. Robot. Syst.},
keywords = {MO4,commercial software,mobile robot simulation,rapid prototyping,transfer to real robots,webots tm},
mendeley-tags = {MO4},
pmid = {14599324},
primaryClass = {cs},
title = {{"Webots TM : Professional Mobile Robot Simulation"}},
year = {2004}
}
@inproceedings{WW13,
abstract = {The UTP theories for {CSP} and Circus can be built by the combination of the theories of designs and reactive processes. Defining the {CSP} operators using reactive design provides a more concise, readable and uniform UTP semantics, and, more importantly, exposes the pre-postcondition semantics of the operators. For Circus Time, a few operators have been defined as reactive designs, but some important operators are still be considered. In this paper, we develop the reactive design semantics of sequential composition, hiding and recursion within Circus Time, and show how to prove some subtle laws using the new semantics. {\textcopyright} Springer-Verlag 2013.},
author = {Wei, Kun and Woodcock, Jim and Cavalcanti, Ana},
booktitle = {Lect. Notes Comput. Sci. (including Subser. Lect. Notes Artif. Intell. Lect. Notes Bioinformatics)},
doi = {10.1007/978-3-642-35705-3_3},
isbn = {9783642357046},
keywords = {Circus Time,Reactive designs,UTP,WW13},
mendeley-tags = {WW13},
title = {{Circus Time with reactive designs}},
year = {2013}
}
@misc{,
title = {{A domain specific modeling language for multiagent systems.pdf}}
}
@article{LC04,
abstract = {The diversity of robotic research areas along with the complex requirements of hardware and software for robotic systems have always presented a challenge for system developers. Many past robot control platforms were complex, expensive, and not very user friendly. Even though several of the previous platforms were designed to provide an open architecture system, very few of the previous platforms have been reused. To address previous disadvantages, this paper describes the design and implementation of the Robotic Platform, an object-oriented development platform for robotic applications. The Robotic Platform includes hardware interfacing, servo control, trajectory generation, 3D simulation, a graphical user interface, and a math library. As opposed to distributed solutions, the Robotic Platform implements all these components in a homogeneous architecture that utilizes a single hardware platform (a standard PC), a single programming language (C++), and a single operating system (the QNX Real-Time Platform) while guaranteeing deterministic real-time performance. This design leads to an open architecture that is less complex, easier to use, and easier to extend. Particularly, the area of multiple cooperating robots benefits from this kind of architecture, since the Robotic Platform achieves a high integration of its components and provides a simple and flexible means of communication. The architecture of the Robotic Platform builds on the following state-of-the-art technologies and general purpose components to further increase simplicity and reliability: (i) PC technology, (ii) the QNX Real-Time Platform, (iii) the Open Inventor library, (iv) object-oriented design, and (v) the QMotor control environment.},
author = {Loffler, M S and Chitrakaran, V and Dawson, D M},
doi = {10.1023/B:JINT.0000010793.21921.13},
journal = {J. Intell. Robot. Syst. Theory Appl.},
keywords = {C (programming language),Computer operating syste,LC04,Multiple cooperating robots,Robot,Robot control,Robotics},
mendeley-tags = {LC04},
title = {{Design and implementation of the robotic platform}},
year = {2004}
}
@article{HS14,
abstract = {In this paper we present our work in progress towards a domain-specific language called Robot Perception Specification Language (RPSL). RSPL provide means to specify the expected result (task knowledge) of a Robot Perception Architecture in a declarative and framework-independent manner.},
archivePrefix = {arXiv},
arxivId = {1408.2933},
author = {Hochgeschwender, Nico and Schneider, Sven and Voos, Holger and Kraetzschmar, Gerhard K.},
eprint = {1408.2933},
keywords = {HS14},
mendeley-tags = {HS14},
title = {{Towards a Robot Perception Specification Language}},
url = {http://arxiv.org/abs/1408.2933},
year = {2014}
}
@article{TH13,
abstract = {This paper introduces the new robot programming language LightRocks(Light Weight Robot Coding for Skills), a domain specific language (DSL) for robot programming. The language offers three different level of abstraction for robot programming. On lowest level skills are coded by domain experts. On a more abstract level these skills are supposed to be combined by shop floor workers or technicians to define tasks. The language is designed to allow as much flexibility as necessary on the lowest level of abstraction and is kept as simple as possible with the more abstract layers. A Statechart like model is used to describe the different levels of detail. For this we apply the UML/P and the language workbench MontiCore. To this end we are able to generate code while hiding controller specific implementation details. In addition the development in LightRocks is supported by a generic graphical editor implemented as an Eclipse plugin.},
author = {Thomas, Ulrike and Hirzinger, Gerd and Rumpe, Bernhard and Schulze, Christoph and Wortmann, Andreas},
doi = {10.1109/ICRA.2013.6630615},
isbn = {9781467356428},
issn = {1050-4729},
journal = {IEEE Int. Conf. Robot. Autom.},
keywords = {Compliant Assembly,Discrete Event Dynamic Automation Systems,Middleware and Programming Environments,Robotic Software,TH13},
mendeley-tags = {TH13},
pages = {461--466},
title = {{A New Skill Based Robot Programming Language Using UML / P Statecharts}},
year = {2013}
}
@book{HJ98,
author = {Hoare, C. A. R and Jifeng, He},
keywords = {HJ98},
mendeley-tags = {HJ98},
publisher = {Prentice Hall College Division.},
title = {{Unifying Theories of Programming}},
url = {http://www.unifyingtheories.org/},
year = {1998}
}
@misc{,
title = {{Genom}}
}



@misc{PRG16,
keywords = {PRG16},
mendeley-tags = {PRG16},
title = {Progression Report Guide},
note = { Available at https://www.cs.york.ac.uk/staff/researchstudy/phdincomputerscience/phdstartedafter31aug2016/studentsfirstyearreport/
(Accessed: 4th September, 2017)}
}


@misc{RafconLink,
keywords = {RafconLink},
mendeley-tags = {RafconLink},
title = {{RAFCON: visual state machine programming}},
note = { Available at http://www.dlr.de/rmc/rm/en/desktopdefault.aspx/tabid-4845/20104{\_}read-47199/  (Accessed: 14th August, 2017)}
}
@article{MR17Auto,
author = {{Alvaro Miyazawa} and {Pedro Ribeiro} and {Wei Li} and {Ana Cavalcanti} and {Jon Timmis}},
keywords = {MR17Auto},
mendeley-tags = {MR17Auto},
journal = {IEEE/RSJ Int. Conf. Intell. Robot. Syst. (forthcoming)},
title = {{Automatic Property Checking of Robotic Applications}},
year = {2017}
}
@article{Schneider2014,
author = {Schneider, Sven and Hochgeschwender, Nico and Kraetzschmar, Gerhard K},
doi = {10.1007/978-3-319-11900-7_20},
issn = {16113349},
journal = {Simulation, Model. Program. Auton. Robot.},
keywords = {SH},
mendeley-tags = {SH},
pages = {231--242},
title = {{Structured Design and Development of Domain-Specific Languages in Robotics}},
year = {2014}
}
@misc{Genom3link,
keywords = {Genom3link},
mendeley-tags = {Genom3link},
title = {{Genom3}},
note = {Available https://git.openrobots.org/projects/genom3/wiki/Wiki}
}
@inproceedings{DP16,
author = {Djuki{\'{c}}, V. and Popovi{\'{c}}, A. and Tolvanen, J. P.},
booktitle = {Proc. 3rd Work. Model. Robot Softw. Eng. (pp. 47-54). ACM.},
keywords = {DP16},
mendeley-tags = {DP16},
title = {{Domain-Specific Modeling for Robotics: From Language Construction to Ready-made Controllers and End-user Applications}},
year = {2016}
}
@article{KW09,
abstract = {This paper discusses the importance and realizability of the$\backslash$n{\&}ldquo;high-level programmability{\&}rdquo; concept for wheeled mobile$\backslash$nrobots. A new high-level mobile robot language, called motion$\backslash$ndescription language (MDL), is proposed. This language has a strong and$\backslash$nstable theoretical foundation. The Java-based object-oriented MDL$\backslash$nimplements the structured robot geometry into its class hierarchy$\backslash$nperfectly. The language MDL is not only {\&}ldquo;a{\&}rdquo; mobile robot$\backslash$nlanguage, but is a strong candidate for {\&}ldquo;the standard{\&}rdquo;$\backslash$nmobile robot language. This innovation will thrust the mobile robotics$\backslash$nfield forward to meet the challenges of the new century head on},
author = {Kanayama, Y.J. and Wu, C.T.},
doi = {10.1109/ROBOT.2000.844078},
isbn = {0-7803-5886-4},
issn = {1050-4729},
journal = {Proc. 2000 ICRA. Millenn. Conf. IEEE Int. Conf. Robot. Autom. Symp. Proc. (Cat. No.00CH37065)},
keywords = {KW09},
mendeley-tags = {KW09},
number = {April},
pages = {329--334},
title = {{It's time to make mobile robots programmable}},
url = {http://ieeexplore.ieee.org/lpdocs/epic03/wrapper.htm?arnumber=844078},
volume = {1},
year = {2000}
}
@article{BD06,
abstract = {UPPAAL 4.0 is the result of over two and a half years of development and contains many new features, additions to the modeling language, performance improvements, enhancements and polish to the easy to use graphical user interface, and is accompanied by several open source libraries. The tool and libraries are available free of charge for academic, educational and evaluation purposes from http://www.uppaal.com/. We describe three of the new features: user defined functions, priorities and symmetry reduction},
author = {Behrmann, Gerd and David, Alexandre and Larsen, Kim G and H{\aa}kansson, John and Petterson, Paul and Wang, Yi and Hendriks, Martijn},
doi = {10.1109/QEST.2006.59},
isbn = {0769526659},
issn = {0-7695-2665-9},
journal = {Third Int. Conf. Quant. Eval. Syst. QEST 2006},
keywords = {BD06},
mendeley-tags = {BD06},
pages = {125--126},
title = {{UPPAAL 4.0}},
year = {2006}
}
@misc{cycabtklink,
keywords = {cycabtklink},
mendeley-tags = {cycabtklink},
title = {{MobileRobotToolkit Website}},
note = { Available at http://cycabtk.gforge.inria.fr/wiki/doku.php  (Accessed: 14th August, 2017) }
}
@inproceedings{urbiscript,
abstract = {Urbi SDK is a software platform for the development of portable robotic applications. It features the Urbi UObject C++ middleware, to manage hardware drivers and/or possibly remote software components, and urbiscript, a domain specific programming language to orchestrate them. Reactivity is a key feature of Urbi SDK, embodied in events in urbiscript. This paper presents the support for events in urbiscript.},
archivePrefix = {arXiv},
arxivId = {1010.5694},
author = {Baillie, Jean-Christophe and Demaille, Akim and Hocquet, Quentin and Nottale, Matthieu},
booktitle = {Work. Domain-Specific Lang. Model. Robot. Syst.},
eprint = {1010.5694},
keywords = {urbiscript},
mendeley-tags = {urbiscript},
title = {{Events! (Reactivity in urbiscript)}},
year = {2010}
}
@article{AL14,
author = {Adam, Sorin and Larsen, Morten and Jensen, Kjeld and Schultz, Ulrik Pagh},
doi = {10.1007/978-3-319-11900-7_18},
isbn = {978-3-319-11900-7},
issn = {16113349},
journal = {Simulation, Model. Program. Auton. Robot. 4th Int. Conf. SIMPAR 2014, Bergamo, Italy, Oct. 20-23, 2014. Proc.},
keywords = {AL14},
mendeley-tags = {AL14},
pages = {207--218},
title = {{Towards Rule-Based Dynamic Safety Monitoring for Mobile Robots}},
url = {http://dx.doi.org/10.1007/978-3-319-11900-7{\_}18},
year = {2014}
}
@article{RK12,
author = {Raman, Vasumathi and Kress-gazit, Hadas},
keywords = {RK12},
mendeley-tags = {RK12},
number = {1},
pages = {1--11},
title = {{Explaining Impossible High-Level Robot Behaviors}},
volume = {14853},
year = {2012}
}
@article{BG09,
abstract = {Autonomous robots are complex systems that require the interaction or cooperation of numerous heterogeneous software components. Nowadays, robots are getting closer to humans and as such are becoming critical systems that must meet safety properties including logical, temporal, and real-time constraints. {\&}copy; 2009 IEEE.},
author = {Bensalem, Saddek and Gallien, Matthieu and Ingrand, F{\'{e}}lix and Kahloul, Imen and Thanh-Hung, Nguyen},
doi = {10.1109/MRA.2008.931631},
journal = {IEEE Robot. Autom. Mag.},
keywords = {BG09,Correct by construction robot controller,Dependable autonomous robot,Validable and verifiable autonomous systems},
mendeley-tags = {BG09},
title = {{Designing autonomous robots: Toward a more dependable software architecture}},
year = {2009}
}
@misc{Ceballos2011,
author = {Ceballos, Antonio and de Silva, Lavindra and Herrb, Matthieu and Ingrand, F{\'{e}}lix and Mallet, Anthony and Medina, Alberto and Prieto, M},
booktitle = {Astra},
number = {2},
pages = {1--7},
title = {{GenoM as a Robotics Framework for Planetary Rover Surface Operations}},
url = {message:{\%}3CE32EBAA6777C584699EDBBDDFA6C2F5C3C9C3EB982@GMVMAIL3.gmv.es{\%}3E},
year = {2011}
}
@article{Gordillo1991,
abstract = {The author describes, {\textless}e1{\textgreater}L{\textless}/e1{\textgreater}{\textless}sub{\textgreater}E{\textless}/sub{\textgreater}, a visual language for specifying verification tasks in the context of the execution of assembly plans. The instructions of {\textless}e1{\textgreater}L{\textless}/e1{\textgreater}{\textless}sub{\textgreater}E{\textless}/sub{\textgreater} have a predicative form, which, being linked in conjunction, imposes conditions on the application of robot actions. These instructions are related to the identification and localization of assembly parts, the verification of the computed trajectory, the verification of the correctness of the object positions, and the verification of the fact that the geometric relations between objects characterizing the manipulation process have been attained. To automatically transform these vision verification tasks into vision programs, the authors defined several data structures by using exhaustively the geometrical and physical object models supporting the system},
author = {Gordillo, J. L.},
doi = {10.1109/ROBOT.1991.131816},
isbn = {0-8186-2163-X},
issn = {10504729},
journal = {Proceedings. 1991 IEEE Int. Conf. Robot. Autom.},
number = {April},
pages = {1433--1439},
title = {{LE: A High Level Language for Specifying Vision Verification Tasks}},
url = {http://ieeexplore.ieee.org/lpdocs/epic03/wrapper.htm?arnumber=131816},
year = {1991}
}
@misc{PR2link,
keywords = {PR2link},
mendeley-tags = {PR2link},
title = {pr2{\_}pbd},
note = { Available at http://wiki.ros.org/pr2{\_}pbd   (Accessed: 14th August, 2017)}
}
@article{SS12,
abstract = {Engineering the software development process in robotics is one of the basic necessities towards industrial- strength service robotic systems. A major challenge is to make the step from code-driven to model-driven systems. This is essential to replace hand-crafted single-unit systems by systems composed out of components with explicitly stated proper- ties. Furthermore, this fosters reuse by separating robotics knowledge from short-cycled implementational technologies. Altogether, this is one but important step towards “able” robots. This paper reports on a practical approach to gain more insights into how a model-driven software approach can be applied to robotics systems.},
author = {Schlegel, Christian and Ha{\ss}ler, T},
doi = {10.5772/25896},
isbn = {978-3-8396-0035-1},
journal = {Int. Conf. Adv. Robot.},
keywords = {SS12},
mendeley-tags = {SS12},
title = {{Robotic software systems: From code-driven to model-driven designs}},
year = {2009}
}
@techreport{Urbi,
author = {Baillie, J. C and {M. Nottale} and {B. Pothier}},
keywords = {Urbi},
mendeley-tags = {Urbi},
title = {{The URBI Tutorial v. 1.5.}},
year = {2007}
}
@article{JH02,
abstract = {This paper introduces means to specify system randomness within UML statecharts, and to verify probabilistic temporal proper-ties over such enhanced statecharts which we call probabilistic UML statecharts. To achieve this, we develop a general recipe to extend a statechart semantics with discrete probability distributions, resulting in Markov decision processes as semantic models. We apply this recipe to the requirements-level UML semantics of [8]. Properties of interest for probabilistic statecharts are expressed in PCTL, a probabilistic variant of CTL for processes that exhibit both non-determinism and probabili-ties. Verification is performed using the model checker Prism. A model checking example shows the feasibility of the suggested approach.},
author = {Jansen, David N and Hermanns, Holger and Katoen, Joost-Pieter},
file = {:home/abdul/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Jansen, Hermanns, Katoen - Unknown - A Probabilistic Extension of UML Statecharts Specification and Verification.pdf:pdf},
keywords = {JH02,Markov decision processes,UML statecharts,model checking,probabilities,semantics},
mendeley-tags = {JH02},
title = {{A Probabilistic Extension of UML Statecharts Specification and Verification}}
}
@book{L09,
abstract = {{\{}In Software Abstractions Daniel Jackson introduces a new approach to software design that draws on traditional formal methods but exploits automated tools to find flaws as early as possible. This approach--which Jackson calls "lightweight formal methods" or "agile modeling"--takes from formal specification the idea of a precise and expressive notation based on a tiny core of simple and robust concepts but replaces conventional analysis based on theorem proving with a fully automated analysis that gives designers immediate feedback. Jackson has developed Alloy, a language that captures the essence of software abstractions simply and succinctly, using a minimal toolkit of mathematical notions. The designer can use automated analysis not only to correct errors but also to make models that are more precise and elegant. This approach, Jackson says, can rescue designers from "the tarpit of implementation technologies" and return them to thinking deeply about underlying concepts. Software Abstractions introduces the key elements of the approach: a logic, which provides the building blocks of the language; a language, which adds a small amount of syntax to the logic for structuring descriptions; and an analysis, a form of constraint solving that offers both simulation (generating sample states and executions) and checking (finding counterexamples to claimed properties). The book uses Alloy as a vehicle because of its simplicity and tool support, but the book's lessons are mostly language-independent, and could also be applied in the context of other modeling languages.{\}}},
author = {Sloane, Anthony M.},
booktitle = {J. Funct. Program.},
doi = {10.1017/S0956796808006977},
isbn = {0262101149},
keywords = {L09},
mendeley-tags = {L09},
title = {{Software Abstractions: Logic, Language, and Analysis by Daniel Jackson, The MIT Press, 2006, 366pp, ISBN 978-0262101141.}},
year = {2009}
}
@article{TP14,
abstract = {FDR3 is a complete rewrite of the {CSP} refinement checker FDR2, incorporating a significant number of enhancements. In this paper we describe the operation of FDR3 at a high level and then give a detailed description of several of its more important innovations. This includes the new multi-core refinement-checking algorithm that is able to achieve a near linear speed up as the number of cores increase. Further, we describe the new algorithm that FDR3 uses to construct its internal representation of {CSP} processes—this algorithm is more efficient than FDR2's, and is able to compile a large class of {CSP} processes to more efficient internal representations. We also give some experimental results that compare FDR3 to related tools, which show it has particularly strong performance in the use of memory and backing store.},
author = {Gibson-Robinson, Thomas and Armstrong, Philip and Boulgakov, Alexandre and Roscoe, A. W.},
file = {:home/abdul/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Gibson-Robinson et al. - 2016 - FDR3 a parallel refinement checker for {CSP}.pdf:pdf},
isbn = {9783642548611},
journal = {Int. J. Softw. Tools Technol. Transf.},
keywords = {{CSP},{FDR},Model-checking,Process algebras,Refinement,TP14},
mendeley-tags = {TP14},
title = {{FDR3: a parallel refinement checker for {CSP}}},
year = {2016}
}

@misc{RPLlink,
keywords = {RPLlink},
mendeley-tags = {RPLlink},
title = {Robot programming languages, Fabryka-robotow.pl},
note = { Available at http://fabryka-robotow.pl/2015/01/programming-languages-to-control-robot   (Accessed: 14th August, 2017) }
}

@article{BF14,
author = {Biggs, Geoffrey and Fujiwara, Kiyoshi and Anada, Keiju},
keywords = {BF14},
mendeley-tags = {BF14},
pages = {146--157},
title = {{Modelling and Analysis of a Redundant Mobile Robot Architecture Using AADL}},
year = {2014}
}
@book{RN14,
abstract = {The long-anticipated revision of this {\#}1 selling book offers the most comprehensive, state of the art introduction to the theory and practice of artificial intelligence for modern applications. Intelligent Agents. Solving Problems by Searching. Informed},
archivePrefix = {arXiv},
arxivId = {arXiv:gr-qc/9809069v1},
author = {Russell, Stuart and Norvig, Peter},
booktitle = {Prentice Hall},
doi = {10.1017/S0269888900007724},
eprint = {9809069v1},
isbn = {9781292024202},
keywords = {RN14},
mendeley-tags = {RN14},
pmid = {15003161},
primaryClass = {arXiv:gr-qc},
title = {{Artificial Intelligence: A Modern Approach, Third edition}},
year = {2014}
}
@article{BS10,
abstract = {—With the increasing complexity of exploration rovers, satellites, and space probes, it has now become a challenge to prove that these systems will behave appropriately/safely in all situations that they may encounter. Such systems make use of complex hardware equipment, but also increasingly complex software. For hardware, one can typically use well known and mastered scientific models (e.g. thermal models, electrical models, mechanical models, and aerodynamic models) to predict how the equipment will behave alone and when integrated into the system. For the software, however, despite the confidence of the programmers who think that their piece of code is as " solid as a rock " and has no flaw (when used alone or with other components), unlike hardware, no scientific formal model exists which can take into account the ever increasing complexity of all the software components. To this end, we present an evolution of the LAAS architecture for autonomous systems, and its tool G en oM. This evolution relies on the BIP component-based design framework, which has been successfully used in other domains such as embedded systems. We integrate BIP into our existing methodology for developing the lowest (functional) level of robots. Particularly, we discuss the componentization of the functional level, the synthesis of an execution controller for it, and how we verify whether the resulting functional level conforms to properties such as deadlock-freedom. Our approach has been fully implemented in the LAAS architecture, and the implementation has been used in several experiments on a real rover.},
author = {Bensalem, Saddek and {De Silva}, Lavindra and Gallien, Matthieu and Ingrand, F{\'{e}}lix and Yan, Rongjie},
file = {:home/abdul/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Bensalem et al. - Unknown - {\&}quot Rock Solid {\&}quot Software A Verifiable and Correct-by-Construction Controller for Rover and Spacecraft.pdf:pdf},
keywords = {BS10},
mendeley-tags = {BS10},
title = {{" Rock Solid " Software: A Verifiable and Correct-by-Construction Controller for Rover and Spacecraft Functional Levels *}}
}
@article{KB12,
abstract = {Coordination is a system-level concern defining execution and interaction semantics of functional computations. Separating coordination from functional computations is a key principle for building complex, robust and reusable robotic systems. This work introduces a minimal variant of Harel statecharts called rFSM designed to model coordination of robotic tasks and systems with a minimal number of semantic primitives. Firstly, the semantics of the rFSM language are derived by analyzing state-of-the-art discrete event models and implementations and extracting a motivated and semantically well-defined subset that is considered best practice for the domain of robotic coordination. Secondly, a real-time capable reference implementation of rFSM is presented, which has been loosely integrated into the OROCOS/RTT framework. The application of rFSM is illustrated using a detailed description of a dual robot coordination problem. Lastly, several best practices and patterns are presented with the goal of i) supporting development of robust Coordination models, ii) illustrating how limitations of the statechart model can be overcome by extending the execution semantics, and iii) offering guidance in designing pure coordination components that optimize reusability.},
author = {Klotzb{\"{u}}cher, Markus and Bruyninckx, Herman},
issn = {2035-3928},
journal = {J. Softw. Eng. Robot.},
keywords = {Component-based system design,Control,Coordination,Domain Specific Language,KB12,Statecharts},
mendeley-tags = {KB12},
number = {January},
pages = {28--56},
title = {{Coordinating Robotic Tasks and Systems with rFSM Statecharts}},
volume = {1},
year = {2012}
}
@article{Gat1991,
abstract = {The author introduces ALFA, a language for programming reactive$\backslash$ncontrol mechanisms for autonomous mobile robots. ALFA programs consist$\backslash$nof networks of computational modules connected by communications$\backslash$nchannels. These channels are themselves computational entities which$\backslash$nperform mediation tasks. This makes it possible to design modular$\backslash$nbehaviors which may be inserted and removed without having to$\backslash$nrestructure the interconnections among modules and allows the system to$\backslash$ninterface cleanly with higher-level reasoning processes. ALFA supports a$\backslash$ndataflow computation model as well as a state-machine model. The results$\backslash$nof two experiments using ALFA to control real robots are briefly$\backslash$ndiscussed},
author = {Gat, E.},
doi = {10.1109/ROBOT.1991.131743},
isbn = {0-8186-2163-X},
issn = {10504729},
journal = {Proceedings. 1991 IEEE Int. Conf. Robot. Autom.},
number = {April},
pages = {1--6},
title = {{ALFA: a language for programming reactive robotic control systems}},
year = {1991}
}
@article{KW17,
abstract = {Ensuring the safety of fully autonomous ve- hicles requires a multi-disciplinary approach across all the levels of functional hierarchy, from hardware fault tolerance, to resilient machine learning, to coop- erating with humans driving conventional vehicles, to validating systems for operation in highly unstructured environments, to appropriate regulatory approaches. Significant open technical challenges include validat- ing inductive learning in the face of novel environ- mental inputs and achieving the very high levels of dependability required for full-scale fleet deployment. However, the biggest challenge may be in creating an end-to-end design and deployment process that inte- grates the safety concerns of a myriad of technical spe- cialties into a unified approach. IEEE},
author = {Koopman, Philip and Wagner, Michael},
doi = {10.1109/MITS.2016.2583491},
isbn = {1939-1390 VO - 9},
journal = {IEEE Intell. Transp. Syst. Mag.},
keywords = {KW17},
mendeley-tags = {KW17},
title = {{Autonomous Vehicle Safety: An Interdisciplinary Challenge}},
year = {2017}
}
@inproceedings{RS13,
abstract = {From exploring planets to cleaning homes, the reach and versatility of robotics is vast. The integration of actuation, sensing and control makes robotics systems powerful, but complicates their simulation. This paper introduces a versatile, scalable, yet powerful general-purpose robot simulation framework called V-REP. The paper discusses the utility of a portable and flexible simulation framework that allows for direct incorporation of various control techniques. This renders simulations and simulation models more accessible to a general-public, by reducing the simulation model deployment complexity. It also increases productivity by offering built-in and ready-to-use functionalities, as well as a multitude of programming approaches. This allows for a multitude of applications including rapid algorithm development, system verification, rapid prototyping, and deployment for cases such as safety/remote monitoring, training and education, hardware control, and factory automation simulation.},
author = {Rohmer, Eric and Singh, Surya P.N. and Freese, Marc},
booktitle = {IEEE Int. Conf. Intell. Robot. Syst.},
doi = {10.1109/IROS.2013.6696520},
isbn = {9781467363587},
issn = {21530858},
pmid = {6696520},
title = {{V-REP: A versatile and scalable robot simulation framework}},
year = {2013}
}
@article{W14,
abstract = {In this paper we present a workflow to design and control robot manipulation behavior. To remain independent from particular robot hardware and an explicit area of application, an embedded domain specific language (eDSL) is used to describe the particular robot and a controller network that drives the robot. We make use of a) a component-based software framework, b) model-based algorithms for motionand sensor processing representations, c) an abstract model of the control system, and d) a plan management software, to describe a sequence of software component networks that generate the desired robot behavior. As first results, we present an eDSL for the description of a robotic system composed of mechatronic subsystems, and for the creation of a multi-stage control network.},
archivePrefix = {arXiv},
arxivId = {1412.3247},
author = {Wirkus, Malte},
doi = {arXiv:1411.7148 [cs.RO]},
eprint = {1412.3247},
journal = {Proc. 5th Int. Work. Domain-Specific Lang. Model. Robot. Syst.},
keywords = {W14},
mendeley-tags = {W14},
title = {{Towards Robot-independent Manipulation Behavior Description}},
year = {2014}
}
@article{Peterson1999,
abstract = {We have applied methodologies developed for domain-specific embedded languages to create a high-level robot control language called Frob, for functional robotics. Frob supports a programming style that cleanly separates the what from the how of a robotic control program. That is, the what is a simple, easily understood definition of the control strategy using groups of equations and primitives which combine sets of these control system equations into a complex system. The how aspect of the program addresses the unpleasant details, such as the method used to realize these equations, the connection between the control equations and the sensors and effectors in the robot, and communication with other elements of the system. Frob is a system that supports rapid prototyping of new control strategies, enables software reuse through composition, and defines a system in a way that can be formally reasoned about and transformed},
author = {Peterson, J. and Hager, G.D. and Hudak, P.},
doi = {10.1109/ROBOT.1999.772516},
isbn = {0-7803-5180-0},
issn = {1050-4729},
journal = {Proc. 1999 IEEE Int. Conf. Robot. Autom. (Cat. No.99CH36288C)},
number = {May},
pages = {1144--1151},
title = {{A language for declarative robotic programming}},
url = {http://ieeexplore.ieee.org/lpdocs/epic03/wrapper.htm?arnumber=772516},
volume = {2},
year = {1999}
}
@article{CW96,
abstract = {Note: OCR errors may be found in this Reference List extracted from the full text article. ACM has opted to expose the complete List rather than only correct and linked references.},
author = {Clarke, Edmund M. and Wing, Jeannette M.},
doi = {10.1145/242223.242257},
journal = {ACM Comput. Surv.},
keywords = {CW96},
mendeley-tags = {CW96},
title = {{Formal methods: state of the art and future directions}},
year = {1996}
}
@article{Fleurey2009,
author = {Fleurey, F and Solberg, A},
doi = {10.1007/978-3-642-04425-0_47},
isbn = {978-3-642-04424-3},
journal = {Model. ACM/IEEE 12th Int. Conf. Model. Eng. Lang. Syst.},
pages = {606--621},
title = {{A Domain Specific Modeling Language supporting Specification, Simulationand Execution of Dynamic Adaptive Systems}},
year = {2009}
}
@article{B05,
abstract = {The growing diversity and complexity of existing robotic devices like humanoids, animal-like robots or wheeled robots, lead to the development of several incompatible software interfaces to control these robots. We believe that there is a need for a standard which could be universal, powerful and easy to use. The open source project URBI, a universal robotic body interface, aims at providing the ground for such a standard. It is based on a client/server architecture where the server is running on the robot and accessed by the client, on the robot or remotely via TCP/IP. The URBI language is a scripted language used by the client and capable of controlling the joints of the robot or access its sensors, camera, speakers or any accessible part of the machine. We present in this article an introduction to URBI and we describe how URBI differs from currently existing solutions. As an example making use of URBI-specific features, we present a simple perturbative approach to walk pattern generation, with URBI running on a ERS7 Aibo robot.},
author = {Baillie, Jean Christophe},
doi = {10.1109/IROS.2005.1545467},
isbn = {0780389123},
issn = {2153-0858},
journal = {2005 IEEE/RSJ Int. Conf. Intell. Robot. Syst. IROS},
keywords = {Aibo,B05,Control architecture and programming,Human-robot interfaces,Programming language,Standard},
mendeley-tags = {B05},
pages = {3219--3224},
title = {{URBI: Towards a universal robotic low-level programming language}},
year = {2005}
}
@inproceedings{KA04,
abstract = {Simulators have played a critical role in robotics research as tools for quick and efficient testing of new concepts, strategies, and algorithms. To date, most simulators have been restricted to 2D worlds, and few have matured to the point where they are both highly capable and easily adaptable. Gazebo is designed to fill this niche by creating a 3D dynamic multi-robot environment capable of recreating the complex worlds that would be encountered by the next generation of mobile robots. Its open source status, fine grained control, and high fidelity place Gazebo in a unique position to become more than just a stepping stone between the drawing board and real hardware: data visualization, simulation of remote environments, and even reverse engineering of blackbox systems are all possible applications. Gazebo is developed in cooperation with the Player and Stage projects (Gerkey, B. P., et al., July 2003), (Gerkey, B. P., et al., May 2001), (Vaughan, R. T., et al., Oct. 2003), and is available from http://playerstage.sourceforge.net/gazebo/ gazebo.html.},
author = {Koenig, N. and Howard, A.},
booktitle = {2004 IEEE/RSJ Int. Conf. Intell. Robot. Syst. (IEEE Cat. No.04CH37566)},
doi = {10.1109/IROS.2004.1389727},
isbn = {0-7803-8463-6},
keywords = {Computational modeling,Educational robots,Friction,Gazebo,KA04,Mobile robots,Open source software,Packaging,Player project,Robot sensing systems,Service robots,Stage project,Testing,Vehicle dynamics,application program interfaces,control engineering computing,digital simulation,grained control,mobile robots,multi-robot systems,open-source multi-robot simulator},
mendeley-tags = {KA04},
title = {{Design and use paradigms for gazebo, an open-source multi-robot simulator}},
year = {2004}
}
@article{PM14,
abstract = {Developing applications considering reactiveness, scalability and re-usability has always been at the center of attention of robotic researchers. Behavior-based architectures have been proposed as a programming paradigm to develop robust and complex behaviors as integration of simpler modules whose activities are directly modulated by sensory feedback or input from other models. The design of behavior based systems, however, becomes increasingly difficult as the complexity of the application grows. This article proposes an approach for modeling and coordinating behaviors in distributed architectures based on port arbitration which clearly separates representation of the behaviors from the composition of the software components. Therefore, based on different behavioral descriptions, the same software components can be reused to implement different applications.},
archivePrefix = {arXiv},
arxivId = {1412.4847},
author = {Paikan, Ali and Metta, Giorgio and Natale, Lorenzo},
eprint = {1412.4847},
journal = {Work. Domain-Specific Lang. Model. Robot. Syst.},
keywords = {PM14},
mendeley-tags = {PM14},
title = {{A Representation of Robotic Behaviors using Component Port Arbitration}},
url = {http://arxiv.org/abs/1412.4847},
year = {2014}
}
@article{ML91,
abstract = {The object-oriented Robot Independent Programming Environment (RIPE), which is being used for the rapid design and implementation of a variety of applications, is described. A system architecture based on hierarchies of distributed multiprocessors provides the computing platform for a layered programming structure that models the application as a set of software objects. These objects are designed to support model-based automated planning and programming, real-time sensor-based activity, error handling, and robust communication. The object-oriented paradigm provides mechanisms such as inheritance and polymorphism which allow the implementation of the system to satisfy the goals of software reusability, extensibility, reliability, and portability. Designing a hierarchy of generic parent classes and device-specific subclasses which inherit the same interface allows a Robot Independent Programming Language (RIPL) to be realized. Workcell tasks demonstrating robot cask handling operations for nuclear waste facilities, which are successfully implemented using this object-oriented software environment, are discussed},
author = {Miller, David J. and Lennox, R. Charleene},
doi = {10.1109/37.67671},
isbn = {0-8186-9061-5},
journal = {IEEE Control Syst.},
keywords = {ML91},
mendeley-tags = {ML91},
title = {{An Object-Oriented Environment for Robot System Architectures}},
year = {1991}
}
@article{NH16,
abstract = {The design, simulation and programming of robotics systems is chal- lenging as expertise from multiple domains needs to be integrated conceptually and technically. Domain-specific modeling promises an efficient and flexible con- cept for developing robotics applications that copes with this challenge. It allows to raise the level of abstraction through the use of specific concepts that are closer to the respective domain concerns and easier to understand and validate. Further- more, it focuses on increasing the level of automation, e.g. through code gen- eration, to bridge the gap between the modeling and the implementation levels and to improve the efficiency and quality of the software development process. Within this contribution, we survey the literature available on domain-specific (modeling) languages in robotics required to realize a state-of-the-art real-world example from the RoboCup@Work competition. We classify 41 publications in the field as reference for potential DSL users. Furthermore, we analyze these con- tributions from a DSL-engineering viewpoint and discuss quantitative and quali- tative aspects such as the methods and tools used for DSL implementation as well as their documentation status and platform integration. Finally, we conclude with some recommendations for discussion in the robotics programming and simula- tion community based on the insights gained with this survey.},
author = {Nordmann, Arne and Hochgeschwender, Nico and Wrede, Sebastian},
doi = {10.1007/978-3-319-11900-7_17},
isbn = {978-3-319-11900-7},
journal = {J. Softw. Eng. Robot.},
keywords = {NH16},
mendeley-tags = {NH16},
number = {July},
pages = {195--206},
title = {{A Survey on Domain-Specific Languages in Robotics}},
volume = {1},
year = {2016}
}
@article{Jacob2012,
author = {Jacob, Jeremy L},
number = {October},
pages = {1--9},
title = {{Selected Solutions to PCOC Practical Exercises Week 3}},
year = {2012}
}
@article{MF02,
abstract = {Robotics systems and software are becoming more and more complex: the need of standard specifications is certainly a key issue in the near future. There is a need to define, from the software point of view, a generic robot. The Orocos project was started to address this problem. It aims at developing a set of robotics software in particular domains and, as a first step, will define a software framework to do that. This paper presents the future evolutions of GenoM (component generator) which we propose as a programming framework in the context of the project. GenoM proposes the definition of generic components that are used to implement robotics functionalities (vision, control, motion planning, ...), and the paper presents the definition of those components. They have been designed so that they can be connected together and externally controlled to form a modular functional layer on robots. We have defined three main entities of which components are made: a set of algorithms, an execution engine, and a communication library. The paper explains their role and presents a formal description language that let us achieves a real decoupling between code of the components (the algorithms) and the execution engine.},
author = {Mallet, a. and Fleury, S. and Bruyninckx, H.},
doi = {10.1109/IRDS.2002.1041609},
isbn = {0-7803-7398-7},
journal = {IEEE/RSJ Int. Conf. Intell. Robot. Syst.},
keywords = {MF02},
mendeley-tags = {MF02},
number = {October},
pages = {2292--2297},
title = {{A specification of generic robotics software components: future evolutions of G/sup en//sub o/M in the Orocos context}},
url = {http://ieeexplore.ieee.org/lpdocs/epic03/wrapper.htm?arnumber=1041609},
volume = {3},
year = {2002}
}
@misc{RapidManual,
author = {{Cortona3D 2017}},
keywords = {RapidManual},
mendeley-tags = {RapidManual},
title = {{Rapid Manual}},
note = { Available at http://www.cortona3d.com/rapidmanual  (Accessed: 14th August, 2017) },
urldate = {2017-08-13},
year = {2017}
}
@inproceedings{DK12,
abstract = {A large number of robotic software have been developed but cannot or can hardly interoperate with each other because of their dependencies on specific hardware or software platform is hard-wired into the code. Consequently, robotic software is hard and expensive to develop because there is little opportunity of reuse and because low-level details must be taken into account in early phases. Moreover, robotic experts can hardly develop their application without programming knowledge or the help of programming experts and robotic software is difficult to adapt to hardware or target-platform changes. In this paper we report on the development of RobotML, a Robotic Modeling Language that eases the design of robotic applications, their simulation and their deployment to multiple target execution platforms. RobotML, a Domain-Specific Language to Design, Simulate and Deploy Robotic Applications (PDF Download Available). Available from: http://www.researchgate.net/publication/232715328{\_}RobotML{\_}a{\_}Domain-Specific{\_}Language{\_}to{\_}Design{\_}Simulate{\_}and{\_}Deploy{\_}Robotic{\_}Applications [accessed Sep 14, 2015].},
author = {Dhouib, Saadia and Kchir, Selma and Stinckwich, Serge and Ziadi, Tewfik and Ziane, Mikal},
booktitle = {Lect. Notes Comput. Sci. (including Subser. Lect. Notes Artif. Intell. Lect. Notes Bioinformatics)},
doi = {10.1007/978-3-642-34327-8_16},
isbn = {9783642343261},
keywords = {DK12,Domain-Specific Languages,Generative Programming,MDE,robotic application},
mendeley-tags = {DK12},
title = {{RobotML, a domain-specific language to design, simulate and deploy robotic applications}},
year = {2012}
}
@article{DZ10,
abstract = {Today's software systems are becoming increasingly configurable and designed for deployment on a plethora of architectures, ranging from sequential machines via multicore and distributed architectures to the cloud. Examples of such systems are found in, e.g., software product lines, service-oriented computing, information systems, embedded systems, operating systems, and telephony. To model and analyze systems without a fixed architecture, the models need to naturally capture and range over relevant deployment scenarios. For this purpose, it is interesting to lift aspects of low-level deployment concerns to the abstraction level of the modeling language. In this paper, the object-oriented modeling language Creol is extended with a notion of dynamic deployment components with parametric processing resources, such that processor resources may be explicitly reallocated. The approach is compositional in the sense that functional models and reallocation strategies are both expressed in Creol, and functional models can be run alone or in combination with different reallocation strategies. The formal semantics of deployment components is given in rewriting logic, extending the semantics of Creol, and executes on Maude, which allows simulations and test suites to be applied to models which vary in their available resources as well as in their resource reallocation strategies.},
author = {Dong, Jin and Zhu, Huibiao and Johnsen, Einar and Owe, Olaf and Schlatte, Rudolf and {Tapia Tarifa}, Silvia},
doi = {10.1007/978-3-642-16901-4},
isbn = {978-3-642-16900-7},
keywords = {DZ10},
mendeley-tags = {DZ10},
pages = {646--661--661},
title = {{Formal Methods and Software Engineering}},
url = {http://www.springerlink.com/content/049033u652453725/},
volume = {6447},
year = {2010}
}
@misc{DSMLtoolLink,
keywords = {DSMLtoolLink},
mendeley-tags = {DSMLtoolLink},
title = {{DiVA Adaptation Modelling Toolkit}},
note = { Available at https://sites.google.com/site/divawebsite/divastudio/diva-adaptation-modelling-toolkit  (Accessed: 14th August, 2017) }
}
@article{CT97,
author = {Coste-Maniere, Eve and Turro, N},
doi = {10.1109/IROS.1997.655107},
journal = {IEEE/RSJ Int. Conf. Intell. Robot. Syst.},
keywords = {CT97,MAESTRO programming language,autonomous underwater vehicle,discrete event system,formal specification,marine systems,mobile robots,program environment,program verification,programming environments,programming languages,robot mission,robot programming,validation},
mendeley-tags = {CT97},
pages = {836----841 vol.2},
title = {{The MAESTRO language and its environment: specification, validation and control of robotic missions}},
year = {1997}
}
@article{PH12,
abstract = {We present our experiences using a purely functional language, Haskell, in what has been traditionally the realm of low-level languages: robot control. Fro b (Functional Robotics) is a domain-specific language embedded in Haskell for robot control. Frob is based on Functional Reactive Programming (FRP), as initially developed for Fran, a language of reactive animations. Frob presents the interaction between a robot and its stimuli, both onboard sensors and messages from other agents, in a purely functional manner. This serves as a basis for composable high level abstractions supporting complex control regimens in a concise and reusable manner. {\textcopyright} Springer-Verlag Berlin Heidelberg 1998.},
author = {Peterson, John and Hudak, Paul and Elliott, Conal M.},
doi = {10.1.1.36.8118},
isbn = {3540655271},
journal = {Lect. Notes Comput. Sci. (including Subser. Lect. Notes Artif. Intell. Lect. Notes Bioinformatics)},
keywords = {PH12},
mendeley-tags = {PH12},
title = {{Lambda in motion: Controlling robots with Haskell}},
year = {1999}
}
@misc{,
title = {{A domain specific modeling language for multiagent systems.pdf}}
}
@article{RH10,
abstract = {The development of robot control programs is a complex task. Many robots are different in their electrical and mechanical structure which is also reflected in the software. Specific robot software environments support the program development, but are mainly text-based and usually applied by experts in the field with profound knowledge of the target robot. This paper presents a graphical programming environment which aims to ease the development of robot control programs. In contrast to existing graphical robot programming environments, our approach focuses on the composition of parallel action sequences. The developed environment allows to schedule independent robot actions on parallel execution lines and provides mechanism to avoid side-effects of parallel actions. The developed environment is platform-independent and based on the model-driven paradigm. The feasibility of our approach is shown by the application of the sequencer to a simulated service robot and a robot for educational purpose.},
archivePrefix = {arXiv},
arxivId = {1010.0886},
author = {Reckhaus, Michael and Hochgeschwender, Nico and Ploeger, Paul G. and Kraetzschmar, Gerhard},
eprint = {1010.0886},
journal = {Appl. Sci.},
keywords = {RH10},
mendeley-tags = {RH10},
title = {{A Platform-independent Programming Environment for Robot Control}},
url = {http://arxiv.org/abs/1010.0886},
year = {2010}
}
@article{Mallet2010a,
abstract = {The topic of reusable software in robotics is now largely addressed. Components based architectures, where components are independent units that can be reused accross applications, have become more popular. As a consequence, a long list of middlewares and integration tools is available in the community, often in the form of open-source projects. However, these projects are generally self contained with little reuse between them. This paper presents a software engineering approach that intends to grant middleware independance to robotic software components so that a clear separation of concerns is achieved between highly reusable algorithmic parts and integration frameworks. Such a decoupling let middle-wares be used interchangeably, while fully benefitting from their specific, individual features. This work has been integrated into a new version of the open-source GenoM component generator tool: GenoM3},
author = {Mallet, Anthony and Pasteur, C{\'{e}}dric and Herrb, Matthieu and Lemaignan, S{\'{e}}verin and Ingrand, F{\'{e}}lix},
doi = {10.1109/ROBOT.2010.5509539},
isbn = {9781424450381},
issn = {10504729},
journal = {Proc. - IEEE Int. Conf. Robot. Autom.},
keywords = {`},
mendeley-tags = {`},
pages = {4627--4632},
title = {{GenoM3: Building middleware-independent robotic components}},
year = {2010}
}
@misc{RT{CSP}ecifLink,
keywords = {RT{CSP}ecifLink},
mendeley-tags = {RT{CSP}ecifLink},
title = {{Robotic Technology Component™ (RTC)}},
note = { Available at http://www.omg.org/spec/RTC/1.1  (Accessed: 14th August, 2017)},
urldate = {2017-08-10},
year = {2012}
}
@article{BM03,
abstract = {Robots have become significantly more power- ful and intelligent over the last decade, and are moving in to more service oriented roles. As a result robots will more often be used by peo- ple with minimal technical skills and so there is a need for easier to use and more flexible programming systems. This paper reviews the current state of the art in robot programming systems. A distinction is made between manual and automatic programming systems. Manual systems require the user/programmer to create the robot program directly, by hand, while au- tomatic systems generate a robot program as a result of interaction between the robot and the human; there are a variety of methods in- cluding learning, programming by demonstra- tion and instructive systems.},
author = {Biggs, Geoffrey and Macdonald, Bruce},
doi = {10.1109/ROBOT.2001.932554},
isbn = {0-7803-6576-3},
journal = {Proc. Australas. Conf. Robot. Autom.},
keywords = {BM03},
mendeley-tags = {BM03},
pages = {1--3},
title = {{A Survey of Robot Programming Systems}},
url = {http://pdf.aminer.org/000/355/292/towards{\_}programming{\_}tools{\_}for{\_}robots{\_}that{\_}integrate{\_}probabilistic{\_}computation{\_}and.pdf},
year = {2003}
}
@article{RP99,
abstract = {Describes the enhancement of XVision, a large library of C++ code for real-time vision processing, into FVision (pronounced "fission"), a fully-featured domain-specific language (DSL) embedded in Haskell. The resulting prototype system substantiates the claims of increased modularity, effective code reuse and rapid prototyping that characterize the DSL approach to systems design. It also illustrates the need for judicious interface design: relegating computationally expensive tasks to XVision (pre-existing C++ components) and leaving modular compositional tasks to FVision (Haskell). At the same time, our experience demonstrates how Haskell's advanced language features (specifically, parametric polymorphism, lazy evaluation, higher-order functions and automatic storage reclamation) permit a rapid DSL design that is itself highly modular and easily modified. Overall, the resulting hybrid system exceeded our expectations: visual tracking programs continue to spend most of their time executing low-level image processing code, while Haskell's advanced features allow us to quickly develop and test small prototype systems within a matter of a few days, and to develop realistic applications within a few weeks.},
author = {Reid, Alastair and Peterson, John and Hudak, Paul and Hager, Greg},
isbn = {1-58113-074-0},
issn = {0270-5257},
journal = {Int. Conf. Softw. Eng. (ICSE 1999), Los Angeles, Calif.},
keywords = {RP99,an area that is,and high-,and the,at a criti-,cal juncture,digitizers,inexpensive cameras,now plentiful,performance video devices are,real-time computer vision is},
mendeley-tags = {RP99},
pages = {1--10},
title = {{Prototyping real-time vision systems: an experiment in DSL design}},
year = {1999}
}
@article{CS11,
author = {Ceballos, Antonio and de Silva, Lavindra and Herrb, Matthieu and Ingrand, F{\'{e}}lix and Mallet, Anthony and Medina, Alberto and Prieto, M},
journal = {Astra},
keywords = {CS11},
mendeley-tags = {CS11},
number = {2},
pages = {1--7},
title = {{GenoM as a Robotics Framework for Planetary Rover Surface Operations}},
url = {message:{\%}3CE32EBAA6777C584699EDBBDDFA6C2F5C3C9C3EB982@GMVMAIL3.gmv.es{\%}3E},
year = {2011}
}
@misc{RDTFLink,
keywords = {RDTFLink},
mendeley-tags = {RDTFLink},
title = {{Domain Level Task Force}},
note = { Available at http://robotics.omg.org   (Accessed: 14th August, 2017) }
}
@misc{robotMLlink,
keywords = {robotMLlink},
mendeley-tags = {robotMLlink},
title = {{Eclipse Papyrus RobotML project a Papyrus DSML for robotic applications.}},
note = { Available at https://eclipse.org/papyrus/components/robotml/1.2.0/   (Accessed: 14th August, 2017)},
urldate = {2017-08-10}
}
@article{FH97,
abstract = {This paper presents a general methodology for the spec-ification and the integration of functional modules in a distributed reactive robot architecture. The approach is based on a hybrid architecture basically composed of two levels: a lower distributed functional level con-trolled by a centralized decisional level. Thanks to this methodology, synchronous or asyn-chronous operating capabilities (servo-control, data processing, event monitoring) can be easily added to the functional level. They are encapsulated into mod-ules, built according a generic model, that are seen by the decisaonal level as homogeneous, programmable, re-active and robust communicant services. Each module is simply described with a specific lan-guage and i s automatically produced by a generator of modules (Gen{\~{}}oM) according to the generic model. GenoM also produces an interactive test program and interface libraries to control the module and to read the resulting data, which allow to directly integrate the module into the architecture.},
author = {Fleury, Sara and Herrb, Matthieu and Chatila, Raja},
doi = {10.1109/IROS.1997.655108},
isbn = {0-7803-4119-8},
issn = {09205489},
journal = {IEEE/RSJ Int. Conf. Intell. Robot. Syst.},
keywords = {FH97},
mendeley-tags = {FH97},
pages = {842 -- 849 vol.2},
title = {{GenJVl: A Tool for the Specification and the Implementation of Operating Modules in a Distributed Robot Architecture}},
year = {1997}
}
@article{AB12,
abstract = {We have recently started an effort to combine a state of the art tool for developing functional modules of robotic systems (G enoM) with a component based framework for implementing embedded real-time systems (BIP). Unlike some works which study the connection between formal approaches and the highest (decisional) level of the robot software architecture, where deliberative activities such as planning, diagnostics, and execution control are conducted, we tackle the problem of using formal methods for developing modules of the functional level of robots. Little attention has been drawn to the development of these modules whose robustness is paramount to the robustness of the overall platform. To this end, we have successfully developed the G enoM/BIP component based design approach and applied it to the functional level of a complex exploration rover. Here, we report on this work, and show how we: (i) produce a very fine grained formal computational model of the robot functional level; (ii) run the BIP engine on the real robot, which executes and enforces the model semantics at runtime; and (iii) check the model offline for deadlock-freedom, as well as other safety properties. Moreover, we also extended this paradigm in a number of promising directions: (i) introduced a real-time BIP engine which can now use and control a timed BIP model; (ii) distributed the model and the engine over multiple CPUs; (iii) proposed a user-friendly language for specifying constraints on the model; and (iv) linked the model with a temporal plan execution controller. Interestingly, although our approach was initially proposed for the lowest level of robot architectures, these more recent extensions now allow us to model and manage the deliberation taking place at the decisional layer. {\textcopyright} 2012 Elsevier Ltd. All rights reserved.},
author = {Abdellatif, Tesnim and Bensalem, Saddek and Combaz, Jacques and {De Silva}, Lavindra and Ingrand, Felix},
doi = {10.1016/j.robot.2012.09.005},
journal = {Rob. Auton. Syst.},
keywords = {AB12,Controller synthesis,Robotic functional layer,Robotic software architecture,Robust software,Verification and validation},
mendeley-tags = {AB12},
title = {{Rigorous design of robot software: A formal component-based approach}},
year = {2012}
}
@article{NV01,
abstract = {We will present an overview of the CLARAty architecture which aims at developing reusable software components for robotic systems. These com- ponents are to support autonomy software which plans and schedules robot activities. The CLARAty architec- ture modifies the conventional three-level robotic archi- tecture into a new two-layered design: the Functional Layer and the Decision Layer. The Functional Layer pro- vides a representation of the system components and an implementation of their basic functionalities. The Deci- sion Layer is the decision making engine that drives the Functional Layer. It globally reasons about the intended goals, system resources, and state of the system and its environment. The Functional Layer is composed of a set of interrelated object-oriented hierarchies consisting of active and passive objects that represent the different levels of system abstractions. In this paper, we present an overview of the design of the Functional Layer. The Functional Layer is decomposed into a set of reusable core components and a set of extended components that adapt the reusable set to different hardware implemen- tations. The reusable components: (a) provide interface definitions and implementations of basic functionality, (b) provide local executive capabilities, (c) manage local resources, and (d) support state and resource queries by the Decision Layer.},
author = {Nesnas, Issa and Volpe, Richard and Estlin, Tara and Das, Hari and Petras, Richard and Mutz, D},
doi = {10.1109/IROS.2001.976425},
isbn = {0-7803-6612-3},
journal = {Proc. 2001 IEEE/RSJ Int. Conf. Intell. Robot. Syst. Expand. Soc. Role Robot. Next Millenn. (Cat. No.01CH37180)},
keywords = {NV01},
mendeley-tags = {NV01},
title = {{Toward developing reusable software components for robotic applications}},
year = {2001}
}
@misc{RoboticPrediction,
author = {Demaitre, E.},
keywords = {RoboticPrediction},
mendeley-tags = {RoboticPrediction},
title = {{Five robotics predictions for 2016. Robotics Business Review." (2016).}},
note = { Available at https://www.roboticsbusinessreview.com/uncategorized/five{\_}robotics{\_}predictions{\_}for{\_}2016/    (Accessed: 14th August, 2017)},
year = {2016}
}

@article{LP97,
  title={\uppaal in a nutshell},
  author={Larsen, Kim G and Pettersson, Paul and Yi, Wang},
  journal={International journal on software tools for technology transfer},
  volume={1},
  number={1-2},
  pages={134--152},
  year={1997},
  publisher={Springer}
}


@misc{,
title = {{A survey DSL{\_}bibliography}}
}

@misc{AutoNavLink,
keywords = {AutoNavLink},
mendeley-tags = {AutoNavLink},
title = {pr2{\_}navigation},
note = { Available at http://wiki.ros.org/pr2{\_}navigation    (Accessed: 14th August, 2017)}
}

@article{AD94,
abstract = {We propose timed (finite) automata to model the behavior of real-time systems over time. Our definition provides a simple, and yet powerful, way to annotate state-transition graphs with timing constraints using finitely many real-valued clocks. A timed automaton accepts timed words-infinite sequences in which a real-valued time of occurrence is associated with each symbol. We study timed automata from the perspective of formal language theory: we consider closure properties, decision problems, and subclasses. We consider both nondeterministic and deterministic transition structures, and both B??chi and Muller acceptance conditions. We show that nondeterministic timed automata are closed under union and intersection, but not under complementation, whereas deterministic timed Muller automata are closed under all Boolean operations. The main construction of the paper is an (PSPACE) algorithm for checking the emptiness of the language of a (nondeterministic) timed automaton. We also prove that the universality problem and the language inclusion problem are solvable only for the deterministic automata: both problems are undecidable (??11-hard) in the nondeterministic case and PSPACE-complete in the deterministic case. Finally, we discuss the application of this theory to automatic verification of real-time requirements of finite-state systems. ?? 1994.},
author = {Alur, Rajeev and Dill, David},
isbn = {0304-3975},
journal = {Theor. Comput. Sci.},
keywords = {AD94},
mendeley-tags = {AD94},
title = {{A theory of timed automata}},
year = {1994}
}
@inproceedings{NH04,
abstract = {Simulators have played a critical role in robotics research as tools for quick and efficient testing of new concepts, strategies, and algorithms. To date, most simulators have been restricted to 2D worlds, and few have matured to the point where they are both highly capable and easily adaptable. Gazebo is designed to fill this niche by creating a 3D dynamic multi-robot environment capable of recreating the complex worlds that would be encountered by the next generation of mobile robots. Its open source status, fine grained control, and high fidelity place Gazebo in a unique position to become more than just a stepping stone between the drawing board and real hardware: data visualization, simulation of remote environments, and even reverse engineering of blackbox systems are all possible applications. Gazebo is developed in cooperation with the Player and Stage projects (Gerkey, B. P., et al., July 2003), (Gerkey, B. P., et al., May 2001), (Vaughan, R. T., et al., Oct. 2003), and is available from http://playerstage.sourceforge.net/gazebo/ gazebo.html.},
author = {Koenig, N. and Howard, A.},
booktitle = {2004 IEEE/RSJ Int. Conf. Intell. Robot. Syst. (IEEE Cat. No.04CH37566)},
doi = {10.1109/IROS.2004.1389727},
isbn = {0-7803-8463-6},
keywords = {Computational modeling,Educational robots,Friction,Gazebo,KH04,Mobile robots,Open source software,Packaging,Player project,Robot sensing systems,Service robots,Stage project,Testing,Vehicle dynamics,application program interfaces,control engineering computing,digital simulation,grained control,mobile robots,multi-robot systems,open-source multi-robot simulator},
mendeley-tags = {KH04},
title = {{Design and use paradigms for gazebo, an open-source multi-robot simulator}},
year = {2004}
}



@article{BB06,
abstract = {We present a methodology for modeling heterogeneous real-time components. Components are obtained as the superposition of three layers: behavior, specified as a set of transitions; Interactions between transitions of the behavior; Priorities, used to choose amongst possible interactions. A parameterized binary composition operator is used to compose components layer by layer. We present the BIP language for the description and composition of layered components as well as associated tools for executing and analyzing components on a dedicated platform. The language provides a powerful mechanism for structuring interactions involving rendezvous and broadcast. We show that synchronous and timed systems are particular classes of components. Finally, we provide examples and compare the BIP framework to existing ones for heterogeneous component-based modeling},
author = {Basu, Ananda and Bozga, Marius and Sifakis, Joseph},
doi = {10.1109/SEFM.2006.27},
isbn = {0769526780},
journal = {Proc. - 4th IEEE Int. Conf. Softw. Eng. Form. Methods, SEFM 2006},
keywords = {BB06},
mendeley-tags = {BB06},
pages = {3--12},
title = {{Modeling heterogeneous real-time components in BIP}},
year = {2006}
}
@article{S10,
abstract = {From the Publisher:The {CSP} approach has been widely used in the specification, analysis and verification of concurrent and real-time systems, and for understanding the particular issues that can arise when concurrency is present. It provides a language which enables specifications and designs to be clearly expressed and understood, together with a supporting theory which allows them to be analyzed and shown to be correct.This book supports advanced level courses on concurrency covering timed and untimed {CSP}. The first half introduces the language of {CSP}, the primary semantic models (traces, failures, divergences and infinite traces), and their use in the modelling, analysis and verification of concurrent systems. The second half of the book introduces time into the language, brings in the timed semantic model (timed failures) and finally presents the theory of timewise refinement which links the two halves together.Containing the following: -Exercises and solutions -Instructors resources - Example {CSP} programs to run on {FDR} and ProBe -Links to useful sitesPartial Contents: Part I: The Language of {CSP}; Sequential Processes; Concurrency; Abstraction and Control Flow; Part II: Analyzing Processes; Traces; Specification and Verification with Traces; Stable Failures; Specification and Verification with Failures; Failures, Divergences, and Infinite Traces; Part III: Introducing Time; The Timed Language; Timed transition systems; Part IV: Timed Analysis; Semantics of Timed {CSP}; Timed Specification and Verification; Timewise Refinement; Appendix A: Event-based Time; A.1 Standard {CSP} and {\$}tock{\$}; A.2 Translating from Timed {CSP}; A.3 Notes; Appendix B:Model-checking with {FDR}; B.1 Interacting with {FDR}; B.2 How {FDR} Checks Refinement; B.3 Machine readable {CSP}; Index of Processes.},
author = {Schneider, Steve},
isbn = {0471623733 (alk. paper)},
journal = {Worldw. Ser. Comput. Sci.},
keywords = {Parallel processing (Electronic computers),Real-time data processing.,S10},
mendeley-tags = {S10},
title = {{Concurrent and real time systems : the {CSP} approach}},
year = {2010}
}
@misc{KarelManual,
keywords = {KarelManual},
mendeley-tags = {KarelManual},
publisher = {FANU C Robotics America, Inc},
title = {{FANUC Robotics SYSTEM R-J3 i B Controller KAREL Reference Manual}},
note = { Available at http://www.aip-primeca.net/DesktopModules/Bring2mind/DMX/Download.aspx?Command=Core{\_}Download\&EntryId=147\&PortalId=1\&TabId=150   (Accessed: 14th August, 2017)},
year = {2003}
}
@article{PHH99,
abstract = {We have applied methodologies developed for domain-specific embedded languages to create a high-level robot control language called Frob, for functional robotics. Frob supports a programming style that cleanly separates the what from the how of a robotic control program. That is, the what is a simple, easily understood definition of the control strategy using groups of equations and primitives which combine sets of these control system equations into a complex system. The how aspect of the program addresses the unpleasant details, such as the method used to realize these equations, the connection between the control equations and the sensors and effectors in the robot, and communication with other elements of the system. Frob is a system that supports rapid prototyping of new control strategies, enables software reuse through composition, and defines a system in a way that can be formally reasoned about and transformed},
author = {Peterson, J. and Hager, G.D. and Hudak, P.},
doi = {10.1109/ROBOT.1999.772516},
isbn = {0-7803-5180-0},
journal = {Proc. 1999 IEEE Int. Conf. Robot. Autom. (Cat. No.99CH36288C)},
keywords = {PHH99},
mendeley-tags = {PHH99},
title = {{A language for declarative robotic programming}},
year = {1999}
}
@inproceedings{BK05,
abstract = {This paper gives an overview of Component-Based Software Engineering (CBSE), motivates its application to the field of mobile robotics, and proposes a particular component model. CBSE is an approach to system-building that aims to shift the emphasis from programming to composing systems from a mixture of off-the-shelf and custom-built software components. This paper argues that robotics is particularly well-suited for and in need of component-based ideas. Furthermore, now is the right time for their introduction. The paper introduces Orca – an open-source component-based software engineering framework proposed for mobile robotics with an associated repository of free, reusable components for building mobile robotic systems.},
author = {Brooks, Alex and Kaupp, Tobias and Makarenko, Alexei and Williams, Stefan and Oreb{\"{a}}ck, Anders},
booktitle = {2005 IEEE/RSJ Int. Conf. Intell. Robot. Syst. IROS},
doi = {10.1109/IROS.2005.1545523},
isbn = {0780389123},
keywords = {BK05,Component-based design,Distributed robotics,Robotic architectures,Software re-use,Standardization},
mendeley-tags = {BK05},
pmid = {1545523},
title = {{Towards component-based robotics}},
year = {2005}
}
@article{PH99,
abstract = {We present our experiences using a purely functional language, Haskell, in what has been traditionally the realm of low-level languages: robot control. Fro b (Functional Robotics) is a domain-specific language embedded in Haskell for robot control. Frob is based on Functional Reactive Programming (FRP), as initially developed for Fran, a language of reactive animations. Frob presents the interaction between a robot and its stimuli, both onboard sensors and messages from other agents, in a purely functional manner. This serves as a basis for composable high level abstractions supporting complex control regimens in a concise and reusable manner. {\textcopyright} Springer-Verlag Berlin Heidelberg 1998.},
author = {Peterson, John and Hudak, Paul and Elliott, Conal M.},
doi = {10.1.1.36.8118},
isbn = {3540655271},
journal = {Lect. Notes Comput. Sci. (including Subser. Lect. Notes Artif. Intell. Lect. Notes Bioinformatics)},
keywords = {PH99},
mendeley-tags = {PH99},
title = {{Lambda in motion: Controlling robots with Haskell}},
year = {1999}
}
@article{PN02,
abstract = {Software for (semi-) autonomous robots tends to be a complex combination of components from many different application domains such as control theory, vision, and artificial intelligence. Components are often developed using their own domain-specific tools and abstractions. System integration can thus be a significant challenge, in particular when the application calls for a dynamic, adaptable system structure in which rigid boundaries between the subsystems are a performance impediment. We believe that, by identifying suitably abstract notions common to the different domains in question, it is possible to create a broader framework for software integration and to recast existing domain-specific frameworks in these terms. This approach simplifies integration and leads to improved reliability. In this paper, we show how Functional Reactive Programming (FRP) can serve as such a unifying framework for programming vision-guided, semi-autonomous robots and illustrate the benefits this approach entails. The key abstractions in FRP, reactive components describing continuous or discrete behavior in a declarative style, are first class entities, allowing the resulting systems to exhibit a dynamic, adaptable structure which we regard as especially important in the area of autonomous robots.},
author = {Pembeci, Izzet and Nilsson, Henrik and Hager, Gregory D},
doi = {doi: 10.1145/571157.571174},
isbn = {1581135289},
journal = {Princ. Pract. Declar. Program.},
keywords = {PN02,reactive-system},
mendeley-tags = {PN02},
pages = {168--179},
title = {{System presentation - Functional reactive robotics: an exercise in principled integration of domain-specific languages}},
url = {citeulike-article-id:2761819{\%}5Cnhttp://dx.doi.org/10.1145/571157.571174{\%}5Cnhttp://www.cs.nott.ac.uk/{~}nhn/Publications/ppdp2002.pdf},
year = {2002}
}
@article{RM17,
abstract = {Designing robotic systems can be very challenging, yet con-trollers are often specified using informal notations with development driven primarily by simulations and physical experiments, without rela-tion to abstract models of requirements. The ability to perform formal analysis and replicate results across different robotic platforms is hindered by the lack of well-defined formal notations. In this paper we present a timed state-machine based formal notation for robotics that is informed by current practice. We motivate our work with an example from swarm robotics and define a compositional {CSP}-based discrete timed semantics suitable for refinement. Our results support verification and, importantly, enable rigorous connection with sound simulations and deployments.},
author = {Ribeiro, Pedro and Miyazawa, Alvaro and Li, Wei and Cavalcanti, Ana and Timmis, Jon and Woodcock, Jim},
file = {:home/abdul/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ribeiro et al. - Unknown - Modelling and Verification of Timed Robotic Controllers.pdf:pdf},
keywords = {{CSP},RM17,process algebra,refinement,semantics},
mendeley-tags = {RM17},
journal = {Integr. Form. Methods (forthcoming) },
year = {2017},
title = {{Modelling and Verification of Timed Robotic Controllers}}
}
@article{SH14,
abstract = {Grasping objects and using them in a task-oriented manner is challenging for a robot. It requires an understanding of the object, the robot's capabilities, and the task to be executed. We argue that an explicit representation of these domains increases reusability and robustness of the resulting system. We present the declarative Grasp Domain Definition Language (GDDL) which enables the explicit grasp-planner-independent specification of grasping problems. The formal model underlying GDDL enables the definition of formal constraints that are validated during design time and run time. Our approach has been realized on two real robots.},
author = {Schneider, Sven and Hochgeschwender, Nico and Kraetzschmar, Gerhard K.},
doi = {10.1109/IROS.2014.6942669},
isbn = {9781479969340},
issn = {21530866},
journal = {IEEE Int. Conf. Intell. Robot. Syst.},
keywords = {SH14},
mendeley-tags = {SH14},
number = {Iros},
pages = {919--926},
title = {{Declarative specification of task-based grasping with constraint validation}},
year = {2014}
}
@inproceedings{KD16,
abstract = {Robotic systems are a typical example of complex systems. Their design involves a combination of different technologies, requiring a multi-disciplinary approach. This is particularly challenging when a robotic system is required to interact either with humans or other entities within its environment. To tackle this complexity, we propose a design and validation approach based on MDE (Model-Driven Engineering) principles for industrial manipulators. We propose an extension of RobotML for manipulation, a modelling environment based on the Papyrus tool, which was developed specifically for the robotics domain. The extension is aiming to model a complete robotic setting, including protagonists, objects, their properties, the interactions between them, the services provided by the robots, and the actions they can perform. Then we propose to use model execution techniques to validate the design models. We illustrate our approach on a robotic scenario dedicated to the Sybot collaborative robot. {\textcopyright} 2016 IEEE.},
author = {Kchir, Selma and Dhouib, Saadia and Tatibouet, Jeremie and Gradoussoff, Baptiste and {Da Silva Simoes}, Max},
booktitle = {IEEE Int. Conf. Emerg. Technol. Fact. Autom. ETFA},
doi = {10.1109/ETFA.2016.7733727},
isbn = {9781509013142},
keywords = {KD16},
mendeley-tags = {KD16},
title = {{RobotML for industrial robots: Design and simulation of manipulation scenarios}},
year = {2016}
}
@misc{MH04,
abstract = {The OWL Web Ontology Language is designed for use by applications that need to process the content of information instead of just presenting information to humans. OWL facilitates greater machine interpretability of Web content than that supported by XML, RDF, and RDF Schema (RDF-S) by providing additional vocabulary along with a formal semantics. OWL has three increasingly-expressive sublanguages: OWL Lite, OWL DL, and OWL Full. This document is written for readers who want a first impression of the capabilities of OWL. It provides an introduction to OWL by informally describing the features of each of the sublanguages of OWL. Some knowledge of RDF Schema is useful for understanding this document, but not essential. After this document, interested readers may turn to the OWL Guide for more detailed descriptions and extensive examples on the features of OWL. The normative formal definition of OWL can be found in the OWL Semantics and Abstract Syntax.},
author = {W3C},
booktitle = {W3C Recomm. 10 Febr. 2004},
keywords = {MH04},
mendeley-tags = {MH04},
title = {{OWL Web Ontology Language}},
year = {2004}
}
@inproceedings{FB16,
author = {Foughali, Mohammed and Berthomieu, Bernard and {Dal Zilio}, Silvano and Ingrand, F{\'{e}}lix and Mallet, Anthony},
booktitle = {Lect. Notes Comput. Sci. (including Subser. Lect. Notes Artif. Intell. Lect. Notes Bioinformatics)},
doi = {10.1007/978-3-319-47846-3_24},
file = {:home/abdul/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Foughali et al. - 2016 - Model checking real-time properties on the functional layer of autonomous robots.pdf:pdf},
isbn = {9783319478456},
keywords = {FB16},
mendeley-tags = {FB16},
title = {{Model checking real-time properties on the functional layer of autonomous robots}},
year = {2016}
}
@article{ZW10,
abstract = {In this paper we present a formal approach to robot motion specification. This motion specification takes into account three elementary behaviors that suffice to define any robot interaction with the environment, i.e. free motion, exerting generalized forces and the transition between both of these behaviors. These behaviors provide a foundation for general motion generation taking into account any sensors, any effectors and the capability to exchange information between embodied agents. This specification can be used both for the definition of robot tasks and implementation of robot control software, hence both of those aspects are presented in this paper. This formal approach was used for the implementation of the MRROC++ robot programming framework. Two-handed manipulation of a Rubik's cube is used as an exemplary task. Extensive experimentation both with the presented formalism and the MRROC++ framework showed that the imposed formal rigor eliminates many errors at the software specification phase, produces well-structured control software and significantly speeds up and simplifies its implementation. These advantages are mainly due to the fact that the proposed formal specification tool is derived from operational semantics used in computer science for the definition of programming languages, thus a close relationship between abstract definition and the implementation of the control system resulted. {\textcopyright} The Author(s), 2010.},
author = {Zieli{\~{n}}ski, C and Winiarski, T},
doi = {10.1177/0278364909348761},
journal = {Int. J. Rob. Res.},
keywords = {Cognitive robotics,Cognitive systems,Comp,Computer control systems,Control software,Elementary b,Robot programming,ZW10},
mendeley-tags = {ZW10},
title = {{Motion generation in the MRROC++ robot programming framework}},
year = {2010}
}
@article{HG13,
abstract = {Deploying a complex robot software architecture on real robot systems and getting it to run reliably is a challenging task. We argue that software deployment decisions should be separated as much as possible from the core development of software functionalities. This will make the developed software more independent of a particular hardware architecture (and thus more reusable) and allow it to be deployed more flexibly on a wider variety of robot platforms. This paper presents a domain-specific language (DSL) which supports this idea and demonstrates how the DSL is used in a model-driven engineering-based development process. A practical example of applying the DSL to the development of an application for the KUKA youBot platform is given.},
author = {Hochgeschwender, Nico and Gherardi, Luca and Shakhirmardanov, Azamat and Kraetzschmar, Gerhard K. and Brugali, Davide and Bruyninckx, Herman},
doi = {10.1109/IROS.2013.6696915},
isbn = {9781467363587},
issn = {21530858},
journal = {IEEE Int. Conf. Intell. Robot. Syst.},
keywords = {HG13},
mendeley-tags = {HG13},
pages = {3907--3914},
title = {{A model-based approach to software deployment in robotics}},
year = {2013}
}
@article{AS12,
abstract = {Industrial robotics is characterized by sophisticated mechanical components and highly-developed real-time control algorithms. However, the efficient use of robotic systems is very much limited by existing proprietary programming methods. In the research project SoftRobot, a software architecture was developed that enables the programming of complex real-time critical robot tasks with an object-oriented general purpose language. On top of this architecture, a graphical language was developed to ease the specification of complex robot commands, which can then be used as part of robot application workflows. This paper gives an overview about the design and implementation of this graphical language and illustrates its usefulness with some examples. I. I NTRODUCTION When programming robots to perform long-lasting and complex tasks, the programmer usually wants to abstract from the technical details of controlling the robot hardware, e.g. hard real-time constraints, closed-loop controllers, or controller parameters. The focus should rather lie on the what aspect of the task [1]. In the research project SoftRobot, an extensible software architecture [2] has been developed to both facilitate the development of robotic applications with the aforementioned level of abstraction, and at the same time keep real-time constraints in mind. This multilayer architecture (cf. Fig. 1) allows to program industrial robots using a standard, high-level programming language (e.g. Java) and, at the same time, ensures that commands are executed on the robot hardware with real-time guarantees. The SoftRobot architecture provides application programmers with the Java-based Robotics API [3], an objectoriented, extensible application programming interface for robot applications. The Robotics API contains an open domain model of (industrial) robotics describing the available actuators and devices, as well as possible actions and tasks, and also includes ways of maintaining a world model of the relevant parts of the environment. The Robotics API allows to specify actions to be executed by actuators (for example, a linear movement by a robot), and to combine multiple actions in different ways to create more complex commands. Every such command is guaranteed to be executed with certain realtime guarantees considering the timing of all actions and their combination. As an example, consider the case of a line welding application in the automotive industry: robots The authors are with the Institute for Software and Systems Engineering, University of Augsburg, D-86135 Augsburg, Germany. E-mail of corresponding author: angerer@informatik.uni-augsburg.de This work presents results of the research project SoftRobot which is funded by the European Union and the Bavarian government within the High-Tech-Offensive Bayern. The project is carried out together with KUKA Labs GmbH and MRK-Systeme GmbH and is kindly supported by VDI/VDE-IT GmbH. Robot Control Core Realtime Primitives Interface Implementation Application Application Robotics API Robot Hardware Automated transformation into real-time dataflow graphs Real-},
archivePrefix = {arXiv},
arxivId = {arXiv:1303.6777v1},
author = {Angerer, Andreas and Smirra, Remi and Hoffmann, Alwin and Schierl, Andreas and Vistein, Michael and Reif, Wolfgang},
eprint = {arXiv:1303.6777v1},
journal = {Proc. Third Int. Work. Domain-Specific Lang. Model. Robot. Syst. (DSLRob 2012)},
keywords = {AS12},
mendeley-tags = {AS12},
title = {{A Graphical Language for Real-Time Critical Robot Commands}},
year = {2012}
}
@inproceedings{Angerer2010,
abstract = {During the last two decades, software development has evolved continuously into an engineering discipline with systematic use of methods and tools to model and implement software. For example, object-oriented analysis and design is structuring software models according to real-life objects of the problem domain and their relations. However, the industrial robotics domain is still dominated by old-style, imperative robot programming languages, making software development difficult and expensive. For this reason, we introduce the object-oriented Robotics Application Programming Interface (Robotics API) for developing software for industrial robotic applications. The Robotics API offers an abstract, extensible domain model and provides common functionality, which can be easily used by application developers. The advantages of the Robotics API are illustrated with an application example.},
author = {Angerer, Andreas and Hoffmann, Alwin and Schierl, Andreas and Vistein, Michael and Reif, Wolfgang},
booktitle = {2010 IEEE/RSJ Int. Conf. Intell. Robot. Syst.},
doi = {10.1109/IROS.2010.5649098},
isbn = {978-1-4244-6674-0},
issn = {2153-0858},
keywords = {application program interfaces,application programming interface,imperative robot programming languages,industrial robotics,industrial robots,object-oriented analysis,object-oriented design,object-oriented framework,object-oriented programming,robot programming,robotics API,software development,software engineering,software models},
title = {{The Robotics API: An object-oriented framework for modeling industrial robotics applications}},
year = {2010}
}
@inproceedings{VK13,
abstract = {Current state-of-the-art robot program development needs expert programmers. Moreover, most robot programs developed today are robot hardware and software specific, and therefore little reusable without modifications. This paper realizes easier robot (re-)programming, by software framework independent models that can be executed using different hard- and software platforms. First, the paper focuses on the formalization of the tasks to be fulfilled by a robot, more specifically constraint-based programming tasks using a Domain Specific Language (DSL). Second, it gives a reference implementation in Lua [1]. The presented DSL makes it easy to develop applications, yet is powerful to execute. It enables automatic model verification and code generation for different hard- and software platforms, diminishing code debugging efforts. Experimental validation shows the ease of creating an application and adapting it, the reduction of the amount of hand-written code, and the debugging aid offered through meaningful errors returned by model verification.},
author = {Vanthienen, Dominick and Klotzbuucher, Markus and {De Schutter}, Joris and {De Laet}, Tinne and Bruyninckx, Herman},
booktitle = {IEEE Int. Conf. Intell. Robot. Syst.},
doi = {10.1109/IROS.2013.6696602},
isbn = {9781467363587},
issn = {21530858},
keywords = {VK13},
mendeley-tags = {VK13},
title = {{Rapid application development of constrained-based task modelling and execution using domain specific languages}},
year = {2013}
}
@misc{KRLManual,
keywords = {KRLManual},
mendeley-tags = {KRLManual},
publisher = {KUKA Roboter GmbH},
title = {{SOFTWARE KR C1 / KR C2 / KR C3 Reference Guide}},
note = { Available at http://robot.zaab.org/wp-content/uploads/2014/04/KRL-Reference-Guide-v4{\_}1.pdf   (Accessed: 14th August, 2017)}
}
@book{P07,
abstract = {Industrial Robots Programming focuses on designing and building robotic manufacturing cells, and explores the capabilities of today's industrial equipment as well as the latest computer and software technologies. Special attention is given to the input devices and systems that create efficient human-machine interfaces, and how they help non-technical personnel perform necessary programming, control, and supervision tasks.Drawing upon years of practical experience and using numerous examples and illustrative applications, J. Norberto Pires covers robotics programming as it applies to:The current industrial robotic equipment including manipulators, control systems, and programming environments. Software interfaces that can be used to develop distributed industrial manufacturing cells and techniques which can be used to build interfaces between robots and computers. Real-world applications with examples designed and implemented recently in the lab.This book is supported by a website http://robotics.dem.uc.pt/indrobprog that includes software code for the examples presented, various software applications developed by the author and videos of all examples presented and discussed.For more information about Industrial Robotics, please find the author's Industrial Robotics collection at the iTunesU University of Coimbra channel at the following link: http://itunes.apple.com/itunes-u/id413183592},
author = {Pires, J. Norberto},
booktitle = {Ind. Robot. Program. Build. Appl. Factories Futur.},
doi = {10.1007/b101252},
isbn = {0387233253},
keywords = {P07},
mendeley-tags = {P07},
title = {{Industrial robots programming: Building applications for the factories of the future}},
year = {2007}
}
@misc{RoboToolLink,
keywords = {RoboToolLink},
mendeley-tags = {RoboToolLink},
title = {{RoboTool}},
note = { Available at https://www.cs.york.ac.uk/circus/RoboCalc/robotool/      (Accessed: 14th August, 2017)}
}
@article{H00,
author = {Hager, G},
journal = {Robot. Res.},
keywords = {H00},
mendeley-tags = {H00},
title = {{FROB: A Transformational Approach to the Design of Robot Software}},
year = {2000}
}
@article{PP16,
abstract = {Robotics systems have special needs often related with their real-time nature and environmental properties. Often, control and communication paths within the system are tightly coupled to the actual physical configuration of the robot. As a consequence, these robots can only be assembled, configured, and programmed by robot experts. Traditional approaches, based on mainly writing the code without using software engineering techniques, are still used in the development process of these systems. Even when these robotic systems are successfully used, several problems can be identified and it is widely accepted that new approaches should be explored. The contribution of this research consists in delineating guidelines for the construction of robotic software systems, taking advantage of the application of the OMG standard robotic specifications which adhere to the model-driven approach MDA. Thereby the expert knowledge is captured in standard abstract models that can then be reused by other less expe‐ rienced developers. In addition part of the code is automatically generated, reducing costs and improving quality.},
author = {Pons, Claudia and P{\'{e}}rez, Gabriela and Giandini, Roxana and Baum, Gabriel},
doi = {10.1007/978-3-319-46613-2_4},
file = {:home/abdul/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Pons et al. - Unknown - Applying MDA and OMG Robotic Specification for Developing Robotic Systems(2).pdf:pdf},
keywords = {Model driven software development {\textperiodcentered} OMG standard,PP16,Robotic software system {\textperiodcentered}},
mendeley-tags = {PP16},
title = {{Applying MDA and OMG Robotic Specification for Developing Robotic Systems}}
}
@article{Dhouib2014,
abstract = {This article focuses on robot domain specific language(DSL) that helps in robot design and architecture. DSL simpllifies the deliberative, reactive, and hybrid architecures and also the communicaiton between the components. One of the domain specific language researchl project discussed in this article is Proteus. Developed a domain model based DSL and using tools like eclipse it was easy to build UML diagrams to represent ronbotic ontologies and arthitecture, and code is generated for those models. This helps to visualization of architecure, simplified design and reusing domain experts knowledge.},
author = {Dhouib, Saadia and Kchir, Selma and Stinckwich, Serge and Ziadi, Tewfik and Ziane, Mikal and Robotml, Mikal Ziane},
keywords = {MDE,domain-specific languages,generative program},
pages = {149--160},
title = {{RobotML , a Domain-Specific Language to Design , Simulate and Deploy Robotic Applications To cite this version : RobotML , a Domain-Specific Language}},
year = {2014}
}
@article{FS09,
author = {Fleurey, F and Solberg, A},
doi = {10.1007/978-3-642-04425-0_47},
isbn = {978-3-642-04424-3},
journal = {Model. ACM/IEEE 12th Int. Conf. Model. Eng. Lang. Syst.},
keywords = {FS09},
mendeley-tags = {FS09},
pages = {606--621},
title = {{A Domain Specific Modeling Language supporting Specification, Simulationand Execution of Dynamic Adaptive Systems}},
year = {2009}
}
@incollection{FB13,
abstract = {The DEPLOY project has provided a rare opportunity to explore and document the potential benefits of and challenges to creating and exploiting usable formal methods. Using the results of an updated review of 98 industrial applications, we identify trends relating to analytic power, robustness, stability and usability of tools, as well as to the quality of evidence on costs and benefits of deployment. A consideration of the DEPLOY applications reinforces these trends, additionally emphasising the importance of selecting formalisms suited to the problem domain and of effectively managing traceable links between requirements and models.},
author = {Fitzgerald, John and Bicarregui, Juan and Larsen, Peter Gorm and Woodcock, Jim},
booktitle = {Ind. Deploy. Syst. Eng. Methods},
isbn = {9783642331701},
keywords = {FB13},
mendeley-tags = {FB13},
title = {{Industrial deployment of formal methods: Trends and challenges}},
year = {2013}
}
@misc{,
title = {{DSLs}}
}
@article{AT15,
abstract = {General-purpose robots can perform a range of useful tasks in human environments; however, programming them to robustly function in all possible environments that they might encounter is unfeasible. Instead, our research aims to develop robots that can be programmed by its end-users in their context of use, so that the robot needs to robustly function in only one particular environment. This requires intuitive ways in which end-users can program their robot. To that end, this paper contributes a flow-based visual programming language, called RoboFlow, that allows programming of generalizable mobile manipulation tasks. RoboFlow is designed to (i) ensure a robust low-level implementation of program procedures on a mobile manipulator, and (ii) restrict the high-level programming as much as possible to avoid user errors while enabling expressive programs that involve branching, looping, and nesting. We present an implementation of RoboFlow on a PR2 mobile manipulator and demonstrate the generalizability and error handling properties of RoboFlow programs on everyday mobile manipulation tasks in human environments.},
author = {Alexandrova, S and Tatlock, Z and Cakmak, M},
doi = {10.1109/ICRA.2015.7139973},
isbn = {1050-4729 VO -},
journal = {2015 IEEE Int. Conf. Robot. Autom.},
keywords = {AT15,Computer languages,Mobile communication,Navigation,PR2 mobile manipulator,Programming profession,RoboFlow programs,Robots,Visualization,control engineering computing,flow-based visual programming language,general-purpose robots,high-level programming,human environments,manipulators,mobile manipulation tasks,mobile robots,visual languages,visual programming},
mendeley-tags = {AT15},
pages = {5537--5544},
title = {{RoboFlow: A flow-based visual programming language for mobile manipulation tasks}},
year = {2015}
}
@article{Horswill2000,
abstract = {The paper describes a simple functional programming language, GRL,$\backslash$nin which most of the characteristic features of the popular$\backslash$nbehavior-based robot architectures can be concisely written as reusable$\backslash$nsoftware abstractions. This makes it easier to write a clear modular$\backslash$ncode, to {\&}ldquo;mix and match{\&}rdquo; arbitration mechanisms, and to$\backslash$nexperiment with variations on existing mechanisms. The author describes$\backslash$nthe compilation process for the language, his experiences with it, and$\backslash$nissues of efficiency expressiveness, and code size relative to other$\backslash$nlanguages},
author = {Horswill, Ian Douglas},
doi = {10.1023/A:1008932520090},
isbn = {0-7803-5806-6},
issn = {09295593},
journal = {Auton. Robots},
number = {1},
pages = {83--93},
title = {{Functional programming of behavior-based systems}},
volume = {9},
year = {2000}
}
@misc{morselink,
keywords = {morselink},
mendeley-tags = {morselink},
title = {{MORSE, the Modular OpenRobots Simulation Engine}},
note = { Available at https://www.openrobots.org/wiki/morse    (Accessed: 14th August, 2017)}
}
@article{VK00,
author = {Deursen, Arie Van and Visser, Joost},
keywords = {VK00},
mendeley-tags = {VK00},
title = {{Domain-Specific Languages : An Annotated Bibliography}}
}
@misc{,
title = {{Genom}}
}
@techreport{MR16refMan,
author = {{Alvaro Miyazawa} and {Ana Cavalcanti} and {Pedro Ribeiro Wei Li} and {Jim Woodcock} and {Jon Timmis}},
institution = {University of York},
keywords = {MR16refMan},
mendeley-tags = {MR16refMan},
title = {{RoboChart Reference Manual}},
year = {2016}
}
@misc{robotCLink,
keywords = {robotCLink},
mendeley-tags = {robotCLink},
title = {{ROBOTC Word Logo a C Programming Language for Robotics}},
note = { Available at http://www.robotc.net/    (Accessed: 14th August, 2017)}
}
@article{MR16,
author = {Miyazawa, Alvaro and Ribeiro, Pedro and Li, Wei and Cavalcanti, Ana and Timmis, Jon and Woodcock, Jim},
journal = {Tech. Rep.},
keywords = {MR16TechReport},
mendeley-tags = {MR16TechReport},
pages = {1--18},
title = {{RoboChart: a State-Machine Notation for Modelling and Verification of Mobile and Autonomous Robots}},
year = {2016}
}
@article{BL95,
abstract = {Upp aal is a tool suite for automatic v erication of safet y and bounded liv eness properties of realtime systems modeled as net orks of w timed automata It includes a graphical in terface that supports graphi cal and textual represen tations of net orks of timed automata and auto w matic transformation from graphical represen tations to textual format a compiler that transforms a certain class of linear h ybrid systems to net orks of timed automata and a modelc w hec er whic k h is implemen ted based on constrain tsolving tec hniques Upp aal also supports diagnos tic modelc hec king pro viding diagnostic information in case v erication of a particular realtime systems fails},
author = {Bengtsson, Johan and Larsen, Kim G and Larsson, Fredrik and Pettersson, Paul and Yi, Wang},
doi = {10.1007/BFb0020949},
isbn = {354061155X},
journal = {Work. Verif. Control Hybrid Syst. III},
keywords = {BL95},
mendeley-tags = {BL95},
number = {1066},
pages = {232--243},
title = {{Uppaal --- a Tool Suite for Automatic Verification of Real--Time Systems}},
url = {http://www.springerlink.com/index/52011553gkv24578.pdf},
year = {1995}
}
@misc{RoboToolLink,
keywords = {RoboToolLink},
mendeley-tags = {RoboToolLink},
title = {{RoboTool}},
note = { Available at https://www.cs.york.ac.uk/circus/RoboCalc/robotool/    (Accessed: 14th August, 2017)},
urldate = {2017-08-10}
}
@article{PNH02,
abstract = {Software for (semi-) autonomous robots tends to be a complex combination of components from many different application domains such as control theory, vision, and artificial intelligence. Components are often developed using their own domain-specific tools and abstractions. System integration can thus be a significant challenge, in particular when the application calls for a dynamic, adaptable system structure in which rigid boundaries between the subsystems are a performance impediment. We believe that, by identifying suitably abstract notions common to the different domains in question, it is possible to create a broader framework for software integration and to recast existing domain-specific frameworks in these terms. This approach simplifies integration and leads to improved reliability. In this paper, we show how Functional Reactive Programming (FRP) can serve as such a unifying framework for programming vision-guided, semi-autonomous robots and illustrate the benefits this approach entails. The key abstractions in FRP, reactive components describing continuous or discrete behavior in a declarative style, are first class entities, allowing the resulting systems to exhibit a dynamic, adaptable structure which we regard as especially important in the area of autonomous robots.},
author = {Pembeci, Izzet and Nilsson, Henrik and Hager, Gregory D},
doi = {doi: 10.1145/571157.571174},
isbn = {1581135289},
journal = {Princ. Pract. Declar. Program.},
keywords = {PNH02,reactive-system},
mendeley-tags = {PNH02},
title = {{System presentation - Functional reactive robotics: an exercise in principled integration of domain-specific languages}},
year = {2002}
}
@article{SN14,
abstract = {This paper presents an approach for defining Unmanned Aerial Vehicle (UAV) missions on a high level. Current methods for UAV mission specification are evaluated and their deficiencies are analyzed. From these findings, a new graphical specification language for UAV missions is proposed, which is targeted towards typical UAV users from various domains rather than computer science experts. The research is ongoing, but a first prototype is presented.},
archivePrefix = {arXiv},
arxivId = {1412.1961},
author = {Schwartz, Benjamin and N{\"{a}}gele, Ludwig and Angerer, Andreas and MacDonald, Bruce A.},
eprint = {1412.1961},
journal = {Work. Domain-Specific Lang. Model. Robot. Syst.},
keywords = {SN14},
mendeley-tags = {SN14},
title = {{Towards a Graphical Language for Quadrotor Missions}},
url = {http://arxiv.org/abs/1412.1961},
year = {2014}
}
@article{SW12,
abstract = {Model-driven software development is a promising way to cope with the complexity of system integration in advanced robotics, as it already demonstrated its benefits in domains with comparably challenging system integration requirements. This paper reports on work in progress in this area which aims to improve the research and experimentation process in a collaborative research project developing motor skill architectures for compliant robots. Our goal is to establish a model-driven development process throughout the project around a domain-specific language (DSL) facilitating the compact description of adaptive modular architectures for rich motor skills. Incorporating further languages for other aspects (e.g. mapping to a technical component architecture) the approach allows not only the formal description of motor skill architectures but also automated code-generation for experimentation on technical robot platforms. This paper reports on a first case study exemplifying how the developed AMARSi DSL helps to conceptualize different architectural approaches and to identify their similarities and differences.},
archivePrefix = {arXiv},
arxivId = {arXiv:1302.6436v1},
author = {Nordmann, Arne and Wrede, Sebastian},
eprint = {arXiv:1302.6436v1},
journal = {Work. Domain-Specific Lang. Model. Robot. Syst.},
keywords = {SW12,domain-specific language,mdsd,modeling},
mendeley-tags = {SW12},
title = {{A Domain-Specific Language for Rich Motor Skill Architectures}},
year = {2012}
}
@article{BD11,
abstract = {UPPAAL is a tool suitable for model checking real-time systems described as networks of timed automata communicating by channel synchronizations and extended with integer variables. Its first version was released in 1995 and its development is still very active. It now features an advanced modeling language, a user-friendly graphical interface, and a performant model checker engine. In addition, several flavors of the tool have matured in recent years. In this paper, we present how we managed to maintain the tool during 15 years, its current architecture with its challenges, and we give the future directions of the tool. Copyright {\textcopyright} 2011 John Wiley {\&} Sons, Ltd.},
author = {Behrmann, Gerd and David, Alexandre and Larsen, Kim Guldstrand and Pettersson, Paul and Yi, Wang},
doi = {10.1002/spe.1006},
journal = {Softw. Pract. Exp.},
keywords = {BD11,UPPAAL,development,model-checker,real-time},
mendeley-tags = {BD11},
title = {{Developing UPPAAL over 15 years}},
year = {2011}
}
@article{BR16,
abstract = {Smart factories that allow flexible production of highly individualized goods require flexible robots, usable in efficient assembly lines. Compliant robots can work safely in shared environments with domain experts, who have to program such robots easily for arbitrary tasks. We propose a new domain-specific language and toolchain for robot assembly tasks for compliant manipulators. With the LightRocks toolchain, assembly tasks are modeled on different levels of abstraction, allowing a separation of concerns between domain experts and robotics experts: externally provided, platform-independent assembly plans are instantiated by the domain experts using models of processes and tasks. Tasks are comprised of skills, which combine platform-specific action models provided by robotics experts. Thereby it supports a flexible production and re-use of modeling artifacts for various assembly processes.},
archivePrefix = {arXiv},
arxivId = {1601.02452},
author = {Butting, Arvid and Rumpe, Bernhard and Schulze, Christoph and Thomas, Ulrike and Wortmann, Andreas},
eprint = {1601.02452},
journal = {Work. Domain Specif. Lang.},
keywords = {BR16},
mendeley-tags = {BR16},
title = {{Modeling Reusable, Platform-Independent Robot Assembly Processes}},
url = {http://arxiv.org/abs/1601.02452},
year = {2015}
}
@article{T11,
abstract = {In this paper we apply a model-driven engineering approach to designing domain-specific solutions for robot control system development. We present a case study of the complete process, including identification of the domain metamodel, graphical notation definition and source code generation for subsumption architecture – a well-known example of robot control architecture. Our goal is to show that both the definition of the robot-control architecture and its supporting tools fits well into the typical workflow of model-driven engineering development.},
archivePrefix = {arXiv},
arxivId = {arXiv:1302.5085v1},
author = {Trojanek, Piotr},
eprint = {arXiv:1302.5085v1},
journal = {Proc. Second Int. Work. Domain-Specific Lang. Model. Robot. Syst. (DSLRob 2011)},
keywords = {T11},
mendeley-tags = {T11},
title = {{Model-driven engineering approach to design and implementation of robot control system}},
year = {2011}
}
@article{Z99,
abstract = {The paper proposes a structure for open, hierarchical, multi-device controllers. The proposed structure takes into account that the system may contain several robots of different type, a certain number of cooperating devices, diverse sensors and also the fact that the task, the system has to execute, and the number and type of its components may vary considerably over time. The concept has been verified by designing a controller for a prototype RNT robot and an ASEA IRb-6 type robot. The flexibility of the system is due to the software, so the programming aspect is treated in detail.},
author = {{Cezary Zielihski}},
file = {:home/abdul/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Cezary Zielihski - 1999 - The MRROC System.pdf:pdf},
journal = {Robot Motion Control. 1999. RoMoCo '99. Proc. First Work.},
keywords = {Z99},
mendeley-tags = {Z99},
title = {{The MRROC++ System}},
url = {http://ieeexplore.ieee.org/abstract/document/791067/},
year = {1999}
}
@misc{,
title = {{DSLs}}
}
@article{CF02,
abstract = {Computational fluid dynamics (CFD) computer codes have become an integral part of the analysis and scientific investigation of complex, engineering flow systems. Unfortunately, inherent in the solutions from simulations performed with these computer codes is error or uncertainty in the results. The issue of numerical uncertainty addresses the development of methods to define the magnitude of error or to bound the error in a given simulation. This paper reviews the status of methods for evaluation of numerical uncertainty, and provides a direction for the effective use of some techniques in estimating uncertainty in a simulation. {\textcopyright} 2002 Elsevier Science Inc. All rights reserved.},
author = {Freitas, Christopher J.},
doi = {10.1016/S0307-904X(01)00058-0},
isbn = {0307-904X},
journal = {Appl. Math. Model.},
keywords = {CF02},
mendeley-tags = {CF02},
title = {{The issue of numerical uncertainty}},
year = {2002}
}
@article{Mallet2002a,
abstract = {Robotics systems and software are becoming more and more complex: the need of standard specifications is certainly a key issue in the near future. There is a need to define, from the software point of view, a generic robot. The Orocos project was started to address this problem. It aims at developing a set of robotics software in particular domains and, as a first step, will define a software framework to do that. This paper presents the future evolutions of GenoM (component generator) which we propose as a programming framework in the context of the project. GenoM proposes the definition of generic components that are used to implement robotics functionalities (vision, control, motion planning, ...), and the paper presents the definition of those components. They have been designed so that they can be connected together and externally controlled to form a modular functional layer on robots. We have defined three main entities of which components are made: a set of algorithms, an execution engine, and a communication library. The paper explains their role and presents a formal description language that let us achieves a real decoupling between code of the components (the algorithms) and the execution engine.},
author = {Mallet, a. and Fleury, S. and Bruyninckx, H.},
doi = {10.1109/IRDS.2002.1041609},
isbn = {0-7803-7398-7},
journal = {IEEE/RSJ Int. Conf. Intell. Robot. Syst.},
number = {October},
pages = {2292--2297},
title = {{A specification of generic robotics software components: future evolutions of G/sup en//sub o/M in the Orocos context}},
url = {http://ieeexplore.ieee.org/lpdocs/epic03/wrapper.htm?arnumber=1041609},
volume = {3},
year = {2002}
}
@inproceedings{MH11,
abstract = {This paper presents recent developments of the LAAS architecture for autonomous systems: the GenoM3 component generator for functional components design. The GenoM tool was originally designed for autonomous and terrestrial mobile robots. This tool remains fairly general and is supported by a consistently integrated set of tools and methodologies, in order to properly design, integrate, test and validate a complex autonomous system. GenoM3 intends to grant middleware independance to robotic software components so that a clear separation of concerns is achieved between highly reusable algorithmic parts and integration frameworks. Such a decoupling let middlewares be used interchangeably, while fully benefitting from their specific, individual features.},
author = {Mallet, Anthony and Herrb, Matthieu},
booktitle = {6th Natl. Conf. Control Archit. Robot.},
keywords = {MH11},
mendeley-tags = {MH11},
title = {{Recent developments of the GenoM robotic component generator}},
year = {2011}
}
@inproceedings{RC13,
abstract = {From exploring planets to cleaning homes, the reach and versatility of robotics is vast. The integration of actuation, sensing and control makes robotics systems powerful, but complicates their simulation. This paper introduces a versatile, scalable, yet powerful general-purpose robot simulation framework called V-REP. The paper discusses the utility of a portable and flexible simulation framework that allows for direct incorporation of various control techniques. This renders simulations and simulation models more accessible to a general-public, by reducing the simulation model deployment complexity. It also increases productivity by offering built-in and ready-to-use functionalities, as well as a multitude of programming approaches. This allows for a multitude of applications including rapid algorithm development, system verification, rapid prototyping, and deployment for cases such as safety/remote monitoring, training and education, hardware control, and factory automation simulation.},
author = {Rohmer, Eric and Singh, Surya P.N. and Freese, Marc},
booktitle = {IEEE Int. Conf. Intell. Robot. Syst.},
doi = {10.1109/IROS.2013.6696520},
isbn = {9781467363587},
keywords = {RC13},
mendeley-tags = {RC13},
pmid = {6696520},
title = {{V-REP: A versatile and scalable robot simulation framework}},
year = {2013}
}
@article{Thomas2013,
abstract = {This paper introduces the new robot programming language LightRocks(Light Weight Robot Coding for Skills), a domain specific language (DSL) for robot programming. The language offers three different level of abstraction for robot programming. On lowest level skills are coded by domain experts. On a more abstract level these skills are supposed to be combined by shop floor workers or technicians to define tasks. The language is designed to allow as much flexibility as necessary on the lowest level of abstraction and is kept as simple as possible with the more abstract layers. A Statechart like model is used to describe the different levels of detail. For this we apply the UML/P and the language workbench MontiCore. To this end we are able to generate code while hiding controller specific implementation details. In addition the development in LightRocks is supported by a generic graphical editor implemented as an Eclipse plugin.},
author = {Thomas, Ulrike and Hirzinger, Gerd and Rumpe, Bernhard and Schulze, Christoph and Wortmann, Andreas},
doi = {10.1109/ICRA.2013.6630615},
isbn = {9781467356428},
issn = {1050-4729},
journal = {IEEE Int. Conf. Robot. Autom.},
keywords = {Compliant Assembly,Discrete Event Dynamic Automation Systems,Middleware and Programming Environments,Robotic Software},
pages = {461--466},
title = {{A New Skill Based Robot Programming Language Using UML / P Statecharts}},
year = {2013}
}
@article{JT13,
abstract = {Programming robots is a complicated and time-consuming task. A robot is essentially a real-time, distributed embedded system. Often, control and communication paths within the system are tightly coupled to the actual physical configuration of the robot. Thus, programming a robot can hardly be achieved by experts of the domain in which the robot is used. In this paper we present an approach towards a domain specific language, which is intended to empower domain experts or even end users to specify robot programs with a dedicated background in programming techniques, but not with special knowledge in the robotics domain. Furthermore we introduce an idea to integrate a software product-line for a hardware and software transparent plug and play mechanism. Copyright {\textcopyright} 2013 SCITEPRESS.},
author = {Baumgartl, J and Buchmann, T and Henrich, D and Westfechtel, B},
isbn = {9789898565686 (ISBN)},
journal = {8th Int. Jt. Conf. Softw. Technol. ICSOFT 2013},
keywords = {Code Generation,Code generation,Computer software,DSL,Distributed embedded system,Domain specific languages,Easy programming,Hardware and software,JT13,Model driven development,Model-driven development,Programming technique,Robot,Robot programming,Robots,Software Product Line,Software product lines,Time-consuming tasks},
mendeley-tags = {JT13},
pages = {548--554},
title = {{Towards easy robot programming: Using DSLs, code generators and software product lines}},
url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-84887046815{\&}partnerID=40{\&}md5=6f68a556866eda0b643e4788ddd7004e},
year = {2013}
}
@misc{,
title = {{LightRocks-A New Skill Based Robot Programming Language Using}}
}

@book{R10,
author = {Roscoe, Andrew William},
keywords = {R10},
mendeley-tags = {R10},
publisher = {Springer Science {\&} Business Media},
title = {{Understanding Concurrent Systems.}},
year = {2010}
}
@inproceedings{MP10,
abstract = {The topic of reusable software in robotics is now largely addressed. Components based architectures, where components are independent units that can be reused accross applications, have become more popular. As a consequence, a long list of middlewares and integration tools is available in the community, often in the form of open-source projects. However, these projects are generally self contained with little reuse between them. This paper presents a software engineering approach that intends to grant middleware independance to robotic software components so that a clear separation of concerns is achieved between highly reusable algorithmic parts and integration frameworks. Such a decoupling let middle-wares be used interchangeably, while fully benefitting from their specific, individual features. This work has been integrated into a new version of the open-source GenoM component generator tool: GenoM3},
author = {Mallet, Anthony and Pasteur, C{\'{e}}dric and Herrb, Matthieu and Lemaignan, S{\'{e}}verin and Ingrand, F{\'{e}}lix},
booktitle = {Proc. - IEEE Int. Conf. Robot. Autom.},
doi = {10.1109/ROBOT.2010.5509539},
isbn = {9781424450381},
issn = {10504729},
keywords = {MP10},
mendeley-tags = {MP10},
title = {{GenoM3: Building middleware-independent robotic components}},
year = {2010}
}
@article{C73,
abstract = {This paper discusses human semantic knowledge and processing in terms of the SCHOLAR system. In one major section we discuss the imprecision, the incompleteness, the open-endedness, and the uncertainty of people's knowledge. In the other majo rsetion we discuss strategies people use to make different types of deductive, negative and functional inferences and the way uncertainties combine in these inferences.},
author = {Carbonell, Jaime R. and Collina, Allan M.},
journal = {IJCAI},
keywords = {C73,a n s w,c e s s,c o g n,c t i o,d e d u,e,e p r o,e r i n,e s,e s s i,g systems,human memory,i n f e,i t i v,n,n a t u,n g,p r o c,q u e s,r a l language,r e n c,semantics,t i o n},
mendeley-tags = {C73},
title = {{Natural semantics in artificial intelligence}},
year = {1973}
}
@misc{siriuslink,
keywords = {siriuslink},
mendeley-tags = {siriuslink},
title = {{Sirius}},
note = { Available at https://www.eclipse.org/sirius/  (Accessed: 14th August, 2017) }
}
@misc{xtextlink,
keywords = {xtextlink},
mendeley-tags = {xtextlink},
title = {{Xtext}},
note = { Available at https://eclipse.org/Xtext/   (Accessed: 14th August, 2017)}
}

@inproceedings{BS16,
abstract = {Robotic tasks are becoming increasingly complex, and with this also the robotic systems. This requires new tools to manage this complexity and to orchestrate the systems to fulfill demanding autonomous tasks. For this purpose, we developed a new graphical tool targeting at the creation and execution of robotic tasks, called RAFCON. These tasks are described in hierarchical state machines supporting concurrency. A formal notation of this concept is given. The tool provides many debugging mechanisms and a GUI with a graphical editor, allowing for intuitive visual programming and fast prototyping. The application of RAFCON for an autonomous mobile robot in the SpaceBotCamp competition has already proved to be successful.},
author = {Brunner, Sebastian G. and Steinmetz, Franz and Belder, Rico and D??mel, Andreas},
booktitle = {IEEE Int. Conf. Intell. Robot. Syst.},
doi = {10.1109/IROS.2016.7759506},
isbn = {9781509037629},
issn = {21530866},
keywords = {BS16},
mendeley-tags = {BS16},
title = {{RAFCON: A graphical tool for engineering complex, robotic tasks}},
year = {2016}
}
@article{KR10,
abstract = {Domain specific languages (DSLs) are increasingly used today. Coping with complex language definitions, evolving them in a structured way, and ensuring their error freeness are the main challenges of DSL design and implementation. The use of modular language definitions and composition operators are therefore inevitable in the independent development of language components. In this article, we discuss these arising issues by describing a framework for the compositional development of textual DSLs and their supporting tools. We use a redundance-free definition of a readable concrete syntax and a comprehensible abstract syntax as both representations significantly overlap in their structure. For enhancing the usability of the abstract syntax, we added concepts like associations and inheritance to a grammar-based definition in order to build up arbitrary graphs (as known from metamodeling). Two modularity concepts, grammar inheritance and embedding, are discussed. They permit compositional language definition and thus simplify the extension of languages based on already existing ones. We demonstrate that compositional engineering of new languages is a useful concept when project-individual DSLs with appropriate tool support are defined.},
author = {Krahn, Holger and Rumpe, Bernhard and V{\"{o}}lkel, Steven},
doi = {10.1007/s10009-010-0142-1},
isbn = {9781605580791},
issn = {14332779},
journal = {Int. J. Softw. Tools Technol. Transf.},
keywords = {Composition,Domain specific language,Grammarware,KR10},
mendeley-tags = {KR10},
title = {{MontiCore: A framework for compositional development of domain specific languages}},
year = {2010}
}
@misc{TC15,
abstract = {General-purpose robots can perform a range of useful tasks in human environments; however, programming them to robustly function in all possible environments that they might encounter is unfeasible. Instead, our research aims to develop robots that can be programmed by its end-users in their context of use, so that the robot needs to robustly function in only one particular environment. This requires intuitive ways in which end-users can program their robot. To that end, this paper contributes a flow-based visual programming language, called RoboFlow, that allows programming of generalizable mobile manipulation tasks. RoboFlow is designed to (i) ensure a robust low-level implementation of program procedures on a mobile manipulator, and (ii) restrict the high-level programming as much as possible to avoid user errors while enabling expressive programs that involve branching, looping, and nesting. We present an implementation of RoboFlow on a PR2 mobile manipulator and demonstrate the generalizability and error handling properties of RoboFlow programs on everyday mobile manipulation tasks in human environments.},
author = {Alexandrova, S and Tatlock, Z and Cakmak, M},
booktitle = {Robot. Autom. (ICRA), 2015 IEEE Int. Conf.},
doi = {10.1109/ICRA.2015.7139973},
isbn = {VO -},
keywords = {Computer languages,Mobile communication,Navigation,PR2 mobile manipulator,Programming profession,RoboFlow programs,Robots,TC15,Visualization,control engineering computing,flow-based visual programming language,general-purpose robots,high-level programming,human environments,manipulators,mobile manipulation tasks,mobile robots,visual languages,visual programming},
mendeley-tags = {TC15},
title = {{RoboFlow: A flow-based visual programming language for mobile manipulation tasks}},
year = {2015}
}
@misc{RoboFlowEditorLink,
keywords = {RoboFlowEditorLink},
mendeley-tags = {RoboFlowEditorLink},
title = {{RoboFlow Editor}},
note = { Available at https://github.com/sonyaa/roboflow  (Accessed: 14th August, 2017)}
}


@article{G91,
abstract = {The author introduces ALFA, a language for programming reactive$\backslash$ncontrol mechanisms for autonomous mobile robots. ALFA programs consist$\backslash$nof networks of computational modules connected by communications$\backslash$nchannels. These channels are themselves computational entities which$\backslash$nperform mediation tasks. This makes it possible to design modular$\backslash$nbehaviors which may be inserted and removed without having to$\backslash$nrestructure the interconnections among modules and allows the system to$\backslash$ninterface cleanly with higher-level reasoning processes. ALFA supports a$\backslash$ndataflow computation model as well as a state-machine model. The results$\backslash$nof two experiments using ALFA to control real robots are briefly$\backslash$ndiscussed},
author = {Gat, E.},
doi = {10.1109/ROBOT.1991.131743},
isbn = {0-8186-2163-X},
issn = {10504729},
journal = {Proceedings. 1991 IEEE Int. Conf. Robot. Autom.},
keywords = {G91},
mendeley-tags = {G91},
title = {{ALFA: a language for programming reactive robotic control systems}},
year = {1991}
}

@inproceedings{NW12,
abstract = {Model-driven software development is a promising way to cope with the complexity of system integration in advanced robotics, as it already demonstrated its benefits in domains with comparably challenging system integration requirements. This paper reports on work in progress in this area which aims to improve the research and experimentation process in a collaborative research project developing motor skill architectures for compliant robots. Our goal is to establish a model-driven development process throughout the project around a domain-specific language (DSL) facilitating the compact description of adaptive modular architectures for rich motor skills. Incorporating further languages for other aspects (e.g. mapping to a technical component architecture) the approach allows not only the formal description of motor skill architectures but also automated code-generation for experimentation on technical robot platforms. This paper reports on a first case study exemplifying how the developed AMARSi DSL helps to conceptualize different architectural approaches and to identify their similarities and differences.},
archivePrefix = {arXiv},
arxivId = {arXiv:1302.6436v1},
author = {Nordmann, Arne and Wrede, Sebastian},
booktitle = {Work. Domain-Specific Lang. Model. Robot. Syst.},
eprint = {arXiv:1302.6436v1},
keywords = {NW12,domain-specific language,mdsd,modeling},
mendeley-tags = {NW12},
title = {{A Domain-Specific Language for Rich Motor Skill Architectures}},
year = {2012}
}



@article{H78,
  title={Communicating sequential processes},
  author={Hoare, Charles Antony Richard},
  journal={Communications of the ACM},
  volume={21},
  number={8},
  pages={666--677},
  year={1978},
  publisher={ACM}
}


@book{JJ96,
  title={Using Z: Specification ‚Refinement ‚and Proof},
  author={Woodcock, Jim and Davies, Jim},
  year={1996},
  publisher={Prentice Hall International}
}
 
@book{J06,
  title={Software abstractions},
  author={Jackson, Daniel},
  volume={2},
  year={2006},
  publisher={MIT press Cambridge}
}



@article{LB18,
  title={Sampling-Based Approximation Algorithms for Reachability Analysis with Provable Guarantees},
  author={Liebenwein, Lucas and Baykal, Cenk and Gilitschenski, Igor and Karaman, Sertac and Rus, Daniela},
  year={2018}
}

@inproceedings{DO95,
  title={The tool KRONOS},
  author={Daws, Conrado and Olivero, Alfredo and Tripakis, Stavros and Yovine, Sergio},
  booktitle={International Hybrid Systems Workshop},
  pages={208--219},
  year={1995},
  organization={Springer}
}

@article{F08,
  title={PHAVer: algorithmic verification of hybrid systems past HyTech},
  author={Frehse, Goran},
  journal={International Journal on Software Tools for Technology Transfer},
  volume={10},
  number={3},
  pages={263--279},
  year={2008},
  publisher={Springer}
}

@article{HH97,
  title={HyTech: A model checker for hybrid systems},
  author={Henzinger, Thomas A and Ho, Pei-Hsin and Wong-Toi, Howard},
  journal={International Journal on Software Tools for Technology Transfer},
  volume={1},
  number={1-2},
  pages={110--122},
  year={1997},
  publisher={Springer}
}


@article{M89,
  title={Communication and concurrency},
  author={Milner, R},
  year={1989},
  publisher={Prentice-Hall, Inc.}
}



@book{R12,
  title={Implementing programming languages. An introduction to compilers and interpreters},
  author={Ranta, Aarne},
  year={2012},
  publisher={College Publications}
}


@book{H16,
  title={Programming in haskell},
  author={Hutton, Graham},
  year={2016},
  publisher={Cambridge University Press}
}


@article{H89,
  title={Why functional programming matters},
  author={Hughes, John},
  journal={The computer journal},
  volume={32},
  number={2},
  pages={98--107},
  year={1989},
  publisher={Oxford University Press}
}



%FRP
@inproceedings{WH00,
  title={Functional reactive programming from first principles},
  author={Wan, Zhanyong and Hudak, Paul},
  booktitle={Acm sigplan notices},
  volume={35},
  number={5},
  pages={242--252},
  year={2000},
  organization={ACM}
}


@inproceedings{PH99,
  title={Lambda in motion: Controlling robots with Haskell},
  author={Peterson, John and Hudak, Paul and Elliott, Conal},
  booktitle={International Symposium on Practical Aspects of Declarative Languages},
  pages={91--105},
  year={1999},
  organization={Springer}
}


@inproceedings{HC02,
  title={Arrows, robots, and functional reactive programming},
  author={Hudak, Paul and Courtney, Antony and Nilsson, Henrik and Peterson, John},
  booktitle={International School on Advanced Functional Programming},
  pages={159--187},
  year={2002},
  organization={Springer}
}


@inproceedings{HH07,
  title={A history of Haskell: being lazy with class},
  author={Hudak, Paul and Hughes, John and Peyton Jones, Simon and Wadler, Philip},
  booktitle={Proceedings of the third ACM SIGPLAN conference on History of programming languages},
  pages={12--1},
  year={2007},
  organization={ACM}
}


@book{L11,
  title={Learn you a haskell for great good!: a beginner's guide},
  author={Lipovaca, Miran},
  year={2011},
  publisher={no starch press}
}



@misc{Haskelllink,
keywords = {Haskelllink},
mendeley-tags = {Haskelllink},
title = {{Haskell}},
note = { Available at https://www.haskell.org   (Accessed: 08th September, 2019)}
}


@article{DH08,
  title={Timed automata patterns},
  author={Dong, Jin Song and Hao, Ping and Qin, Shengchao and Sun, Jun and Yi, Wang},
  journal={IEEE Transactions on Software Engineering},
  volume={34},
  number={6},
  pages={844--859},
  year={2008},
  publisher={IEEE}
}


@article{F05,
  title={{From Circus to Java}: Implementation and verification of a translation strategy},
  author={de Freitas, Angela Figueiredo},
  journal={Master's thesis, University of York},
  year={2005}
}







@inproceedings{LM04,
  title={Online testing of real-time systems using uppaal},
  author={Larsen, Kim G and Mikucionis, Marius and Nielsen, Brian},
  booktitle={International Workshop on Formal Approaches to Software Testing},
  pages={79--94},
  year={2004},
  organization={Springer}
}

% Larsen K, Mikučionis M, Nielsen B. Online testing of real-time systems using U PPAAL . FATES’04 (Lecture
% Notes in Computer Science). Springer: Berlin, Linz, Austria, September 2004; 79–94.





@inproceedings{LM05,
  title={Testing real-time embedded software using UPPAAL-TRON: an industrial case study},
  author={Larsen, Kim G and Mikucionis, Marius and Nielsen, Brian and Skou, Arne},
  booktitle={Proceedings of the 5th ACM international conference on Embedded software},
  pages={299--306},
  year={2005},
  organization={ACM}
}

% 24. Larsen KG, Mikucionis M, Nielsen B. Testing real-time embedded software using uppaal-tron: An industrial
% case study. The 5th ACM International Conference on Embedded Software. ACM Press: New York, NY, U.S.A.,
% 2005; 299–306.



@inproceedings{BA07,
  title={Uppaal-tiga: Time for playing games!},
  author={Behrmann, Gerd and Cougnard, Agnes and David, Alexandre and Fleury, Emmanuel and Larsen, Kim G and Lime, Didier},
  booktitle={International Conference on Computer Aided Verification},
  pages={121--125},
  year={2007},
  organization={Springer}
}






@inproceedings{FP02,
  title={Timed automata with asynchronous processes: Schedulability and decidability},
  author={Fersman, Elena and Pettersson, Paul and Yi, Wang},
  booktitle={International Conference on Tools and Algorithms for the Construction and Analysis of Systems},
  pages={67--82},
  year={2002},
  organization={Springer}
}



@article{HS12,
  title={Analysis of a clock synchronization protocol for wireless sensor networks},
  author={Heidarian, Faranak and Schmaltz, Julien and Vaandrager, Frits},
  journal={Theoretical Computer Science},
  volume={413},
  number={1},
  pages={87--105},
  year={2012},
  publisher={Elsevier}
}



@inproceedings{GV06,
  title={Analysis of the zeroconf protocol using UPPAAL},
  author={Gebremichael, Biniam and Vaandrager, Frits and Zhang, Miaomiao},
  booktitle={Proceedings of the 6th ACM \& IEEE International conference on Embedded software},
  pages={242--251},
  year={2006},
  organization={ACM}
}

@article{AH09,
  title={Adaptive scheduling of data paths using Uppaal Tiga},
  author={AlAttili, Israa and Houben, Fred and Igna, Georgeta and Michels, Steffen and Zhu, Feng and Vaandrager, Frits},
  journal={arXiv preprint arXiv:0912.1897},
  year={2009}
}

@inproceedings{AB09,
  title={Using uppaal for the secure and optimal control of agv fleets},
  author={Arnaud, Yoann and Boimond, Jean-Louis and Cury, Jose and Loiseau, Jean Jacques and Martinez, Claude},
  year={2009}
}


@article{JP19,
  title={Reasoning in tock-{CSP} with {FDR}},
  author={Baxter, James and Ribeiro, Pedro and Cavalcanti, Ana}
}

@article{CE86,
  title={Automatic verification of finite-state concurrent systems using temporal logic specifications},
  author={Clarke, Edmund M. and Emerson, E Allen and Sistla, A Prasad},
  journal={ACM Transactions on Programming Languages and Systems (TOPLAS)},
  volume={8},
  number={2},
  pages={244--263},
  year={1986},
  publisher={ACM}
}

@inproceedings{MP86,
  title={An automata-theoretic approach to automatic program verification},
  author={Vardi, Moshe Y and Wolper, Pierre},
  booktitle={Proceedings of the First Symposium on Logic in Computer Science},
  pages={322--331},
  year={1986},
  organization={IEEE Computer Society}
}

@book{HM08,
  title={Introduction to automata theory, languages, and computation},
  author={Hopcroft, John E},
  year={2008},
  publisher={Pearson Education India}
}


@article{KJ17,
  title={Model checking of state-rich formalism by linking to  {$CSP \parallel B$ } },
  author={Ye, Kangfeng and Woodcock, Jim},
  journal={International Journal on Software Tools for Technology Transfer},
  volume={19},
  number={1},
  pages={73--96},
  year={2017},
  publisher={Springer}
}




@article{A93,
  title={Model-checking in dense real-time},
  author={Alur, Rajeev and Courcoubetis, Costas and Dill, David},
  journal={Information and computation},
  volume={104},
  number={1},
  pages={2--34},
  year={1993},
  publisher={Elsevier}
}


@book{A15,
  title={Principles of cyber-physical systems},
  author={Alur, Rajeev},
  year={2015},
  publisher={MIT Press}
}

@article{A13,
  title={Can we verify cyber-physical systems? technical perspective},
  author={Alur, Rajeev},
  journal={Communications of the ACM},
  volume={56},
  number={10},
  pages={96--96},
  year={2013},
  publisher={ACM New York, NY, USA}
}


@inproceedings{P12,
  title={Logical analysis of hybrid systems},
  author={Platzer, Andr{\'e}},
  booktitle={International Workshop on Descriptional Complexity of Formal Systems},
  pages={43--49},
  year={2012},
  organization={Springer}
}


@inproceedings{P19, place={S.l.}, title={LOGICAL FOUNDATIONS OF CYBER-PHYSICAL SYSTEMS}, publisher={SPRINGER}, author={PLATZER, ANDRE}, year={2019}}

@inproceedings{P18,
  title={Logical Foundations of Cyber-Physical Systems},
  author={Platzer, Andre},
  booktitle={Logical Foundations of Cyber-Physical Systemsw},
  year={2018},
  publisher={Springer}
}


@inproceedings{DO02,
  title={Formal verification of UML statecharts with real-time extensions},
  author={David, Alexandre and M{\"o}ller, M Oliver and Yi, Wang},
  booktitle={International Conference on Fundamental Approaches to Software Engineering},
  pages={218--232},
  year={2002},
  organization={Springer}
}


@article{MP01,
  title={Formal design and analysis of a gear controller},
  author={Lindahl, Magnus and Pettersson, Paul and Yi, Wang},
  journal={International Journal on Software Tools for Technology Transfer},
  volume={3},
  number={3},
  pages={353--368},
  year={2001},
  publisher={Springer}
}

@inproceedings{CB19,
  title={Testing Robots Using {CSP}},
  author={Cavalcanti, Ana and Baxter, James and Hierons, Robert M and Lefticaru, Raluca},
  booktitle={International Conference on Tests and Proofs},
  pages={21--38},
  year={2019},
  organization={Springer}
}


@inproceedings{NS00,
  title={Analysing time dependent security properties in {CSP} using PVS},
  author={Evans, Neil and Schneider, Steve},
  booktitle={European Symposium on Research in Computer Security},
  pages={222--237},
  year={2000},
  organization={Springer}
}

@inproceedings{YF12,
  title={Safety and line capacity in railways--an approach in Timed {CSP}},
  author={Isobe, Yoshinao and Moller, Faron and Nguyen, Hoang Nga and Roggenbach, Markus},
  booktitle={International Conference on Integrated Formal Methods},
  pages={54--68},
  year={2012},
  organization={Springer}
}



@misc{VC20,
url={https://www.cs.york.ac.uk/robostar/case_studies/vacuum_cleaner/index.html},
journal={Cs.york.ac.uk},
year={2020}
}


@phdthesis{C13,
  title={Verification of liveness properties on hybrid dynamical systems},
  author={Carter, Rebekah},
  year={2013},
  school={The University of Manchester (United Kingdom)}
}



@article{G08,
  title={Specification of communicating processes: temporal logic versus refusals-based refinement},
  author={Lowe, Gavin},
  journal={Formal Aspects of Computing},
  volume={20},
  number={3},
  pages={277--294},
  year={2008},
  publisher={Springer}
}


@inproceedings{TS13,
  title={Automatic validation of infinite real-time systems},
  author={G{\"o}thel, Thomas and Glesner, Sabine},
  booktitle={2013 1st FME Workshop on Formal Methods in Software Engineering (FormaliSE)},
  pages={57--63},
  year={2013},
  organization={IEEE}
}



@inproceedings{DP06,
  title={A reasoning method for timed {CSP} based on constraint solving},
  author={Dong, Jin Song and Hao, Ping and Sun, Jun and Zhang, Xian},
  booktitle={International Conference on Formal Engineering Methods},
  pages={342--359},
  year={2006},
  organization={Springer}
}


@article{KM19,
  title={Survey and classification of model transformation tools},
  author={Kahani, Nafiseh and Bagherzadeh, Mojtaba and Cordy, James R and Dingel, Juergen and Varr{\'o}, Daniel},
  journal={Software \& Systems Modeling},
  volume={18},
  number={4},
  pages={2361--2397},
  year={2019},
  publisher={Springer}
}


@phdthesis{O00,
  title={Discrete analysis of continuous behaviour in real-time concurrent systems},
  author={Ouaknine, Joel},
  year={2000},
  school={University of Oxford}
}




@inproceedings{MP98,
  title={Formal design and analysis of a gear controller},
  author={Lindahl, Magnus and Pettersson, Paul and Yi, Wang},
  booktitle={International Conference on Tools and Algorithms for the Construction and Analysis of Systems},
  pages={281--297},
  year={1998},
  organization={Springer}
}

@inproceedings{D02,
  title={Formal verification of UML statecharts with real-time extensions},
  author={David, Alexandre and M{\"o}ller, M Oliver and Yi, Wang},
  booktitle={International Conference on Fundamental Approaches to Software Engineering},
  pages={218--232},
  year={2002},
  organization={Springer}
}




@inproceedings{NS08,
  title={Guided test generation from {CSP} models},
  author={Nogueira, Sidney and Sampaio, Augusto and Mota, Alexandre},
  booktitle={International Colloquium on Theoretical Aspects of Computing},
  pages={258--273},
  year={2008},
  organization={Springer}
}



@inproceedings{K11,
  title={Translating {Timed Automata} to tock-{CSP}},
  author={Khattri, Maneesh},
  booktitle={Proceedings of the 10th IASTED International Conference on Software Engineering, SE 2011},
  year={2011}
}


@inproceedings{HL14,
  title={Translating {B to TLA+ for validation with TLC} },
  author={Hansen, Dominik and Leuschel, Michael},
  booktitle={International Conference on Abstract State Machines, Alloy, B, TLA, VDM, and Z},
  pages={40--55},
  year={2014},
  organization={Springer}
}


@inproceedings{HL12,
  title={Translating {TLA+ to B for validation with ProB}},
  author={Hansen, Dominik and Leuschel, Michael},
  booktitle={International Conference on Integrated Formal Methods},
  pages={24--38},
  year={2012},
  organization={Springer}
}


@inproceedings{LP07,
  title={Generating trace-sets for model-based testing},
  author={Lindstrom, Birgitta and Pettersson, Paul and Offutt, Jeff},
  booktitle={The 18th IEEE International Symposium on Software Reliability (ISSRE'07)},
  pages={171--180},
  year={2007},
  organization={IEEE}
}



@misc{extendedVersion,
title = {Archives repository of this work},
note = {https://github.com/ahagmj/TemporalReasoning.git}
}





@article{T06,
  title={A taxonomy of model transformation},
  author={Mens, Tom and Van Gorp, Pieter},
  journal={Electronic notes in theoretical computer science},
  volume={152},
  pages={125--142},
  year={2006},
  publisher={Elsevier}
}

@book{NN07,
  title={Semantics with applications: an appetizer},
  author={Nielson, Hanne Riis and Nielson, Flemming},
  year={2007},
  publisher={Springer Science \& Business Media}
}



@phdthesis{O05,
  title={Formal derivation of state-rich reactive programs using Circus},
  author={Oliveira, Marcel Vinicius Medeiros},
  year={2005},
  school={University of York}
}

@phdthesis{thesis,
title={Temporal Reasoning About Robotics Applications: Refinement and Temporal Logic},
author={Abdulrazaq Abba},
year={2021},
school={The University of York, UK}
}

@article{B81,
  title={On correct refinement of programs},
  author={Back, RJR},
  journal={Journal of Computer and System Sciences},
  volume={23},
  number={1},
  pages={49--68},
  year={1981},
  publisher={Elsevier}
}


@incollection{CO95,
  title={Verifying et-lotos Programs with Kronos},
  author={Daws, Conrado and Olivero, Alfredo and Yovine, Sergio},
  booktitle={Formal Description Techniques VII},
  pages={227--242},
  year={1995},
  publisher={Springer}
}


@article{HG98,
  title={Automatic verification of a lip-synchronisation protocol using \uppaal},
  author={Bowman, Howard and Faconti, Giorgio and Katoen, J-P and Latella, Diego and Massink, Mieke},
  journal={Formal Aspects of Computing},
  volume={10},
  number={5-6},
  pages={550--575},
  year={1998},
  publisher={Springer}
}




@article{B09,
  title={Model-checking timed temporal logics},
  author={Bouyer, Patricia},
  journal={Electronic Notes in Theoretical Computer Science},
  volume={231},
  pages={323--341},
  year={2009},
  publisher={Elsevier}
}


@article{DR16,
  title={Reducing complex CSP models to traces via priority},
  author={Mestel, David and Roscoe, AW},
  year={2016},
  publisher={Elsevier}
}


@inproceedings{ST18,
  title={LTL Semantic Tableaux and Alternating $ \omega$-automata via Linear Factors},
  author={Sulzmann, Martin and Thiemann, Peter},
  booktitle={International Colloquium on Theoretical Aspects of Computing},
  pages={11--34},
  year={2018},
  organization={Springer}
}


@article{R05,
  title={The theory and practice of concurrency. 2005},
  author={Roscoe, AW and Hoare, CAR and Bird, R},
  journal={Revised edition. Only available online},
  year={2005}
}


@inproceedings{SL09,
  title={PAT: Towards flexible verification under fairness},
  author={Sun, Jun and Liu, Yang and Dong, Jin Song and Pang, Jun},
  booktitle={International Conference on Computer Aided Verification},
  pages={709--714},
  year={2009},
  organization={Springer}
}

==> zz_del/BNF.tex <==

\vspace{0.2cm}
\begin{tcolorbox} %[title=Title]
\begin{definition} \textbf{Data definition of \lstinline{CSPproc}} 
\label{dfn_CSPproc}
\end{definition}
\tcblower
\lstset{frameround=fttt}
\vspace{-0.2cm}
\begin{lstlisting}[mathescape, language=Haskell, basicstyle=\ttfamily, columns=flexible]
data CSPproc =   STOP
               | SKIP
               | Prefix       Event       CSPproc
               | IntChoice    CSPproc     CSPproc
               | GenPar       CSPproc     CSPproc  [Event]
\end{lstlisting}
\end{tcolorbox}




%  This section describes the characterisation of tock-CSP using BNF grammar. The following BNF in \autoref{BNF_tockCSP} defines a valid syntax for constructing a tock-CSP process that we consider within the scope of this work.


% This section describes the characterisation of tock-CSP using BNF grammar for the tock-CSP language. The following BNF in \autoref{BNF_tockCSP} defines a valid syntax for constructing a tock-CSP process that we consider within the scope of this work.

%A tock-CSP process is constructed according to the following BNF grammar.        


% \begin{figure}

% \begin{align*}
% NamedProc  &::= Name \  CSPproc   \ \\
%                 & \ \ \ | \ Name \ CSPexpression \ CSPproc
% \end{align*}

% \begin{align*}
% CSPproc &::=  STOP \ \\
%         & | \ Stopu \ \\ 
%         & | \ SKIP \ \\
%         & | \ Skipu \ \\         
%         & | \ Wait(Expression) \ \\ 
%         & | \ Waitu(Expression) \ \\ 
%         & | \ Event \rightarrow CSPproc \ \\
%         & | \ CSPproc \ \square \ CSPproc \ \\   %External choice
%         & | \ CSPproc \ \sqcap\ Proc \ \\     %Internal choice
%         & | \ CSPproc;CSPproc \ \\               %Sequential 
%         %& | \ Proc \mathbin{_{Event}{\|}_{Event}} Proc   \\     %Alphabetized par
%         & | \ CSPproc|||CSPproc \ \\       %Interleaving
%         & | \ CSPproc \ \underset{\{Event\}}{||} \ CSPproc \ \\       % Gen par
%         & | \ CSPproc \vartriangle  CSPproc \\            % Interrupt
%         & | \ CSPproc \ \Theta \  CSPproc   \  \\    %Exception        
%         & | \ CSPproc \ \backslash \ \{Event\} \ \\    % Hiding
%         & | \ CSPproc[\{Event\}/\{Event\}] \ \\        % Renaming
%         & | \ EDeadline( Event, Expression) \ \\         
%         %& | \ Countdown(Expression) \ \\                 
%         %& | \ Proc \overset{Expression} {\rhd} Proc   \ \\  % Deadline
% \end{align*}

% \begin{align*}        
% Event  &::= eventIdentifier  \ | \ tock \\ \\
% \end{align*}

%     % \centering
%     % \includegraphics{}
%     \caption{BNF of tock-CSP for the translation technique}
%     \label{BNF_tockCSP}
% \end{figure}


%%%%%%%%%  CSP Expression as defined in the https://www.cs.ox.ac.uk/projects/fdr/manual/cspm/syntax.html#csp-expressions

% Expression &::= <digit> \ \\ 
%         & | \ <Expression> <mathOperator>  <Expression>  \ \\ 
%         & |   ( <Expression>) \\ \\
% digit &::= 0 \ | \ 1 \ | \ 2 \ | \ 3 \ | \ 4 \ | \ 5 \ | \ 6 \ | \ 7 \ | \ 8 \ | \ 9  \ | \  <digit><digit> \\ \\
% mathOperator  &::= + \ | \  - \ | \  \times  \ | \ / \\ \\
%


%The BNF is implemented into AST using Haskell in the following Definition \ref{dfn_CSPproc}.


% \begin{tcolorbox} %[title=Title]
% \begin{definition} \textbf{Data definition of \lstinline{CSPproc}} 
% \label{dfn_CSPproc}
% \end{definition}
% \tcblower
% \lstset{frameround=fttt}
% \vspace{-0.5cm}
% \begin{lstlisting}[mathescape, language=Haskell, basicstyle=\ttfamily, columns=flexible]
% data CSPproc =   STOP
%               | Stopu
%               | SKIP
%               | Skipu
%               | WAIT         Int
%               | Waitu        Int 
%               | Prefix       Event       CSPproc
%               | IntChoice    CSPproc     CSPproc
%               | ExtChoice    CSPproc     CSPproc
%               | Seq          CSPproc     CSPproc
%               | Interleave   CSPproc     CSPproc
%               | GenPar       CSPproc     CSPproc  [Event]
%               | Interrupt    CSPproc     CSPproc
%               | Timeout      CSPproc     CSPproc  Int
%               | Hiding       CSPproc     [Event]
%               | Rename       CSPproc     [(Event, Event)]
%               | Proc         NamedProc
%               | Exception    CSPproc     CSPproc  [Event]
%               | EDeadline    Event       Int  
%               | ProcID       String  
% \end{lstlisting}
% \end{tcolorbox}




% In the following explanation, we use two metavariables $P$ and $Q$, and decorations on these names, to denote elements of the syntactic category $CSPproc$. We use the symbol $e$ to represent an element of the set Event. Also, the symbols $A$ and $B$ are used to represent a set of events.  Lastly, the parameter $d$ represents a $CSP$ expression that evaluates to a positive integer \footnote{Details in \url{https://www.cs.ox.ac.uk/projects/fdr/manual/cspm/syntax.html#csp-expressions}}. 


% \paragraph{$STOP$} specifies a process at a stable state in which only the event tock is allowed to happen. This means that the process enables passage of time only, no other events are allowed to happen.

% \paragraph{$Stopu$} specifies a process that immediately deadlocks. Unlike the previous process $STOP$, this process $Stopu$ does not allow any time to pass before the deadlock.

%  \paragraph{$SKIP$} specifies a process that reaches a successful termination point, where it can either terminate or allow time to pass using the event $tock$ before termination. In essence, only two events are possible at that state, $tock$ for time or  $tick$ for termination.

% \paragraph{$Skipu$} specifies a process that immediately terminates. Unlike the previous process $Skipu$, this process does not allow time to pass before termination. In essence, the process immediately performs the termination event $tick$.


% \paragraph{$WAIT(d)$} specifies a delay process that remains idle for a certain amount of unit time $d$. After the idle time elapses, either the process terminates with the event $tick$ or allows arbitrary units of times to pass before termination.


% \paragraph{$Waitu(d)$} specifies an urgent delay process that remains idle for a fixed amount of unit time $d$. The process terminates immediately after the fixed delay time $d$.




% \paragraph{$e \rightarrow P$} Prefix describes a process that offers to engage with an event $e$ and then subsequently perform the behaviour of the process $P$.
% %The prefixing process waits as long as possible for that specific event to happen for the other subsequent series of events to follow.
% % otherwise the following events will never happen.


% \paragraph{$P \ \sqcap\ Q $} Internal choice specifies a process that has different autonomous choices of behaviour, $P$ and $Q$.  Independently the process $P \ \sqcap\ Q $ behaves either as $P$ or $Q$,  regardless of the choice of the environment. In the case of this internal choice the environment has no control over the two possible choices of $P$ and $Q$.


% \paragraph{$ P\ \square\ Q$ } External choice specifies a process that is ready to engage in the behaviour of either $P$ or $Q$ depending on the choice of the environment. The process offers to engage with the initials of both $P$ and $Q$, for each chosen initials the process $P\ \square\ Q$ provides the corresponding behaviour of either process $P$ or $Q$. In the case of this external choice, the environment has control in choosing the behaviour of the process. This is the complement of the previous internal choice where the process has control over the choice of the behaviour.

% \paragraph{Well-formedness} In the case of external choice, there is a restriction that the event tock is not allowed to appear in the initials of either of the processes. That is $tock  \notin (initials(P) \cup initials(P))$. This is because having the event tock as part of the initials will cause non-determinism between the process behaviour and progress of time.



% \paragraph{$P;Q$} Sequential Composition specifies a composition of two processes $P$ and $Q$ that run one process after the other. The first process $P$ begins until it terminates, then follow with the behaviour of the subsequent process $Q$.


% \paragraph{$P|||Q$} Interleaving specifies a parallel composition where both the processes run independently without any interaction. In this case, the processes have no common interaction points except for the termination point. Interleaving processes do not synchronise in any of their events.
% %
% \paragraph{Well-formedness} Implicitly, the processes $P$ and $Q$ have to match the flow of time. If both the two processes perform the time event $tock$, they synchronise with the flow of time on the event $tock$, which implies that the two processes implicitly synchronise on the flow of time and the time event $tock$.


% \paragraph{$ P \ \underset{A}{||} \ Q $} Generalised parallel specifies a parallel composition of two processes $P$ and $Q$ that run in parallel and synchronise on specified set of events $A$. Independently, each of the processes performs its events that are outside the set $A$
% %, at least the event tock.
% \paragraph{Well-formedness} The set $A$ implicitly contains the event $tock$.



% \paragraph{$P \overset{d} {\rhd} Q $} Timeout delay specifies a composition of two processes $P$ and $Q$, where a deadline $d$ is specified for the first process $P$ to engage with performing an event from it initials $initials(P)$. If the first process $P$ engagee, then the whole process behaves as the process $P$. After the deadline $d$ time unit, if the first process $P$ did not engages, the second process $Q$ take over the control, and the whole process behaves like the second process $Q$.
 
 

% \paragraph{Well-formedness} The expression $d$ should be an expression that evaluates to a natural number.  This is because tock-CSP is based on a discrete-time model that records time-progress with discrete-event tock. Also, both the two processes $P$ and $Q$ are not allowed to begins with the timed event $tock$.


% \paragraph{$ P \vartriangle  Q $} Interrupt operator describes a process $P$ that can be interrupted by another process $Q$ at any time during the execution of $P$. The first process $P$ runs until the second process $Q$ performs a visible event. Whenever the second process performs an external action, it interrupts the execution of the first process. The interrupted process is blocked, and the second process takes over the control, then the whole process behaves as the second process $Q$. If the second process $Q$ did not interrupt the whole process behave as the first process $P$. % up to its completion.
% %and runs up to its termination point.

% \paragraph{Well-formedness}  There is restriction that the event $tock$ is not allowed to be in the initials of the second (interrupt) process. This means that an interruption cannot begin with the event tock. This is because time event $tock$ can cause non-determinism between the interrupt and the process of time.

% \paragraph{$ P \ \backslash \ A $ } Hiding specifies the behaviour of a process $P$ which hide all the events in set A. The hidden events $A$  becomes special event $tau$ that are not visible to the environment, as such the environment has no control over the hidden events.



% \paragraph{Well-formedness}  In the case of hidden, there is a restriction that hidden events should not include the time event $tock$. This is because a process should not control the progress of time.



% %Renaming operator
%  \paragraph{$P[A/B]$} Renaming specifies a process that renames a list of its events $A$ with corresponding names of events in list $B$, in one to one mapping. The renaming operator transforms a process into another process with the same structure but appears with different names of the renamed events $A$.
 
%  %of the behaviour but appears with different names events.
 
% \paragraph{Well-formedness} There is restriction that the event $tock$ cannot be renamed to another event, and no other event can be renamed to be $tock$. This is because the time-event tock is a special event dedicated for recording the progress of time.

% \paragraph{$Edeadline(e, d)$} The process event deadline specifies a process that must perform the event $e$ within a specific deadline $d$. So the event $e$ must happen within the deadline $d$.



% \paragraph{}
% The language that we define above and call tock-CSP language is the language used in defining the discrete-time semantics of RoboChart. 




==> zz_del/C4.tex <==
\section{Evaluation of the Translation Technique}

This chapter discusses the experimental approach that we follow in evaluating the translation technique.  First, we discuss an experiment, which we carried out to translate a list of processes that pair the constructs of the BNF,  which has been previously presented in Section \ref{bnf}. Second, we discuss and illustrate a translation of a RoboChart model. Third, we discuss a performance evaluation that we carried out in comparing the performance of FDR and UPPAAL in the verification. The results show a significant performance increase of UPPAAL over FDR for verification. Finally, we summarise and conclude the chapter.


\subsection{Experimental Evaluations}
\subfile{C4.1}

\subsection{Performance Evaluations}
\subfile{C4.3}


%Summary of Gavin paper
\subsection{Comparing tock-CSP and TA for verification}
Verification using tock-CSP (Refinement) and TA (CTL) 

%\subfile{}



%Translation of Robochart
\subfile{C4.2}


\subsection{Limitations}
%\subfile{}


%\subsection{Final Consideration}
\subfile{C4.4}

% \begin{cmt}
% This section summarises and concludes the chapter, as well as establishes a link to the next chapter.
% \end{cmt}


% In conclusion, this section discussed the evaluation of the translation technique. First, we discussed the a list of processes we used in evaluating the translation technique. Second, we discuss and illustrates a translation of RoboChart models. Third, we discuss the experiment we carryout in comparing the performance of using  using FDR and UPPAAL for automatic verification. The result of the comparison shows a significant improvement of using UPPAAL in the verification RoboChart models and also tock-CSP models.


==> zz_del/C4_1.tex <==
%\subsection{Examples for Experimental Evaluation}



This section discusses the list of processes that we use in evaluating the translation technique. In evaluating the translation technique, we consider an experimental approach, which enables us to use trace semantics in justifying the correctness of the translation technique. We begin with formulating a list of various processes that covers interesting conditions (test cases), ranging from basic processes in Table \ref{basicproc} to processes in Table \ref{pairproc} that pair the tock-CSP constructors in BNF, as discussed in Section \ref{BNF}. 


Tables \ref{basicproc} and \ref{pairproc}  summarise the processes that we used in evaluating the translation technique. Details of all these processes are provided in Appendix \ref{detailsProc}. The numbers in Tables \ref{basicproc}  and  \ref{pairproc} correspond to the numeric label of each process in Appendix \ref{detailsProc}. Processes 10-1J are processes that pair the constructor prefix with basic processes and all the other constructors from the BNF. Similarly, processes 20-2J pair the constructor internal choice with basic processes and all the other constructors from the BNF. In this similar way, we pair all the constructors in the first column of Table \ref{} with the basic processes and constructors in the first row of the table.




After formulating the processes in Table \ref{}, we use the translation tool, which we developed in Section \ref{}, to generate, collect, compare and analyse the traces of these processes in Tables  \ref{basicproc} and \ref{pairproc}. The results of comparing and analysing the traces enable us to reason about the correctness of the translation technique. We see that, for each of the finite processes in Table  \ref{basicproc} and \ref{pairproc} within a specific length (currently length 3), the traces of the translated UPPAAL model contains the traces of the original input tock-CSP process. This result ensures that the translated UPPAAL captures the semantics of the input tock-CSP model.



Additionally, the processes in Tables \ref{basicproc} and \ref{pairproc} are part of the built-in processes that we provide in the translation tool we developed in Section \ref{}. The provided process help users to explore and understand the tool. We provide an interface for selecting each of the process using the process number as provided in Tables \ref{basicproc} and \ref{pairproc}. On entering a process number, the system displays the selected process and then translates the process into TA, and then generates and compares the traces of the selected process, as we discussed in Section \ref{}. Subsequently, the system displays a summary of the results for comparing the traces. This list of built-in processes and the interface provide a good starting point for interacting and understanding the system. On top of that, the interface enables users to enter or upload tock-CSP specifications, (Currently, in AST using the BNF of Section \ref{bnf}).



\begin{table} []
    \centering
    \begin{tabular}{|c|l|l|}   \hline \hline

01  &  STOP     &  Deadlock (Dl)              \\ \hline \hline
02  &  Stopu    &  Urgent Deadlock (UD)       \\ \hline \hline
03  &  SKIP     &  Termination (Tn)           \\ \hline \hline
04  &  Skipu    &  Urgent Termination (UT)    \\ \hline \hline
05  &  WAIT(n)  &  Delay  (Dy)                \\ \hline \hline
06  &  Waitu(n) &  Strict Delay (SD)          \\ \hline \hline

   \end{tabular}
    \caption{Constant processes}
    \label{basicproc}
\end{table}



\begin{landscape}

\begin{table} []
    \centering
%    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|l|l|l|l|l|l|}   \hline \hline
    \begin{tabular}{|l|| l| l| l| l| l| l| l| l| l| l| l| l| l|l|l|l|l|l|l|}   \hline \hline
% Constructors  &  Dl &  UD  &  Tn  &  UT  &  Dy  &  SD  &  Px  &  IC  &  EC  &  SC  &  Il  &  GP  &  RP  &  It  &  ED   \\  \hline  \hline

\textbf{BNF Constructors}  &  Dl &  UD  &  Tn  &  UT  &  Dy  &  SD  &  Px  &  IC  &  EC  &  Il  &  GP  &  SC  &  RP  &  To  &  It  &  ED  & Hd  &  Rn  &  Ex    
\\  \hline  \hline

Prefix (Px)  &  10  &  11  &  12  &  13  &  14  &  15  &  16  &  17  &  18  &  19  &  1A  &  1B  &  1C  &  1D  &  1E  &  1F  &  1G  &  1H  &  1J                  \\  \hline  \hline  
Internal Choice (IC)    &  20  &  21  &  22  &  23  &  24  &  25  &  26  &  27  &  28  &  29  &  2A  &  2B  &  2C  &  2D  &  2E  &  2F  &  2G  &  2H  &  2J                  \\  \hline  \hline
External Choice (EC)    &    30  &  31  &  32  &  33  &  34  &  35  &  36  &  37  &  38  &  39  &  3A  &  3B  &  3C  &  3D  &  3E  &  3F  &  3G  &  3H  &  3J                  \\  \hline  \hline
Interleaving (Il) &    40  &  41  &  42  &  43  &  44  &  45  &  46  &  47  &  48  &  49  &  4A  &  4B  &  4C  &  4D  &  4E  &  4F  &  4G  &  4H  &  4J                  \\  \hline  \hline
Generallise Parallel (GP)    &   50  &  51  &  52  &  53  &  54  &  55  &  56  &  57  &  58  &  59  &  5A  &  5B  &  5C  &  5D  &  5E  &  5F  &  5G  &  5H  &  5J                  \\  \hline  \hline
Sequential (SC)  &    60  &  61  &  62  &  63  &  64  &  65  &  66  &  67  &  68  &  69  &  6A  &  6B  &  6C  &  6D  &  6E  &  6F  &  6G  &  6H  &  6J                  \\  \hline  \hline
Recursive  Process (RP)    &      70  &  71  &  72  &  73  &  74  &  75  &  76  &  77  &  78  &  79  &  7A  &  7B  &  7C  &  7D  &  7E  &  7F  &  7G  &  7H  &  7J                  \\  \hline  \hline
Interrupt (It)                &   80  &  81  &  82  &  83  &  84  &  85  &  86  &  87  &  88  &  89  &  8A  &  8B  &  8C  &  8D  &  8E  &  8F  &  8G  &  8H  &  8J                  \\  \hline  \hline
Timeout (To)      &    90  &  91  &  92  &  93  &  94  &  95  &  96  &  97  &  98  &  99  &  9A  &  9B  &  9C  &  9D  &  9E  &  9F  &  9G  &  9H  &  9J                  \\  \hline  \hline
Event Deadline (ED)          &    A0  &  A1  &  A2  &  A3  &  A4  &  A5  &  A6  &  A7  &  A8  &  A9  &  AA  &  AB  &  AC  &  AD  &  AE  &  AF  &  AG  &  AH  &  AJ                  \\  \hline  \hline
Hiding (Hd)                 &     B0  &  B1  &  B2  &  B3  &  B4  &  B5  &  B6  &  B7  &  B8  &  B9  &  BA  &  BB  &  BC  &  BD  &  BE  &  BF  &  BG  &  BH  &  BJ                  \\  \hline  \hline
Renaming (Rn)                 &   C0  &  C1  &  C2  &  C3  &  C4  &  C5  &  C6  &  C7  &  C8  &  C9  &  CA  &  CB  &  CC  &  CD  &  CE  &  CF  &  CG  &  CH  &  CJ                  \\  \hline  \hline
Exception (Ex)               &    D0  &  D1  &  D2  &  D3  &  D4  &  D5  &  D6  &  D7  &  D8  &  D9  &  DA  &  DB  &  DC  &  DD  &  DE  &  DF  &  DG  &  DH  &  DJ                  \\  \hline  \hline

    \end{tabular}
    \caption{A summary of processes for the exhaustive possible pairing of the constructors. Details of these processes is in Appendix \ref{DetailProcesses}. Also, all these processes are part of the builtin processes in the translation tool we developed in Section \ref{}} 
    \label{pairproc}
\end{table}

\end{landscape}







==> zz_del/C4_2.tex <==
\subsection{Translation of A RoboChart Model}
\label{rc}

This section discusses the translation of a RoboChart model into UPPAAL. Figure \ref{RCmodel} illustrates a simple RoboChart model of a mobile system. The system moves at a specified linear velocity $vl$ and observes the presence of an obstacle. When the system detects an obstacle, it turns at a specified angular velocity $av$ and then continues moving in a straight line with the velocity $v$ while detecting and avoiding obstacles.


\begin{frame}{}
 \begin{figure}[H]
     \centering
   \fbox{ \includegraphics [width=\textwidth]{_SF_RoboChart.png}}
    \caption{A RoboChart model for a simple mobile system}
    \label{RCmodel}
 \end{figure}
\end{frame}


\subsubsection{tock-CSP specification of the RoboChart model}
Below \ref{} is a short version of the tock-CSP specification of the RoboChart model in Figure \ref{rc}. At the current development of RoboTool \cite{RoboTool}, the generated tock-CSP specifications of the model in Figure \ref{rc} from RoboTool span multiple files, which is illustrated in Appendix \ref{rc_model_generated tockCSP}. Here we use a shorter version of the tock-CSP specification of the model.

To ensure the equivalence of the shorter version of the tock-CSP specification with the generated version of the tock-CSP, we check the equivalence of the two versions of the specification using refinement relations in Line 21 and 22.  Line 21 asserts that the short tock-CSP specification \lstinline{Tspec} is refined by the generated tock-CSP \lstinline{T_CFootBot} in failure divergence. Likewise, Line 22 asserts that the generated tock-CSP \lstinline{T_CFootBot} is also refined by the short tock-CSP specification \lstinline{Tspec} in failure divergence mode.



\begin{tcolorbox} %[title=Title]
\begin{Verbatim}[numbers=left,numbersep=7pt]
Timed(OneStep) {

Tspec = EntryMoving; 
        obstacle -> SKIP0; 
        EntryTurning;
        Countdown(SMovement_PI/SMovement_av); 
        Tspec

EntryMoving  = EDeadline(moveCall, 0); 
               EDeadline(moveRet, 0); 
               Countdown(1) 

EntryTurning = EDeadline(moveCall, 0); 
               EDeadline(moveRet,0) 
      }

-- The following refinement checks ensure that the short tock-CSP
-- specification Tspec is equivalent to the generated 
-- specification T_CFootBot

assert Tspec [FD= T_CFootBot  -- passes FDR test
assert T_CFootBot [FD= Tspec  -- passes FDR test

-- include the generated tock-CSP specification from RoboTool
include "SimFW.csp"

\end{Verbatim}
\end{tcolorbox}



\subsubsection{Abstract Syntax Tree (AST) of the RoboChart model}
In this section, we generate an AST of the RoboChart model. We consider the short version of the tock-CSP specification of the RoboChart model in \autoref{RCmodel}.  The AST is in \autoref{AST_RC}. The tock-CSP specification is highlighted as comments and is then followed by its corresponding AST using the BNF presented in Section \ref{bnf}. For example, Lines 4-5 are tock-CSP specification of Tspec, and its corresponding AST follows in Lines 6-13.


\begin{tcolorbox} %[title=Title]
\begin{Verbatim}[numbers=left,numbersep=7pt]
-- The AST of the RoboChart model


-- Tspec = EntryMoving; obstacle-> SKIP0; EntryTurning;
           Countdown(SMovement_PI/SMovement_av); Tspec
   Tspec = NamedProc "Tspec" 
           (Seq 
           (Seq (entryMovingT)
           (Seq (Prefix (ID "obstacle") SKIP0 ) 
           (Seq (entryTurningT)  (Countdown 3)
           )))
           (ProcID "Tspec")
           )
           
-- EntryMoving = EDeadline(moveCall, 0);EDeadline(moveRet, 0);WAIT(1) 
   entryMovingT = Seq 
                 (EDeadline (ID "moveCall")  0)
                 (Seq (EDeadline (ID "moveRet")  0)  
                 (Countdown 1))


-- EntryTurning = EDeadline(moveCall, 0);EDeadline(moveRet,0) 
   entryTurningT = Seq 
                  (EDeadline (ID "moveCall")  0)
                  (EDeadline (ID "moveRet" )  0)
    


\end{Verbatim}
\end{tcolorbox} %[title=Title]

\subsubsection{Translated Timed Automata of the RoboChart model}
This section discusses the output of translating the RoboChart model in Section \autoref{rc}. Using the translation technique discussed in Section \ref{}, we translate the AST \ref{} into UPPAAL TA, which produces the following list of 17 small TA. The first TA is environment TA defined in \ref{dfn_env_TA}. The remaining TA are  small TA that capture the specification of the RoboChart model in \autoref{RCmodel}. The last TA is synchronisation TA defined in Section \ref{dfn_sync_TA}. For this model, the synchronisation TA has no transitions because there is no multi-synchronisation action.


 \begin{figure}[H]
     \centering
    \fbox{ \includegraphics [width=\textwidth, height=0.5\textheight]{TAspec.png} }
     \caption{ Translated UPPAAL TA for the mobile system} 
    \label{translated_ta}
\end{figure}





The resulting translated TA in \autoref{translated_ta} facilitate verification using UPPAAL toolbox. Table \ref{sampleUppalQuerry} provides a sample verification check with UPPAAL. The first specification S1 is for checking deadlock, which is one of the common interesting specification that can be specified in both tock-CSP and TA, which can also be checked automatically using their supporting tools FDR and UPPAAL respectively. The second specification S2, illustrates an example of a specification for a behaviour that involves an operator for eventually, which is a kind of specification that is difficult to specify with tock-CSP, but can easily be specified with TA using Timed Computational Tree Logic (TCTL) \cite{G08, Gavin paper}. Third specification S3 illustrates a specification that involves the negation of eventuality.




\begin{table}[H]
\caption {Sample specifications for UPPAAL verification}
\label{sampleUppalQuerry}
\begin{center}
%\begin{tabular}{|C{2cm}|L{9cm} |C{2cm}| }
\begin{tabular}{|p{0.5cm}|p{13cm} | } % p{3cm}|  p{2cm} | }
\hline\hline

\textbf{No.} & \textbf{Specification}  % &  \textbf{tock-CSP}   & \textbf{TA} \\ % & \textbf{Single TA}  \\ 
\\ \hline \hline

S1. & Deadlock Free  \\ 
\hline
S2. & The system eventually moves after detecting an obstacle  \\ \hline

S3. & Is it possible that the system never detects an obstacle?
(In other words, is there a behaviour where the system never detects an obstacle?) 
\\ \hline


\hline
\end{tabular}
\end{center}
\end{table}





==> zz_del/C4_3.tex <==
%\subsection{Performance Evaluations}


In this section, we evaluate the performance of the two verification tools, FDR and UPPAAL, specifically for automatic verification. We describe the resources as well as the procedure we used for the experimental evaluation.


%In this section, we discuss the performance comparison between FDR and UPPAAL. Evaluating the performance is another experiment we carryout in determining the performance of using FDR in verifying tock-CSP specification and using UPPAAL in the verification of TA. 

%we describe another experiment we carryout in illustrating the significance of the work. In this section, we evaluate the performance of the two verification tools, FDR and UPPAAL, specifically for automatic verification. We describe the resources as well as the procedure we used for experimental evaluation.

% \begin{cmt}
% How did we carry out the experiment?
% \end{cmt}


%\section{Performance analysis for the examples}
Evaluating the performance is another experiment that we carry-out in determining the performance of FDR in verifying tock-CSP specifications and using UPPAAL in the verification of the translated TA. The graph in \autoref{perfEgs} summarises the timing for checking deadlock using both FDR and UPPAAL. Considering that checking deadlock is one of the common interesting checks that can be done with both FDR and UPPAAL. Secondly, deadlock checks require an exhaustive verification for checking each state of the model.


%in each of the processes in Table \ref{} and \ref{}.
For each process in Tables \ref{basicproc} and \ref{pairproc}, we run verification checks for checking deadlock using both FDR for the tock-CSP and using UPPAAL in the corresponding translated TA, and we record the average timing after repeating each of the checks 10 times. Details of the recorded values for the timing are in  Appendix \autoref{performanceTable}.  

We compare the recorded timings in the following Graph \ref{performanceGraph}, which provides a summary of comparing the recorded timing, using both FDR and UPPAAL. The graph at the top (blue) shows the recorded timing for FDR, while the graph at the bottom (red) shows the recorded time for UPPAAL. From the graph, it is clear that average performance timing for FDR is above 0.03 unit time while the average performance timing for UPPAAL is below 0.01. This result shows that using UPPAAL is at least 3 times faster than using FDR for verification. In short, this experiment shows a significant performance increase in using UPPAAL for verification of RoboChart models. 


%The following graph illustrates a summary of comparing the recorded timing in using FDR and UPPAAL. The graph shows a significant performance increase in using UPPAAL for verification.  The graph at the top (blue) shows the recorded timing for FDR. While the graph at the bottom (red) shows the recorded time for UPPAAL. From the graph, it is clear that average timing for FDR is above 0.03 unit time while the average timing for UPPAAL is below 0.01. This result shows that using UPPAAL is at least 3 times faster, then using FDR for verification.

%Timing for each verification was repeated 10 times, and the average time and standard deviation are recorded in  \autoref{perftable}. The following graph illustrates a summary of comparing the timing recorded in using FDR and UPPAAL.


  \begin{figure}[H]
     \centering
    \includegraphics [width=1\textwidth]{PerformanceEgs.png}
    \caption{Performance analysis for FDR and UPPAAL}
    \label{performanceGraph}
\end{figure}


%I carried out the following verification using both FDR and UPPAAL. Each verification was repeated 10 times, and the average time is recorded in table \autoref{performance}. Overall, there is a significant performance increase in using UPPAAL for the verification. 




==> zz_del/Eg.tex <==
\begin{example} \textbf{A translation of Automatic Door System (ADS)}\\
\label{ads}
This example illustrates a translation of an automatic door system (ADS). Consider a simple tock-CSP model of a system that opens a door, and then after at least one time unit, the system closes the door. \\
\verb!          ADS = open -> tock -> close -> SKIP!. 

A translation of process ADS produces the following list of TA in Figure \ref{ta_env}.


\begin{figure}
\subfigure{\includegraphics [width=0.25\textwidth]{fig/taPrefix00.png}}
\hspace{0.05\textwidth}
\subfigure{\includegraphics [width=0.25\textwidth]{fig/taPrefix01.png}}
\hspace{0.05\textwidth}
\subfigure{\includegraphics [width=0.25\textwidth]{fig/taPrefix02.png}}
\end{figure}


\begin{figure}
\subfigure{\includegraphics [width=0.2\textwidth]{fig/taSKIP.png}}
\hspace{0.05\textwidth}
\includegraphics [width=0.5\textwidth]{fig/Env.png}
\label{ta_env}
\end{figure}

\end{example}

%The process ADS is translated into a list containing 5 TA. 


The list of network TA in Figure \ref{ta_env} expresses the behaviour of the original tock-CSP process. Starting from the top-left corner, the first TA captures the occurrence of the event \lstinline{open}. The second TA captures the occurrence of the event \lstinline{tock}. The third TA captures the occurrence of the event \lstinline{close}. The fourth TA captures the occurrence of the event \lstinline{tick}. Finally, the last TA is an environment TA provides separate transitions for each co-actions of all the event in the original tock-CSP process, that is \lstinline{open}, \lstinline{tock}, \lstinline{close} and \lstinline{tick}.


==> zz_del/a1_abs02.tex <==

We present a technique for translating tock-CSP into TA for UPPAAL. tock-CSP is a process algebra that provides textual notations for modelling discrete-time behaviours of CPS. Automatic verification is supported with FDR that facilitates formal analysis and verification of tock-CSP models. TA is a finite state machine that provides graphical notations for modelling real-time systems and verification with TCTL. Automatic verification is supported with real-time verification toolbox UPPAAL. tock-CSP differs from TA in terms of both modelling and verification and also the kind of requirements that can be verified in their models.


Here, we translate tock-CSP into TA that facilitates using  UPPAAL for the verification of tock-CSP. We provide a list of translation rules for translating the constructs of the tock-CSP into small TA that address the complexity of capturing the compositionality of tock-CSP, which is not available in TA. We compose the small TA into various shapes that capture the behaviour tock-CSP process.


We utilised the expressive power of Haskell in both expressing and implementing the translation technique into a tool, which enables us to use trace analysis in justifying the correctness of the translation techniques. Firstly, we find a significant performance increase in using UPPAAL for the verification of tock-CSP. Secondly, the work provides an easier alternative for both expressing and verifying liveness requirements that are difficult to specify in tock-CSP. Lastly, we provide an extension for verifying RoboChart models, which relies on tock-CSP for verifying temporal specifications.



==> zz_del/a1_abs03.tex <==
tock-CSP is a process algebra that provides textual notations for modelling discrete-time behaviours. Automatic verification of tock-CSP is supported by FDR that facilitates formal analysis and verification. Similarly, automatic verification of Timed Automata (TA) is supported by real-time verification toolbox UPPAAL. tock-CSP differs from TA in terms of both modelling and verification as well as the kind of requirements that can be verified in their models. In this work, we translate tock-CSP into TA that facilitates using UPPAAL for the verification of tock-CSP. We provide a list of translation rules for translating the constructs of the tock-CSP into collection small TA that address the complexity of capturing the compositionality of tock-CSP, which is not available in TA. 
%
We compose the small TA into various shapes that capture the behaviour of tock-CSP process. We utilise the expressive power of Haskell in both expressing and implementing the translation technique into a tool, which enables us to use trace analysis in justifying the correctness of the translation techniques. The result shows significant performance increase in using UPPAAL for the verification of deadlock freedom, a promising check for measuring performance in both FDR and UPPAAL. 


==> zz_del/a1_abs1.tex <==
% Full research papers: full papers of not more than 14 pages in LNCS format, which have to be original, unpublished and not submitted elsewhere.


%One of the complexities of verifying CPS systems is due to the number of concurrent processes that interacts to provide the behaviour of the intended systems. 

In this work, we present a technique for translating tock-CSP into TA for UPPAAL. tock-CSP is a process algebra that provides textual notations for modelling discrete-time behaviours of CPS. Automatic verification is supported with FDR that facilitates formal analysis and verification of tock-CSP models. While, TA is a finite states machine that provides graphical notations for modelling real-time systems and verification with TCTL. Automatic verification is supported with real-time verification toolbox UPPAAL.
tock-CSP differs from TA in terms of both modelling and verification of systems and the kind of requirements that can be checked with each one.
%and also their supporting tools. 

Here, we translate tock-CSP into TA that facilitates using  UPPAAL for the verification of tock-CSP. We provide a list of translation rules for translating the constructs of the tock-CSP into small TA that address the complexity of capturing the compositionality of tock-CSP, which is not available in TA. We compose the small TA into various shapes for capturing the behaviour tock-CSP process.

%In this work, we use small TA that are composed into various shapes to capture the behaviour of the translated tock-CSP process.
%We address the complexity of compositionality of tock-CSP that is not available in the TA.

We utilised the expressive power of Haskell in both expressing and implementing the translation technique into a tool, which enables us to perform various experiments for justifying the correctness of the translation techniques. Firstly, we find a significant performance increase in using UPPAAL for the verification of tock-CSP. Secondly, the work provides an easier approach for verifying liveness requirements that are difficult to specify in tock-CSP. Lastly, we provides an extension for verifying RoboChart models, which relies on tock-CSP for verifying temporal specifications.


% The result of this work can be categorise into three.
% The result of this work significantly improves performance of the verification aspect with UPPAAL.
% Provides an easier way of specifications requirements that are difficult to specify with tock-CSP, specifically specification requirements that involves eventual behaviour, such as <>a.
% Provides an extension for RC, which facilitates verifying RC models using UPPAAL model checker. Also, other existing works that are based on tock-CSP can benefit from this traslation work.





% that is supported with automatic verification tool FDR.

%tock-CSP is a process algebra that provides textual notations for modelling discrete-time behaviours of CPS that is supported with automatic verification tool FDR.

%tock-CSP is a process algebra that provides textual notations for modelling discrete-time behaviours of CPS.  
%Both automatic verification and analysis with tockCSP is supported with a supporting tool FDR
%that is supported with automatic verification tool FDR.

% tock-CSP provides a textual notation for modelling CPS, that facilitates formal reasoning and verification of systems. This facilitates verification with concept of refinement.


% What is CSP?
% TA and UPPAAL?
% Relationship between TA?



%tock-CSP models systems in textual format while TA is finite-state machine that models system in graphical models.

% Scope?
% In this work, we developed a translation techniques for translating tockCSP into TA, that facilitates verification with UPPAAL. We provide a list of translation rules for translating the essential constructs of the tock-CSP for modelling temporal specifications.

% One of the challenging points is capturing compositionality of tockCSP that is not available in TA. We address this issues/challenge with using small size TA that enable composing small TA

% Compositionality?
% On of the challenging point is capturing the compositionality of tock-CSP that is not available in TA. In this work, we use small TA that are composed into various shapes to capature the behavaiour of the translated tock-CSP process.
% %We address the complexity of compositionality of tock-CSP that is not available in the TA.

% We utilised the expressive power of Haskell in both expressing the translation technique and also implementing the technique into a software tool, which enable us to perform verious expriment to generate traces for justifying the correctness of the translation techniques. Additionally, also find/identify a significant increase in performance of using UPPAAL in the verification of the translated tock-CSP. Also, the work provides an alternative approach for verifying specifications that are difficult to specify with tock-CSP.
% As a result of this work we also provides an extenstion for verifyig RoboChart models, a modelling tool that relies on tock-CSP for verifying temporal specifications.


% Based on this work, we developed automatic tool for translating tock-CSP into TA. And also a validation tool for validating the translation work.

% Todo: translating verification requirements from tock-CSP into TA, 
% Improving the interface and displaying the result 
% Todo: series of case studies for the future work



%tockCSP provides notations for modelling CPS. The notations is supported with automatic verification using FDR, which was initially designed for modelling untimmed systems. In this work, we translates tock-CSP into TA for automatic verifications using UPPAAL, which was developed specifically for modelling and verification of RTS.


% ----------------------------------------------




% Haskell: Functional translation of tock-CSP to Timed Automata
% Haskell: Functional translation of tock-CSP to UPPAAL



% To read (in drive)
% Translation of UML 2 Activity Diagrams into Finite State Machines for Model Checking

% ABZ proceeding 2018


% %Related work
% Timed CSP has been translated into tock-CSP which establish a connection between timed CSP and tock-CSP, and also enable using FDR for the verification of Timed CSP that is translated into tock-CSP \ref{O00}.






==> zz_del/a1_abs_.tex <==

In this work we consider the advantage of model transformation in the verification liveness specification. A process algebra \verb!tock-CSP! provides textual notations for modelling discrete-time behaviours. Automatic verification of tock-CSP is supported by FDR. Similarly, automatic verification of Timed Automata (TA) is supported by real-time verification toolbox UPPAAL. However, \verb!tock-CSP! differs from TA in terms of both modelling and verification as well as the kind of requirements that can be addressed with each one of them, specifically in the verification of liveness specifications that can not be verify in tock-CSP and in general with simple refinement checks but possible with temporal logic.

In this work, we translate \verb!tock-CSP! into TA so that we can take advantage of TA and its supporting tool UPPAAL in the verifications of liveness specification using temporal logic.  We developed a translation technique that enables us to work out a list of translation rules for translating the constructs of \verb!tock-CSP! into a network of small TA, which address the complexity of capturing the compositionality of \verb!tock-CSP! that is not available in TA. In verifying the correctness of the translation we implement the technique into tool that enable us to use trace semantics in justifying the correctness of the translation technique based on finite approximations to trace sets. For the infinite traces, we plan to use mathematical proof for each of the translation rule to justify the correctness of the technique that will justify the correctness of the translation technique that will cover infinite traces.

%of each of the translation rule

%We plan to use mathematical proof to justify the translation each of the translation of the translation rule using mathematical proof.

%The correctness of the translation is justified by testing based on finite approximations to trace sets. 

%The results show significant performance increase in using UPPAAL for the verification of deadlock freedom.

%We compose the small TA into various shapes that capture the behaviour of tock-CSP process. We utilise the expressive power of Haskell in both expressing and implementing the translation technique into a tool, which enables us to use trace analysis in justifying the correctness of the translation techniques. 

%, a promising check for measuring performance in both FDR and UPPAAL. 


%First, we find a significant performance increase in using UPPAAL for the verification of tock-CSP. Secondly, the work provides an easier alternative for both expressing and verifying liveness requirements that are difficult to specify in tock-CSP. 

==> zz_del/a1_abs_1.tex <==
A process algebra \verb!tock-CSP! provides textual notations for modelling discrete-time behaviours, with the support of FDR for automatic verification. Similarly, automatic verification of Timed Automata (TA) is supported by real-time verification toolbox UPPAAL. TA and \verb!tock-CSP! differ in terms of both modelling and verification, as well as the kind of requirements that can be addressed with each one of them, specifically in verifying requirement that are difficult to specify and check with tock-CSP, and in general with simple refinement. For instance, liveness requirements are difficult to specify with \verb!tock-CSP!, but they are easy to specify with the constructs of temporal logic. In this work, we translate \verb!tock-CSP! into TA to take the advantages of TA and its supporting tool UPPAAL in using temporal logic.  We developed a translation technique that is implemented as a tool. And we come up with a list of translation rules for translatisng the constructs of \verb!tock-CSP! into a network of small TA, which address the complexity of capturing the compositionality of \verb!tock-CSP!. In validating the translation technique, the developed tool enables us to use experimental approach with trace semantics in justifying the correctness of the translation technique based on finite approximations to trace sets. We plan to use mathematical proof to work out the correctness of the translation rules that will cover infinite set of traces.



==> zz_del/a1_abs__.tex <==
A process algebra \verb!tock-CSP! provides textual notations for modelling discrete-time behaviours, with the support of FDR for automatic verification. Similarly, automatic verification of Timed Automata (TA) is supported by real-time verification toolbox UPPAAL. However, \verb!tock-CSP! differs from TA in terms of both modelling and verification, as well as the kind of requirements that can be addressed with each one of them, specifically in the verification of liveness specifications that can not be verify in tock-CSP, and in general with simple refinement checks, but can be verify with temporal logic. In this work, we consider the advantage of model transformation in the verification of liveness specification. Thus, we translate \verb!tock-CSP! into TA to take the advantages of TA and its supporting tool UPPAAL in using temporal logic.  We developed a translation technique that is implemented as a tool, which enables us to work out a list of translation rules for translating the constructs of \verb!tock-CSP! into a network of small TA, which address the complexity of capturing the compositionality of \verb!tock-CSP!, which is not available in TA. In verifying the correctness of the translation techniques, the developed tool enables us to use trace semantics in justifying the correctness of the translation technique based on finite approximations to trace sets. For the infinite traces, we plan to use mathematical proof to work out the correctness of the translation rules that will cover infinite traces.

% n each of the translation rule to justify the correctness of the technique that will justify the correctness of the translation technique that will cover infinite traces.

%of each of the translation rule

%We plan to use mathematical proof to justify the translation each of the translation of the translation rule using mathematical proof.

%The correctness of the translation is justified by testing based on finite approximations to trace sets. 

%The results show significant performance increase in using UPPAAL for the verification of deadlock freedom.

%We compose the small TA into various shapes that capture the behaviour of tock-CSP process. We utilise the expressive power of Haskell in both expressing and implementing the translation technique into a tool, which enables us to use trace analysis in justifying the correctness of the translation techniques. 

%, a promising check for measuring performance in both FDR and UPPAAL. 


%First, we find a significant performance increase in using UPPAAL for the verification of tock-CSP. Secondly, the work provides an easier alternative for both expressing and verifying liveness requirements that are difficult to specify in tock-CSP. 

==> zz_del/a1_abs__1.tex <==
The process algebra \verb!tock-CSP! provides textual notations for modelling discrete-time behaviours, with the support of FDR for automatic verification. Similarly, automatic verification of Timed Automata (TA) is supported by the real-time verification toolbox UPPAAL. TA and \verb!tock-CSP! differ in terms of both modelling and verification, as well as the kind of requirements that can be addressed with each one of them. For instance, liveness requirements are difficult to specify with the constructs of \verb!tock-CSP!, but they are easy to specify with the constructs of temporal logic. In this work, we translate \verb!tock-CSP! into TA to take advantage of TA and its supporting tool UPPAAL in using temporal logic.  We developed a translation technique and its tool; and we come up with a list of translation rules for translating \verb!tock-CSP! into a network of small TA, which address the complexity of capturing the compositionality of \verb!tock-CSP!. For validating the translation technique, we use experimental approach based on finite approximations to trace sets. Finally, we plan to use mathematical proof to work out the correctness of the translation rules that will cover an infinite set of traces.

%We plan to use mathematical proof to work out the correctness of the translation rules that will cover an infinite set of traces.

==> zz_del/a1_abs___.tex <==
% We present a technique for translating tock-CSP into Timed Automata (TA) for UPPAAL. 

A process algebra \verb!tock-CSP! provides textual notations for modelling discrete-time behaviours. Automatic verification of tock-CSP is supported by FDR that facilitates formal analysis and verification. Similarly, automatic verification of Timed Automata (TA) is supported by real-time verification toolbox UPPAAL. \verb!tock-CSP! differs from TA in terms of both modelling and verification as well  requirements that addressed. In this work, we translate tock-CSP into TA so that we can take advantage of TA and its supporting tool UPPAAL.  We provide a list of translation rules for translating the constructs of the tock-CSP into a collection of small TA that address the complexity of capturing the compositionality of \verb!tock-CSP!, which is not available in TA. The translation is justified by testing based on finite approximations to the traces sets of both the original \verb!tock-CSP! and the translated TAs.
%We compose the small TA into various shapes that capture the behaviour of tock-CSP process. We utilise the expressive power of Haskell in both expressing and implementing the translation technique into a tool, which enables us to use trace analysis in justifying the correctness of the translation techniques. 
The result shows significant performance increase in using UPPAAL for the verification of deadlock freedom.
%, a promising check for measuring performance in both FDR and UPPAAL. 


%First, we find a significant performance increase in using UPPAAL for the verification of tock-CSP. Secondly, the work provides an easier alternative for both expressing and verifying liveness requirements that are difficult to specify in tock-CSP. 

==> zz_del/a2_intro.tex <==
%Why is it hard? (E.g., why do naive approaches fail?) 
 
% todo: Modelling and Verification of Timed Robotic Controller
% todo: /home/userfs/a/aha526/Documents/LinktoStuff/Downloads/MN06_ From MITL to Timed Automata.pdf



%CSP-----------------------------------------------------------------------------
Communicating Sequential Processes (CSP) is an established process algebra that provides notations for both modelling and verification of concurrent systems \cite{R10, S10}. Using CSP for verification has been supported with an automatic model-checker FDR \cite{TP14}. CSP and its modelling approaches have significantly contribute in understanding the complexity of concurrent systems  \cite{S10}. 


%tockCSP------------------------------------------------------------------------
Afterwards, \verb!tock-CSP! provides an additional event $tock$ to record a progress of time. This facilitates using CSP for modelling temporal specifications in a suitable format for formal analysis and verification. tock-CSP retains the structure of CSP and utilises the existing works and tools build for CSP. Thus, automatic verification is supported by FDR \cite{TP14, R10}. As a result of that,  \verb!tock-CSP! has been used in the verification of case studies such as security protocols \cite{NS00} and Railways system \cite{YF12}. Recently tock-CSP has been used for capturing the semantics of RoboChart, a DSML for modelling robotics system. Additionally, a recent extension of tock-CSP provides additional notations for specifying budgets and deadlines for effective modelling and verification of temporal specifications \cite{JP19}.



%In this work, we extend the 
%Translation -------------------------------------------------

%In an  effort to improve the verification aspect of CPS,  in this work, we present a model transformation technique for translating tock-CSP into TA that will enable us to use UPPAAL in the verification of tock-CSP.

%In an  effort to improve the verification aspect of CPS,  in this work we present a model transformation technique for translating tock-CSP into TA that will enable us to use UPPAAL in the verification of tock-CSP.


Based on this foundation, we add a step forward by developing a technique for translating tock-CSP into TA that enable using the facilities of UPPAAL for verification of tock-CSP models.  UPPAAL is a tool-suite for modelling and verification of real-time systems \cite{BD06}.  So, in this work we develop both a translation technique and a supporting tool for automatically translating tock-CSP into a network of TA that capture the behaviour of the input tock-CSP models. 


The results of this translation work show a significant increased performance for using UPPAAL in the verification of deadlock freedom in the translated tock-CSP. In comparing the performance, first, we formulate various tock-CSP processes for the possible pairs of the tock-CSP operators that we consider for the scope of this work. Second, we use the developed translation tool to translate the formulated processes into TA for UPPAAL. Third, we used both FDR and UPPAAL to compare the performance of checking deadlock freedom in both tock-CSP models and translated TA, respectively. 

% The results of these comparisons show a significant increasing performance for using UPPAAL in the verification of deadlock freedom in the translated tock-CSP. 


% TO return this paragraph
% % UPPAAL ----------------------------------------------------------------------
% Currently, UPPAAL toolsuite provides tool support for verification \cite{BD06}, testing \cite{LM04, LM05}, simulation \cite{BA07} and scheduling   \cite{FP02}. UPPAAL has been used in the verification of various case studies, such as,  Gear-Box Controller \cite{MP98}   UML Statecharts \cite{D02},  wireless sensor \cite{HS12}, internet protocols  \cite{GV06}, vehicle control system \cite{AB09} and scheduling \cite{AH09}.
% %Developing UPPAAL over 15 years, for additional success of UPPAAL
 
% Contribution  --------------------------------------------------------------------

 


% Outline of the paper  ----------------------------------------------------------------------
The structure of the paper is as follows. Next, Section \ref{background} provides brief backgrounds that are essential for understanding the translation technique.  Section \ref{trans_rule} describes the translation technique and provides sample of the translation rules. Section \ref{evaluation} discusses an evaluation of the translation technique. Section \ref{related_work} highlights related work and also provides brief comparison with this work. Finally, Section \ref{conclusion} highlights future work and concludes the paper.
 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%From R10
%David Jackson wrote his doctoral thesis [70], from R10
%continuous Timed CSP language of Reed (Oxford University D.Phil. Thesis, 1988),
%The first to be developed, and probably the most elegant, is Timed CSP [110–112].
%in tock CSP, and usually the overall system is built so that it does not terminate
 
%From  https://cs.stanford.edu/people/widom/paper-writing.html


% What is the problem?
% Why is it interesting and important?
% Why is it hard? (E.g., why do naive approaches fail?)
% Why hasn't it been solved before? (Or, what's wrong with previous proposed solutions? How does mine differ?)
% What are the key components of my approach and results? Also include any specific limitations.
 
 


==> zz_del/a2_intro_.tex <==
%Why is it hard? (E.g., why do naive approaches fail?) 
 
% todo: Modelling and Verification of Timed Robotic Controller
% todo: /home/userfs/a/aha526/Documents/LinktoStuff/Downloads/MN06_ From MITL to Timed Automata.pdf


Verification of Cyber-Physical Systems (CPS) is becoming an interesting concern due to the increasing advancement of their capability. This leads to increasing acceptance of CPS for universal use, ranging from automatic cooker, autopilot to nuclear reactor. However, the verification aspect remains a questionable concern, which is currently attracting significant research input for developing better techniques and tools for improving the verification of CPS \cite{A13, A15}.

 
%Verification of Cyber-Physical Systems (CPS) is an interesting concern due to the increasing advancement of the technology driven the systems. This successful advancement leads to increasing acceptance CPS for universal use, ranging from automatic toaster, autopilot to nuclear reactor. However, the verification aspect remains a questionable concern, which attracts significant research input in developing better techniques and tools for the verification of CPS \cite{A13, A15}.
 

 
%Successful advancement of Cyber-Physical Systems (CPS) is increasingly become visible with their universal acceptance, ranging from automatic toaster, autopilot to nuclear reactor. As a result of this, verification of such kind of system is becoming an interesting concern that is attracting significant research input \ref{A13}. This is because, 

%Cyber-physical systems combine cyber capabilities with physical capabilities to solve problems that neither part could solve alone.

% ??? from p18
% understand opportunities and challenges in CPS and verification. While the
% beneficial prospects of CPS for society are substantial, it is crucial to also de-
% velop an understanding of their inherent challenges and of approaches to mini-
% mize the impact of potential safety hazards. Likewise, it is important to under-
% stand the ways in which formal verification can best help improve the safety of
% system designs.
% ??


Mostly, CPS are complex system due to the number of multiple components that run concurrently to realised the correct behaviour of the developed system.  Also, each component composes multiple processes for controlling parts of the system, such as sensing, localisation, moving. These processes interact with one another and the physical environment to provide the behaviour of a system. Verifying the possible interactions of these processes require a well equipped systematic verification approach \cite{P18, P12, A15, O00}.

%that makes verification to become a challenging task. 
%and their record of success 
%Cyber-Physical systems are becoming widely used for universal purpose.  The kind of system that involve/encomposes concurrent processes. Verification of such system is becoming an interesting concern.  One of the established formal approach for modelling and verification of concurrent systems is Communicating Sequential Processes (CSP) \ref{R10. R05}. CSP provides notations and supporting tools for specifying and analysing concurrent systems, which contribute to understanding/handling the complexity of concurrent systems \ref{S05}. 

%CSP-----------------------------------------------------------------------------
Communicating Sequential Processes (CSP) is an established process algebra that provides notation for both modelling and verification of concurrent systems \cite{R10, S10}. Using CSP for verification has been supported with an automatic model-checker FDR \cite{TP14}. CSP and its modelling approaches has significantly contributes in both understanding the complexity of concurrent systems  \cite{S05}. 

%Using CSP for verification has been supported with automatic tool, FDR \cite{TP14}.
%This contributes to understanding of concurrent systems. 

However, lack of facilities for modelling temporal specifications motivate the development of an extension, which provides facilities for capturing temporal specification. tock-CSP \cite{R10} and timed-CSP \cite{S10} are the popular approaches for using CSP in modelling temporal specifications.

%One of the successful extensions are tock-CSP \cite{R10} and timed-CSP \cite{S10}. 

% One of the established formal approach for modelling and verification of concurrent systems is Communicating Sequential Processes (CSP) \cite{R10, R05, S10}. CSP is a process algebra that provides notations for formal specification and analysis of concurrent systems, which contribute to understanding/handling the complexity of concurrent systems \cite{S05}. Using CSP for verification has been supported with automatic tool, FDR \cite{TP14}.



%tockCSP------------------------------------------------------------------------
%tock-CSP is another version that provides temporal specification with the deadline facilities but lack urgent facilities for urgent specifications. In this case a special event tock is used to record progress of time. An extension of tock-CSP that provides facilities for urgent specification has been developed, which is called tick-tock-CSP \cite{Pedro}.



% ??????? From tick-tock
% "Extensive use of tock -CSP has been reported, including, for example,
% in the verification of security properties [10], the design of general-purpose I/O
% controllers [11], the study of railways [12], the verification of distributed adaptive
% systems [13], and more recently, in the verification of simulations for robotics [14]."

tock-CSP provides an additional event $tock$ to record progress of time. This facilitates using CSP for modelling temporal specifications in a suitable format for formal analysis and verification. Automatic verification is supported with FDR \cite{TP14, R10}. tock-CSP retains the structure of CSP and utilises the existing works and tools build for CSP. tock-CSP has been used in the verification of case studies such as security protocols \cite{NS00}, Railways system \cite{YF12} and   \cite{??}. Recently tock-CSP has been used for capturing the semantics of RoboChart, a DSML for modelling robotics system. Additionally, a recent extension of tock-CSP provides additional notations for specifying budgets and deadlines for effective modelling and verification of CPS \cite{JP19}.


% tock-CSP is an extension of CSP that provides additional notations for capturing temporal specifications. tock-CSP facilitates modelling temporal specification for formal analysis and verification.  A support for automatic verification is provided using FDR \cite{TP14, R10}. tock-CSP utilises the existing research works and tools build for CSP. tock-CSP has been used in the verification of case studies such as security protocols \cite{NS00}, Railways system \cite{YF12} and   \cite{??}.
% Recent extension of tock-CSP provides additional notations for specifying budgets and deadlines for effective modelling and verification of CPS \cite{JP19}.


%Recent extension of tock-CSP provides additional notations for specifying budgets and deadlines for effective modelling and verification of CPS \cite{JP19}. Additionally, tock-CSP is used to capture the semantics of a domain specific modelling language RoboChart, which has been developed specifically for modelling robotics applications \cite{MR16}, RoboChart has been used in the verification of case studies, such as chemical detector \cite{MR16}, rescue drone \cite{CB19} and  Vacuum cleaner \cite{VC20}.

%Recent extension of tock-CSP provides additional notations for specifying budgets and deadlines for effective modelling and verification of CPS\cite{JP19}   Additionally, tock-CSP is used to capture the semantics of a domain specific modelling language RoboChart, which has been developed specifically for modelling robotics applications \cite{MR16}, RoboChart has been used in the verification of case studies, such as chemical detector \cite{MR16}, rescue drone \cite{CB19} and  Vacuum cleaner \cite{VC20}.


 
%tock-CSP is an extension of timed version of CSP that facilitate capturing temporal specification, An automatic verification is provided using FDR, which is a de facto supporting tool for the verification CSP specification \cite{R10}. Recently, tock-CSP is used to capture the semantics of a domain specific modelling language RC, specifically for modelling robotics applications \cite{MR16}.  Another recent extension of the tock-CSP provides additional notations for specifying budgets and deadlines \cite{JP19}

% Introduction:
% tock-CSP provides textual notations for formal modelling and verification of systems.
% While TA provides graphical notations for modelling systems.

% With the increasing availability of CPS need for verifying their correctness also become a crucial concern. To maintain their integrity,


%BNF ----------------------------------------------------------------------------
%In this work we used the BNF of tick-tock-CSP to translate tock-CSP into TA that facilitates using UPPAAL toolbox for verifying tock-CSP models.

%We developed a translation technique that produces xx translations for translating tock-CSP into TA.
 
%In this work, we extend the 
%Translation -------------------------------------------------

In an  effort to improve the verification aspect of CPS,  in this work we present a model transformation technique for translating tock-CSP into TA that will enable us to use UPPAAL in the verification of tock-CSP.

In an  effort to improve the verification aspect of CPS,  in this work we present a model transformation technique for translating tock-CSP into TA that will enable us to use UPPAAL in the verification of tock-CSP.


Based on this foundation, we add a step forward with developing a technique for translating tock-CSP into TA that enable using the facilities of UPPAAL for verification of tock-CSP models.  UPPAAL is a toolsuite for modelling and verification of real time systems \cite{BD06}.  So in this work we develop both translation technique and a supporting tool for automatically translating tock-CSP into network of TA that capture the behaviour of the input tock-CSP models. 


 
% UPPAAL ----------------------------------------------------------------------
% for the verification of systems modelled with tock-CSP. UPPAAL has been used successfully used in the verification of real-time systems \cite{BD04, BD11}.UPPAAL was developed based on the theory of TA. 

Currently, UPPAAL toolsuite provides tool support for verification \cite{BD04}, testing \cite{LM04, LM05}, simulation \cite{BA07} and scheduling   \cite{FP02}. UPPAAL has been used in the verification of various case studies, such as,  Gear-Box Controller \cite{}   UML Statecharts \cite{},  wireless sensor \cite{HS12}, internet protocols  \cite{GV06}, vehicle control system \cite{AB09} and scheduling \cite{AH09}.
%Developing UPPAAL over 15 years, for additional success of UPPAAL
 
% Contribution  --------------------------------------------------------------------
The result of this translation work shows a significant increasing performance for using UPPAAL in the verification of the translated tock-CSP. Secondly, this translation work facilitates using Timed Computational Tree Logic (TCTL) \cite{A93} in the verification of tock-CSP models. TCTL provides an easier alternative way of specifying liveness requirement. Gavin shows that it is impossible to liveness using tock-CSP in trace model \cite{G08}, but may be possible using tricks with advanced refinement techniques in failure refinement model \cite{R10}.
%, which is beyond the scope of this research.


%Liveness requirement are the form of properties that are impossible to specify tock-CSP using trace refinement \cite{G08}, but may be possible using tricks \cite{G08} with advanced refinement techniques that is failure refinement model \cite{R10}, which is beyond the scope of this research.
% 3 provide an extension for RoboChart, a state-machine based notation for modelling robotics systems. This extension facilitates using UPPAAL for the verification of RoboChart models.


% lIVENESS WITH TCTL
% Liveness requirements are the kind of interesting requirement in the verification hybrid systems \cite{C13}. However, it is very difficult to express liveness in tock-CSP. Gavin shows that it is impossible to express liveness using trace analysis  \cite{G08}, but may be possible using advanced refinement techniques that is failure refinement model \cite{R10}, which is beyond the scope of this research.

% In TA, TCTL provides an easier way of expressing liveness requirements. So, this work contributes in filling this gap for using tock-CSP in the verification of liveness requirements. 

% The result of this work enables us to verify RoboChart models. Secondly, we find a significant increase in performance of using UPPAAL in the verification of the translated tock-CSP specifications. Thirdly, with UPPAAL  we are able to use TCTL \cite{A93} to specify liveness properties, the form of properties that are difficult to specify using refinement in tock-CSP \cite{G08}

% So we developed a translation technique for translating tockcsp into UPPAAL such that we can use the verification facilities of UPPAAL in the analysis and verification of tockcsp models.

% Recently tockcsp has been used to capture semantics of rc, which enable using FDR for the verification. Here we translate tock-CSP into TA that enable using UPPAAL for the verification of temporal specifications. 
%We use small size ta that are easier to compose which enable us to reasonably handle the compositional structure of ta, which is not available in tockcsp.


%Firstly, there is increasing performance in using UPPAAL for the verification of tock CSP then using FDR. 
%we find a significant performance increase in using UPPAAL for the verification of tock-CSP. 

% Secondly, the work provides an easier approach for verifying liveness requirements that are difficult to specify in tock-CSP. 

% Lastly, we provides an extension for verifying RoboChart models, which relies on tock-CSP for verifying temporal specifications.


% Liveness requirements are the kind of interesting requirement in the verification hybrid systems \cite{C13}. However, it is very difficult to express liveness in tock-CSP. Gavin shows that it is impossible to express liveness using trace analysis  \cite{G08}, but may be possible using advanced refinement techniques that is failure refinement model \cite{R10}, which is beyond the scope of this research.

% In TA, TCTL provides an easier way of expressing liveness requirements. So, this work contributes in filling this gap for using tock-CSP in the verification of liveness requirements. 

%timed computational tree logic (TCTL)

% From A91 thesis
%We present two conservative extensions of the existing temporal logics to allow them to specify timing properties. The metric interval temporal logic (MITL) uses linear-time semantics, and its syntax allows temporal operators to be subscripted with intervals restricting their scope in time. The timed computation tree logic (TCTL) uses branching-time semantics, and its syntax provides access to time through a novel kind of time quantifier



% The result of this translation work can be divided into 3. First
% 1 improving efficiency of the verification aspect.
% 2. Provide an alternative for specification that are difficult to specify in tock-CSP. For instance specification that involves eventual occurrence of an event.
% 3 provide an extension for RoboChart, a state-machine based notation for modelling robotics systems. This extension facilitates using UPPAAL for the verification of RoboChart models.

% Extending RC model
% Improve efficiency using UPPAAL
% Verifying RC specs with UPPAAL

% Outline of the paper  ----------------------------------------------------------------------
The structure of the paper is as follows. Next, Section \ref{background} provides a brief backgrounds that are essential for understanding the translation technique.  Section \ref{trans_rule} describes the translation technique and lay down the translation rules together with examples that illustrate using the rules in translating tock-CSP process into TA. Section \ref{evaluation} discuss an evaluation of the translation techniques. Section \ref{related_work} highlights related work, and also provides brief comparison with this work. Then, finally Section \ref{conclusion} highlights future work and concludes the paper.
 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%From R10
%David Jackson wrote his doctoral thesis [70], from R10
%continuous Timed CSP language of Reed (Oxford University D.Phil. Thesis, 1988),
%The first to be developed, and probably the most elegant, is Timed CSP [110–112].
%in tock CSP, and usually the overall system is built so that it does not terminate
 
%From  https://cs.stanford.edu/people/widom/paper-writing.html


% What is the problem?
% Why is it interesting and important?
% Why is it hard? (E.g., why do naive approaches fail?)
% Why hasn't it been solved before? (Or, what's wrong with previous proposed solutions? How does mine differ?)
% What are the key components of my approach and results? Also include any specific limitations.
 
 


==> zz_del/a3_background.tex <==
% CSP
% tock-CSP
% tick-tock-CSP
% BNF
% TA 
% UPPAAL
% Haskell
% ??Bashscript???

% Automatic Validation of Infinite Real-Time Systems
% Model checking Timed CSP


% Advantage of UPPAAL
% Facilities for verifying temporal specifications
% Gavin paper for specifying temporal specs

%Background

This section discusses the required background for understanding the translation work. We begin with discussing the notations of tock-CSP and then discuss the target outcome of the translation work, that is a list of suitable TA for UPPAAL. 

%Then, we briefly describe the structure of Haskell, the language we used for expressing, implementing and evaluating the translation technique.


%CSP and tock-CSP
\subsubsection{tock-CSP} is an extension of CSP, which provides notations for modelling processes and their interactions. There are varieties of basic constant processes such as \verb!SKIP! and \verb!STOP!. \verb!SKIP! expresses a successful termination while \verb!STOP! expresses a deadlock. Also, there are operators such as an operator \verb!prefix (->)! that prefixes an event to a process. For example, the process \verb!move->SKIP! specifies the behaviour of a system that moves and then terminates. 

%So \lstinline{P1 = e->SKIP} is a process that performs the event $e$ and then behaves as SKIP, which terminates the process.  So the process \verb!move->SKIP! specifies the behaviour of a system that moves and then terminate. 

Additionally, there are various binary operators such as sequential composition (;), which composes two processes one after the other. So a process P1;P2 is a process that behaves as P1, and then after P1 terminates, the process behaves as P2. For example, the process \verb!(move->SKIP);(turn->SKIP)!, specifies a system that moves, turns and then terminates.


There are other binary operators for composing processes in different shapes, such as concurrency, choice and interrupt. The collection of the operators provides a rich set of constructs for modelling untimed systems. Details of the CSP operators is available in these books \cite{R10, S10}. 
%Automatic verifications with CSP is supported with a verification tool FDR \cite{TP14}



%TODO: alternative of
%In the same way; 
%correspondingly.

tock-CSP enriches the notations with an additional event \verb!tock! for recording the progress of time \cite{R10}. Each event \verb!tock! indicates a passage of a single time unit. For example,  \verb!move->tock->tock->turn->SKIP! specifies a behaviour of a system that moves, and then after at least two time units, the system turns and then terminates. This additional event tock enables specifying temporal specification in a format that is suitable for formal analysis \cite{TP14}. 

%tock-CSP retains the original structure of CSP which enables using  FDR for the verification of tock-CSP specifications and also utilises the existing works and tools developed for CSP \cite{TP14}. 

For this work, we provide a BNF that defines the \verb!tock-CSP! operators we consider. Part of the BNF is presented in Definition \ref{dfn_CSPproc} as Haskell data definition. The complete BNF is available in an extended report of the work \cite{extendedVersion}. The BNF provides a basic foundation for the translation work.

\vspace{0.2cm}
\begin{tcolorbox} %[title=Title]
\begin{definition} \textbf{Data definition of \lstinline{CSPproc}} 
\label{dfn_CSPproc}
\end{definition}
\tcblower
\lstset{frameround=fttt}
\vspace{-0.2cm}
\begin{lstlisting}[mathescape, language=Haskell, basicstyle=\ttfamily, columns=flexible]
data CSPproc =   STOP
               | SKIP
               | Prefix       Event       CSPproc
               | GenPar       CSPproc     CSPproc  [Event]
\end{lstlisting}
\end{tcolorbox}


% For this work, we consider the following BNF from the recent extension of \verb!tock-CSP! \cite{JP19}. The BNF is presented here as Haskell data definition, which we use as the basic foundation of the translation work. 
%Skipu and Stopu are additional constant process for urgent termination and urgent deadlock respectively.







\subsubsection{Timed Automata for UPPAAL}
TA provides graphical notations for modelling Hybrid systems. In UPPAAL, systems are modelled as a network of TA. Mathematically, TA is defined as a tuple $(L, l_0, C, A, E, I)$, where L defines a set of locations such that $l_0$  is the initial location, C is the set of clocks, A is the set of actions, E is the set of possible edges that connects the locations and \verb!I! is an invariant that is associated with a location. An edge E is defined as $E \subseteq (L \times A \times B(C) \times 2^C \times L)$, which describes an edge from location L that is triggered by an action A associated with a set of clocks B(C) that are reset on following the edge E to a location L  \cite{BD06, B11}.



% Formal reasoning with TA was established based on the semantics of TA. The semantics of TA is defined as a labelled transition system (LTS), which is a tuple $(S, s_0, \rightarrow)$, where $S  \subseteq (L  \times R^C)$, combination of location and an associated clocks value, $s_0$ is the initial state, transition $(\rightarrow)$ in the form of $S \times  A \times S$. There are two forms of transitions. A transition triggered by either time delay (d) or an action (a) or combination of both\cite{BD06, B11}.
% % This defines the two possible transitions with action or delay.


% \paragraph{1. Delay transition}  over time delay: \[  (l,u) \xrightarrow{\text{d}}  (l, u+d) \iff (\forall d : 0 \le d' \le d \implies u+d' \in I(l)  \]
% %\item 
% \paragraph{2. Action transition} triggered by an action:
% \[ (l, u)  \xrightarrow{ \text{a}}  (l', u') \iff  \exists  e = (l, a, g, r, l') \in E \]
% %\vspace{- 0.9cm}
% \[  such \ that \ u \in g, \ u' =[r \rightarrow 0] u \ and \ also \ u' \in I(l) \]


In UPPAAL, a TA performs an action over an edge, synchronously with the environment and possibly with some other TA in the case of broadcast action. An action triggered a transition from one location to another or possibly returns to the same location. A state of a system comprises of three elements:  a list of the locations for all the network of TA, a list of values for both  associated clocks and variables. So, a transition changes the state of the whole system, which defines the traces of a model that is used for both reasoning and verification of a system, together with the automatic support of UPPAAL.
  


 Haskell \cite{H16} is the functional programming language we use for expressing, implementing and evaluating the translation technique. Both concise and expressive power of Haskell helps us in providing a precise description of the translation technique in the form of translation rules.


% \subsubsection{Structure of Haskell}
% Here, we briefly describe the structure of Haskell \cite{H16}, a functional programming language, which we use for expressing, implementing and evaluating the translation technique. We discuss both the style of functional programming approach and highlights some of the provided constructs of Haskell that are essential in understanding this work.



% % Why Haskell
% We choose to use Haskell for 3 reasons.  First, the concise structure of Haskell helps us in providing a precise description of the translation technique in the form of translation rules. Expressing the rules in an executable format maintains the consistency of the translation technique. Secondly, Haskell provides an easier way of representing an abstract syntax tree (AST)\cite{R12}, which plays an essential role in providing a solid foundation for the translation work. Thirdly, in the future, we are planning to use the reasoning facilities of Haskell to reason about the translation rules.



% % Description of function
% In Haskell, a computation is evaluation of expression and application of a function to its argument, which produces a result. A function has parameters and a body. The parameters describe the input of the function, while the body describes the evaluation of the input to get an output. Normally, a function has a name for identification. However, an anonymous function is also possible using $Lambda\ expression$. \footnote{ For example, \lstinline{\x -> x*x}, is an anonymous function that takes input $x$ and computes the square of the input number x.}  Also, both the argument and output can be a function, a concept known as higher-order functions.  This concept provides an interesting way of composing a chain of function for expressing complex computation \cite{H89, H16}.

% %Example 1
% %\begin{exl}  
% \begin{example}
% An example of a simple Haskell program for computing a Fibonacci number.
% \label{fib}
% %todo: change to lstlisten
% \begin{lstlisting}
% fibonacci :: Int -> Int
% fibonacci    0   =  0
% fibonacci    1   =  1
% fibonacci    n   =  fibonacci (n-1) + fibonacci (n-2)
% \end{lstlisting}
% \end{example}
% %\end{exl}
% % 1.   fibonacci :: Int -> Int
% % 2.   fibonacci    0   =  0
% % 3.   fibonacci    1   =  1
% % 4.   fibonacci    n   =  fibonacci (n-1) + fibonacci (n-2)


% % Explanation of the example
% Example  \ref{fib} demonstrates basic Haskell’s constructs, such as type, pattern matching, and recursive call.  Details of Example \ref{fib} is as follows. Line 1 specifies a type for the function. The function \lstinline{fibonacci} takes an argument of type integer and returns an output of type integer. Line 2 and 3 specify the base cases of the function. For the input values 0 and 1, the function returns the same input value 0 and 1 respectively. While for any other value the function returns the sum of two previous terms. This illustrates using the concept of pattern matching to determine the appropriate evaluation of each input. While Line 4 illustrates using recursive calls in evaluating the input. Overall, this example illustrates a complete Haskell program, which is a function \lstinline{fibonacci}.









==> zz_del/a3_bg.tex <==
% CSP
% tock-CSP
% tick-tock-CSP
% BNF
% TA 
% UPPAAL
% Haskell
% ??Bashscript???

% Automatic Validation of Infinite Real-Time Systems
% Model checking Timed CSP


% Advantage of UPPAAL
% Facilities for verifying temporal specifications
% Gavin paper for specifying temporal specs

%Background

This section discusses the required background for understanding the translation work. We begin with discussing the notations of tock-CSP and then discuss the target outcome of the translation work, that is list of suitable TA for UPPAAL. Then, we briefly describe the structure of Haskell, the language we used for expressing, implementing and evaluating the translation technique.


%CSP and tock-CSP
\subsubsection{tock-CSP} is an extension of CSP, which provides notations for modelling process and their interactions. The basic constant processes are SKIP and STOP that express a behaviour of a process that terminates successful and deadlock respectively. A prefix operator  \lstinline{->} prefixes an event to a process. So the process \verb!move->SKIP! specifies the behaviour of a system that moves and then terminate. 

%So \lstinline{P1 = e->SKIP} is process that performs the event $e$ and then behave as SKIP, which terminates the process.  So the process \verb!move->SKIP! specifies the behaviour of a system that moves and then terminate. 

Additional binary operators include sequential composition (;), which composes two processes one after the other. So a process P1;P2 is a process that behaves as P1 and then after P1 terminates, the process behaves as P2. For example, the process \lstinline{(move->SKIP; turn->SKIP)}, specifies a system that moves, turns and then terminates.


There are other binary operators for composing processes in different shapes, such as concurrency, choice, interrupt. The collection of the operators provides a rich set of constructs for modelling untimed system. Details of the CSP operators is available in these books \cite{R10, S10}. Automatic verifications with CSP is supported with a verification tool FDR \ref{TP14}


%However the notations of CSP did not specify time, which means that the process can not specify timing and temporal specifications. This means that there is no possible way for expressing a specification of budget and deadline.  essential specifications for modelling cyber-physical systems.

%tock-CSP
tock-CSP enrich the notations with an additional event $tock$ for recording a progress of time \cite{R10}. Each event tock is a time frame which indicates a passage of a single time unit. For example, the process \lstinline{move->tock->tock->SKIP} specifies a behaviour of a system that moves and then after at least 2 time units the system terminates. This enables specifying temporal specification in a format that is suitable for formal analysis. tock-CSP retains the original structure of CSP which enables using  FDR for the verification of tock-CSP specifications, and also utilises the existing works and tools developed for CSP \cite{TP14}. 

%tock-CSP builds on that with providing additional event tock for recording a progress of time \ref{}. Each event tock is a timeframe which indicates a passage of a single time unit. For example, move -> tock -> tock -> SKIP, is a process that moves and then after at least 2 time unit and then terminates. This enables specifying timing information between events. 

%Support for automatic verification has been provided in FDR, which provides a separate timed section for writing tock-CSP specifications \cite{TP14}. 

%is supported in the automatic verification tool FDR. This is provided in a time-section of a CSP file. 



%We  provide a good foundation for the translation work, with providing BNF base on the tock-CSP extension \ref{JP19}. The BNF describes the selected operators we chose for this translation work.

%Based on this series we develop a translation techniques that translates tock-CSP into UPPAAL that enable using the facilities UPPAAL for the verification.

%Put the BNF here



%Alur, Courcoubetis, and Dill’s seminal work on region graphs [ACD90, ACD93] provided the first algorithm to model check (continuous-time) timed graphs with respect to satisfiability of formulas expressed in the temporal logic TCTL. Timed graphs consist of a finite set of nodes together with a finite set of real-valued clocks, giving rise to an uncountable number of states. However, Alur et al. showed that it was possible to construct an equivalence relation on the state space, partitioning it into a finite number of regions, in such a way that no TCTL formula can distinguish states belonging to the same region. This led naturally to a model checking algorithm. The technique is however computationally expensive—deciding satisfiability of TCTL formulas by timed graphs can be shown to be PSPACE-complete— and much subsequent research has concentrated on finding ways to curb the resulting complexity [HNSY94, LL95, SS95, HKV96, HK97].


% Brief about Timed Automata and  UPPAAL
% summary of UPPAAL section


For this work, we consider the following BNF from the recent extension of tock-CSP \cite{JP19}. The BNF is presented here as Haskell data definition, which we use as the basic foundation of the translation work.

\subfile{BNF}




% %Automata - TA - UPPAAL
% Automata has being used substantially for reasoning about systems \cite{MP86, HM08}. Automata is finite state machine that reads words, which is an infinite sequence of actions that trigger change of states. A list of accepted words describes the possible behaviours the system/model. This enables using traces to modelled the behaviour of a system, which facilitates analysis and verification of a system \ref{CE86, MP86}. Various researchers have explore using Automata for system analysis, which establish theories, techniques and formalism for using automata in system analysis \ref{HM08} 

% % TA -----------------------------------------------------------------------------------------
% Considering the crucial role of time in the operation of cyber-physical systems, Timed Automata was developed as an extension of automata, which provides additional facilities for using clock in specifying temporal specifications \ref{AD94, B05, B11}. This extension of automata facilitates modelling and verifications of real-time systems that includes CPS. Like automata, Timed-automata reads timed-words, which assigns real-valued time to the occurrence of each action \ref{AD94, B05, DH08}. 


% %Timed Control Tree Logic (TCTL) \cite{A93} --------------------------------------------
% Verification with TA has been supported with an automatic tool, UPPAAL \cite{BD06, BL95, LP97}, which is developed for modelling and verification of real-time systems. In UPPAAL, systems are model as a network of timed automata (TA) that have an external clock.  The clock modelled the progress of time with a real value in which time progresses synchronously with the global clock \cite{BD04, BD11, FP02} . 





\subsubsection{Timed Automata for UPPAAL}
TA provides graphical models for modelling Hybrid systems. On top of that, the theory of TA provides a foundation for developing real-time verification system, UPPAAL.  In UPPAAL, systems are modelled as a network of TA, which modelled a process. Mathematically, TA is defined as a tuple $(L, l_0, C, A, E, I)$, where L defines the set of locations, $l_0$  is the initial location, C is the set of clocks, A is the set of actions, E is the set of possible edges that connects the locations. An edge E is defined as $E \subset L \times A \times B(C) \times 2^C \times L$, which describes an edge from location L that is triggered by an action A associated with set of clocks B(C) that are reset on following the edge E to a location L  \cite{BD06, B11}.


%TA provides suitable models for modelling Hybrid systems. Thus, TA provides the a foundation for developing RT verification system, UPPAAL.  In UPPAAL, systems are modelled as a network of TA, in which TA modelled a process. Mathematically, a TA is defined as a tuple $(L, l_0, C, A E, I)$, where L describes the set of possible locations, $l_0$  is the initial location, C is the set of clocks, A is the set of actions, E is the set of possible edges that connects the locations of the TA, which is defined as $E \subset L \times A \times B(C) \times 2^C \times L$.  This describes an edge from location L that is triggered by an action A associated with set of clocks B(C), which is a set of clocks that are reset on following the edge E to a location L  \ref{BD04, B12}.

Formal reasoning with TA was established based on the semantics of TA. The semantics of TA is defined as a labelled transition system (LTS), which is a tuple $(S, s_0, \rightarrow)$, where $S  \subset L  \times R^C$, combination of location and an associated clocks value, $s_0$ is the initial state, transition $(\rightarrow)$ in the form of $S \times  A \times S$. There are two forms of transitions. A transition triggered by either time delay (d) or an action (a) or combination of both\cite{BD06, B11}.
% This defines the two possible transitions with action or delay.

%NOT CLEAR
% The operational semantics is defined as follows, given a $TA = (L, l_0, C, A, E, I)$ with a LTS as $(S, s_0, \rightarrow)$, the two possible transitions are

\paragraph{1. Delay transition}  over time delay, as follow:
\[  (l,u) \xrightarrow{\text{d}}  (l, u+d) \iff (\forall d : 0 \le d' \le d \implies u+d' \in I(l)  \]
%\item 
\paragraph{2. Action transition} triggered by an action, as follow.
\[ (l, u)  \xrightarrow{ \text{a}}  (l', u') \iff  \exists  e = (l, a, g, r, l') \in E \]
%\vspace{- 0.9cm}
\[  such \  that \ u \in g, \ u' =[r \rightarrow 0] u \ and \ also \ u' \in I(l) \]

% \begin{cmt}
% \textit{
% %The Z specification for the above transition is incomplete yet. The above mathematical expressions will be replaced with Z specification
% %After completing the Z specification, it will replace t
% The above mathematical expressions will be replace with Z specifications. At the moment the specifications are incomplete.}
% \end{cmt}
% \textit{Suggestion: They do not necessarily need to be replace with Z *specifications*, but they do need to be in Z syntax. In particular, consider the syntax of the quantified predicates. \\ \\
% I did not understand the above suggestion.}
% \vspace{0.3cm}

In UPPAAL, a TA performs an action over an edge, synchronously with the environment and possibly with some other TA in the case of broadcast action. An action triggered a transition from one location to another or possibly return to the same location. A state of a system comprises of 3 elements,  a list of locations for all the network of TA, a list of associated clock values and value of the variables. So a transition changes the state of the whole system, which defines the traces of the model that is used for both reasoning and verification of a system, together with the automatic support of UPPAAL.
  

%%%%%%%%%%  Example





\subsubsection{Structure of Haskell}
Here, we briefly describe the structure of Haskell \cite{H16}, a functional programming language, which we use for expressing, implementing and evaluating the translation technique. We discuss both the style of functional programming approach and highlights some of the provided constructs of Haskell that are essential in understanding this work.


%Here, we briefly introduce Haskell \cite{H16} as a functional programming language, which we use for expressing, implementing and evaluating the translation technique. We discuss both the style of functional programming approach and highlights some of the provided constructs of Haskell that will help in understanding the work.


% Why Haskell
We choose to use Haskell for 3 reasons.  First, the concise structure of Haskell helps us in providing a precise description of the translation technique in the form of translation rules. Expressing the rules in an executable format maintains the consistency of the translation technique. Secondly, Haskell provides an easier way of representing an abstract syntax tree (AST)\cite{R12}, which plays an essential role in providing a solid foundation for the translation work. Thirdly, in the future, we are planning to use the reasoning facilities of Haskell to reason about the translation rules.

%Thirdly, in the future, the reasoning facilities in Haskell is another important features, which will enable us to reason about the translation rules.


%makes the translation rule to remain consistent with one another. Secondly, Haskell provides an easier way of representing an abstract syntax tree (AST)\cite{R12}. This plays a major role in the foundation of this translation work. Thirdly, the provision of reasoning facilities in Haskell is another important features, which will enable us to reason about the translation rules.



% Description of function
In Haskell, a computation is evaluation of expression and application of a function to its argument, which produces a result. A function has parameters and a body. The parameters describe the input of the function, while the body describes the evaluation of the input to get an output. Normally, a function has a name for identification. However, an anonymous function is also possible using $Lambda\ expression$. \footnote{ For example, \lstinline{\x -> x*x}, is an anonymous function that takes input $x$ and computes the square of the input number x.}  Also, both the argument and output can be a function, a concept known as higher-order functions.  This concept provides an interesting way of composing a chain of function for expressing complex computation \cite{H89, H16}.

%Example 1
%\begin{exl}  
\begin{example}
An example of a simple Haskell program for computing a Fibonacci number.
\label{fib}
%todo: change to lstlisten
\begin{lstlisting}
fibonacci :: Int -> Int
fibonacci    0   =  0
fibonacci    1   =  1
fibonacci    n   =  fibonacci (n-1) + fibonacci (n-2)
\end{lstlisting}
\end{example}
%\end{exl}
% 1.   fibonacci :: Int -> Int
% 2.   fibonacci    0   =  0
% 3.   fibonacci    1   =  1
% 4.   fibonacci    n   =  fibonacci (n-1) + fibonacci (n-2)


% Explanation of the example
Example  \ref{fib} demonstrates basic Haskell’s constructs, such as type, pattern matching, and recursive call.  Details of Example \ref{fib} is as follows. Line 1 specifies a type for the function. The function \lstinline{fibonacci} takes an argument of type integer and returns an output of type integer. Line 2 and 3 specify the base cases of the function. For the input values 0 and 1, the function returns the same input value 0 and 1 respectively. While for any other value the function returns the sum of two previous terms. This illustrates using the concept of pattern matching to determine the appropriate evaluation of each input. While Line 4 illustrates using recursive calls in evaluating the input. Altogether, this example illustrates a complete Haskell program, which is a function \lstinline{fibonacci}.


%In summary, this section provides a brief background for understanding the work. The section briefly discusses the main components of the translation technique, which takes input tock-CSP and translates it into TA for UPPAAL. And also Haskell, which we used for developing the translation technique. In the next section we will discuss the details of the translation technique.



%---------------------------------------------------------------------------------------------
%Each of the TA is used to model a process in the system.
%UPPAAL is an automatic verification tool for Automata. The tool is developed for modelling real-time system. 

%UPPAAL is a tool for modelling real-time systems. Systems are model as a parallel composition of timed automata (TA) that have an external clock.  The clock modelled the progress of time with a continuous time model, in which time progresses synchronously with the global clock. Time is quantified with a real number value.  Each of the TA is used to model a single process in the system.

%Verification with TA has been supported with an automatic tool, UPPAAL, which is developed for modelling and verification of RTS. In

%UPPAAL is an automatic verification tool for Automata. The tool is developed for modelling real-time system. 

%UPPAAL is a tool for modelling real-time systems. Systems are model as a parallel composition of timed automata (TA) that have an external clock.  The clock is modelled with a  continuous time model, in which time progresses synchronously with the global clock. Time is quantified with a real number value.  Each of the TA is used to model a single process in the system.







==> zz_del/a4Overview.tex <==


% Also, in expressing the translation technique, we use the syntax of Haskell for precise description of the translation technique as a function \verb!transTA!, which defines the translation of each of the BNF's constructs into TA.



%In expressing the translation technique, we use the syntax of Haskell for preciseness description of the translation technique. We describe the translation technique as a function \verb!transTA!, which defines the translation of each of the BNF's constructs into TA.












% For extended version, up to ending

% \begin{exl}
% \label{ex_TA}
% For example, the TA shown in Figure \ref{fig_ex_ta} has a corresponding definition in Listing \ref{lst_ex_ta}. The TA has two locations and one transition, together with a corresponding label of the transition. Listing \ref{lst_ex_ta} shows an example of a definition of TA with the definitions of its components: location, transition as well as label. 





% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.4\textwidth]{fig/ex_ta.png}
%     \caption{A sample output TA with two location and one transition.}
%     \label{fig_ex_ta}
% \end{figure}


% \vspace{1cm}
% \begin{tcolorbox} %[title=Title]
% % \begin{trule} \textbf{Translation of STOP}
% % \label{rule_STOP}
% % \end{trule}
% % \tcblower

% %%[Example of an abstract definition of a TA with two locations and one transition]
% %\lstset{framexleftmargin=5mm, frame=single} %, rulesepcolor=\color{blue}}
% %[caption=Example of an abstract definition of a TA with two locations and one transition]
% \begin{lstlisting}[caption= An abstract definition of a TA that has two locations and one transition., captionpos=b, label=lst_ex_ta, language=Haskell]
% TA  "ta1"   []  []  [loc1, loc2] (Init loc1) [tran1] 
%   where 
%      - -  = Location  ID    Name  Label      LocType
%     loc1  = Location "idA"  "A"   EmptyLabel None
%     loc2  = Location "idB"  "B"   EmptyLabel None
    
%      - -  = Transition  Source  Target  [Label] 
%     tran1 = Transition  loc1    loc2    [lab1]  
    
%     lab1  = Sync (VariableID  "start")  Excl
    
    
% \end{lstlisting}

% \end{tcolorbox}

% \end{exl}


% Line 1 is the definition of TA. Line 3 highlights the definition of location. Line 4 and 5 define the 2 locations of the TA. Line 7 highlights the definition of transition. Then, Line 8 defines a transition that connects the 2 locations of the TA. Finally, Line 10 defines the label of the transition.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%  rename, hiden, interrupt and external choice
% renaming and hiding
%In translating a renamed event

% In handling renaming the translation technique carries along a list of renamed events. So before translating each event the technique check if the event is part of renamed event, and then translate the event appropriately with the corresponding new name. In the like manner, if an event is part of hidden event the techniques carries along a list of hidden events. On translating a hidden event the technique uses a s special name $itau$ to replace the hidden event.

Furthermore, in tock-CSP, a process can be interrupted by another process when the two processes are composed with an interrupt operator (\verb!/\!). This is due to the compositional structure of tock-CSP. However, in the case of TA, an explicit transition is needed for expressing an interrupt,  which enables a TA to interrupt another one. So in this translation work, we provide an additional transition for capturing interrupt using an interrupt action which as defined in the coordination action, Definition \ref{coordinating_action}.
%where an interrupt can happen, which begins in the translation of constant process \verb!SKIP}.

For example, given a process \verb!P = P1/\P2!, the process \verb|P1| can be interrupted by process \verb|P2|. Thus, in translating each event of process \verb|P1|, we provide additional transitions for the initials of the interrupting process \verb|P2|, which enables the translated behaviour of \verb|P2| to interrupt the translated behaviour of \verb|P1| at any event.


% n translating each event of the interrupted process p1 tha

% when the two processes are compose with an interrupt operator (\verb!/\!) as (\verb!p1/\p2!) .  Thus, we provide additional transitions for handling interrupt. In translating each event of the interrupted process p1 we provided additional interrupt transitions that enable the interrupt process p1 to takeover the behaviour of the process.
% %Such that the translated process can be interrupted with additional transition.


% Additionally, in translating external choice, we used mutually exclusive actions (action and co-action) to form transitions that enable choosing one behaviour to block the other behaviours. In the external choice, the translation makes all the initials of the translated process available such that choosing one action blocks the other initials. 



Similarly, in translating external choice, we provide additional transitions that enables the the behaviour of the chosen process to block the behaviour of the other processes. Initially, the translated TA make the initials of the translated processes available such that choosing one of the processes block the other alternative processes with the co-actions of the additional transitions for external choice, as defined in Definition \ref{coordinating_action}.



% In a similar manner, we provide additional transitions for handling external choice. The translation technique makes the initials of the translated processes available such that choosing one process blocks the other alternative processes with its co-action. 


%, one transition for each initial of the processes composed with external choice. Such that choosing one of the two processes composed with external choice blocks the other alternative choice. 





For example, given a process \verb!P = P1[]P2! that composes \verb!P1! and \verb!P2! with an operator for external choice such that \verb!Tp! is a list of TA for the translation of the process \verb!P!. Similarly, \verb!Tp1! and \verb!Tp2! are list of TA for the translation of the processes \verb!P1! and \verb!P2! respectively.  The first TA in the list \verb!Tp1! has additional transitions for the initials of \verb!P2! such that choosing \verb! Tp2! blocks \verb!Tp1!. Similarly, the first TA in the list of TA \verb!Tp2! has additional transitions for the initials of \verb!P1! such that choosing \verb!Tp1! blocks the behaviour \verb!Tp2!. Additional details of this example is available in an extended report of the work \cite{extendedVersion}.



% A list of TA for the translation \verb!Tp!, such that \verb!Tp1! and \verb!Tp2! are translation of the processes \verb!P1! and \verb!P2! respectively.  The first TA in the list \verb!Tp1! has additional transitions for the initials of \verb!P2! such that choosing \verb! Tp2! blocks \verb!Tp1!. Similarly, the first TA in the list of TA \verb!Tp2! has additional transitions for the initials of \verb!P1! such that choosing \verb!Tp1! blocks the behaviour \verb!Tp2!. An example is provided in an extended report  \cite{extendedVersion}.



Also, in \verb!tock-CSP!, an event can be renamed or hidden from the environment. In handling renaming, the translation technique carries along a list of renamed events. Before translating each event, the technique checks if the event is part of renamed events, and then translate the event appropriately with the corresponding new name. In the like manner, if an event is part of the hidden events the techniques carries along a list of hidden events, such that on translating a hidden event the technique uses a special name $itau$ in place of the hidden event.




% Translation of the p1 and p2 that are composed with external choice into a process p = p1[]p2. A list of the translated TA for the process Tp, such that Tp1 and Tp2 are list of translated TA for process p1 and p2. The first TA in the list Tp1 has additional transitions for the initials of p2 such that choosing Tp2 blocks Tp1. Similarly, the first TA in Tp2 has additional transitions for the initials p1 such choosing Tp1 blocks Tp2. An example is provided in the extended report \cite{extendedVersion}.



% For example, given processes p1 and p2 that are composed with external choice into a process p = p1[]p2. A list of the translated TA for the process Tp, such that Tp1 and Tp2 are list of translated TA for process p1 and p2. The first TA in the list Tp1 has additional transitions for the initials of p2 such that choosing Tp2 blocks Tp1. Similarly, the first TA in Tp2 has additional transitions for the initials p1 such choosing Tp1 blocks Tp2. An example is provided in the extended report \cite{extendedVersion}.


% In similar manner, we provide additional transitions for handling external choice, one transition for each initial of the processes composed with external choice. Such that choosing one of the two processes composed with external choice blocks the other alternative choice. For example, given processes p1 and p2 that are composed with external choice into a process p = p1[]p2. A list of the translated TA for the process Tp, such that Tp1 and Tp2 are list of translated TA for process p1 and p2. The first TA in the list Tp1 has additional transitions for the initials of p2 such that choosing Tp2 blocks Tp1. Similarly, the first TA in Tp2 has additional transitions for the initials p1 such choosing Tp1 blocks Tp2. An example is provided in the extended report \cite{extendedVersion}.

%one another on choosing one of the two processes. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  rename, hiden, interrupt and external choice



==> zz_del/a4Overview_.tex <==
In expressing the translation technique we use the syntax of Haskell for precise description of the translation technique. We describe the translation technique as a function \verb!transTA!, which defines the translation of each of the BNF's constructs into TA.



\vspace{0.5cm}
\begin{tcolorbox} %[title=Title]
\begin{definition} \textbf{Function \lstinline{transTA}}
\label{dfn_transTA}
\end{definition}
\tcblower
\begin{verbatim}
transTA :: CSPproc -> ProcName  -> BranchID -> StartID ->
          FinishID -> UsedNames -> ([TA], [Event], [SyncPoint])
\end{verbatim}
\end{tcolorbox}


\vspace{0.5cm}
\begin{tcolorbox} %[title=Title]
\begin{definition} \textbf{Function \lstinline{transTA}}
\label{dfn_transTA}
\end{definition}
\tcblower
%\begin{verbatim}
\begin{lstlisting}[mathescape, language=Haskell, basicstyle=\ttfamily, columns=flexible]
transTA :: CSPproc  -> ProcName  -> BranchID -> StartID ->
           FinishID -> UsedNames -> ([TA], [Event], [SyncPoint])
\end{lstlisting}
%\end{verbatim}
\end{tcolorbox}



The function \lstinline{transTA} has 6 parameters, input tock-CSP process, process name, list of branch identifiers for the translated TA, list of start identifiers for the translated TA, list of finish identifiers for the translated TA, list of names we used in defining the translation function. The output of the function is \lstinline{[TA], [Event], [SyncPoint]}, a tuple containing 3 elements, a list of the translated TA, a list of the translated events into actions for constructing an environment TA at the end of the translation, a list of synchronisation actions for the constructing a synchronising TA.




From the BNF of UPPAAL \cite{LP97}, the key elements of the output TA are the definition of TA itself and the definition of its components: locations, transitions and the corresponding definition of their labels. These are express in the following definitions as Haskell data. 


\vspace{0.5cm}
\begin{tcolorbox} %[title=Title]
\begin{definition} \textbf{TA}  %   {Data definition of TA} 
\label{dfn_TA}
\end{definition}
\tcblower
\begin{verbatim}
data TA = 
 TA Name [Parameter] [Declaration] [Location] Init [Transition]
\end{verbatim}
\end{tcolorbox}


% \vspace{0.5cm}
% \begin{tcolorbox} %[title=Title]
% \begin{definition} \textbf{TA}  %   {Data definition of TA} 
% \label{dfn_TA}
% \end{definition}
% \tcblower
% %\begin{verbatim}
% \begin{lstlisting}[mathescape, language=Haskell, basicstyle=\ttfamily, columns=flexible] 
% data TA = 
%  TA Name [Parameter] [Declaration] [Location] Init [Transition]
% \end{lstlisting}
% %\end{verbatim}
% \end{tcolorbox}
%data TA = TA Name [Parameter] [Declaration] [Location] [Branchpoint]  
%         Init [Transition]


%Definition \ref{dfn_TA} is provides a
The data TA has a constructor \lstinline{TA} with 6 parameters \ref{dfn_TA}. First parameter of type \lstinline{Name} is an identifier for the TA itself. Second parameter of type \lstinline{Parameter} is a list of arguments for the TA. Third parameter of type \lstinline{Declaration} is a list of local definitions inside the TA. Fourth parameter of type \lstinline{Location} is a list of locations in the TA, which is defined in the following Definition \ref{dfn_location}. Fifth parameter of type \lstinline{Init} is an initial location of the TA. Last parameter of type \lstinline{Transitions} is a list of transitions that connect the locations of the TA, also defined below in Definition \ref{dfn_transition}.   


\vspace{0.5cm}
\begin{tcolorbox} %[title=Title]
\begin{definition} \textbf{Location} 
\label{dfn_location}
\end{definition}
\tcblower
%\begin{lstlisting}[mathescape, language=Haskell, basicstyle=\ttfamily, columns=flexible]
\begin{verbatim}
data Location = Location ID Name Label LocType
\end{verbatim}
% \end{lstlisting}
\end{tcolorbox}


Definition \ref{dfn_location} defines a location with a constructor that has 4 parameters, of types \lstinline{ID, Name, Label and LocType}. First parameter of type  \lstinline{ID} is an identifier for the location. Second parameter of type \lstinline{Name} is a tag for the location. Third parameter of type \lstinline{Label} is a constraint label for the location, defined below in Definition \ref{dfn_label}. Last parameter of type \lstinline{LocType} is a format of the location, which can be one of these three: \lstinline{urgent}, \lstinline{committed}, \lstinline{none} (which means normal location that is neither urgent nor committed). 





\vspace{0.5cm}
\begin{tcolorbox} %[title=Title]
\begin{definition} \textbf{Transition} 
\label{dfn_transition}
\end{definition}
\tcblower
\begin{verbatim}
data Transition = Transition Source Target [Label]
\end{verbatim}
\end{tcolorbox}

Similarly, transition has three parameters. Two locations for both source and target of the transition. The third parameter is label. Both location and transition has label, which can be empty (for a silent transition), invariant, Guard, Update, synchronisation action or combinations of them, as defined below.  

\vspace{0.5cm}
\begin{tcolorbox} %[title=Title]
\begin{definition} \textbf{Label} 
\label{dfn_label}
\end{definition}
\tcblower
\begin{verbatim}
data Label = EmptyLabel 
           | Invariant     Expression 
           | Guard         Expression 
           | Update       [Expression] 
           | Sync          Identifier   Direction
\end{verbatim}
\end{tcolorbox}




% \vspace{0.5cm}
% \begin{tcolorbox} %[title=Title]
% \begin{definition} \textbf{TA and its components} 
% \label{dfn_label}
% \end{definition}
% \tcblower
% \begin{verbatim}
% data TA = 
%  TA Name [Parameter] [Declaration] [Location] Init [Transition]

% data Location   = Location ID Name Label LocType

% data Transition = Transition Source Target [Label]

% data Label = EmptyLabel 
%           | Invariant     Expression 
%           | Guard         Expression 
%           | Update       [Expression] 
%           | Sync          Identifier   Direction
% \end{verbatim}
% \end{tcolorbox}




% ------ To remove this begin
% Finally, label is an expression (or list of expressions) that is associated with either a location or a transition. For a location, a label can be empty or invariant that specifies the constraint condition of the location. While for a transition the label can be either empty for silent transition or any combination of these three types: \lstinline{Guard}, \lstinline{Update} and \lstinline{Sync}.  Where \lstinline{Sync} is a type for an UPPAAL action that has an identifier and direction, which is either sender (with question mark) or receiver (with exclamation mark).
% ------ To remove this end
% Label of a state can be empty or invariant
% For state

% While for transition can be ...
% For transition

% Finally, label is either expression or list of expressions an action that is associated to state or transition. For the case of transition the label can be an action. There are five types of label.



%%%%%%%%%%%%%%%%%%%%%%%%   Example of TA

\begin{exl}
\label{ex_TA}



For example, the TA shown in Figure \ref{fig_ex_ta} has a corresponding definition in Listing \ref{lst_ex_ta}. The TA has two locations and one transitions, together with a corresponding label of the transition. Listing \ref{lst_ex_ta} shows an example of a definition of TA with the definitions of its components: location, transition as well as label. 

%that illustrates a definition of TA shown in Figure \ref{fig_ex_ta}, which is defined in Listing \ref{lst_ex_ta} that is express using syntax of Haskell. The examples shows the definition of TA with definitions of both location and transition as well as label. 




\begin{figure}[H]
    \centering
    \includegraphics{fig/ex_ta.png}
    \caption{A sample output TA with two location and one transition.}
    \label{fig_ex_ta}
\end{figure}


\vspace{1cm}
\begin{tcolorbox} %[title=Title]
% \begin{trule} \textbf{Translation of STOP}
% \label{rule_STOP}
% \end{trule}
% \tcblower

%%[Example of an abstract definition of a TA with two locations and one transition]
%\lstset{framexleftmargin=5mm, frame=single} %, rulesepcolor=\color{blue}}
%[caption=Example of an abstract definition of a TA with two locations and one transition]
\begin{lstlisting}[caption= An abstract definition of a TA that has two locations and one transition., captionpos=b, label=lst_ex_ta, language=Haskell]
TA  "ta1"   []  []  [loc1, loc2] (Init loc1) [tran1] 
  where 
     - -  = Location  ID    Name  Label      LocType
    loc1  = Location "idA"  "A"   EmptyLabel None
    loc2  = Location "idB"  "B"   EmptyLabel None
    
     - -  = Transition  Source  Target  [Label] 
    tran1 = Transition  loc1    loc2    [lab1]  
    
    lab1  = Sync (VariableID  "start")  Excl
    
    
\end{lstlisting}

\end{tcolorbox}

\end{exl}


%%%%%%   ---- short version
Line 1 is the definition of TA. Line 4 and 5 define the 2 locations of the TA. Line 8 defines a transition that connects the locations of the TA. Finally, Line defines the label of the transition.

Furthermore, a process can be interrupted when the process is part interruption, we provide an additional transitions for handling the interrupt. Also, we add special transition for handling external choice.
%%%%%%%%%%%%%  -- short version


% %???????????????? Update names 
% ----------- To remove for short version begins
% Line 1 defines a TA using Definition \ref{dfn_TA} with 6 arguments. First, \lstinline{"ta1"} is the name of the TA. Second and third are empty lists for both  parameters of the TA and its local definitions. Fourth,  \lstinline{[loc1, loc2]} is a list of locations for the TA that contains 2 locations,  \lstinline{loc1} and  \lstinline{loc2}. Fifth,  \lstinline{(init loc1)} specifies loc1 as the initial location of the TA. Lastly, \lstinline{[tran1]} is a list of transitions that has one transition for the TA. 

% Line 3 highlights a definition location from Definition \ref{dfn_location}. Then, Line 4 defines  \lstinline{Loc1} as an instance of location with an identifier  \lstinline{"idA"} and name  \lstinline{"A"}, with an empty label that indicates no constraint in the location, and also specify the type of the location to be None. In the like manner, Line 5 defines  \lstinline{loc2} as the second location with an identifier  \lstinline{"idB"}, name  \lstinline{"B"}, also label with empty that specify no constraint in the location, and  specify a type for the location to be None.

% Line 7 is a comment that highlights a definition of a transition from Definition \ref{dfn_transition}. Then, Line 8 defines  \lstinline{tran1} as a transition that connects two locations  \lstinline{loc1} and  \lstinline{loc2} with  \lstinline{[lab1]} as a label of the transition.  \lstinline{lab1} is defined in Line 10 using the definition of label from Definition \ref{dfn_label} as an UPPAAL action with identifier "start" that has direction Excl which specifies the acation as a sender.



% In Listing \ref{lst_ex_ta}, specifically Line 1, we use a simple name "ta1" for the TA. However, in the coming translation rules, We formulate an approach for generating uniforms names for the small TA. We consider the structure of the AST of the tock-CSP process, which is in a form of a binary tree. So we assign an identifier to both the branch and the depth of the tree, using binary number and positive integer respectively. Then, at in the translation rules, we concatenate the two identifiers to generate a name for each small TA. Examples are provided in the translation rules, that illustrate how we formulate the names of the small TA.


% %defined in Line 4 -- 5. Definition of a location is highlighted in Line 


% Furthermore, in tock-CSP, a process can be interrupted by another process when the two processes are composed using interrupt operator (\lstinline{/\}). This is due to the compositional structure of tock-CSP. However, in the case of TA, an explicit transition is needed for expressing an interrupt,  which can enable a TA to interrupt another one. So in this translation work, we provide an additional transition for capturing interrupt where an interrupt can happen, which begins in the translation of constant process \lstinline{SKIP} that will come later in Section \ref{sec_skip}. 


% Additionally, in translating external choice, we used mutually exclusive actions (action and co-action) to form transitions that enable choosing one behaviour to block the other behaviours. In the external choice, the translation makes all the initials of the translated process available such that choosing one action blocks the other initials. 



% The above Example \ref{ex_TA} illustrates a simple form of the output TA produced by the translation function \lstinline{transTA}. However, in the translation rule we will have TA with more than two states and multiple transitions. The upcoming translation rules define the function \lstinline{transTA}. Each rule defines a translation of one of the constructors of the BNF previously presented in Section \ref{BNF}. In the next section, we discuss details of each of the translation rules together with an example for illustrating using the rule in translating a process.
% ----------- To remove for short version ends





==> zz_del/a4Strategy.tex <==
%Translation_Strategy


This section discusses an overview of the translation technique. Then, we illustrate the technique with translating a simple specification of an Automatic Door System (ADS) in Example \ref{ads}. Also, we present  samples of using the translation rules, which summarise the translation technique. Each rule defines a translation of an operator of the \verb!tock-CSP! operators that we consider for this work.




\subsection{Overview of the Translation Technique}



The translation technique produces a list of small TA, such that the occurrence of each \verb!tock-CSP! event is captured in a small TA with an UPPALL action,  which records an occurrence of an event. The action has the same name as the name of the translated event from the input tock-CSP process. Then, the technique composes these small TA into a network of TA that express the behaviour of the original tock-CSP model. The main reason for using small TA is coping with the compositional structure of tock-CSP, which is not available in TA \cite{DH08}. The small TA provides enough flexibility for composing TA in various ways that capture the behaviour of the original \verb!tock-CSP! process.  


Connections between the small TA are developed using additional coordinating actions, which coordinate and link the small TA into a network of TA to establish the flow of the translated \verb!tock-CSP! process.  Each coordinating action \verb|a!| (with an exclamation mark) synchronises with the corresponding co-action  \verb|a?| (with a question mark) to link two TA, in such a way that the first TA (with \verb|a!|) communicates with the second TA that has the corresponding co-action (\verb|a?|).


 \vspace{0.2cm}
\begin{tcolorbox} %[title=Title]
\begin{definition} \textbf{Coordinating Action}
\label{coordinating_action}
\end{definition}
\tcblower
A coordinating action is an UPPAAL action that is not part of the original tock-CSP process. There are six types of coordinating actions:
\begin{itemize}
    
\item \textbf{Flow action} only coordinates a link between two TA for capturing the flow of the behaviour of the original tock-CSP process. 
    
\item \textbf{Terminating action} records termination information, in addition to coordinating a link between two TA.


\item \textbf{Synchronisation action} coordinates a link between a TA that participate in a multi-synchronisation action and a TA for controlling the multi-synchronisation. 


\item \textbf{External choice action} coordinates the translation of external choice such that choosing one of the processes composed with external choice blocks the other alternative choices.


\item \textbf{Interrupt action} initiates an interruption of a process that enables a process to interrupt another process that are composed with interrupt operator.

\item \textbf{Exception action} coordinates a link between a TA that raises an exception and a control TA for handling the exception. 


\end{itemize}
\end{tcolorbox}



\vspace{0.5cm}


The name of each coordinated action is unique to establish correct flow. The name of a flow action is in the form \verb!startIDx!, where \verb!x! is either a natural number or the name of the original tock-CSP process. Likewise, the name of the remaining coordinating action follows in the same pattern \verb!keywordIDx! where  \verb!keyword! is a designated word for each of the coordinating action: \verb!finish! for terminating action,  \verb!ext! for external choice action, \verb!intrp! for interrupting action, and \verb!excp! for exception action. Similarly, the name of a synchronising action is in the form \verb!eventName___sync!, that is an event name appended with the keyword \verb!___sync! to differentiate the synchronisation event from other events. 

% of type UPPAAL broadcast channel.

% \verb!sync! for synchronisation action,

Termination actions are provided to capture essential termination information from the input tock-CSP in the cases where a TA needs to communicate a successful termination for another TA to proceed. For example, like in the case of sequential composition \lstinline{P1;P2} where the process \lstinline{P2} begins after successful termination of the process \lstinline{P1}.  



% The name of each coordinated action is unique to establish correct flow. The name of a flow action is in the form \lstinline{startIDx}, where \lstinline{x} is either a natural number or the name of the original tock-CSP process. Likewise, the name of a terminating action is in the form \lstinline{finishIDx}, where \lstinline{x} is a natural number. This termination action captures essential termination information from the input tock-CSP in the cases where a TA needs to communicate a successful termination for another TA to proceed. For instance, in the case of sequential composition \lstinline{P1;P2} where the process \lstinline{P2} begins after successful termination of the process \lstinline{P1}.  


% The name of each coordinated action is unique, which forms a unique link that ensures that each TA connects with the correct TA to form a network of TA, which correctly captures the behaviour of the original tock-CSP. The name of a flow action is in the form \lstinline{startIDx}, where \lstinline{x} is either a natural number or the name of the original tock-CSP process. Likewise, the name of a terminating action is in the form \lstinline{finishIDx}, where \lstinline{x} is a natural number. This termination action captures essential termination information from the input tock-CSP in the cases where a TA needs to communicate a successful termination for another TA to proceed. For instance, in the case of sequential composition \lstinline{P1;P2} where the process \lstinline{P2} begins after successful termination of the process \lstinline{P1}.  



 


% Finally, the name of an exception action is in the form of \lstinline{startExcpIDx}, where x is a natural number. A TA raises an exception with a coordinating action \lstinline{startExcpIDx!} and a TA for controlling the exception responds with the corresponding coordinating co-action  \lstinline{startExcpIDx?}. 


% So far, the translated actions of the input tock-CSP process do not have the corresponding co-actions. So,

For each translated tock-CSP specification, we provide an environment TA that has corresponding co-actions for all the translated events of the input tock-CSP process. In addition, the environment TA has two coordinating actions that link the environment TA with the network of the translated TA. First, a flow action that links the environment with the first TA in the list of the translated TA. Also, this first flow action is the starting action that activates the behaviour of the translated TA. Second, a terminating action that links back the final TA in the list of the translated TA to the environment TA, and also records a successful termination of the whole process. 


% \vspace{0.2cm}
\begin{tcolorbox} %[title=Title]
\begin{definition} 
\textbf{Environment TA}
\label{environment_TA}
\end{definition}
\tcblower
An environment TA models an explicit environment for UPPAAL models. The environment TA has one state and transitions for each co-action of all the events in the original tock-CSP process, in addition to two transitions for the first starting flow action and the final termination co-action. 
\end{tcolorbox}


Also, for translating multi-synchronisation events, we adopt a centralised approach developed in \cite{O05} and implemented using Java in \cite{F05}. The approach describes using a separate centralised controller for controlling multi-synchronisation events. Here, we use UPPAAL broadcast channel to communicates synchronisation between the synchronisation controller and the TA that participate in the synchronisation. 


%(\lstinline{sync_IDx?}).
%Here we adopt and implement the approach in Haskell.

% \vspace{0.5cm}
\begin{tcolorbox} %[title=Title]
\begin{definition} \textbf{Synchronisation TA}
\label{dfn_syncTA}
\end{definition}
\tcblower
A synchronisation TA coordinates a translated multi-synchronisation action. The structure of synchronisation TA has an initial state and a committed state for each multi-synchronisation action. And for each of the committed state, there are two transitions. The first transition connects the initial state to the committed state. This first transition has a guard that is enable only when all the TA that participate in that multi-synchronisation become ready for the synchronisation, which enables the TA to synchronise first with the environment TA on the first transition and then immediately broadcast the synchronisation action in the second transition, which connects the committed state back to the initial state of the synchronisation TA. 

%The second transition connects the committed state back to the initial state.

\end{tcolorbox}




When all the participating TA become ready, a synchronisation TA broadcasts the multi-synchronisation action such that all the corresponding participating TA synchronise using their corresponding co-action. The provided guard ensures that the TA synchronises with the required number of TA that participate in a multi-synchronisation action. The guard blocks the broadcast multi-synchronisation action until all the participating TA become ready, which enables the corresponding guard for broadcasting the multi-synchronisation action. 
% Example \ref{ads} illustrates the technique. 

%with translating a tock-CSP process.



% %Simple Example
% \subfile{Eg}


%Concurency example
\subfile{EgGenPar/EgGen}








==> zz_del/a4Strategy_.tex <==
%Translation_Strategy


This section discusses an overview of the translation technique, which discusses our strategy in translating tock-CSP processes. We illustrate the strategy with translating a simple specification of an Automatic Door System (ADS)
%, which is provided as an example in this section.


%This section discusses an overview of the translation technique forour strategy in translating tock-CSP processes. We illustrate the strategy with translating a simple specification of an Automatic Door System (ADS), which is provided as an example in this section.

The translation technique produces a list of small TA, such that the occurrence of each tock-CSP event is captured by a small TA with an UPPALL action,  which records an occurrence of an event. The action has the same name as the name of the translated event from the input tock-CSP process. Then, the strategy composes these small TA into a network of TA that express the behaviour of the original tock-CSP model. The main reason for using small TA is coping with the compositional structure of tock-CSP, which is not available in TA \cite{DH08}. The small TA provides enough flexibility for composing TA in various ways that capture the behaviour of the original tock-CSP process.  



% In carrying out the translation, we produce small TA, such that the occurrence of each tock-CSP event is captured by a small TA with an UPPALL action,  which records an occurrence of an event. The action has the same name as the event in the input tock-CSP process. 



%The strategy composes these small TA into a network of TA that express the behaviour of the original tock-CSP model. The main reason for using small TA is coping with the compositional structure of tock-CSP, which is not available in TA \cite{DH08}.  Details of this compositionality will be discussed in both the subsequent Section \ref{rules} and Chapter 4. The small TA provides enough flexibility for composing TA in various ways that capture the behaviour of the original tock-CSP process.  


The connection between the small TA is developed using additional coordinating actions, which link the small TA to establish the flow of the original tock-CSP process.  Each coordinating \lstinline{action!} (with an exclamation mark) synchronises with the corresponding co-action \lstinline{action?} (with a question mark) to link two TA, in such a way that the first TA (with \lstinline{action!}) activates the second TA (with the corresponding co-action \lstinline{action?}).

%We next characterise precisely the set of coordinating actions.
%All these coordinating actions are designed to have unique names that are not part of the original tock-CSP process.



\vspace{0.5cm}
\begin{tcolorbox} %[title=Title]
\begin{definition} \textbf{Coordinating Action}
\label{coordinating_action}
\end{definition}
\tcblower
A coordinating action is an UPPAAL action that is not part of the original tock-CSP process. There are four types of coordinating actions:
\begin{itemize}
    
\item \textbf{Flow action} only coordinates a link between two TA for capturing the flow of the behaviour of the original tock-CSP process. 
    
\item \textbf{Terminating action} records termination information, in addition to coordinating a link between two TA.


\item \textbf{Synchronisation action} coordinates a link between a TA that participate in a multi-synchronisation action and a TA for controlling the multi-synchronisation. 

\item \textbf{Exception action} coordinates a link between a TA that raises an exception and a control TA for handling the exception. 

\end{itemize}
\end{tcolorbox}



\vspace{0.5cm}

The name of each coordinated action is designed to be unique, which ensures that each TA synchronises and connects with the correct TA to form a network of TA, which correctly captures the behaviour of the original tock-CSP. The name of a flow action is in the form \lstinline{startIDx}, where \lstinline{x} is either a natural number or the name of the original tock-CSP process. Likewise, the name of a terminating action is in the form \lstinline{finishIDx}, where \lstinline{"x"} is a natural number. This termination action captures essential termination information from the input tock-CSP in the cases where a TA needs to communicate a successful termination for another TA to proceed. For instance, in the case of sequential composition \lstinline{P1;P2} where the process \lstinline{P2} begins after successful termination of the process \lstinline{P1}.  



% The strategy uses 4 types of coordinating actions, flow action, terminating action, synchronisation action and exception action, as defined in Definition \ref{coordinating_action}. The name of each coordinated action is designed to be unique, which ensures that each TA synchronises and connects with the correct TA to form a network of TA, which correctly captures the behaviour of the original tock-CSP. The name of a flow action is in the form \lstinline{startIDx}, where \lstinline{x} is either a natural number or the name of the original tock-CSP process. 

% Likewise, the name of a terminating action is in the form \lstinline{finishIDx}, where \lstinline{"x"} is a natural number. This termination action captures essential termination information in the cases where a TA needs to communicate a successful termination for another TA to proceed. For instance, in the case of sequential composition \lstinline{P1;P2} where the process \lstinline{P2} begins after successful termination of the process \lstinline{P1}.  


%In the case of synchronisation

%The third type of coordinating action is synchronising action that coordinates a link between a TA for controlling multi-synchronising action and a TA that participates in the multi-synchronising action. 

Similarly, the name of a synchronising action is in the form \lstinline{sync_action!} and has a type UPPAAL broadcast channel. When all the participating TA become ready, the control TA broadcasts the multi-synchronisation action and all the corresponding participating TA synchronise using their corresponding co-action \lstinline{sync_action?}.

%Finally, an exception action is the type of coordinating action that captures information about raising an exception in the translated TA, in addition to coordinating link between a TA that raises an exception and a control TA for controlling the exception. The

Finally, the name of an exception action is in the form of \lstinline{startExcpIDx}, where x is a natural number. A TA raises an exception with a coordinating action \lstinline{startExcpIDx!} and a TA for controlling the exception responds with the corresponding coordinating co-action  \lstinline{startExcpIDx?}. 
% We provide an example exception action in Section \ref{exception}, which comes after discussing a translation exception construct.

%An example is provided in Section \ref{exception}, that is after discussing the translation of construct exception.





%\paragraph{Explicit Environment for UPPAAL model}

So far the translated actions of the original tock-CSP process does not have the corresponding co-actions. So, for each translated tock-CSP specifications, we provide an environment TA that has corresponding co-actions for all of the translated events in the original tock-CSP process. In addition, the environment TA has two coordinating actions that link the environment TA with the network of the translated TA. One of the coordinating action is the first flow action that links the environment with the first TA in the list of the translated TA. This is the first starting action that activates the behaviour of the translated TA. The second coordinating action is a terminating action that links the final TA in the list of the translated TA to the environment TA, and also indicates a successful termination of the whole process. 


%As already discussed in Chapter 2, in UPPAAL each action (\lstinline{action!}) has a corresponding co-action (\lstinline{action?}). Where \lstinline{action!} (with exclamation mark) is the sender while \lstinline{action?} (with question mark) is the receiver \cite{BD06}.


\vspace{0.5cm}
\begin{tcolorbox} %[title=Title]
\begin{definition} 
\textbf{Environment TA}
\label{environment_TA}
\end{definition}
\tcblower
An environment TA is an UPPAAL TA that models an explicit environment for UPPAAL models. The environment TA has one state and transitions for each co-actions of all the events in the original tock-CSP process, in addition to two transitions for the first starting flow action and the final termination co-action. 
\end{tcolorbox}

%in a list of translated TA for a process.



%As a result of that, 


%Accordingly, for each translated tock-CSP process, we provide an environment TA that has corresponding co-actions for all of the translated events in the original tock-CSP process. In addition, the environment TA has two coordinating actions that link the environment TA with the network of the translated TA. One of the coordinating action is the first flow action that links the environment with the first TA in the list of the translated TA. This is the first starting action that enables the environment to activate the behaviour of the translated TA. The second coordinating action is a terminating action that links the final TA in the list of the translated TA to the environment TA, and also indicates a successful termination of the whole process. 

%Accordingly, we provide a TA for modelling the environment, which provides the corresponding co-actions for all of the translated events in the original tock-CSP process. In addition, the environment TA has two coordinating actions that link the environment TA with the network of the translated TA. One action is the first flow action that links the environment with the first TA in the list of the translated TA. This is the first starting action that enables the environment to activate the behaviour of the translated TA. The second action is a terminating action that links the final TA in the list of the translated TA to the environment TA, and also indicates a successful termination of the whole process. 


%\vspace{0.5cm}

%Turning now to
Also, for the translation of multi-synchronisation event, we adopt a centralised approach developed in \cite{O05} and implemented using Java in \cite{F05}. The approach describes using a separate centralised controller for controlling multi-synchronisation events. Here we adopt and implement the approach in Haskell.
%The following Definition \ref{dfn_syncTA} defines a TA for controlling multi-synchronisation action.


%that control multi-synchronisation action. 




\vspace{0.5cm}
\begin{tcolorbox} %[title=Title]
\begin{definition} \textbf{Synchronisation TA}
\label{dfn_syncTA}
\end{definition}
\tcblower
Synchronisation TA is an UPPAAL TA that coordinates the translated multi-synchronisation action. A synchronisation TA has an initial state and a committed state for each multi-synchronisation action. Each of the committed state has two transitions. The first transition connects the initial state to the committed state. The second transition connects the committed state back to the initial state.


%The guard of a synchronisation TA enables the broadcast synchronisation action only when all the required TA are ready for the synchronisation.

\end{tcolorbox}


% Name 
%The name of the multi-synchronisation controller is in the form of\lstinline{syncTA}.




%In translating multi-synchronisation event, we adopt a centralised approach developed in \cite{O05} and implemented using Java in \cite{F05}. The approach describes using a separate centralised controller for controlling multi-synchronisation events. Here we adopt and implement the approach in Haskell.  Definition \ref{dfn_syncTA} defines a separate control synchronisation TA \lstinline{syncTA} that control multi-synchronisation action. 

%In the list of the translated TA,
This synchronisation TA ensures correct synchronisation for the required TA that participate in a multi-synchronisation action. This is achieved with the use of guard and broadcast channel of UPPAAL. The guard blocks the broadcast multi-synchronisation action until all the participating TA becomes ready, which enables the guard for broadcasting the multi-synchronisation action.




%This synchronisation TA ensures that all the required processes that participate in a multi-synchronisation synchronise correctly with the use of additional guard and broadcast channel of UPPAAL. Initially, the guard blocks the broadcast multi-synchronisation action until all the participating TA become ready, which enables broadcasting the multi-synchronisation action.


%Initially, in the list of the translated TA, each TA that participates in a multi synchronisation action has to send a synchronisation request to the corresponding multi-synchronisation control TA and then waits for a broadcast synchronisation action for the requested multi-synchronisation action. Each transition of a multi-synchronisation action has a guard that becomes enabled only when the control TA receives the required synchronisation requests from the required number of participating TA in that multi-synchronisation action. Receiving enough synchronisation requests enables an associated guard for the transition from initial states to a committed state of that multi-synchronisation action. This transition communicates the occurrence of multi-synchronisation action with environment TA and then also immediately broadcasts the multi-synchronisation action, which enables all the participating TA to synchronise and proceed to complete their behaviours.  Further details and example are provided in Section  \ref{GenPar} and Example \ref{ex_genPar} respectively, which come after discussing the translation of construct generalised parallel.




The strategy is illustrated in the following Example \ref{ads}, which demonstrates a translation of a simple tock-CSP specification of an automatic door system from tock-CSP into UPPAAL TA.


%%%%%%%%%%%%%%%%%%%%%%%%%%%   EXAMPLE ADS
%\begin{proof} \textbf{Example for translating a simple automatic door system}\\
\begin{example} \textbf{A translation of Automatic Door System (ADS)}\\
\label{ads}
This example illustrates a translation of an automatic door system (ADS). Let consider a simple model of a system that opens a door, and then after at least one time unit, the system closes the door. A tock-CSP specification of the system is: %model with the following process: \\
\verb!          ADS = open -> tock -> close -> SKIP!. 

A translation of ADS produces the following list of TA in Figures \ref{ta1}, \ref{ta2}, \ref{ta3}, \ref{ta4} and \ref{ta_env}.


\begin{figure}
\subfigure{\includegraphics [width=0.4\textwidth]{fig/taPrefix00.png}}
\hspace{0.05\textwidth}
\subfigure{\includegraphics [width=0.4\textwidth]{fig/taPrefix01.png}}
\end{figure}


\begin{figure}
\subfigure{\includegraphics [width=0.4\textwidth]{fig/taPrefix02.png}}
\hspace{0.05\textwidth}
\subfigure{\includegraphics [width=0.4\textwidth]{fig/taSKIP.png}}
\end{figure}

\begin{figure}%[H]
\centering
\includegraphics [width=0.6\textwidth]{fig/Env.png}
%\caption{TAenv, a TA for an explicit environment of the resulting UPPAAL models}
\label{ta_env}
\end{figure}



% \begin{figure} %[H]
% \centering
% \includegraphics [width=0.4\textwidth]{fig/taPrefix00.png}
% \caption{TA1, a TA for the translation of the event \lstinline{open} in the process ADS.}
% \label{ta1}
% \end{figure}


% \begin{figure}%[H]
% \centering
% \includegraphics [width=0.4\textwidth]{fig/taPrefix01.png}
% \caption{TA2, a TA for the translation of the event \lstinline{tock} in the process ADS.}
% \label{ta2}
% \end{figure}

% \begin{figure}%[H]
% \centering
% \includegraphics [width=0.4\textwidth]{fig/taPrefix02.png}
% \caption{TA3, a TA for the translation of the event \lstinline{close} in the process ADS.}
% \label{ta3}
% \end{figure}

% \begin{figure}%[H]
% \centering
% \includegraphics [width=0.4\textwidth]{fig/taSKIP.png}
% \caption{TA4, a TA for the translation of the termination event \lstinline{tick} in the process ADS.}
% \label{ta4}
% \end{figure}



% \begin{figure}%[H]
% \centering
% \includegraphics [width=0.6\textwidth]{fig/Env.png}
% \caption{TAenv, a TA for an explicit environment of the resulting UPPAAL models}
% \label{ta_env}
% \end{figure}

\end{example}

%The process ADS is translated into a list containing 5 TA. 


The above list of network TA in Figures \ref{ta1}, \ref{ta2}, \ref{ta3} and \ref{ta4} expresses the behaviour of the original tock-CSP process. Where Figure \ref{ta1} captures the occurrence of the event \lstinline{open}. Figure \ref{ta2} captures the occurrence of the event \lstinline{tock}. Figure \ref{ta3} captures the occurrence of the event \lstinline{close}. And Figure \ref{ta4} captures of the occurrence of the event \lstinline{tick}. Finally, Figure \ref{ta_env} environment TA provides separate transitions for each co-actions of all the event in the original tock-CSP process, that is \lstinline{open}, \lstinline{tock}, \lstinline{close} and \lstinline{tick}.



% ?????  To remove in the short version  -------   Begin

% Also in Example \ref{ads}, the coordinating actions link the list of the translated TA into a network of TA as follows. The first coordinating flow action \lstinline{startIDADS!} links the environment TA in \ref{ta_env} with the first TA in \ref{ta1} through its co-action \lstinline{startIDADS?}. The second flow action \lstinline{startID1!} links the first TA with the second TA \ref{ta2} through its co-action  \lstinline{startID2!}. The third flow action links the second TA with the third TA \ref{ta3} through its co-action \lstinline{startID2?}. The fourth flow action \lstinline{startID3!} links the third TA \ref{ta3} with the fourth TA  \ref{ta4} through its co-action \lstinline{startID3?}. Finally, the terminating action links the fourth TA \ref{ta4} with the environment TA \ref{ta_env} to complete the links that connect the list of the translated TA into a network of TA, which expresses the behaviour the original tock-CSP process ADS.


% The behaviour of the translated TA begins with the first flow action that activates the first TA in \lstinline{startIDADS?} and then proceed to performs the action \lstinline{open?} with the cooperation of the environment TA in \ref{ta_env} through its co-action \lstinline{open?}.  Then, TA in \ref{ta1} performs the next coordinating flow action \lstinline{startID1!}, which activates the second TA in \ref{ta2} and then proceeds to perform the time action \lstinline{tock!} at least once, also with the cooperation of the environment TA. And then the second TA in  \ref{ta2} proceeds to performs the next coordinating action \lstinline{startID2!} to activate the third TA in \ref{ta4}, which synchronises with the corresponding co-action \lstinline{startID2?}.  The third TA in \ref{ta4} proceeds to perform the action \lstinline{close!} with the co-action \lstinline{close?} from the environment, and then also performs  the next coordination action \lstinline{startID3!} to activate the last TA in \ref{ta4}. The last TA proceeds to perform the action \lstinline{tick!} with the corresponding co-action \lstinline{tick?} from the environment TA \ref{ta_env}, and then also immediately performs the final coordination action \lstinline{finishID0!}, with the corresponding co-action \lstinline{finishID?}, which records a successful termination of the whole process. This describes the behaviour of the translated networked TA.



% As already discussed, each event in the tock-CSP specification is translated into a pair action (with !) and co-action (with ?). This is illustrated in Example \ref{ads}, specifically in the translation of the event \lstinline{open} into action \lstinline{open!} in \ref{ta1} and the corresponding co-action \lstinline{open?} in \ref{ta_env}. Also, this is similar to the translation of the remaining two events \lstinline{close} and \lstinline{tick} in \ref{ta3} and \ref{ta4} respectively, as well as their corresponding co-actions in \ref{ta_env}. This is the strategy we develop for translating each event except in the cases of two types of events, event \lstinline{tock} and multi-synchronisation event.




% In the case of event \lstinline{tock}, the environment controls the progress of time. Therefore, the environment communicates the progress of time using a broadcast action \lstinline{tock!}, and all other TA synchronises with their co-action \lstinline{tock?} to record the progress of time. 

% While in the case of multi-synchronisation event, we adopt the strategy developed in \cite{O05, F05}, where we provide a separate synchronisation TA Definition \ref{dfn_syncTA} for coordinating multi-synchronisation events. The synchronisation TA in \lstinline{syncTA} communicates multi-synchronisation action by broadcasting action \lstinline{sync_action!} and then all the required TA synchronise with their co-action \lstinline{sync_action?}.  To ensure that each TA synchronises correctly, we used an additional guard to block each multi-synchronisation action until all the required participating TA becomes ready for the synchronisation. Then the guard enables the multi-synchronisation action. Additional details of controlling multi-synchronisation action will be discussed in Section \ref{rules}.


% %In conclusion, it is easy to see that from Example \ref{ads} 
% From Example \ref{ads}, it is clear that each TA captures a translation of one event from the input tock-CSP specification. In \ref{ta1}, TA1 captures the translation of the event \lstinline{open}.  In \ref{ta2}, TA2 captures the translation of the event \lstinline{tock}.  In \ref{ta3}, TA3 captures the translation of the event \lstinline{close}.  Lastly, in \ref{ta4} TA4 captures the translation the basic process \lstinline{SKIP}.  

% We follow this strategy in developing the translation rules. Each translation rules translates one construct into TA, in such a way that the translated TA form a network of TA that express the behaviour of the original tock-CSP process. In the next section, we will discuss the translation rules in details.


% ?????  To remove in the short version  -------   End

==> zz_del/a4_Rules.tex <==
% ????Update this??? 
Here we describe the translation rules. We provide a sample of the translation rules  with a  structure of a rule for translating operator of generallised parallel (concurrency).  Details of the complete list of the translation rules together with examples are available in \cite{extendedVersion}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We develop the translation technique as a function \verb!transTA!, which defines the translation of each of the BNF's constructs into TA.


 \vspace{0.2cm}
\begin{tcolorbox} %[title=Title]
\begin{definition} \textbf{Type of Function \lstinline{transTA}}
\label{dfn_transTA}
\end{definition}
\tcblower
\begin{verbatim}
transTA :: CSPproc -> ProcName  -> BranchID -> StartID ->
          FinishID -> UsedNames -> ([TA], [SyncAction])
\end{verbatim}
\end{tcolorbox}



%  \vspace{0.2cm}
% \begin{tcolorbox} %[title=Title]
% \begin{definition} \textbf{Function \lstinline{transTA}}
% \label{dfn_transTA}
% \end{definition}
% \tcblower
% \vspace{-0.5cm}
% %\begin{verbatim}
% \begin{lstlisting}[language=Haskell, basicstyle=\ttfamily, columns=flexible]
% transTA :: CSPproc -> ProcName  -> BranchID -> StartID ->
%           FinishID -> UsedNames -> ([TA], [Event], [SyncPoint])
% \end{lstlisting}
% \end{tcolorbox}


% \vspace{0.5cm}
% \begin{tcolorbox} %[title=Title]
% \begin{definition} \textbf{Function \lstinline{transTA}}
% \label{dfn_transTA}
% \end{definition}
% \tcblower
% %\begin{verbatim}
% \begin{lstlisting}[mathescape, language=Haskell, basicstyle=\ttfamily, columns=flexible]
% transTA :: CSPproc  -> ProcName  -> BranchID -> StartID ->
%           FinishID -> UsedNames -> ([TA], [Event], [SyncPoint])
% \end{lstlisting}
% %\end{verbatim}
% \end{tcolorbox}


 The function \verb!transTA! has 6 parameters. The type of the parameters are \verb!CSPproc!, \verb!ProcName!, \verb!BranchID!, \verb!StartID!, \verb!FinishID! and \verb!UsedNames!. The first parameter of type \verb!CSPproc! is the input CSP process to be translated. The second parameter is a name for the process, of type \verb!ProcName!. While the third and fourth parameter are of type \verb!BranchID! and \verb!StartID!. Fifth parameter of type \verb!FinishID!, is a termination ID, as defined in the coordination action \ref{coordinating_action}. Last parameter of type \verb!UsedNames! is a collection of names, which we used in defining the translation function, mainly for passing translation information from one recursive call to another. 


% We use the two parameters to to generate an identifier for each small TA in the list of the output TA. In generating the identifiers, we consider the structure of binary tree for the AST of the input process, which has branch and depth. So a combination of these two parameters branch and depth identifies a position of each TA in the list of the output TA. Fifth parameter of type \verb!FinishID!, is a termination ID, as defined in the coordination action \ref{}. Last parameter of type \verb!UsedNames! is a collection of names, which we used in defining the translation function, mainly for passing translation information from one recursive call to another. 
% We will explain the purpose of these names as we introduce them in the translation rules. The first 3 parameters \verb!ProcName!, \verb!BranchID! and \verb!StartID! are essential for each translation rule. 


% The function \verb!transTA! has six parameters: input tock-CSP process, process name, list of branch identifiers for the translated TA, list of start identifiers for the translated TA, list of finish identifiers for the translated TA and list of names we used in defining the translation function. 

The output of the function is pairs: a list of translated TA, and a list of synchronisation actions. From the BNF of UPPAAL \cite{LP97}, the key elements of the output TA are the definition of TA itself and the definition of its components:  \verb!Locations!, \verb!Transitions! and the corresponding definitions of their \verb!Labels!. These are expressed in the following Definition \ref{dfn_tastr} as Haskell data-type. 


% The output of the function \verb!transTA! is a tuple containing 3 elements. The first element is a list of small TA that captures the behaviour of the input tock-CSP process. Here, we define TA in the following Definition \ref{dfn_TA}, which is an extract from the complete AST of TA that is provided in Appendix \ref{TA_AST}. The remaining two elements, second and third are used for translating multi-synchronisation. Details explanation of these two elements will come in discussing a translation of generallised parallel operator, where we are going to discuss multi-synchronisation.




 \vspace{0.2cm}
\begin{tcolorbox} %[title=Title]
\begin{definition} \textbf{Type of TA and its components} 
\label{dfn_tastr}
\end{definition}
\tcblower
\begin{verbatim}
data TA = TA Name        [Parameter] [Declaration] 
             [Location]  Init        [Transition]

data Location   = Location   ID     Name   Label   LocType
data Transition = Transition Source Target [Label]
data Label      = EmptyLabel 
                | Invariant  Expression 
                | Guard      Expression 
                | Update     [Expression] 
                | Sync       Identifier   Direction
\end{verbatim}
\end{tcolorbox}


% \vspace{0.5cm}
% \begin{tcolorbox} %[title=Title]
% \begin{definition} \textbf{TA}  %   {Data definition of TA}
% \label{dfn_TA}
% \end{definition}
% \tcblower
% \begin{verbatim}
% data TA = 
%  TA Name [Parameter] [Declaration] [Location] Init [Transition]
% \end{verbatim}
% \end{tcolorbox}


% \vspace{0.5cm}
% \begin{tcolorbox} %[title=Title]
% \begin{definition} \textbf{TA}  %   {Data definition of TA} 
% \label{dfn_TA}
% \end{definition}
% \tcblower
% %\begin{verbatim}
% \begin{lstlisting}[mathescape, language=Haskell, basicstyle=\ttfamily, columns=flexible] 
% data TA = 
%  TA Name [Parameter] [Declaration] [Location] Init [Transition]
% \end{lstlisting}
% %\end{verbatim}
% \end{tcolorbox}
%data TA = TA Name [Parameter] [Declaration] [Location] [Branchpoint]  
%         Init [Transition]


% TODO: shorter form of the following paragraphs?

%Definition \ref{dfn_TA} is provides a
In Definition \ref{dfn_tastr}, the type \verb!TA! has a constructor \verb!TA! with six parameters. The first parameter of type \verb!Name! is an identifier for the TA itself.  The second parameter of type \verb!Parameter! is a list of arguments for the TA. The third parameter of type \verb!Declaration! is a list of local definitions inside the TA.  The fourth parameter of type \verb!Location! is a list of locations in the TA, which is defined in Definition \ref{dfn_tastr}. The fifth parameter of type \verb!Init! is an initial location of the TA. The last parameter of type \verb!Transitions! is a list of transitions that connect the locations of the TA, also defined in Definition \ref{dfn_tastr}.   


% ??? todo: what’s the difference between an identifier and a tag? explain that the distinction comes from UPPAAL.

% \vspace{0.5cm}
% \begin{tcolorbox} %[title=Title]
% \begin{definition} \textbf{Location} 
% \label{dfn_location}
% \end{definition}
% \tcblower
% %\begin{lstlisting}[mathescape, language=Haskell, basicstyle=\ttfamily, columns=flexible]
% \begin{verbatim}
% data Location = Location ID Name Label LocType
% \end{verbatim}
% % \end{lstlisting}
% \end{tcolorbox}


Also, in Definition \ref{dfn_tastr}, the type \verb!Location! has a constructor that has four parameters of types \verb!ID, Name, Label and LocType!.  \verb!ID! is an identifier for the location. \verb!Name! is a tag that provides visual description of a location. Third parameter of type \verb!Label! is a constraint label for the location as defined in Definition \ref{dfn_tastr}. Last parameter of type \verb!LocType! is a format of the location, which can be one of these three: \verb!urgent!, \verb!committed!, \verb!none! (which means normal location that is neither urgent nor committed). 





% \vspace{0.5cm}
% \begin{tcolorbox} %[title=Title]
% \begin{definition} \textbf{Transition} 
% \label{dfn_transition}
% \end{definition}
% \tcblower
% \begin{verbatim}
% data Transition = Transition Source Target [Label]
% \end{verbatim}
% \end{tcolorbox}

Similarly, the type \verb!Transition! has a constructor \verb!Transition! that has three parameters, two parameters of type Location for both source and target location of a transition. The third parameter of type \verb!Label! provides a label for a transition. Both location and transition have label, which can be empty (for a silent transition), invariant, guard, update and synchronisation action or combinations of them, as defined in Definition \ref{dfn_tastr}.  

% \vspace{0.5cm}
% \begin{tcolorbox} %[title=Title]
% \begin{definition} \textbf{Label} 
% \label{dfn_label}
% \end{definition}
% \tcblower
% \begin{verbatim}
% data Label = EmptyLabel 
%           | Invariant     Expression 
%           | Guard         Expression 
%           | Update       [Expression] 
%           | Sync          Identifier   Direction
% \end{verbatim}
% \end{tcolorbox}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Translation of Constant process STOP}
% Rule \ref{rule_STOP}  describes a translation of constant process \lstinline{STOP}.
% % This section provides a rule for the translation of a constant process \lstinline{STOP} in Rule \ref{rule_STOP}.

% \begin{tcolorbox} %[title=Title]
% \begin{trule} \textbf{Translation of STOP}
% \label{rule_STOP}
% \end{trule}
% \tcblower
% \begin{Verbatim}[numbers=left,numbersep=7pt, fontsize=\small]
% transTA STOP processName bid sid _ _ _ =
%     (([(TA idTA [] [] locs [] (Init loc1) trans)]), [], [] )
%     where 
%       idTA = "taSTOP__" ++ bid ++ show sid
        
%       --   = Location ID      Name    Label       LocType
%       loc1 = Location "id1"   "s1"    EmptyLabel  None
%       loc2 = Location "id2"   "s2"    EmptyLabel  None
%       locs = [loc1, loc2]

%       --    = Transition Source   Target  [Label] 
%       tran1 = Transition loc1     loc2    [lab1]  
%       tran2 = Transition loc2     loc2    [lab2] 
%       trans = [tran1, tran2]

%       lab1 = Sync 
%                 (VariableID (startEvent processName (bid ++ sid)) [])
%                 Ques
%       lab2 = Sync (VariableID "tock" []) Ques     
% \end{Verbatim}

% \end{tcolorbox}


% \begin{tcolorbox} %[title=Title]
% \begin{trule} \textbf{Translation of STOP}
% \label{rule_STOP}
% \end{trule}
% \tcblower
% \vspace{-0.5cm}
% \begin{lstlisting}[language=Haskell, basicstyle=\ttfamily, columns=flexible]
% transTA STOP processName bid sid _ _ _ =
%      (([(TA idTA [] [] locs [] (Init loc1) trans)]), [], [] )
%      where 
%         idTA = "taSTOP__" ++ bid ++ show sid
        
%         --   = Location ID      Name    Label       LocType
%         loc1 = Location "id1"   "s1"    EmptyLabel  None
%         loc2 = Location "id2"   "s2"    EmptyLabel  None
%         locs = [loc1, loc2]

%         --    = Transition Source   Target  [Label] [Edge]
%         tran1 = Transition loc1     loc2    [lab1]  []
%         tran2 = Transition loc2     loc2    [lab2]  []
%         trans = [tran1, tran2]

%         lab1 = Sync 
%                  (VariableID 
%                   (startEvent processName (bid ++ sid)) [])
%                  Ques
%         lab2 = Sync (VariableID "tock" []) Ques     
% \end{lstlisting}
% \end{tcolorbox}



% \subsubsection{Translation of Construct for Internal choice}
% This section provides a rule for the translation of a construct for internal choice in Rule \ref{rule_IntCh}.


% \vspace{0.5cm}
% \begin{tcolorbox} %[title=Title]
% \begin{trule} \textbf{Translation of Internal Choice}
% \label{rule_IntCh}
% \end{trule}
% \tcblower
% \begin{Verbatim}[numbers=left,numbersep=7pt, fontsize=\small]
% transTA (IntChoice p1 p2) procName bid sid fid usedNames =  
%   ([(TA idTA [] [] locs [] (Init loc1) trans )] ++ ta1 ++ ta2, 
%       (sync1 ++ sync2), (syncMap1 ++ syncMap2) )
%   where 
%       idTA  = "taIntCho" ++ bid ++ show sid
      
%       loc1 = Location "id1" "s1" EmptyLabel None
%       loc2 = Location "id2" "s2" EmptyLabel CommittedLoc
%       loc3 = Location "id3" "s3" EmptyLabel CommittedLoc
%       loc4 = Location "id4" "s4" EmptyLabel CommittedLoc
%       locs = [loc1, loc2, loc3, loc4]

%       tran1 = Transition loc1 loc2 [lab1] 
%       tran2 = Transition loc2 loc3 []     
%       tran3 = Transition loc2 loc4 []     
%       tran4 = Transition loc3 loc1 [lab4]                                        
%       tran5 = Transition loc4 loc1 [lab5]                                        
%       trans = [tran1, tran2, tran3, tran4, tran5]

%       lab1 = Sync (VariableID (startEvent procName bid sid) [])
%                   Ques
%       lab4 = Sync (VariableID ("startID" ++ (bid ++ "0") ++ 
%                                 show (sid+1)) []) 
%                   Excl 
%       lab5 = Sync (VariableID ("startID" ++ (bid ++ "1") ++ 
%                                 show (sid+2)) []) Excl
        
%       (ta1, sync1, syncMap1) = 
%             transTA p1 [] (bid ++ "0") (sid+1) fid usedNames
%       (ta2, sync2, syncMap2) = 
%             transTA p2 [] (bid ++ "1") (sid+2) fid usedNames

% \end{Verbatim}
% \end{tcolorbox}



\subsubsection{Translation of Construct for Generalised Parallel}
The following Rule \ref{rule_GenPar} provides a structure of a rule for translating a construct for generalised parallel.
% This rule works with another definition for synchronisation controller which handles multi-synchronisation as defined in Definition \ref{dfn_syncTA}.

\vspace{0.5cm}
\begin{tcolorbox} %[title=Title]
\begin{trule} \textbf{Translation of Generalised Parallel}
\label{rule_GenPar}
\end{trule}
\tcblower
\begin{Verbatim}[numbers=left,numbersep=7pt, fontsize=\small]
transTA (GenPar P1 P2 es) procName bid sid fid usedNames = 
    ([(TA idTA [] [] locs [] (Init loc1) trans )] ++ ta1 ++ ta2, 
    (es ++ sync1 ++ sync2) )
    where
      idTA   = "taGenPar" ++ bid ++ show sid
      loc1   = Location  "id1" "s1" EmptyLabel None
      ...
      -- Definitions of the remaining seven locations follow in 
      -- the same pattern
     
      tran1  = Transition loc1 loc2 [lab1] 
      ...
      -- Definitions of the remaining nine transitions follow in 
      -- the same pattern.                      
      
      lab1 = Sync (VariableID (startEvent procName bid sid) []) Ques
      ...
      -- Definitions of the remaining five labels follow in 
      -- the same pattern.                       

      (syncEv, syncPoint, hide, rename, exChs, intrr, iniIntrr,  
               excps) = usedNames 
      syncEv'    = es ++ syncEv               -- Update synch names
      usedNames' = (syncEv', syncPoint, hide, rename, exChs, intrr, 
                    iniIntrr, excps)
      (ta1, sync1, syncMap1) = 
               transTA P1 [] (bid ++ "0") (sid+1) (fid+1) usedNames'
      (ta2, sync2, syncMap2) = 
               transTA P2 [] (bid ++ "1") (sid+2) (fid+2) usedNames'
\end{Verbatim}
\end{tcolorbox}


Details of Rule \ref{rule_GenPar} is as follows. Line 1 defines the function \verb!transTA! for translating the operator generallised parallel. Lines 2-3 defines the output of the function \verb!transTA!, that is a pair containing two elements. First is a definition of the translated TA concatenated with \verb!ta1! and \verb!ta2!, list of TA for the translation of the two concurrent processes  \verb!P1! and \verb!P2!, respectively (defined subsequently in Line 26 and 28). Second, list of synchronisation action for constructing synchronisation controller. Line 5 defines an identifier for the output TA. Line 6 defines the first location of the TA. Omitted definition of the remaining seven locations follow in the same pattern. Line 11 defines the first transition of the TA. Similarly, omitted definitions of the remaining nine transitions follow in the same pattern. Line 16 defines a label for the first transition. Definitions of the remaining five labels follow in the same pattern. There are five labels because four pairs of the transitions use similar label. Line 21 extracts the synchronisation name from the used names \verb!usedName!. Line 23 updates the synchronisation names with additional synchronisation actions \verb!es! for the translated operator. Line 24 updates the used names \verb!usedNames'! for subsequent translations. Line 26--29 defines two recursive calls for the function \verb!transTA! that translate the concurrent processes \verb!P1! and \verb!P2!.


A sample output TA of this translation rule can be seen in Example \ref{ads}, that is the first TA in the list of the translated TA (top left).


% \vspace{0.5cm}
% \begin{tcolorbox} %[title=Title]
% \begin{trule} \textbf{Translation of Generalised Parallel}
% \label{rule_GenPar}
% \end{trule}
% \tcblower
% \begin{Verbatim}[numbers=left,numbersep=7pt, fontsize=\small]
% transTA (GenPar p1 p2 es) procName bid sid fid usedNames = 
%     ([(TA idTA [] [] locs [] (Init loc1) trans )] ++ ta1 ++ ta2, 
%     (es ++ sync1 ++ sync2), (syncMap1 ++ syncMap2) )
%     where
%       idTA   = "taGenPar" ++ bid ++ show sid
%       loc1   = Location  "id1" "s1" EmptyLabel None
%       loc2   = Location  "id2" "s2" EmptyLabel CommittedLoc
%       loc3   = Location  "id3" "s3" EmptyLabel CommittedLoc
%       loc4   = Location  "id4" "s4" EmptyLabel CommittedLoc
%       loc5   = Location  "id5" "s5" EmptyLabel None
%       loc6   = Location  "id6" "s6" EmptyLabel None
%       loc7   = Location  "id7" "s7" EmptyLabel None
%       loc8   = Location  "id8" "s8" EmptyLabel CommittedLoc
%       locs   = [loc1, loc2, loc3, loc4, loc5, loc6, loc7, loc8]
%       tran1  = Transition loc1 loc2 [lab1] 
%       tran2  = Transition loc2 loc3 [lab3] 
%       tran3  = Transition loc3 loc5 [lab2] 
%       tran4  = Transition loc2 loc4 [lab2] 
%       tran5  = Transition loc4 loc5 [lab3] 
%       tran6  = Transition loc5 loc6 [lab4]                                    
%       tran7  = Transition loc5 loc7 [lab5]  
%       tran8  = Transition loc6 loc8 [lab5]  
%       tran9  = Transition loc7 loc8 [lab4]  
%       tran10 = Transition loc8 loc1 [lab6]                                  
%       trans  = [tran1, tran2, tran3, tran4, tran5, 
%                 tran6, tran7, tran8, tran9, tran10]
%       lab1 = Sync (VariableID (startEvent procName bid sid) []) Ques
%       lab2 = Sync (VariableID ("startID" ++ (bid ++ "0") ++
%                                 show (sid+1              )) []) Excl 
%       lab3 = Sync (VariableID ("startID" ++ (bid ++ "1") ++ 
%                                 show (sid+2              )) []) Excl 
%       lab4 = Sync (VariableID ("finishID" ++ show (fid+1 )) []) Ques
%       lab5 = Sync (VariableID ("finishID" ++ show (fid+2 )) []) Ques
%       lab6 = Sync (VariableID ("finishID" ++ show  fid    ) []) Excl 

%       (syncEv, syncPoint, hide, rename, exChs, intrr, iniIntrr,  
%               excps) = usedNames 
%       syncEv'    = es ++ syncEv               -- Update synch name
%       usedNames' = (syncEv', syncPoint, hide, rename, exChs, intrr, 
%                     iniIntrr, excps)
%       (ta1, sync1, syncMap1) = 
%               transTA p1 [] (bid ++ "0") (sid+1) (fid+1) usedNames'
%       (ta2, sync2, syncMap2) = 
%               transTA p2 [] (bid ++ "1") (sid+2) (fid+2) usedNames'
% \end{Verbatim}
% \end{tcolorbox}

% \vspace{0.5cm}
% \begin{tcolorbox} %[title=Title]
% \begin{trule} \textbf{Translation of Generalised Parallel}
% \label{rule_GenPar}
% \end{trule}
% \tcblower
% \vspace{-0.5cm}
% \begin{lstlisting}[language=Haskell, basicstyle=\ttfamily, columns=flexible]
% transTA (GenPar p1 p2 es) procName bid sid fid usedNames = 
%     ([(TA idTA [] [] locs [] (Init loc1) trans )] ++ ta1 ++ ta2, 
%     (es ++ sync1 ++ sync2), (syncMap1 ++ syncMap2) )
%     where
%       idTA   = "taGenPar" ++ bid ++ show sid
%       loc1   = Location  "id1" "s1" EmptyLabel None
%       loc2   = Location  "id2" "s2" EmptyLabel CommittedLoc
%       loc3   = Location  "id3" "s3" EmptyLabel CommittedLoc
%       loc4   = Location  "id4" "s4" EmptyLabel CommittedLoc
%       loc5   = Location  "id5" "s5" EmptyLabel None
%       loc6   = Location  "id6" "s6" EmptyLabel None
%       loc7   = Location  "id7" "s7" EmptyLabel None
%       loc8   = Location  "id8" "s8" EmptyLabel CommittedLoc
%       locs   = [loc1, loc2, loc3, loc4, loc5, loc6, loc7, loc8]
%       tran1  = Transition loc1 loc2 [lab1] []
%       tran2  = Transition loc2 loc3 [lab3] [] 
%       tran3  = Transition loc3 loc5 [lab2] []
%       tran4  = Transition loc2 loc4 [lab2] []
%       tran5  = Transition loc4 loc5 [lab3] []
%       tran6  = Transition loc5 loc6 [lab4] []                                   
%       tran7  = Transition loc5 loc7 [lab5] [] 
%       tran8  = Transition loc6 loc8 [lab5] [] 
%       tran9  = Transition loc7 loc8 [lab4] [] 
%       tran10 = Transition loc8 loc1 [lab6] []                                 
%       trans  = [tran1, tran2, tran3, tran4, tran5, 
%                 tran6, tran7, tran8, tran9, tran10]
%       lab1 = Sync (VariableID (startEvent procName bid sid) []) Ques
%       lab2 = Sync (VariableID ("startID" ++ (bid ++ "0") ++
%                                 show (sid+1              )) []) Excl 
%       lab3 = Sync (VariableID ("startID" ++ (bid ++ "1") ++ 
%                                 show (sid+2              )) []) Excl 
%       lab4 = Sync (VariableID ("finishID" ++ show (fid+1 )) []) Ques
%       lab5 = Sync (VariableID ("finishID" ++ show (fid+2 )) []) Ques
%       lab6 = Sync (VariableID ("finishID" ++ show  fid    ) []) Excl 

%       (syncEv, syncPoint, hide, rename, exChs, intrr, iniIntrr,  
%               excps) = usedNames 
%       syncEv'    = es ++ syncEv               -- Update synch name
%       usedNames' = (syncEv', syncPoint, hide, rename, exChs, intrr, 
%                     iniIntrr, excps)
%       (ta1, sync1, syncMap1) = 
%               transTA p1 [] (bid ++ "0") (sid+1) (fid+1) usedNames'
%       (ta2, sync2, syncMap2) = 
%               transTA p2 [] (bid ++ "1") (sid+2) (fid+2) usedNames'
% \end{lstlisting}
% \end{tcolorbox}


% \vspace{0.5cm}
% \begin{tcolorbox} %[title=Title]
% \begin{definition} \textbf{Synchronisation TA}
% \label{dfn_syncTA}
% \end{definition}
% \tcblower
% % -- 4. Generate TA for controlling the synchronisations point
% % -- The definition of "trans" below, adds a prefix "v_" to an event name to form a variable name that each TA increments to register its readiness to sync.
% \begin{Verbatim}[numbers=left,numbersep=7pt, fontsize=\small]
% syncTA :: [Event] -> [SyncPoint] -> Template
% syncTA     events     syncMaps   =  
%     Template "SyncTA" [] [] (loc:locs) [] (Init loc) trans 
%     where 
%       loc  = Location "SyncPoint" "SyncPoint" EmptyLabel None 
%       locs = [(Location ("s"++ show e) ("s"++ show e) EmptyLabel 
%                         CommittedLoc) | e <- uniq events]
%       trans = transGen  loc (uniq events) syncMaps events
                    
%     -- Generates transitions for the sync controller
%     transGen :: Location->[Event]->[SyncPoint]->[Event]->[Transition]
%     transGen    l0        []        _            _     = []
%     transGen    l0        (e:es)   syncMaps     syncs  =  
%         [(Transition 
%           l0 l 
%           (Sync (VariableID (show e) []) Excl),
%           (Guard 
%               (ExpID 
%                 ((addExpr 
%                   [("g_" ++ tag)|(e1, tag) <- syncMaps, e == e1 ]) 
%                   ++ " == " ++  
%                   show ((length [e1 | e1 <- syncs, e == e1 ]) + 1) 
%                 )  )  ), 
%           (Update ([ AssgExp (ExpID ("g_" ++ tag)) 
%                      ASSIGNMENT (Val 0) |(e1, tag) <- syncMaps, 
%                      e == e1] )) ] [])] 
%         ++ [Transition 
%              l l0  
%              [(Sync (VariableID ((show e) ++ "___sync") []) Excl)]
%         ] ++ (transGen l0 es syncMaps syncs)  
%         where
%           l = (Location ("s"++ show e) ("s"++ show e)
%                         EmptyLabel CommittedLoc)
                      
% \end{Verbatim}
% \end{tcolorbox}


%% The remaining translation rules do not fit into the available space for this paper. A complete list of the translation rules together with examples are available in a report of the translation work \cite{extendedVersion}.

% An extended version of the paper \cite{extendedVersion} contains all the translation rules together with examples that illustrate using the rules in translating tock-CSP processes.

% The remaining translation rules do not fit into the available space for this paper. An extended version of the paper \cite{extendedVersion} contains all the translation rules together with examples that illustrate using the rules in translating tock-CSP processes.

==> zz_del/a4_ruleGenPar.tex <==
\subsubsection{Translation of Generalised Parallel Construct}
The following Rule \ref{rule_GenPar} provides a structure of a rule for translating generalised parallel construct.
% This rule works with another definition for synchronisation controller which handles multi-synchronisation as defined in Definition \ref{dfn_syncTA}.

\vspace{0.5cm}
\begin{tcolorbox} %[title=Title]
\begin{trule} \textbf{Translation of Generalised Parallel}
\label{rule_GenPar}
\end{trule}
\tcblower
\begin{Verbatim}[numbers=left,numbersep=7pt, fontsize=\small]
transTA (GenPar P1 P2 es) procName bid sid fid usedNames = 
  ([(TA idTA [] [] locs [] (Init loc1) trans )] ++ ta1 ++ ta2, 
  (es ++ sync1 ++ sync2) )
  where
   idTA   = "taGenPar" ++ bid ++ show sid
   loc1   = Location  "id1" "s1" EmptyLabel None
   ...
   -- Definitions of the remaining seven locations follow 
   -- in the same pattern
 
   tran1  = Transition loc1 loc2 [lab1] 
   ...
   -- Definitions of the remaining nine transitions follow 
   -- in the same pattern.                      
  
   lab1 = Sync (VariableID (startEvent procName bid sid) []) 
                Ques
   ...
   -- Definitions of the remaining five labels follow 
   -- in the same pattern.                       

   (syncEv, syncPoint, hide, rename, exChs, intrr, iniIntrr,  
           excps) = usedNames 
   syncEv'    = es ++ syncEv    -- 
   usedNames' = (syncEv', syncPoint, hide, rename, exChs, 
                intrr, iniIntrr, excps)
   (ta1, sync1, syncMap1) = 
           transTA P1 [] (bid ++ "0") (sid+1) (fid+1)
           usedNames'
   (ta2, sync2, syncMap2) = 
           transTA P2 [] (bid ++ "1") (sid+2) (fid+2) 
           usedNames'
\end{Verbatim}
\end{tcolorbox}


Details of Rule \ref{rule_GenPar} is as follows. Line 1 defines the function \verb!transTA! for translating the operator generallised parallel. Lines 2-3 defines the output of the function \verb!transTA!, that is a pair containing two elements. First is a definition of the translated TA concatenated with \verb!ta1! and \verb!ta2!, list of TA for the translation of the two concurrent processes  \verb!P1! and \verb!P2!, respectively (defined subsequently in Line 26 and 28). Second, list of synchronisation action for constructing synchronisation controller. Line 5 defines an identifier for the output TA. Line 6 defines the first location of the TA. Omitted definition of the remaining seven locations follow in the same pattern. Line 11 defines the first transition of the TA. Similarly, omitted definitions of the remaining nine transitions follow in the same pattern. Line 16 defines a label for the first transition. Definitions of the remaining five labels follow in the same pattern. There are five labels because four pairs of the transitions use similar label. Line 21 extracts the synchronisation name from the used names \verb!usedName!. Line 23 updates the synchronisation names with additional synchronisation actions \verb!es! for the translated operator. Line 24 updates the used names \verb!usedNames'! for subsequent translations. Line 26--29 defines two recursive calls for the function \verb!transTA! that translate the concurrent processes \verb!P1! and \verb!P2!.


A sample output TA of this translation rule can be seen in Example \ref{ads}, that is the first TA in the list of the translated TA (top left).


==> zz_del/a4_ruleStop.tex <==

%%%%%%%%%%%%%%%%%%%%%%% STOP
% \subsubsection{Translation of STOP}

Here, we present a structure of the translation rule using one of the translation rule, which describes the translation of the construct  \verb!STOP!. We begin with presenting a rule for translating STOP and then follow with an example that illustrates using the rule in translating a \verb!tock-CSP! process into TA.


%This section describes a translation of a constant process \lstinline{STOP}. The section begins with presenting a rule for translating STOP and then follows with an example that illustrates using the rule in translating a process.



% \vspace{1cm}
\begin{tcolorbox} %[title=Title]
\begin{trule} \textbf{Translation of STOP}
\label{rule_STOP}
\end{trule}
\tcblower
\begin{Verbatim}[numbers=left,numbersep=7pt]
transTA STOP processName bid sid _ usedNames =
  (([(TA idTA [] [] locs [] (Init loc1) trans)]), [] )
  where 
   idTA = "taSTOP__" ++ bid ++ show sid
   
     --   Definition of locations in the TA  
     -- = Location ID     Name  Label       LocType
   loc1 = Location "id1"  "s1"  EmptyLabel  None
   loc2 = Location "id2"  "s2"  EmptyLabel  None
   locs = [loc1, loc2]

     --    Definition of transitions in the TA 
     --  = Transition Source   Target  [Label] [Edge]
   tran1 = Transition loc1     loc2    [lab1]  []
   tran2 = Transition loc2     loc2    [lab2]  []
   intrp = transIntrpt intrptsInits loc1 loc2        
   trans = [tran1, tran2] ++ intrp

   --  Labels of the transitions in the TA
   lab1 = Sync (VariableID 
            (startEvent processName (bid ++ sid)) []) 
             Ques
   lab2 = Sync (VariableID "tock" []) Ques     

   -- Get the initial events of an interrupting process
   (_, _, _, _, _, intrptsInits, _, _) = usedNames

\end{Verbatim}

\end{tcolorbox}

% %%% Previous description
% %\pagebreak
% \vspace{0.3cm}
% \begin{trule} Translation of Deadlock
% \begin{lstlisting}[mathescape, firstnumber=last]
% transTA STOP processName _ startID _ _ =
%    [ 
% \end{lstlisting}
% \begin{figure}[H]
% \centering
% \includegraphics [width=0.4\textwidth]{newImg/trule_stop.png}
% \end{figure}
% \begin{lstlisting}[mathescape, firstnumber=last]
%    ]
% where
%  startEvent = startEvent processName startID
        
% \end{lstlisting}
% \label{trule_STOP}
% \end{trule} 



\begin{figure}[H]
\centering
\includegraphics [width=0.5\textwidth]{figGray/stopMap.png}
 \caption{A structure of an output TA for the translation of STOP.}
\label{STOP_map}
\end{figure}




Rule \ref{rule_STOP} expresses the translation of the construct \verb!STOP!, which produces an output TA that is depicted in Figure \ref{STOP_map}.The structure of the output TA that has 2 locations and 2 transitions as defined in Rule \ref{rule_STOP}, Lines 7--9 and Lines 11--13, respectively. For conciseness, in Figure \ref{STOP_map}, we map the structure of the TA with the names used in the translation rule. The names are \lstinline{loc1, loc2, tran1, tran2, intrpt} 


Detail description of Rule \ref{rule_STOP} is as follow. Starting from the beginning of the translation rule, Line 1 provides a definition of the translation function \lstinline{transTA} for translating the construct \lstinline{STOP} and the four essential parameters for translating the construct \verb!STOP!, \lstinline{processName}, \lstinline{bid} and \lstinline{sid}. While the symbol underscore represents unused arguments for this translation rule. In Haskell, the symbol of underscore indicates a position of unused arguments. For conciseness, we use the underscore to omit unused arguments and provide only the required arguments for each translation rule. 


Line 2 defines the output pairs, a list of output TA and a list of synchronising action. Starting with the simple one, the second element that is empty ([]) because there is no synchronising action in translating the construct \verb!STOP!. The first element is a definition of the output TA (Definition \ref{dfn_TA}) for translating the constant process \verb!STOP!, which has 6 parameters. First, \lstinline{idTA} is an identifier for the TA, which is define subsequently in Line 4, as concatenation of the keyword \lstinline{"taSTOP__"} with the 2nd and 3rd arguments of the function \lstinline{transTA}, that is \lstinline{bid} and \lstinline{sid} respectively. Additionally, still in Line 2, in the definition of the output TA, the 2nd, 3rd and 5th parameters are empty for the output TA. While the 4th parameter \lstinline{locs} is a list of locations for the output TA defined in Lines 7--9. The 6th parameter \lstinline{(Init loc1)} specifies \lstinline{loc1} as the initial location of the output TA. Last parameter \lstinline{trans} describes a list of transitions that connect the locations of the TA, as defined in line 12--13. Line 14 defines interrupting transitions that are generated with the function \verb!transIntrpt!, that is in the case where a process is compose with an interrupting process. Lines 17--20 define the labels of the transitions. Lastly, Line 23 extracts the initials of an interrupting process from the parameter \verb!usedNames!, which collects information about the translation function, as described in Definition \ref{dfn_transTA}.



The behaviour of the output TA begins with the first flow action (Define in Line 17). After that, the TA performs the action \lstinline{tock} (line 18), repeatedly, which allows the progress of time, unless if their is an interrupt, which causes the TA to follow the interrupting transition (Defined in Line 14). An illustration of using this translation rule in translating a process is shown in Example \ref{ex_STOP}.




\vspace{0.3cm}
\begin{example} An example of translating a process \verb!STOP! that produces a list of TA, which contains two TA as shown in Figure \ref{stop_ta1} and \ref{stop_ta2}, as illustrated below.
\label{ex_STOP}
\begin{lstlisting}[mathescape, firstnumber=last]
transTA STOP "p0_1" 1 0 ([], [], [], [], [], [], [], ([],[])) =
        [ 
\end{lstlisting}
\begin{figure}[H]
\centering
\includegraphics [width=0.5\textwidth]{figGray/STOP_T0.png}
%1 \caption{A small TA for the translation of the process STOP.}
\label{stop_ta1}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics [width=0.5\textwidth]{figGray/STOP_env.png}
%1 \caption{Environment TA for the translation of the process STOP.}
\label{stop_ta2}
\end{figure}

\lstinline{  ]}
\end{example}


Example \ref{ex_STOP} demonstrates using Rule \ref{rule_STOP} in translating the process  \verb!STOP!  which produces two TA, a small TA and its corresponding environment TA, as shown in Figure \ref{stop_ta1}. The behaviour of the output TA begins with the environment TA that initiates its first flow action \lstinline{startID00!} with the cooperation of its co-action from the small TA \lstinline{startID00?}. Then, the small TA cooperates in performing the event \lstinline{tock} to record the progress of time, and remains in the same location \lstinline{s2}, deadlock. In short, the behaviour of the translated TA for the constant process \lstinline{STOP} causes a deadlock behaviour in location \verb!s2!.

==> zz_del/a4_ruleStopNew.tex <==
An example of the formalisation of the translation rules in Haskell is provided in Rule 1, which describes the translation of the construct  \verb!STOP!. All the remaining rules can be found in \cite{extendedVersion}. Rule \ref{rule_STOP} produces an output TA that is depicted in Figure \ref{STOP_map}, which has two locations and two transitions as defined in Rule \ref{rule_STOP}, Lines 7--9 and Lines 11--13, respectively. In Figure \ref{STOP_map}, we map the structure of the TA with the names used in the translation rule. The names are \lstinline{loc1, loc2, tran1, tran2, intrpt}. 


A detailed description of Rule \ref{rule_STOP} is as follows. Each rule considers one construct. Line 1 identifies that this a definition of the translation function \lstinline{transTA} for translating the construct \lstinline{STOP}, and it takes three extra parameters: \lstinline{processName}, \lstinline{bid} and \lstinline{sid}. The symbol underscore \footnote{In Haskell, the symbol of underscore indicates a position of unused arguments. For conciseness, we use the underscore to omit unused arguments and provide only the required arguments for each translation rule.} represents unused arguments for this translation rule.







% \vspace{1cm}
\begin{figure}
    \centering

\begin{tcolorbox} %[title=Title]
\begin{trule} \textbf{Translation of STOP}
\label{rule_STOP}
\end{trule}
\tcblower
\begin{Verbatim}[numbers=left,numbersep=7pt]
transTA STOP processName bid sid _ usedNames =
  (([(TA idTA [] [] locs [] (Init loc1) trans)]), [] )
  where 
   idTA = "taSTOP__" ++ bid ++ show sid
   
     --   Definition of locations in the TA  
     -- = Location ID     Name  Label       LocType
   loc1 = Location "id1"  "s0"  EmptyLabel  None
   loc2 = Location "id2"  "s1"  EmptyLabel  None
   locs = [loc1, loc2]

     --    Definition of transitions in the TA 
     --  = Transition Source   Target  [Label] [Edge]
   tran1 = Transition loc1     loc2    [lab1]  []
   tran2 = Transition loc2     loc2    [lab2]  []
   intrp = transIntrpt intrptsInits loc1 loc2        
   trans = [tran1, tran2] ++ intrp

   --  Labels of the transitions in the TA
   lab1 = Sync (VariableID 
            (startEvent processName (bid ++ sid)) []) 
             Ques
   lab2 = Sync (VariableID "tock" []) Ques     

   -- Get the initial events of an interrupting process
   (_, _, _, _, _, intrptsInits, _, _) = usedNames

\end{Verbatim}

\end{tcolorbox}

    % \includegraphics{}
    % \caption{Caption}
    % \label{fig:my_label}
\end{figure}
% %%% Previous description
% %\pagebreak
% \vspace{0.3cm}
% \begin{trule} Translation of Deadlock
% \begin{lstlisting}[mathescape, firstnumber=last]
% transTA STOP processName _ startID _ _ =
%    [ 
% \end{lstlisting}
% \begin{figure}[H]
% \centering
% \includegraphics [width=0.4\textwidth]{newImg/trule_stop.png}
% \end{figure}
% \begin{lstlisting}[mathescape, firstnumber=last]
%    ]
% where
%  startEvent = startEvent processName startID
        
% \end{lstlisting}
% \label{trule_STOP}
% \end{trule} 



\begin{figure}[H]
\centering
\includegraphics [width=0.5\textwidth]{figGray/stopMap.png}
 \caption{A structure of an output TA for the translation of STOP.}
\label{STOP_map}
\end{figure}





%%%%%%%%%%%%%%%%%%%%%%% STOP
% \subsubsection{Translation of STOP}


% Here, we present a structure of the translation rule using one of the translation rule, which describes the translation of the construct  \verb!STOP!. We begin with presenting a rule for translating STOP and then follow with an example that illustrates using the rule in translating a \verb!tock-CSP! process into TA.


%This section describes a translation of a constant process \lstinline{STOP}. The section begins with presenting a rule for translating STOP and then follows with an example that illustrates using the rule in translating a process.

?? You need to explain the fun transTA ?? \\

Line 2 defines the output pairs, a list of output TA and a list of synchronising actions. The second element is empty ([]) in Rule 1 because there is no synchronising action in translating the construct \verb!STOP!. The first element describes the output TA, which has 6 parameters. First, \lstinline{idTA} is an identifier for the TA, which is defined subsequently in Line 4, as the concatenation of the keyword \lstinline{"taSTOP__"} with the 2nd and 3rd arguments of the function \lstinline{transTA}, that is \lstinline{bid} and \lstinline{sid} respectively. Additionally, still in Line 2, in the definition of the output TA, the 2nd, 3rd and 5th parameters are empty for the output TA. While the 4th parameter \lstinline{locs} is a list of locations for the output TA, as defined in Lines 7--9. The 6th parameter \lstinline{(Init loc1)} specifies \lstinline{loc1} as the initial location of the output TA. Last parameter \lstinline{trans} describes a list of transitions that connect the locations of the TA, as defined in line 12--13. Line 14 defines interrupting transitions that are generated with the function \verb!transIntrpt!, that is in the case where a process is composed with an interrupting process. Lines 17--20 define the labels of the transitions. Lastly, Line 23 extracts the initials of an interrupting process from the parameter \verb!usedNames!, which collects essential information about the translation function, such as the names of hidden events and renamed events.
%and interrupting events.
%, as described in Definition \ref{dfn_transTA}.



The behaviour of the output TA begins with the first flow action (defined in Line 17). After that, the TA performs the action \lstinline{tock} (line 18), repeatedly, which allows the progress of time, unless there is an interrupt, which causes the TA to follow the interrupting transition (defined in Line 14). 
%ToReturn
% An illustration of using this translation rule in translating a process is shown in Example \ref{ex_STOP}.


%--------------------- EXAMPLE
\vspace{0.3cm}
\begin{example} \label{ex_STOP}
An example of translating a process \verb!STOP! that produces a list of TA, which contains two TA as shown in Figure \ref{stop_ta1}. The left TA captures the translation of the construct $STOP$, in this case there is no interrupting transition because there is no interrupting process. The right TA is the added environment TA.


% \begin{lstlisting}[mathescape, firstnumber=last]
% transTA STOP "p0_1" 1 0 ([], [], [], [], [], [], [], ([],[])) =
%         [ 
% \end{lstlisting}

\begin{lstlisting}[mathescape, firstnumber=last]
transTA(STOP) = [
\end{lstlisting}

\begin{figure}[H]
\subfigure{\includegraphics [width=0.5\textwidth]{figGray/taSTOP.png}}
\subfigure{\includegraphics [width=0.5\textwidth]{figGray/Env1_g.jpg}}
\caption{A list of TA for the translation of the construct STOP}
\label{stop_ta1}
\end{figure}

% \centering
% \includegraphics [width=0.4\textwidth]{figGray/taSTOP1_g.png}
% %1 \caption{A small TA for the translation of the process STOP.}
% % \label{stop_ta1}
% % \end{figure}

% % \begin{figure}[H]
% % \centering
% \includegraphics [width=0.4\textwidth]{figGray/Env1_g.jpg}
% %1 \caption{Environment TA for the translation of the process STOP.}
% \label{stop_ta1}
% \end{figure}

\lstinline{  ]}
\end{example}




% Example \ref{ex_STOP} demonstrates using Rule \ref{rule_STOP} in translating the process  \verb!STOP!  which produces two TA, a small TA and its corresponding environment TA, as shown in Figure \ref{stop_ta1}.


%To Return
% For illustration, we omit the unused parameters of the function \lstinline{transTA()}. The behaviour of the output TA (Figure \ref{stop_ta1}) begins from the environment TA (first TA) that initiates its first flow action \lstinline{startID00!} with the cooperation of its co-action \lstinline{startID00?} from the second TA, which moves from location \lstinline{s0} to location \lstinline{s1}. Then, the first TA  performs the event \lstinline{tock} to record the progress of time, together with the cooperation of the second TA, which remains in the same location \lstinline{s1} and deadlock. In short, the behaviour of the translated TA for the constant process \lstinline{STOP} causes a deadlock behaviour in location \verb!s1!. The remaining list of the translation rules, together with examples are discussed in details in the technical report \cite{extendedVersion}.



%------------------ END EXAMPLE




% \vspace{0.3cm}
% \begin{example} An example of translating a process \verb!STOP! that produces a list of TA, which contains two TA as shown in Figure \ref{stop_ta1} and \ref{stop_ta2}, as illustrated below.
% \label{ex_STOP}
% \begin{lstlisting}[mathescape, firstnumber=last]
% transTA STOP "p0_1" 1 0 ([], [], [], [], [], [], [], ([],[])) =
%         [ 
% \end{lstlisting}
% \begin{figure}[H]
% \centering
% \includegraphics [width=0.5\textwidth]{figGray/STOP_T0.png}
% %1 \caption{A small TA for the translation of the process STOP.}
% \label{stop_ta1}
% \end{figure}

% \begin{figure}[H]
% \centering
% \includegraphics [width=0.5\textwidth]{figGray/STOP_env.png}
% %1 \caption{Environment TA for the translation of the process STOP.}
% \label{stop_ta2}
% \end{figure}

% \lstinline{  ]}
% \end{example}


% Example \ref{ex_STOP} demonstrates using Rule \ref{rule_STOP} in translating the process  \verb!STOP!  which produces two TA, a small TA and its corresponding environment TA, as shown in Figure \ref{stop_ta1}. The behaviour of the output TA begins with the environment TA that initiates its first flow action \lstinline{startID00!} with the cooperation of its co-action from the small TA \lstinline{startID00?}. Then, the small TA cooperates in performing the event \lstinline{tock} to record the progress of time, and remains in the same location \lstinline{s2}, deadlock. In short, the behaviour of the translated TA for the constant process \lstinline{STOP} causes a deadlock behaviour in location \verb!s2!.

==> zz_del/a5_Eval_Experiment.tex <==


% --------- short version begin
This evaluation tool enables us to evaluate the translation technique by translating a list of formulated processes that pair all the considered constructors in the presented BNF. And then, we compare the performance of verifying deadlock freedom using both FDR and UPPAAL on the formulated processes. Details of the processes are available in a provided repository of the work \cite{extendedVersion}. Each verification was repeated 10 times, and the average timing in the repository \cite{extendedVersion}) was used to construct a graph for comparing the performance in Figure \ref{performanceGraph}. 

% \textit{COMMENT: We can choose between the following two graphs}

%  \begin{figure}[h!]
%      \centering
%     \includegraphics [width=1\textwidth]{fig/PerformanceEgs2.png}
%     \caption{Performance analysis for FDR and UPPAAL}
%     \label{performanceGraph}
% \end{figure}


 \begin{figure} %[t]
     \centering
    \includegraphics [width=1\textwidth]{fig/PerformanceEgsHis.png}
    \caption{Performance analysis for comparing FDR and UPPAAL}
    \label{performanceGraph}
\end{figure}


 The longer (blue) bars show the average timing of FDR, while the shorter (red) bars show the average time of UPPAAL. From the graph, the average performance of FDR is above 0.03 unit time while the average performance timing for UPPAAL is below 0.01. This result shows that using UPPAAL is at least three times faster than using FDR for verification. This shows a significant performance increase of UPPAAL over FDR.


% The second contribution, the translated TA facilitate using TCTL to specify requirements for liveness, in the form $\diamondsuit a$. Checking liveness is difficult in tock-CSP. In his thorough investigation, Gavin concluded that it is impossible to specify liveness requirement in trace model, but it is possible using tricks with advanced techniques in failure model \cite{G08}. 

% ---------  short version end


% ---------  remove upto the end of this tex file
% We pair the operators of the BNF presented in Section \ref{}, to generate list of tock-CSP processes that we translate into TA. And then measure the performance of FDR and UPPAAL in checking deadlock. We chose deadlock mainly for two reasons. One deadlock is one of the interesting requirements that can be check with both UPPAAL and FDR. Second, checking deadlock requires an exhaustive check for all the possible states of the process.




% In this section, we evaluate the performance of the two verification tools, FDR and UPPAAL, specifically for automatic verification. We describe the resources as well as the procedure we used for the experimental evaluation.


% %In this section, we discuss the performance comparison between FDR and UPPAAL. Evaluating the performance is another experiment we carryout in determining the performance of using FDR in verifying tock-CSP specification and using UPPAAL in the verification of TA. 

% %we describe another experiment we carryout in illustrating the significance of the work. In this section, we evaluate the performance of the two verification tools, FDR and UPPAAL, specifically for automatic verification. We describe the resources as well as the procedure we used for experimental evaluation.

% % \begin{cmt}
% % How did we carry out the experiment?
% % \end{cmt}


% %\section{Performance analysis for the examples}
% Evaluating the performance is another experiment that we carry-out in determining the performance of FDR in verifying tock-CSP specifications and using UPPAAL in the verification of the translated TA. The graph in \autoref{perfEgs} summarises the timing for checking deadlock using both FDR and UPPAAL. Considering that checking deadlock is one of the common interesting checks that can be done with both FDR and UPPAAL. Secondly, deadlock checks require an exhaustive verification for checking each state of the model.


% %in each of the processes in Table \ref{} and \ref{}.
% For each process in Tables \ref{basicproc} and \ref{pairproc}, we run verification checks for checking deadlock using both FDR for the tock-CSP and using UPPAAL in the corresponding translated TA, and we record the average timing after repeating each of the checks 10 times. Details of the recorded values for the timing are in  Appendix \autoref{performanceTable}.  

% We compare the recorded timings in the following Graph \ref{performanceGraph}, which provides a summary of comparing the recorded timing, using both FDR and UPPAAL. The graph at the top (blue) shows the recorded timing for FDR, while the graph at the bottom (red) shows the recorded time for UPPAAL. From the graph, it is clear that average performance timing for FDR is above 0.03 unit time while the average performance timing for UPPAAL is below 0.01. This result shows that using UPPAAL is at least 3 times faster than using FDR for verification. In short, this experiment shows a significant performance increase in using UPPAAL for verification of RoboChart models. 


% %The following graph illustrates a summary of comparing the recorded timing in using FDR and UPPAAL. The graph shows a significant performance increase in using UPPAAL for verification.  The graph at the top (blue) shows the recorded timing for FDR. Also, the graph at the bottom (red) shows the recorded time for UPPAAL. From the graph, it is clear that average timing for FDR is above 0.03 unit time while the average timing for UPPAAL is below 0.01. This result shows that using UPPAAL is at least 3 times faster, then using FDR for verification.

% %Timing for each verification was repeated 10 times, and the average time and standard deviation are recorded in  \autoref{perftable}. The following graph illustrates a summary of comparing the timing recorded in using FDR and UPPAAL.


%  \begin{figure}[h!]
%      \centering
%     \includegraphics [width=1\textwidth]{fig/PerformanceEgs.png}
%     \caption{Performance analysis for FDR and UPPAAL}
%     \label{performanceGraph}
% \end{figure}

%  \begin{figure}[h!]
%      \centering
%     \includegraphics [width=1\textwidth]{fig/PerformanceEgs2.png}
%     \caption{Performance analysis for FDR and UPPAAL}
%     \label{performanceGraph}
% \end{figure}


%  \begin{figure}[h!]
%      \centering
%     \includegraphics [width=1\textwidth]{fig/PerformanceEgsHis.png}
%     \caption{Performance analysis for FDR and UPPAAL}
%     \label{performanceGraph}
% \end{figure}


% %I carried out the following verification using both FDR and UPPAAL. Each verification was repeated 10 times, and the average time is recorded in table \autoref{performance}. Overall, there is a significant performance increase in using UPPAAL for the verification. 




==> zz_del/a5_Eval_Imple_.tex <==
% ---- Short version

We evaluate the translation techniques in two steps. First, we implement the translation techniques into a software tool using Haskell, as a function \lstinline{transform} that has the following type in Definition \ref{dfn_transform}. The function takes tock-CSP process and produce a list of TA. 

\vspace{0.5cm}
%\begin{tcolorbox} %[title=---]
\begin{tcolorbox} %[title=Title]
\begin{definition} \textbf{Function \lstinline{transform}}
\label{dfn_transform}
\end{definition}
\tcblower
\begin{verbatim}
transform :: NamedProc -> [TA]
\end{verbatim}    
\end{tcolorbox}



Second, we develop an evaluation tool, which uses the translation tool to translates tock-CSP process and then uses both FDR and UPPAAL as blackboxes for generating traces. Then, the tool analyse the traces to ensure that all the traces of tock-CSP are acceptable traces of the translated TA. The structure of the evaluation tool is illustrated in the Figure \ref{trace_analysis_system}.

% ----- short version end


% --- remove for short version
% In evaluating the translation techniques, we implement the translation techniques into a software tool using Haskell, which we used for precise expression of the translation rule.


% This section describes a mechanism we use in validating the translation technique and translation rule. The section is divided into two parts. First part describes an implementation of the translation rules into a software tool using Haskell. Second part describes another technique we developed for validating the translation technique. We use trace semantics for validating the translation technique. Thus we develop a technique for generating and comparing traces of tock-CSP and UPPAAL. The second part also describes a mechanisation of the second technique for comparing traces.


% \subsubsection{Mechanisation of the translation rules}
% \label{mechanisation}
% In this part we discuss the software tool we developed for automating the translation technique. For the implementation of the software tool, we continue using Haskell, the language we used in presenting the translation rules in the previous section. This reduces the complexity of justifying the translation technique. 

% %in the translation technique, which automates the translation technique. 

% At the top-level we develop another function \lstinline{transform}, which combines three functions \lstinline{transTA, syncTA} and \lstinline{envTA} into one systems. These three functions have been discussed in the previous Section \ref{rules}. The function \lstinline{transTA} defined the translation rules in Section \ref{dfn_transTA}, function \lstinline{syncTA} defined a synchronisation TA in Section \ref{dfn_syncTA} and function \lstinline{envTA} defined an explicit environment for UPPAAL models in Section \ref{dfn_env}. The following Figure \ref{translation_system} illustrates a high-level structure of the translation system.

% --- remove for short version


% \vspace{0.5cm}
% %\begin{tcolorbox} %[title=---]
% \begin{tcolorbox} %[title=Title]
% \begin{definitions} \textbf{Function \lstinline{transform}}
% \label{dfn_transform}
% \end{definitions}
% \tcblower
% \begin{verbatim}
% transform :: NamedProc -> TA
% \end{verbatim}    
% \end{tcolorbox}



% --- remove for short version
% The function \lstinline{transform} takes a named CSP process as input. This is shown in Definition \ref{dfn_transform}. The function \lstinline{transform} initialised the required arguments of both function \lstinline{transTA} and \lstinline{envTA}. The output of the function \lstinline{transform} is a list of TA that describes a suitable model for UPPAAL tool, which captures the behaviour of the input tock-CSP specifications. The following \ref{fig_uppaalTA} describes a high level structure of the UPPAAL model. The structure illustrates the main parts of UPPAAL model. The structure includes a header section for configurations information, a declarations section, definition of a list of TA in the system, definition of system that combines the list of TA into a system, and a section for specifying the verification requirements using TCTL queries. Additional details structure of UPPAAL TA is provided in Appendix \ref{TA_AST}. 
% %The types is highlighted in the following Definition \ref{dfn_TA}

% \begin{figure}%[H]
%     \centering
%     \includegraphics[width=0.7\textwidth]{fig/UPPAAL_TA_structure.png}
%     \caption{Structure of the UPPAAL models}
%     \label{fig_uppaalTA}
% \end{figure}



%Evaluation process
% \subsubsection{Trace Analysis}
% This section describes a mechanism we develop for evaluating the translation rules. The  section begins with discussing another technique we develop for validating the translation technique and a software tool we developed that automates the validation technique. For the evaluation we used trace analysis that enables us to use trace semantics for reasoning about the correctness of the translation technique. 


% Therefore, we developed a technique for generating and comparing traces of the input tock-CSP and the traces of the output translated TA. The result of the comparisons enables us to validate the translation technique. In generating the traces we use FDR as blackbox to generate finite traces of tock-CSP process. In the like manner we use UPPAAL as blackbox to generate finite traces of the translated TA. The following \ref{trace_analysis_system} provides an overview of the developed system for trace analysis.

% --- remove for short version ends 



\begin{figure}[h] %[H]
    \centering
%    \includegraphics[width=0.7\textwidth]{C3_figs/traceAnalysis.png}
    \includegraphics[width=1\textwidth]{fig/traceAnalysis.png}
    \caption{Structure of the trace analysis system}
    \label{trace_analysis_system}
\end{figure}



% --- remove for short version begins
% Figure \ref{trace_analysis_system} illustrates a structure of the trace analysis system and its 5 components, a controller, a translation system we discussed \ref{translation_system}, FDR and UPPAAL as blackboxes, and two additional components for analysing traces in two stages. In stage 1 we compare the traces of FDR and UPPAAL. If the traces does not match we move to stage 2 to check if the traces generated with FDR are valid traces of the translated UPPAAL model.


% The controller invokes each components of the system one after the other, passes input to a component and collects output and then proceeds to pass the collected output as input to the subsequent component of the system for further analysis. Initially, the controller takes input specification in tock-CSP, invokes the translation system to get a translated TA from the translation system, and then invokes FDR to get traces of the tock-CSP, and then invokes UPPAAL to get traces of the translated TA. After collecting traces, the controller initiates the trace comparison in stage 1. If stage 1 fails, the controller invokes stage 2 component of the trace analysis to ask if the traces of FDR are acceptable traces of UPPAAL. The stage 2 components converts each trace of generated trace from FDR into TA (traceTA) and then compose the trace TA in parallel with the translated TA, and then formulate a query that ask if the UPPAAL system can reach the final state. If the UPPAAL tool reaches the final state the trace is an acceptable valid trace of the translated TA, otherwise the trace is not a valid trace. At the end, the trace comparison system provides a final result that includes the result of the comparison and the collection of traces generated during the analysis. The controller is developed using bash script, which provides a neutral ground for communication among the components of the system, FDR, UPPAAL, translation system and trace comparison system. 

% --- remove for short version ends

In generating multiple traces with FDR, it is good to note that FDR was developed to produce only one trace (counterexample) at a time. As such based on the testing technique developed in \cite{CSP_traces_augusto}, we developed a technique that repeatedly invokes FDR for trace until we get the required traces. The technique enables us to generate finite traces of a tock-CSP specification.  The following Example \ref{gen_traces_with_FDR} illustrates using the trace comparison technique we developed in generating a traces of tock-CSP specification.



% --- remove for short version begins

% \begin{exl}
% \label{gen_traces_with_FDR}
% This example illustrates a step by steps technique for using FDR in generating traces of tock-CSP process \\
% \lstinline{         P1 = e1->(e2->SKIP)|||(e3->SKIP)}.

% %P = e1->(e2->SKIP)|||(e3->SKIP)


% \paragraph{Step 1} The technique begins with appending a special event \lstinline{m} to the process \lstinline{P} to form another process \lstinline{Pm}. This is express as \\
% \lstinline{         Pm = P;m->STOP}.  \\

% However, it is necessary that the special event m should not be part of the process \lstinline{P}.

% \paragraph{Step 2}. Then using FDR to verify assertion does the process P contains the traces of Pm, which is express as \\ 
% \lstinline{         P [T= Pm}.  \\

% The assertion fails and yields a counterexample  \\
% \lstinline{         t1 = <e1, e2, e3, m>}, in which the process \lstinline{P} refuses the event m. 

% The counterexample is one of the complete trace of process P with additional special event m. This is because after the complete trace t1, the formulated process Pm performs a special event m in which the process P can not perform.


% %\paragraph{Step 3} Then w
% We proceed to find out if the process Pm has another trace that is different from the trace t1.

% \paragraph{Step 3} We convert the generated trace t1 into a linear process 

% \lstinline{         Pt1 = e1->e2->e3->m->SKIP}

% %???????????? Concatenate m with Pt1

% \paragraph{Step 4} Then, we use external choice to compose the generated process Pt1 with the original process P to produce another process 

% \lstinline{P[]Pt1}. 

% \paragraph{Step 5} After that, then we use FDR again to verify an assertion 'does the new process (P[]Pt1) contains the traces of the process Pm?'. The assertion is express as

% \lstinline{         (P[]Pt1) [T= Pm}

% The assertion fails and generate a counterexample 

% \lstinline{         t2 = <e1, e3, e2, m>} in which the process P refuses the special event m.

% %This enable us to generate another

% \paragraph{Step 6} Again we convert the trace t2 into another linear process 

% \lstinline{         Pt2 = e1->e3->e2-> m->SKIP}

% \paragraph{Step 7} Again we use external choice to compose the process Pt2 with the previously formulated process \lstinline{(P[]Pt1)} to form another process 

% \lstinline{(P[]Pt1[]Pt2)}.

% \paragraph{Step 8} Also, we use FDR to verify the assertion does the process \lstinline{(P[]Pt1[]Pt2)} contains the traces of the process Pm? This assertion is express as 

%  \lstinline{         (TP1[](TP2[]P1)) [T= Pm}
 
% \paragraph{Step 9} Using FDR in verifying this assertions passes. This indicates that the traces \lstinline{t1} and \lstinline{t2} are the only complete traces of the original process P. 

% \vspace{0.5cm}

% If the assertion does does not pass, we take the generated counterexample and repeat steps 7 to 10 until the generated assertions pass, which indicate the end of the finite complete traces of the original process P. 

% %And the we stop collect the traces for
% %will cause the verification to fail, when there is no alternative path that can generate another trace.


% \end{exl}

% --- remove for short version end

However, the technique we developed for generating traces using FDR is not suitable for generating traces using UPPAAL. This is due to the differences between the two systems. FDR was developed based on verification using refinement. Secondly, FDR uses the same language CSP for both specifications and verification of a system. While UPPAAL was developed based on networks of TA. And also UPPAAL uses different languages for specification and verification. That is UPPAAL uses TA for modelling the specifications and TCTL for verification. So, based on the testing technique developed in \cite{cover_UPPAAL}, we developed another technique for generating traces using UPPAAL toolbox.

Based on this analysis we develop the trace comparison in two stages. In stage 1 we generate traces using both FDR and UPPAAL. Then, the we compare the traces, if they did not match we move to the second stage. Since all the traces of FDR have precise order, in stage 2, we verify if all the traces of the FDR are acceptable traces of UPPAAL. Based on these two steps, we are able to justify the correctness of the translation technique. Traces of TA are infinite because of the real time. So it is not possible to verify the reverse, that is to check if traces of FDR contains traces of the translated TA.




% --- remove for short version begins

% However, the technique we developed for generating traces using FDR is not suitable for generating traces using UPPAAL. This is due to the differences between the two systems. FDR was developed based on verification using refinement. Secondly, FDR uses the same language CSP for both specifications and verification of a system. While UPPAAL was developed based on networks of TA. And also UPPAAL uses different languages for specification and verification. That is UPPAAL uses TA for modelling the specifications and TCTL for verification. 



% Based on the testing technique developed in \cite{cover_UPPAAL}, we developed another technique for generating traces using UPPAAL toolbox. This technique resemble the structure of the previous technique, in such a way that this technique also repeatedly invokes UPPAAL for generating traces. We achieved this by formulating a query that generate a trace and then modify the query to block the current trace, and then also ask for another trace. This second technique enables us to generate finite traces of a finite process using UPPAAL. The following Example \ref{gen_traces_UPPAAL} illustrates using this technique in generating traces with UPPAAL tool box.

% \begin{exl}
% \label{gen_traces_UPPAAL}
% This example illustrates the technique we use in generating traces using UPPAAL toolbox. In the case of generating traces with UPPAAL system, we attach two types of auxiliary variables, one in the form \lstinline{ep1, ep2, ep3 ... epn}, and the second variables of the form \lstinline{dp1, dp2, dp3 ... dpn} to each translated event of the tock-CSP specification in the the translated TA. This is shown in the following figures \ref{trg_ta1}, \ref{trg_ta3} and \ref{trg_ta5}, for the translation of the events \lstinline{e1, e2 and e3} respectively. For each event \lstinline{e1} we attached the two variables \lstinline{ep1 and dp1}.

% The event of the forms \lstinline{epx} are Boolean variable that we used for identifying each path, in such a way that each path has unique combination of these events. Initially, the variables are set to the value true, and recording a trace of each path assigns true to all the auxiliary variables in that path.  While other variable of the form \lstinline{dp} are integer types that we used in specifying the required depth of a trace. 



% \begin{figure}%[H]
%     \centering
%     \includegraphics[width=0.8\textwidth]{fig/trg_TA1.png}
%     \caption{TA1 for the translation of the event e1}
%     \label{trg_ta1}
% \end{figure}



% \begin{figure}%[H]
%     \centering
%     \includegraphics[width=\textwidth]{fig/trg_TA2.png}
%     \caption{TA2 for the translation of the operator interleaving}
%     \label{trg_ta2}
% \end{figure}


% \begin{figure}%%[H]
%     \centering
%     \includegraphics[width=0.7\textwidth]{fig/trg_TA3.png}
%     \caption{TA3 for the translation of the event e3}
%     \label{trg_ta3}
% \end{figure}


% \begin{figure}%[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{fig/trg_TA4.png}
%     \caption{TA4 for the translation of the process SKIP}
%     \label{trg_ta4}
% \end{figure}


% \begin{figure}%[H]
%     \centering
%     \includegraphics[width=0.7\textwidth]{fig/trg_TA5.png}
%     \caption{TA5 for the translation of the event e3}
%     \label{trg_ta5}
% \end{figure}


% \begin{figure}%[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{fig/trg_TA6.png}
%     \caption{TA6 for the translation of the process SKIP}
%     \label{trg_ta6}
% \end{figure}

% \begin{figure}%[H]
%     \centering
%     \includegraphics[width=\textwidth]{fig/trg_Env.png}
%     \caption{TA7 that provides an explicit environment for the translated process}
%     \label{trg_ta7}
% \end{figure}

% \end{exl}


%  %%--- Summarise the following paragraph for the short version
% There is another difference in using FDR and UPPAAL for generating traces of a concurrent processes. In FDR, we are able to precisely specify each events and their order in each requirement using assertions. This means that with FDR we are able to generate traces that have same set of events with different permutations. For example, the complete traces of process \lstinline{P = (a -> SKIP)|||(b->SKP)} are \lstinline{ [a, b]} and \lstinline{[b,a]}, the trace have the same events that occur in different order.

% However, this is different from the case of UPPAAL tool which uses predicate logic in the verification aspect. The system evaluates whether a trace satisfies a predicate logic query (requirement)  irrespective of the order of events in a trace. This makes it difficult to generate traces that have the same event with different permutation, unless we provide an additional information that precisely indicates where the order of the traces. For example, in generating the traces of the process \lstinline{P = (a -> SKIP)|||(b->SKP)}, using UPPAAL we are able to generate either \lstinline{<a,b>} or \lstinline{<b,a>} depending on some additional configurations, such as shortest path or fastest trace. Unless if we precisely specify that event \lstinline{b} comes before event \lstinline{a}. This additional information will guide UPPAAL to generate \lstinline{<b,a>} irrespective of other configurations. That is, if we formulate a query that ask "Can the process P perform event b?". UPPAAL system returns a trace [b], unless if we have additional information that precisely say 'Can the process P performs the event b after performing the event a?'. Then UPPAAL returns the trace <a,b>. 

% --- remove for short version end


Based on this analysis we develop the trace comparison in two stages. In stage 1 we generate traces using both FDR and UPPAAL. Then, the we compare the traces, if they did not match we move to the second stage. Since all the traces of FDR have precise order, in stage 2, we verify if all the traces of the FDR are acceptable traces of UPPAAL. Based on these two steps, we are able to justify the correctness of the translation technique.




==> zz_del/a5_Eval_Implementation.tex <==
% ---- Short version

We evaluate the translation technique in two steps. First, we implement the translation techniques into a software tool using Haskell, as a function \verb!transform! that has the following type in Definition \ref{dfn_transform}. The function takes tock-CSP process and produces a list of TA. 

\vspace{0.5cm}
%\begin{tcolorbox} %[title=---]
\begin{tcolorbox} %[title=Title]
\begin{definition} \textbf{Function \lstinline{transform}}
\label{dfn_transform}
\end{definition}
\tcblower
\begin{verbatim}
transform :: NamedProc -> [TA]
\end{verbatim}    
\end{tcolorbox}



Second, in evaluating correctness, we develop an evaluation tool, which uses the translation tool to translate tock-CSP process and then uses both FDR and UPPAAL as black boxes for generating finite set of traces for a given length. The structure of the evaluation tool is illustrated in Figure \ref{trace_analysis_system}. Therefore, correctness of the translation technique is supported by the trace sets being the same, when the coordinating actions are deleted. 

% Then, the tool compares the traces to ensure that either the traces are the same or all the traces of the tock-CSP are acceptable traces of the translated TA. The structure of the evaluation tool is illustrated in Figure \ref{trace_analysis_system}.




\begin{figure}[t!] %[H]
    \centering
%    \includegraphics[width=0.7\textwidth]{C3_figs/traceAnalysis.png}
    \includegraphics[width=\textwidth, height=0.25\textheight]{fig/traceAnalysis.png}
    \caption{Structure of the trace analysis system}
    \label{trace_analysis_system}
\end{figure}




% In generating multiple traces with FDR, it is good to note that 

% Todo ????????
% Regarding X, …
% With regard to X, …


FDR was developed to produce only one trace (counterexample) at a time. So, based on the testing technique developed in \cite{NS08}, we developed a technique that repeatedly invokes FDR for generating traces until we get all the required traces set of the input tock-CSP. This trace generation technique enables us to generate finite traces set of tock-CSP specification with FDR. 

% The following Example \ref{gen_traces_with_FDR} illustrates using the trace comparison technique we developed in generating traces of tock-CSP specification.




%However, this technique for generating traces with FDR is unsuitable for generating traces with UPPAAL. This is due to the differences between the two systems. FDR was developed based on verification using refinement. Secondly, FDR uses the same language CSP for both specifications and verification of a system. In contrast, UPPAAL was developed based on networks of TA. Additionally,  UPPAAL uses different languages for specification and verification, TA and TCTL, respectively. S

Also, based on the testing technique developed in \cite{LP07}, we developed another technique for generating finite discrete traces set of TA with UPPAAL.


%Since all the 

So, based on this trace generation components, we develop the trace analysis in two stages. In stage 1, we generate traces of the input tock-CSP and its corresponding translation using both FDR and UPPAAL, respectively. Then, we compare the traces, and if they did not match, we move to the second stage. FDR trace generation technique distinguishes and generate traces with different permutation. In contrast, generating traces with UPPAAL does not distinguishes traces with different permutations. So, in stage 2, we use UPPAAL to check if the traces of the input tock-CSP process are acceptable traces of the translated TA. 
% This enables us to use trace comparison in justifying the correctness of the translation technique.

%the correctness of the translation technique using traces analysis. 

% ?????? To Remove
% ?????????????????????? So, based on this trace generation components, we develop the trace analysis in two stages. In stage 1, we generate traces of the input tock-CSP and its corresponding translation using both FDR and UPPAAL respectively. Then, we compare the traces, and if they did not match, we move to the second stage. FDR generates traces of tock-CSP with precise permutation order. In contrast, UPPAAL generates traces of TA in nondeterministic permutation order. So, in stage 2, we use UPPAAL to check if all the traces of the tock-CSP are acceptable traces of the translated TA. This enables us justify the correctness of the translation technique using traces analysis. 

%Traces of TA are infinite because of the real-time. So it is not possible to verify the reverse, that is to check if the traces of FDR contains all traces of the translated TA.





%Based on this analysis, we develop the trace comparison in two stages. In stage 1, we generate traces using both FDR and UPPAAL. Then, we compare the traces if they did not match, we move to the second stage. Since all the traces of FDR have precise order, in stage 2, we verify if all the traces of the FDR are acceptable traces of UPPAAL. Based on these two steps, we justify the correctness of the translation technique based on trace analysis.




==> zz_del/a6_RelatedWork.tex <==


%Model transformation is an established area in software engineering, various transformation techniques and tools have been developed.


% Several researches explore finding an alternative for using CSP in the verification of temporal specifications, especially in verifying Real timed systems.

Several types of researches explore using CSP in the verification of temporal specifications, especially in verifying real-time systems. Timed-CSP \cite{S10} is another popular extension of CSP that provides additional notations for capturing temporal specifications. Timed-CSP records the progress of time with a series of positive real numbers, which facilitates reasoning and verification of real-time systems.

%The provided extension facilitates verification of RTS.


%Timed-CSP \cite{S10} provides facilities for capturing temporal specifications. Timed-CSP records progress of time using non-negative real number. 

However, the Timed-CSP does not enable specifying strict progress. Thus, traces of Timed-CSP becomes infinite, which is problematic for automatic analysis and verification \cite{R10}. So far, there is no tool support for verifying Timed-CSP models.

% the added notations make
%This does not facilitate automatic verification, which becomes problematic. So far, there is no tool support for verifying Timed-CSP.

%So it is impossible to specify that an event must happen within a specific amount of time.  
%Read R10 for additional info

As a result of that, many researchers explore model transformations for supporting Timed-CSP with an automatic verification tool. Timed-CSP has been translated into tock-CSP to enable using FDR for automatic verification \cite{O00}. The work provides a link for utilising the facilities of FDR in verifying Timed-CSP model. 

Also, Timed-CSP has been translated into UPPAAL to facilitates using the facilities of UPPAAL in verifying Timed-CSP. The work was initiated in \cite{DH08} and then subsequently improved in \cite{TS13}.


Additionally, Timed-CSP has been translated into Constraint Logic Programming (CLP)  that facilitates reasoning in verifying Timed-CSP, that is supported by constraint solver CLP(R) \cite{DP06}.

%Also, Timed-CSP was translated into tock-CSP to enable using FDR for the verification.

However, there is less attention in applying the same transformation techniques in improving tock-CSP with a better approach for verifying real-time system.
An attempt for transforming TA into tock-CSP was proposed in \cite{K11}. In this work, we consider the opposite direction for translating tock-CSP into TA for UPPAAL to be able to utilise the facilities of UPPAAL in verifying tock-CSP models.
 

Apart from CSP, model transformations have been used for improving other modelling notations. Circus has been translated into \lstinline{CSP||B} to enable using ProB for automatic verification \cite{KJ17}. Additionally, B has been translated into TLA+ for automatic validation with TLC \cite{HL14}. Also, the reverse of translating TLA+ to B has been investigated for automatic validation of TLA+ with ProB \cite{HL12}. Such that both B and TLA+ benefits from the resources of both TLC and ProB. Model transformation is an established field. A recent survey provides rich collections of model transformations techniques and their supporting tools \cite{KM19}.





% Translating B to TLA+ for Validation with TLC \cite{HL14}

% Also, the reverse of translating TLA+ to B for validation with ProB \cite{HL12}



%Difference from the existing related work
%Limitations of our work 


% In this work, we take a different approach, in which we consider translating tock-CSP into TA for UPPAAL to utilise the facilities of UPPAAL in verifying RTS.




%Timed-CSP has been translated into UPPAAL to enable using the facilities of UPPAAL \cite{}, and also improved \cite{}.



























==> zz_del/a6_RelatedWork_.tex <==


%Model transformation is an established area in software engineering various transformation techniques and tools has been developed.


% Several researches explore finding alternative for using CSP in the verification of temporal specifications, especially in verifying Real timed systems.

Several researches explore using CSP in the verification of temporal specifications, especially in verifying Real timed systems. Timed-CSP \cite{S10} is another popular extension of CSP that provides additional notations for capturing temporal specifications. Timed-CSP records progress of time with positive real number, which facilitates reasoning and verification of real-time systems.

%The provided extension facilitates verification of RTS.


%Timed-CSP \cite{S10} provides facilities for capturing temporal specifications. Timed-CSP records progress of time using non-negative real number. 

However, the extension does not enable specifying strict progress. As a result of this, the traces of Timed-CSP becomes infinite in nature, which is problematic for automatic analysis and verification \cite{R10}. So far there is no tool support for verifying Timed-CSP models.

% the added notations make
%This does not facilitate automatic verification, which becomes problematic. So far there is no tool support for verifying Timed-CSP.

%So it is impossible to specify that an event  must happen within a specific amount of time.  
%Read R10 for additional info

As a result of that many researchers explore model transformations for supporting verification with automatic tool. 

Timed-CSP has been translated into tock-CSP to enable using FDR for automatic verification \cite{O00}. This provides a link for utilising the facilities of FDR in verifying Timed-CSP model. 

Also, Timed-CSP has been translated into UPPAAL to facilitates using the facilitiese of UPPAAL in verifying Timed-CSP. The work was initiated in \cite{DH08} and then subsequently improved in \cite{TS13}.


Additionally, Timed-CSP has been translated into Constraint Logic Programming (CLP)  that facilitates reasoning  in verifying Timed-CSP, that is suppoorted with constraint solver CLP(R) \cite{DP06}.

%Also, Timed-CSP was translated into tock-CSP to enable using FDR for the verification.

However, there is less attantions is applying the same techniques in complementing tock-CSP with a better approach for the verifying RTS. 

An attempt for transforming TA into CSP was proposed in \cite{A94}

Also model transformations has been used for improving/complementing other modelling notations.

Additionally, Circus has been translated into CSP||B to enable using ProB for automatic verification \cite{KJ17}.

Translating B to TLA+ for Validation with TLC \cite{HL14}

Also, the reverese of translating TLA+ to B for validation with ProB \cite{HL12}

Model transformation is an established field. A recent survey provides a rich collections of model transformations techniques and their supporting tools \cite{KM19}.


%Difference from the existing related work
%Limitations of our work 


In this work, we take different approach, in which we consider translating tock-CSP into TA for UPPAAL to utilised the facilities of UPPAAL in verifying RTS.




%Timed-CSP has been translated into UPPAAL to enable using the facilities of UPPAAL \cite{}, and also improved \cite{}.



























==> zz_del/a7_Conc.tex <==
% -------------------------------------
% Conclusion

In this work, we presented a translation of tock-CSP into TA for UPPAAL. The translation work facilitates using UPPAAL for the verification of tock-CSP. We find a significant increase in performance for using UPPAAL in the verification of tock-CSP specifications. 

Additionally, this work would provide an easier alternative of using TCTL in specifying liveness requirements that are difficult to specify and verify in tock-CSP. Such possibility will be explored in the future work.

So far, we used trace analysis in justifying the correctness of the work. In the future, we are planning to apply mathematical reasoning to formally prove the translation technique. Secondly, we are planning to explore using the translation technique in translating extensive case studies, from tock-CSP to UPPAAL. 
%The efficiency of the translation technique is another topic for investigation in future work.


%Any Limitation?


==> zz_del/all_.tex <==



\section{Introduction}   %%%-----------------------------------------------------

Communicating Sequential Processes (CSP) is an established process algebra that provides formal notations for both modelling and verification of concurrent systems \cite{R10, S10, H78}. Using CSP for verification has been supported with an automatic model-checker FDR \cite{TP14}. CSP and its modelling approaches have contributed in understanding the complexity of concurrent systems  \cite{S10}. 


%tockCSP------------------------------------------------------------------

Interest in CSP motivates the introduction of time into its constructs; \verb!tock-CSP! provides an additional event $tock$ to record progress of time. This facilitates using CSP for modelling temporal specifications in a format that is suitable for formal analysis and verification. The structure of \verb!tock-CSP! retains the original structure of CSP and utilises the existing works and tools for CSP. Thus, automatic verification is supported by FDR \cite{TP14, R10}. As a result of that,  \verb!tock-CSP! has been used in the verification of real-time systems such as security protocols \cite{NS00} and railways system \cite{YF12}. Recently, \verb!tock-CSP! has been used for capturing the semantics of RoboChart, a domain specific modelling language (DSML) for modelling robotics system \cite{MR16}. Additionally, a recent extension of \verb!tock-CSP! provides additional notations for specifying budgets and deadlines for effective modelling and verification of temporal specifications \cite{JP19}.



In this work, we add a technique for translating \verb!tock-CSP! into TA that enables using the facilities of UPPAAL in verifying of \verb!tock-CSP! models. UPPAAL is a tool-suite for modelling and verification of real-time systems using TA and temporal logic \cite{BD06}. Both temporal logic and refinement are powerful approaches for model-checking \cite{G08}. However, each one of these two approaches has different concept of modelling and verifying system behaviour. 

On the one hand, refinement approach models both the system and its specifications with the same constructs, like \verb!tock-CSP!, which enables asking a question if the system captures the specification of its requirement \cite{R10, S10}. On the other hand,  temporal logic has logical constructs for formulating system specifications, which enables asking a question, if a system satisfies a logical formula of the specification, that is $system \models formula$ \cite{CE86}. Both temporal logic and refinement have support for automatic verification such as UPPAAL \cite{BD06} and FDR \cite{TP14}, respectively.


Previously, Lowe has investigated the relationship between refinement oriented approach (with CSP) and temporal logic oriented approach. The result shows that, in expressing temporal logic with refinement approach, it is necessary to use  (infinite) refusal testing model of CSP. The work highlights that the most challenging part is capturing the expressiveness power of temporal logic in specifying the availability of an event (liveness specification). These are desirable specifications that ensure that a system will either perform something good or something bad will never happen in the system. 

Additionally, the work \cite{G08} proves that simple refinement check can not cope with the expressive power of three operators: eventuality $(\diamond)$,  until ($\mathcal{U}$) and negation ($ \neg$), that are interconnected for the verification of eventual behaviour of a system. In addition, due to the difficulty of capturing refusal testing, automatic support becomes problematic. Although, the previous version of FDR supports refusal testing, but not the recent efficient version of FDR \cite{fdr}.



In the case of TA for UPPAAL, temporal logic provides constructs for expressing liveness specifications. Therefore, this translation work will facilitate using the resources of temporal logic (and UPPAAL) in checking liveness specifications of \verb!tock-CSP! models, including requirements that involve an operator for specifying eventual behaviour $(\diamond)$. The same also applies to the remaining two operators  $ until (\mathcal{U}$) and  $negation (\neg) $. This is illustrated in Example \ref{ads}.



\begin{example} %{A translation of an Automatic Door System (ADS)} \\
\label{ads}
An example of an Automatic Door System (ADS) that opens a door, and then after at least one-time unit, the system closes the door in synchronisation with a lighting controller, which turns-off the light after closing the door. A \verb!tock-CSP! specification of the system is as follows.



\begin{lstlisting}
Controller = open -> tock -> close -> Controller

Lighting = close -> offLight -> Lighting

ADS = Controller [|{close}|] Lighting

\end{lstlisting}



\end{example}



ADS system has two components, \lstinline{Controller} and \lstinline{Lighting}.  \verb!Controller! opens and closes the system after an interval of at least one unit time. \lstinline{Lighting} turns-off the light after closing the door. The two components synchronise on the event \lstinline{close}, which enables the lighting controller to turns-off the light. 


The concise compositional structure of \verb!tock-CSP! make it suitable for modelling component and compose them into a system.
However, there are certain interesting desirable requirements that are difficult to specify with \verb!tock-CSP!, and in general they are difficult to specify using simple refinement testing \cite{G08}. For instance, in the case of Example \ref{ads}, there is no easy way of using \verb!tock-CSP! to specify requirements for checking 'if the system will eventually turns-off the light when the environment is ready to switch-of the light'. Also, there is no straightforwad way for specifying and checking requirements such as 'closing the door will always leads to switching-up the light'. However, temporal logic provides direct construct for specifying these kind of requirements in a simple form. For instance, in temporal logic these requirements are specify as follow.
\begin{enumerate}
    \item $E\diamond$ \lstinline{offLight}  \\ 
    - - \textit{Can the system always turns-off the light after closing the door, if the environment agrees on closing the door}
    
    \item \lstinline{close} $\leadsto$ \lstinline{offLights} \\
    % \item \verb!close --> offLight! \\
    - - \textit{Can closing the door leads to turning-off the light, if the environment agrees on turning-off the light.}
\end{enumerate}

Translating \verb!tock-CSP! into TA will enable using the best of these worlds, \verb!tock-CSP! and TA. An early result of this translation work indicates a potential result of utilising the resources of UPPAAL and its verification facilities in the translated \verb!tock-CSP! models, specifically the constructs of temporal logic in the verification of certain specifications that are difficult to specify with \verb!tock-CSP!. 

For verifying the correctness of the translation work. First, we formulate a list of interesting \verb!tock-CSP! processes, which pair all the constructs of \verb!tock-CSP! that we consider within the scope of this work. Second, we use the developed translation technique to translate the formulated processes into TA for UPPAAL.  Third, we developed another tool that assists us in generating and comparing traces of the input \verb!tock-CSP! processes and the traces of the translated TA, with the support of both FDR and UPPAAL, respectively. This ensures that the translated TA captures the behaviour of \verb!tock-CSP! models.



% Outline of the paper  ----------------------------------------------------------------------
The structure of the paper is as follows. Next, Section \ref{background} provides a brief backgrounds that are essential for understanding the translation technique.  In Section \ref{trans_rule}, we describe the translation technique and also provide an overview of the translation rules. In Section \ref{evaluation}, we discuss an evaluation of the translation technique. In Section \ref{related_work}, we highlight relevant related work, and also provides a brief comparison with this work. Finally, Section \ref{conclusion} highlights future work and provides a conclusion for the paper.
 


%%  --------------------  BACKGROUND -----------------------
\section{Background}
\label{background}

This section discusses the required background for understanding the translation work. We begin with discussing the notations of \verb!tock-CSP! and then discuss the target outcome of the translation work, that is a list of TA that is suitable for UPPAAL tool. 


%CSP and \verb!tock-CSP!
\subsubsection{A tock-CSP model} is an extension of CSP that provides notations for modelling processes and their interactions. In \verb!CSP!, there are varieties of construct that includes basic processes such as \verb!SKIP! and \verb!STOP!. \verb!SKIP! expresses a successful termination while \verb!STOP! expresses a deadlock. Also, there are operators such as an operator \verb!prefix (->)! that prefixes an event to a process. For example, the process \verb!move->SKIP! specifies the behaviour of a system that moves and then terminates. 



Additionally, there are binary operators such as sequential composition (;), which composes two processes one after the other. So, a process \verb!P3 = P1;P2! is a process that behaves as process \verb!P1!, and then after a successful termination of the process \verb!P1!, the process behaves as process \verb!P2!. For example, the process \verb!Ps = (move->SKIP);(turn->SKIP)!, specifies a system that moves, turns and then terminates.


There are other binary operators for composing processes in different shapes, such as concurrency, choice and interrupt. The collection of these operators provides a rich set of constructs for modelling untimed systems. Comprehensive details of CSP operators are available in these books \cite{R10, S10}. 


Thus, \verb!tock-CSP! enriches the notations with adding a special event \verb!tock! for recording the progress of time \cite{R10}. Each event \verb!tock! indicates a passage of a single time unit. For example,  a process \verb!Pt= move->tock->tock->turn->SKIP! specifies a behaviour of a system that moves, and then after at least two time units, the system turns and then terminates. The addition of the special event \verb!tock! enables specifying temporal specification in a format that is suitable for formal analysis \cite{TP14}. 


For this work, we provide a BNF that describes the scope of the \verb!tock-CSP! operators we consider in developing the translation technique. Part of the BNF is presented in Definition \ref{dfn_CSPproc} using the syntax of Haskell data definition. Due to limited space, the complete BNF is available in an extended report of the work \cite{extendedVersion}. We use this BNF as the basic foundation of this translation work.

\begin{definition} \textbf{Data definition of \lstinline{CSPproc}} 
\label{dfn_CSPproc}


\begin{verbatim}
data CSPproc =   STOP | SKIP | Prefix Event CSPproc |
                 Interleave CSPproc CSPproc |
                 GenPar CSPproc CSPproc [Event] |
                 Interrupt CSPproc CSPproc |
                 ...
\end{verbatim}
\end{definition}




\subsubsection{Timed Automata for UPPAAL}
TA provides graphical notations for modelling Hybrid systems. In UPPAAL, systems are modelled as a network of TA. Mathematically, TA is defined as a tuple $(L, l_0, C, A, E, I)$, where L is a set of locations such that $l_0$  is the initial location, C is the set of clocks, A is the set of actions, E is the set of possible edges that connects the locations \verb!L!, and \verb!I! is an invariant that is associated with a location $l \in L$. So, an edge $E$ is defined as $E \subseteq (L \times A \times B(C) \times 2^C \times L)$, which describes an edge from location $l \in L$ that is triggered by an action $a \in A$ associated with a set of clocks B(C) that are reset on following an edge $e \in E$ to a location $l \in L$.  \cite{BD06, B11}.



In UPPAAL, a TA performs an action over an edge, synchronously with the environment and possibly with some other TA in the case of broadcast action. An action triggers a transition from one location to another or possibly returns to the same location. A state of a system comprises of three elements:  a list of the locations for all the networked TA, a list of values for both  associated clocks and variables. Thus, a transition changes the state of the whole system, which defines the traces that are suitable for reasoning and verification of a system, together with the automatic support of UPPAAL.
  


Lastly, for consistency, we use the concise constructs of Haskell \cite{H16} is describing the technical part of the work. Haskell is the functional programming language that we use for expressing, implementing and evaluating the translation technique. Both concise and expressive power of Haskell helps us in providing a precise description of the translation technique as a list of translation rules.









%%%%% ------------------------------  TRANSLATION TECHNIQUE  ------------------

\section{Translation Technique}
\label{trans_rule}

% \begin{cmt}
% To be updated.
% The introduction will be updated after updating the section.
% \end{cmt}

This section discusses an overview of the translation technique.  Also, we present a sample of the translation rules, which summarise the translation technique. Each rule defines a translation of one construct of \verb!tock-CSP! operators into TA, in a form that are networked to establish the flow of the translated \verb!tock-CSP!.

%that we consider for this work.




\subsection{An Overview of the Translation Technique}



The translation technique produces a list of small TA, such that the occurrence of each \verb!tock-CSP! event is captured in a small TA with an UPPALL action,  which records an occurrence of the translated event. The action has the same name as the name of the translated event from the input \verb!tock-CSP! process. The technique composes these small TA into a network of TA, which captures the behaviour of the input \verb!tock-CSP! model. 


% \begin{cmt}
% Update:\\
% I add the following paragraph to address the reason for using small TA.
% \end{cmt}


We use the small TA to capture the compositional structure of \verb!tock-CSP!. Capturing the compositional structure is complex because the compositionality may change the behaviour of a process when compose with another process without changing the definition a process. For example, the process \verb!P = e -> SKIP! has different behaviour when compose concurrently with another process, such as in the process  \verb!Pb = P|[{e}]SKIP!.  Even though the definition of the process \verb!P! remains the same but the behaviour is different, because the process \verb!P! can not perform the event \verb!e! alone, without the cooperation of the LHS process \verb!SKIP!. Thus, the behaviour of the process \verb!P! becomes deadlock, because the process \verb!SKIP! never cooperates in performing the event \verb!e!.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \begin{figure} %[H]
 
\subfigure{\includegraphics [width=0.9\textwidth, height=0.4\textwidth]{EgGenParGray/taGenPar0_0.png}}

\subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix00_1.png}}
 \hspace{0.1\textwidth}
\subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix00_2.png}}

\subfigure{\includegraphics [width=0.55\textwidth]{EgGenParGray/taPrefix00_3.png}}
\subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/SyncTA.png}}

\subfigure{\includegraphics [width=0.55\textwidth]{EgGenParGray/taPrefix01_2.png}}
\subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix01_3.png}}

 \hspace{0.1\textwidth}
% \subfigure{\includegraphics [width=0.3\textwidth]{EgGenParGray/taWait_n01_4.png}}
\subfigure{\includegraphics [width=0.9\textwidth]{EgGenParGray/Env.png}}
\caption{A list of networked TA for the translation of the process ADS}
\label{ta_ads}

\end{figure}



For example, a translation of the process ADS from Example \ref{ads} produces a network of small TA in Figure \ref{ta_ads}. Details of the translated TA are as follows. Starting from the top-left corner, the first TA captures the translation of concurrency that starts the two processes \lstinline{Controller} and \lstinline{Lighting} concurrently in two possible orders, either \lstinline{Controller} then \lstinline{Lighting} or vice versa, and then also waits on state \lstinline{s5} for their termination actions in the two possible orders, either \lstinline{Controller} then \lstinline{Lighting} or vice versa, and then the whole system terminates with the action \lstinline{finishID0}.


The second, third and fourth TA capture the translation of the process \lstinline{Controller}. The second TA captures the occurrence of the event \verb!open!. The third TA captures the occurrence of the events \verb!tock?! (with question mark) because the environment controls the progress of time because all processes synchronise with time.  The fourth TA captures the occurrence of the event \verb!close!, which needs to synchronise with a synchronisation controller, that is the fifth TA in the list of the TA.


The sixth TA captures the event \verb!close! for the process  \lstinline{Lighting}, which also needs to synchronise with the synchronisation controller on the event \verb!close!. The eighth TA captures the event \verb!offLight!. Finally, the last TA is an environment TA that provides co-actions for all the translated events. Also, the environment TA serves the purpose of 'closing' the overall system (in contrast to having an "open system") as required for the model checker.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Explanation of TA for ADS

\paragraph{}
An alternative of using a list of small TA is using a single large TA that captures the behaviour of the translated \verb!tock-CSP! process. However, the main reason for using a list of small TA is coping with the compositional structure of \verb!tock-CSP!, which is not available in TA \cite{DH08}. For instance, it can be argue that a linear process constructed with series of prefix operators can be translated into linear TA. However, the compositional structure of \verb!tock-CSP! for this straight forward translation. In particular, composing a process $P1$ with another process $P2$ using an interrupt operator changes the original behaviour of the process $P1$, even though the definition of the process $P1$ remains the same. Thus brings the need of a network of small TA that provides enough flexibility for composing TA in various ways to capture the behaviour of the original \verb!tock-CSP! process.  


In constructing the the network of TA, we use additional action, \textbf{\textit{coordinating actions}} that links the small TA into a network.  For example, \verb!startIDADS!, \verb!startID01_1!, \verb!startID00_2! in Figure \ref{ta_ads}. These coordinating actions coordinate and link the small TA into a network of TA to establish the flow of the translated \verb!tock-CSP! process.  Each coordinating action is pair of action, an action and its corresponding co-action. An action has exclamation mark (\verb|a!|) that synchronises with its corresponding co-action, which has a question (\verb|a?|).  This provides a link between two TA in such a way that the first TA (with \verb|a!|) communicates with the second TA that has the corresponding co-action (\verb|a?|). A precise definition of the coordinating action is provided in Definition \ref{coordinating_action}, which includes the types of coordinating action we use in developing the translation technique.




\begin{definition}

\textbf{Coordinating Action} is an additional UPPAAL action that is not part of the input \verb!tock-CSP! process. In developing the translation technique, we use six types of coordinating actions as follows:
\begin{itemize}
\item \textbf{Flow action} coordinates a link between two TA for capturing the flow of the behaviour of the original \verb!tock-CSP! process. 
    
\item \textbf{Terminating action} records termination information, in addition to coordinating a link between two TA.


\item \textbf{Synchronisation action} coordinates a link between a TA that participate in a multi-synchronisation action and a TA for controlling the multi-synchronisation. 


\item \textbf{External choice action} coordinates and capture the translation of external choice, such that choosing one of the processes composed with external choice blocks the other alternative choices.


\item \textbf{Interrupt action} initiates an interrupting transition that enables a processes to interrupt other processes, for the case of translating processes that are composed with an interrupt operator in \verb!tock-CSP!.

\item \textbf{Exception action} coordinates a link between a TA that raises an exception and a control TA for handling the exception. 

\end{itemize}
\label{coordinating_action}.
\end{definition}


The name of each coordinated action is unique, which ensures a correct flow of the translated TA. The name of the flow action is in the form \verb!startIDx!, where \verb!x! is either a natural number or the name of the original \verb!tock-CSP! process. For instance, in Example \ref{ads}, the name \verb!startID00_1! connects the first TA with the second TA.

Likewise, the name of the remaining coordinating action follow the same pattern; \verb!keywordIDx! where  \verb!keyword! is a designated word for each of the coordinating action: \verb!finish! for terminating action,  \verb!ext! for external choice action, \verb!intrp! for interrupting action, and \verb!excp! for exception action. Similarly, the name of a synchronising action is in the form \verb!eventName___sync!, that is an event name appended with the keyword \verb!___sync! to differentiate the synchronisation action from other actions. 



We provide termination actions that capture essential termination information from the input \verb!tock-CSP!. This is essential is the cases where a TA needs to communicate a successful termination for another TA to proceed. For example, in the case of translating sequential composition \lstinline{P1;P2} where the process \lstinline{P2} begins only after a successful termination of the process \lstinline{P1}.  



Additionally, for each translated \verb!tock-CSP! specification, we provide an environment TA that has corresponding co-actions for all the translated events of the input \verb!tock-CSP! model. Also, the environment TA closes the overall model as part of the requirements for UPPAAL model checker.  In addition, the environment TA has two coordinating actions that link the environment TA with the network of the translated TA. First, a flow action that links the environment with the first TA in the list of the translated TA. Also, this first flow action is the starting action that activates the behaviour of the translated TA. Second, a terminating action that links back the final TA in the list of the translated TA to the environment TA, and also records a successful termination of a process and close the whole system. A precise definition of the structure of environment TA is provided in Definition \ref{environment_TA}.



% \vspace{0.2cm}

\begin{definition} 
\textbf{Environment TA} models an explicit environment for UPPAAL model. The environment TA has one state and transitions for each co-action of all the events in the original \verb!tock-CSP! process, in addition to two transitions for the first starting flow action and the final termination co-action. 

\label{environment_TA}
\end{definition}



Next, in translating multi-synchronisation, we adopt a centralised approach developed in \cite{O05} and implemented using Java in \cite{F05}. The approach describes using a separate centralised controller for controlling multi-synchronisation events. Here, we use UPPAAL broadcast channel to communicates synchronising information among the synchronising TA and the control TA that control the synchronising action.

In Example \ref{ads}, we illustrate the strategy of translating synchronisation action, in translating the event \verb!close!, which synchronises the two processes \verb!Controller! and \verb!Lighting!. The fifth TA captures the translation the action close, which synchronise the process \lstinline{Controller} and the process \lstinline{Lighting}, that is fourth and sixth TA in the translated TA in Figure \ref{ta_ads}. A precise definition of the synchronisation TA is provided in Definition \ref{dfn_syncTA}.



\begin{definition} \textbf{Synchronisation TA} coordinates a multi-synchronisation action. The structure of synchronisation TA has an initial state and a committed state for each multi-synchronisation action, such that each committed state is connected to the initial state with two transitions. The first transition from the initial state, has a guard and an action. The guard is conjunction of guards for each of the process that synchronises on that synchronisation action. The guard becomes enable when all the process are ready for the synchronisation, which also enables the TA to performs the associated action that notifies the environment for the occurrence of the synchronisation action. Then, in the second transition, the TA broadcasts  the synchronisation action to all the processes that synchronise on the synchronisation action.


\label{dfn_syncTA}
\end{definition}



When all the synchronising TA become ready, a synchronisation TA broadcasts the multi-synchronisation action such that all the participating TA synchronise using their corresponding co-action. The provided guard ensures that the synchronisation TA synchronises with the required number of TA that participate in a multi-synchronisation action. The guard blocks the broadcast multi-synchronisation action until all the participating TA become ready, which enables the corresponding guard in broadcasting the multi-synchronisation action. 





%%%%%%%%%%%%%%%%%% ---  OVERVIEW OF THE TRANSLATION TECHNIQUE
Furthermore, in \verb!tock-CSP!, a process can be interrupted by another process when the two processes are composed with an interrupt operator (\verb!/\!). This is due to the compositional structure of \verb!tock-CSP!. However, in the case of TA, an explicit transition is needed for expressing an interrupt,  which enables a TA to interrupt another one. Thus, in this translation work, we provide an additional transition for capturing interrupt using an interrupt action, as defined in Definition \ref{coordinating_action}.


For example, given a process \verb!Pi = P1/\P2!, the process \verb|P1| can be interrupted by process \verb|P2|. Thus, in translating each event of process \verb|P1|, we provide additional transitions for the initials of the interrupting process \verb|P2|. The additional transitions enable the translated behaviour of process \verb|P2| to interrupt the translated behaviour of process \verb|P1| at any of its action.




Similarly, in translating external choice, we provide additional transitions that enable the behaviour of the chosen process to block the behaviour of the other processes. Initially, in the translated TA, all the initials of the translated processes are available such that choosing one of the processes block the other alternative processes with the co-actions of the provided additional transitions for translating  external choice, as defined in Definition \ref{coordinating_action}.



For example, given a process \verb!Pe = P1[]P2! that composes \verb!P1! and \verb!P2! with operator external choice; such that \verb!Tp! is a list of TA for translating the process \verb!P!. Similarly, let \verb!Tp1! and \verb!Tp2! are list of TA for the translation of the processes \verb!P1! and \verb!P2!, respectively.  The first TA in the list \verb!Tp1! has additional transitions for the initials of \verb!P2! such that choosing \verb! Tp2! blocks \verb!Tp1!. Similarly, the first TA in the list of TA \verb!Tp2! has additional transitions for the initials of \verb!P1! such that choosing \verb!Tp1! blocks the behaviour \verb!Tp2!. Additional examples are also provided in an extended report of this work \cite{extendedVersion}.




Also, in \verb!tock-CSP!, an event can be renamed or hidden from the environment. In translating renaming, the translation technique carries a list of renamed events. Before translating each event, the translation technique checks if the event is part of renamed events, and then translate the event appropriately with the corresponding new name. In the like manner, if an event is part of the hidden events, the translation technique carries a list of hidden events, such that on translating hidden event the technique uses a special name $itau$ in place of the hidden event. The event $itau$ has similar meaning with the event $tau$. We make them different to differentiate the translated hidden event $itau$ from the event $tau$ that comes from FDR, mainly for the purpose of analysis.


In \verb!tock-CSP!, the event \verb!tock! records the progress of time. So, we translate the event \verb!tock! into a corresponding action \verb!tock! in the translated TA with a broadcast channel that enables all the process to synchronise with the progress time. The translated action \verb!tock! is guarded with clock $clk<=1$ which trigger the action tock and reset the clock $clk=0$. The action tock is broadcast by the environment TA, which forces all the TA to synchronise and record the progress of time. An example of translating the event \verb!tock! is in Example \ref{ta_ads}, the last TA, Environment TA in the list of the translated TA Figure \ref{ta_env}, also together with the corresponding clock in the last TA of Figure \ref{ta_ads}.


In translating non-determinism, TA has a non-determinism facilities. We translated non-deterministic choice into silent transitions, such that the translated TA follow one of the silent transitions non-deterministically. While urgency translated into the corresponding urgent channel in UPPAAL. However, divergence is another concern that we did not included in this work because divergence process is a sign of bad behaviour and does not terminate.



This completes an overview description of the strategy we follow in developing the translation technique. The following section describes the details the translation rules, and provides examples that demonstrate using each rule in translating a \verb!tock-CSP! process.















%%  ----------------------------- RULES
\subsection{An Overview of the Translation Rules}

Based on this translation technique, we come-up with a list of translation rules that describe a translation \verb!tock-CSP! constructs into a network of TA.  Here, we provide an overview description of the translation rules. The first rule, which translates the construct STOP, describes the structure of the translation rule.  Additional details of the complete list of the translation rules together with examples are available in \cite{extendedVersion}.





We develop the translation technique as a function \verb!transTA!, which defines the translation of each of the BNF's constructs into TA. For preciseness, consistency and uniformity the translation rule are describe with Haskell, as follow.




\begin{definition} \textbf{Type of Translation Function \lstinline{transTA}}
\begin{verbatim}
transTA :: CSPproc -> ProcName  -> BranchID -> StartID ->
          FinishID -> UsedNames -> ([TA], [SyncAction])
\end{verbatim}

\label{dfn_transTA}
\end{definition}





The function \verb!transTA! has 6 parameters. The first parameter of type \verb!CSPproc! is the input \verb!tock-CSP! process. The second parameter is a name of the input process, of type \verb!ProcName!, an alias of string. While the third and fourth parameter are of type \verb!BranchID! and \verb!StartID!. Fifth parameter of type \verb!FinishID!, is a termination ID, as defined in Definition \ref{coordinating_action}. We use these IDs in constructing a network of TA that capture the behaviour of the translated process. Last parameter of type \verb!UsedNames! is a tuple for the collection of names, which we used in developing the translation function, mainly for passing the required translation information from one recursive call of the translation function to another call. 






The output of the translation function is a pairs of list of translated TA and another list of synchronisation actions. From the BNF of UPPAAL \cite{LP97}, the key elements of the output TA are the definition of TA itself and the definition of its components:  \verb!Locations!, \verb!Transitions! and the corresponding definitions of their \verb!Labels!. These elements are expressed in  Definition \ref{dfn_tastr} as Haskell data-type, which define the structe of the output TA. 




\begin{definition} \textbf{Type of TA and its components} 
\label{dfn_TA}

\begin{verbatim}
data TA = TA Name        [Parameter] [Declaration] 
             [Location]  Init        [Transition]

data Location   = Location   ID     Name   Label   LocType
data Transition = Transition Source Target [Label]
data Label      = EmptyLabel 
                | Invariant  Expression 
                | Guard      Expression 
                | Update     [Expression] 
                | Sync       Identifier   Direction
\end{verbatim}
\label{dfn_tastr}
\end{definition}



%Definition \ref{dfn_TA} is provides a
In Definition \ref{dfn_tastr}, the type \verb!TA! has a constructor \verb!TA! with six parameters. The first parameter of type \verb!Name! is an identifier for the TA itself.  The second parameter of type \verb!Parameter! is a list of arguments for the TA. The third parameter of type \verb!Declaration! is a list of local definitions inside the TA.  The fourth parameter of type \verb!Location! is a list of locations in the TA, which is defined in Definition \ref{dfn_tastr}. The fifth parameter of type \verb!Init! is an initial location of the TA. The last parameter of type \verb!Transitions! is a list of transitions that connect the locations of the TA, also defined in Definition \ref{dfn_tastr}.  These definition of TA for UPPAAL corresponds to the Mathematical definition of TA, as described in Section \ref{background} .



Also, in Definition \ref{dfn_tastr}, the definition of the remaining three parameters are as follow. The type \verb!Location! has a constructor that has four parameters of types \verb!ID, Name, Label and LocType!.  \verb!ID! is an identifier for the location. \verb!Name! is a tag that provides visual description of a location. Third parameter of type \verb!Label! is a constraint label of the location as defined in Definition \ref{dfn_tastr}. Last parameter of type \verb!LocType! donates a format of the location, which can be one of these three: \verb!urgent!, \verb!committed!, \verb!none!. An urgent location does not allow time to pass. While committed location is an urgent location that must take the next transition before any other transition. Lastly, none is ordinary location that is neither urgent nor committed.



Similarly, the type \verb!Transition! has a constructor \verb!Transition! that has three parameters, two parameters of type \verb!Location! for both source and target location of a transition. The third parameter of type \verb!Label! donate a label for a transition. Both location and transition have label, which can be empty (for a silent transition), invariant for a location only. And a transition can have any combination of guard, update and synchronisation action, as defined in Definition \ref{dfn_tastr}.  








% Translation of stop
\subfile{a4_ruleStop}


% Translation of gen parallel
\subfile{a4_ruleGenPar}



The remaining translation rules follow similar pattern and format. Due to limited space, we made them available in an extended report \cite{extendedVersion} accompanying this work.


%  ---------------------------------- EVALUATION 
\section{Evaluation}
\label{evaluation}




To ensure that the translation work is correct we have to verify the correctness of the translation work. A translation of formal models like \verb!tock-CSP! and TA can be verify in semantics correctness, which deals with verifying that interesting properties of the source model are preserved in the target models. This can be verify by comparing the  behaviours of the source model and the behaviours of the translated model \cite{T06, NN07, KM19, B81}. 

In most cases, verifying semantics correctness require solving a complex task [T06]. However, there are two popular approaches of verifying semantics correctness, that is either partial correctness or total correctness. Partial correctness relates the initial and final state of a system with respect to the correct specification of the system. A system is partially correct if the final state of the system satisfies the correct specification, given that the initial state satisfies the specification of the  system \cite{NN07, T06}.

In the case of partial correctness, axiomatic semantics  provides a system of expressing and relating both the initial and final states of a system (precondition and post-condition, before and after transformation). The axiomatic semantics system is express with Hoare triple in the form of P\{C\}Q, where P, Q and C are pre and post-condition program respectively \cite{NN07}

However, partial correctness does not guarantee that a program terminate. Total correctness complements that with ensuring that the program terminates, and establish a relationship between the initial and final states of the program. Proving total correctness involve using direct mathematical proof to prove that each construct of the input model is translated into an equivalent construct or statements in the target output. While using mathematical induction to proof infinite behaviour of the system in the case of an non-terminating system [NN07]

We start with using traces to prove the partial correctness of the translation technique with using trace semantics to compare the behaviour of the source model and the translated models. First, we develop a software tool that automate the translation technique. Second, we develop an evaluation tool, which uses the translation tool to translate \verb!tock-CSP! process and then uses both FDR and UPPAAL as black boxes for generating finite set of traces for a given length. The structure of the evaluation tool is illustrated in Figure \ref{trace_analysis_system}. Therefore, partial correctness of the translation technique is supported by the trace sets being the same, when the coordinating actions are deleted. 






\begin{figure}[t!] %[H]
    \centering
%    \includegraphics[width=0.7\textwidth]{C3_figs/traceAnalysis.png}
    \includegraphics[width=\textwidth, height=0.25\textheight]{fig/traceAnalysis.png}
    \caption{Structure of the trace analysis system}
    \label{trace_analysis_system}
\end{figure}






In generating the trance, FDR was developed to produce only one trace (counterexample) at a time. So, based on the testing technique developed in \cite{NS08}, we developed a technique that repeatedly invokes FDR for generating traces until we get all the required traces set of the input \verb!tock-CSP!. This trace generation technique enables us to generate finite traces set of \verb!tock-CSP! specification with FDR. 



Similarly, based on the testing technique developed in \cite{LP07}, we developed another technique for generating finite discrete traces set of TA with UPPAAL.



So, based on this trace generation components, we develop the trace analysis in two stages. In stage 1, we generate traces of the input \verb!tock-CSP! and its corresponding translation using both FDR and UPPAAL, respectively. Then, we compare the traces, and if they did not match, we move to the second stage. FDR trace generation technique distinguishes and generate traces with different permutation. In contrast, generating traces with UPPAAL does not distinguishes traces with different permutations. So, in stage 2, we use UPPAAL to check if the traces of the input \verb!tock-CSP! process are acceptable traces of the translated TA. 







% --------- short version begin
This evaluation tool enables us to evaluate the translation technique by translating a list of formulated processes that pair all the considered constructors in the presented BNF in Definition \ref{dfn_CSPproc}. Also, we compare the performance of verifying deadlock freedom using both FDR and UPPAAL on the formulated processes. Details of the processes are available in a repository that contains the achieve of this work \cite{extendedVersion}. 


 \begin{figure}[t] 
     \centering
    \includegraphics [width=1\textwidth]{fig/PerformanceEgsHis.png}
    \caption{Performance analysis for comparing FDR and UPPAAL}
    \label{performanceGraph}
\end{figure}



For the analysis we conducted with the list of the processes, which cover the \verb!tock-CSP! operators we consider within the scope of this work, the results show that that using UPPAAL is at least three times faster than using FDR for verification. This shows a significant performance increase of UPPAAL over FDR.

A summary of the result is shown in graph Figure \ref{performanceGraph}. For the FDR, the maximum, minimum, average and standard deviation times are 0.0337s, 0.0312s, 0.03261801802s, 0.000573220281s respectively. While for UPPAAL, the maximum, minimum, average and standard deviation times are 0.0126s 0.0057s, 0.007948648649s, 0.001025126588s respectively.


For each process we measure the execution time for verifying deadlock freedom in each of the process ten times, and the average is recorded. Details of all the recorded times including the average times are in the repository that contains the research archieve \cite{extendedVersion}). Then we use the list of the average times to construct the graph in Figure \ref{performanceGraph}.  The longer (blue) bars show the average timing of FDR, while the shorter (red) bars show the average time of UPPAAL. This shows a significant performance increase of UPPAAL over FDR.



\subsection{Mathematical Proof}

\begin{cmt}
I will add the mathematical proof here.
\end{cmt}



%% ----------------------------- RELATED WORK
\section{Related Work}
\label{related_work}



Several types of researches explore using CSP in the verification of temporal specifications, especially in verifying real-time systems. Timed-CSP \cite{S10} is another popular extension of CSP that provides additional notations for capturing temporal specifications. Timed-CSP records the progress of time with a series of positive real numbers, which facilitates reasoning and verification of real-time systems.



However, the Timed-CSP does not enable specifying strict progress. Thus, traces of Timed-CSP becomes infinite, which is problematic for automatic analysis and verification \cite{R10}. So far, there is no tool support for verifying Timed-CSP models.



As a result of that, many researchers explore model transformations for supporting Timed-CSP with an automatic verification tool. Timed-CSP has been translated into \verb!tock-CSP! to enable using FDR for automatic verification \cite{O00}. The work provides a link for utilising the facilities of FDR in verifying Timed-CSP model. 

Also, Timed-CSP has been translated into UPPAAL to facilitates using the facilities of UPPAAL in verifying Timed-CSP. The work was initiated in \cite{DH08} and then subsequently improved in \cite{TS13}.


Additionally, Timed-CSP has been translated into Constraint Logic Programming (CLP)  that facilitates reasoning in verifying Timed-CSP, that is supported by constraint solver CLP(R) \cite{DP06}.


However, there is less attention in applying the same transformation techniques in improving \verb!tock-CSP! with a better approach for verifying real-time system.
An attempt for transforming TA into \verb!tock-CSP! was proposed in \cite{K11}. In this work, we consider the opposite direction for translating \verb!tock-CSP! into TA for UPPAAL to be able to utilise the facilities of UPPAAL in verifying \verb!tock-CSP! models.
 

Apart from CSP, model transformations have been used for improving other modelling notations. Circus has been translated into \lstinline{CSP||B} to enable using ProB for automatic verification \cite{KJ17}. Additionally, B has been translated into TLA+ for automatic validation with TLC \cite{HL14}. Also, the reverse of translating TLA+ to B has been investigated for automatic validation of TLA+ with ProB \cite{HL12}. Such that both B and TLA+ benefits from the resources of both TLC and ProB. 


\begin{cmt}  %---------------------------------------------------
New addition begins
\end{cmt}

Another approach of reducing the complexity refusal testing was provided in \cite{DR16}, which introduces a translation technique for using priority operator \cite{R10} to transform a question for refusal testing refinement into trace refinement. The technique is generalised to be applicable to the remaining three observational CSP models, namely acceptances, revivals, and finite linear observations \cite{R09}, all with the same motivation of reducing complexity and providing support for automatic verification for these four behavioural models. 

However, their translation technique \cite{DR16} is limited to finite linear-time. While our translation work targets at using  Timed Computation Tree Logic (TCTL) that is powerful enough to cover branching time. Part of the future work will expand the comparison of our translation work with their approach of translating the refusal testing into trace models. 

\begin{cmt}  %---------------------------------------------------
Addition ends
\end{cmt}





Model transformation is an established field which has been used for many decades in addressing computational problem. The novelty of this work is trace back to early model translation work, such as the translation of the timed variants of LOTOS into TA \cite{CO95, HG98}.  A recent survey provides rich collections of model transformations techniques and their supporting tools \cite{KM19}.



\section{Conclusion}
\label{conclusion}

%-------------  CONCLUSION  --------------------------------------------------

In this work, we presented a technique for translating \verb!tock-CSP! into TA for UPPAAL, which facilitates using UPPAAL for the verification of \verb!tock-CSP!. The result of this work shows significant increase in performance for using UPPAAL in the verification of \verb!tock-CSP! specifications. 

Additionally, this would provide an easier alternative of using TCTL in specifying liveness requirements that are difficult to specify and verify in \verb!tock-CSP!. Such possibility will be explored in the future work.

So far, we used trace analysis in justifying the partial correctness of the translation work. In the future, we are planning to apply mathematical reasoning to formally prove the total correctness of the translation technique.

Secondly, we are planning to explore using the translation technique in translating extensive case studies in translating \verb!tock-CSP! to UPPAAL. 


So far in this work, we translated the event tock into an action that is control by timed clock in UPPAAL. 
A next step in the work would be to relate the notion of tock to the notion of time in TA and get rid of tock.  This will help us to explore other interesting facilities of UPPAAL in verifying temporal specifications.





==> zz_del/all__.tex <==



\section{Introduction}   %%%-----------------------------------------------------

Communicating Sequential Processes (CSP) is an established process algebra that provides formal notations for both modelling and verification of concurrent systems \cite{R10, S10, H78}. Using CSP for verification has been supported with an automatic model-checker FDR \cite{TP14, R10}. CSP and its modelling approaches have contributed to understanding the complexity of concurrent systems  \cite{S10}. 


%tockCSP------------------------------------------------------------------

Interest in using CSP motivates the introduction of time into its constructs; \verb!tock-CSP! provides an additional event $tock$ to record the progress of time. This addition enables using CSP for modelling temporal specifications in a format that is suitable for formal analysis and verification. The structure of \verb!tock-CSP! retains the original structure of CSP and utilises the existing works and tools for CSP. Thus, automatic verification is supported by FDR. As a result of that,  \verb!tock-CSP! has been used in the verification of real-time systems such as security protocols \cite{NS00} and railways systems \cite{YF12}. Recently, \verb!tock-CSP! has been used for capturing the semantics of RoboChart, a domain-specific language for modelling robotics system \cite{MR16}. Additionally, a recent extension of \verb!tock-CSP! provides notations for specifying budgets and deadlines for effective modelling and verification of temporal specifications \cite{JP19}.



In this work, we add a technique for translating \verb!tock-CSP! into TA that enables using the facilities of UPPAAL \cite{BD06} in verifying \verb!tock-CSP! models. UPPAAL is a tool-suite for modelling and verifying real-time systems using TA and temporal logic. Both temporal logic and refinement are powerful approaches for model checking \cite{G08}. However, each one of these two approaches has different concept of modelling and verifying system behaviour. 

On one hand, the refinement approach models both the system and its specifications with the same constructs, like in \verb!tock-CSP!, which enables asking a question if the system captures the specification of its requirement \footnote{Generally, a model-checker is used to determine if the system behaviours are subset of the requirement specification, in other word if the system refines the specification} \cite{R10, S10}. On the other hand,  temporal logic has logical constructs for formulating system specifications, which enables asking a question, if a system is a model for a logical formula of the specification ($system \models formula$) \cite{CE86}. Using both temporal logic and refinement have been supported with automatic verification tools, such as UPPAAL \cite{BD06} and FDR \cite{TP14}, respectively.


Previously, Lowe has investigated the relationship between the refinement oriented approach (with CSP) and the temporal logic-oriented approach. The result shows that, in expressing temporal logic checks using the refinement approach, it is necessary to use the infinite refusal testing model of CSP. The work highlights that the most challenging part is capturing the expressiveness power of temporal logic in specifying the availability of an event (liveness specification). A desirable specification that ensure that a system performs something good.
% or something bad will never happen in the system. 

In addition, due to the difficulty of capturing refusal testing, automatic support becomes problematic. A previous old version of FDR supports refusal testing, but not the recent efficient version of FDR \cite{fdr}.


Additionally, the work \cite{G08} proves that simple refinement checks cannot cope with the expressive power temporal logic, specifically in expressing three operators: $eventually$  ($\diamond p$: $p$ will hold in some subsequent state),  $until$ ($p  \mathcal{U} q$: $p$ holds in every state until $q$ hold)  and $negation$  ($\neg ( \diamond p$): $p$ will never hold in the subsequent states). The problem of capturing negation operator is  mainly due to its connection with operator $eventually$. All these three operators expresses a behaviour that is captured by infinite traces. 




In the case of TA for UPPAAL, temporal logic formula is capable of expressing  specifications of an infinite trace of a system \cite{ST18}, which can be seen in expressing liveness specifications. Therefore, this translation work will facilitate using the resources of temporal logic (and UPPAAL for automatic support) in checking requirements specifications that are difficult to specify with refinement models, specifically \verb!tock-CSP! models.  This will include liveness specifications, in addition to the three operators that cannot be specify in refinement models. The operators are eventually $(\diamond)$,  $ until (\mathcal{U}$) and  $negation (\neg) $, as illustrated in Example \ref{ads}.



\begin{example} %{A translation of an Automatic Door System (ADS)} \\
\label{ads}
Consider an Automatic Door System (ADS) that opens a door, and then after at least one-time unit, the system closes the door in synchronisation with a lighting controller, which turns-off the light after closing the door. In \verb!tock-CSP!, a description of ADS is as follows:

\begin{lstlisting}
Controller = open -> tock -> close -> Controller

Lighting = close -> offLight -> Lighting

ADS = Controller [|{close}|] Lighting

\end{lstlisting}



\end{example}



The system ADS has two components, \lstinline{Controller} and \lstinline{Lighting}. The component \verb!Controller! opens and closes the door after an interval of at least one unit time. \lstinline{Lighting} turns-off the light after closing the door. The two components synchronise on the event \lstinline{close}, which enables the lighting controller to turn-off the light. 



In particular, in using \verb!tock-CSP!, there is no straightforward way of specifying requirements for checking `if the system will eventually turn-off the light when the environment is ready to switch-of the light'. However, temporal logic provide a direct construct for specifying these kinds of requirements in a simple form. For instance, in temporal logic, using the syntax of UPPAAL \footnote{UPPAAL uses $A\diamond$ for specifying liveness specifications, while the symbol $\diamond$ or $F$ are also commonly use symbols for specifying liveness in the litereture of temporal logic} for specifying liveness specification, the requirement is specified as follow.
\begin{itemize}
    \item $A\diamond$ \lstinline{offLight}  \\ 
        - - \textit{Eventually the system should turn-off the light, if the environment permits.}
    % - - \textit{Can the system always turns-off the light, if the environment permits.}
\end{itemize}
    



In verifying the correctness of the translation technique, we follow a series of steps.  First, we formulate a systematic list of interesting \verb!tock-CSP!  processes, which pair all the constructs of \verb!tock-CSP! within the scope of this translation work. Second, we use the developed translation technique and its tool to translate the formulated processes into TA for UPPAAL.  Third, we developed another tool that assists us in generating and comparing finite traces of the input \verb!tock-CSP! models and the traces of the translated TA models, with the support of both FDR and UPPAAL, respectively. This provides evidence that the translated TA captures the behaviour of the input \verb!tock-CSP! models.

Describing the translation technique is one of the challenging task we faced in this work,
So, we take advantage of the concise construct of Haskell \cite{H16} in describing the technical part of the work. Haskell is a functional programming language, which we use for expressing, implementing and evaluating the translation technique. Both concise and expressive power of Haskell helps us in providing a precise description of the translation technique as a list of translation rules.




% Outline of the paper  ----------------------------------------------------------------------
The structure of the paper is as follows. Next, Section \ref{background} provides brief backgrounds that are essential for understanding the translation technique.  In Section \ref{trans_rule}, we describe an overview of the translation technique. In Section \ref{evaluation}, we discuss an evaluation of the translation technique. In Section \ref{related_work}, we highlight relevant related work, and also discuss a brief comparison with this work. Finally, Section \ref{conclusion}, we highlight future work and also provide a conclusion for the paper.





%%  --------------------  BACKGROUND -----------------------
\section{Background}
\label{background}

This section discusses the required background for understanding the translation work. We begin by discussing the notations of \verb!tock-CSP! and then discuss the target outcome of the translation work, that is a list of TA that is suitable for UPPAAL tool. 


%CSP and \verb!tock-CSP!
\subsubsection{tock-CSP} is an extension of CSP that provides notation for modelling processes and their interactions. In \verb!CSP!, there are varieties of constructs, which includes basic processes such as \verb!SKIP! and \verb!STOP!. \verb!SKIP! expresses a successful termination while \verb!STOP! expresses a deadlock behaviour that can no longer perform any communication. Also, there are operators such as \verb!prefix (->)!, which describes an event that leads up to a process. For example, the process \verb!move->SKIP! specifies the behaviour of a system that moves and then terminates. 



Furthermore, there are additional binary operators such as sequential composition (;), which concatenates two processes serially. For instance, a process \verb!P3 = P1;P2!, which expresses a process that behaves as process \verb!P1!, and then after successful termination of the process \verb!P1!, the process \verb!P3! behaves as process \verb!P2!. For example, the process \verb!Ps = (move->SKIP);(turn->SKIP)!, specifies a system that moves, turns and then terminates, successfully.


There are other binary operators for composing processes in different shapes, such as concurrency, choice and interrupt. Also, CSP provides a special event $tau \ ( \tau ) $ that represents invisible actions that are internal to a system, specifically for internal communication of a system that are hidden from the operating environment. The collection of these operators provides a rich set of constructs for modelling untimed systems. A comprehensive detail of CSP constructs, together with examples, are available in these books \cite{R10, S10}. 


Consequently, \verb!tock-CSP! enriches the notations with adding a special event \verb!tock!, which records the progress of time \cite{R10}. Each event \verb!tock! specifies a single unit of time. For example,  a process \verb!Pt= move->tock->tock->turn->SKIP! specifies the behaviour of a system that moves, and then after at least two-time units, the system turns and then terminates. The addition of the special event \verb!tock! enables specifying temporal specification in a format that is suitable for formal analysis of timed system \cite{TP14}. 


In this work, we provide a translation techniques that facilitates using the expressive power of temporal logic in verifying real-time system. We provide a BNF for \verb!tock-CSP! that describes the essential constructs we consider in developing the translation technique and its supporting tool. Part of the BNF is presented in Definition \ref{dfn_CSPproc} using the syntax of Haskell. The complete BNF is available in an extended report of this work \cite{extendedVersion}. The BNF forms the basic foundation of this translation work, and provides a good link for other related works and tools that are associated to \verb!tock-CSP!.

\begin{definition} \textbf{Data definition of \lstinline{CSPproc}} 
\label{dfn_CSPproc}


\begin{verbatim}
data CSPproc =   STOP | SKIP | Prefix Event CSPproc 
                | Interleave CSPproc CSPproc 
                | GenPar CSPproc CSPproc [Event] 
                | Interrupt CSPproc CSPproc 
                | ...
\end{verbatim}
\end{definition}




\subsubsection{Timed Automata for UPPAAL}
TA provides graphical notations for modelling hybrid systems. In UPPAAL, systems are modelled as a network of TA with additional variables. Mathematically, a TA is defined as a tuple $(L, l_0, C, A, E, I)$, where $L$ is a set of locations such that $l_0$  is the initial location, $C$ is a set of clocks, $A$ is a set of actions, $E$ is a set of edges that connects the locations $L$, and $I$ is an invariant that is associated with a location $l \in L$. So, an edge $E$ is defined as $E \subseteq (L \times A \times B(C) \times 2^C \times L)$, which describes an edge from location $l \in L$ that is triggered by an action $a \in A$, guarded with a guard $B(C)$, and associated clocks $C$  that are reset on following an edge $e \in E$ to a location $l \in L$. Finally, $I$ is a function that assigns invariant to a location $I:L \longrightarrow B(C)$   \cite{BD06, B11}.


In UPPAAL, a system is modelled as network of TA that communicate over channels or variables. A sending channel is decorated with exclamation mark $(c!)$ while the corresponding receiving channel is decorated with question $(c?)$. This enables TA to communicate by synchronising over complementary actions  $a!$ and $a?$, for sending and receiving over the channel $a$. For urgency, there are urgent channels that do not allow delay. Also, there is broadcast channel that communicates with multiple TA, in the form of one-to-many communication simultaneously (one sender with multiple receivers). For instance, in a broadcast channel $b$, a single TA with the action $b!$ synchronises with all the TA that performs $b?$.

In addition, there are other constructs, such as urgent and committed types of location. An urgent location does not allow time to pass. While the committed location is an urgent location that must take the next transition before any other transition. The committed location expresses atomicity, specifically for expressing compound action, which spans multiple transition that must be executed as a unit. An invariant expressions is also provided for specifying and enforcing progress in a location. 




%Env TA
Overall, UPPAAL provides graphical notations for modelling system as a network of TA for the components of a system that communicate with one another and the operating environment, which is also modelled as a TA. For instance, the collection of TA in Figure \ref{ta_ads}, which will be explain later in more details. For specifications, UPPAAL uses subset of Timed Computational Tree Logic (TCTL) \cite{B09}  for specifying system properties that can be verify automatically  \cite{LP07, LP97, BD06}.  


\section{An Overview of the Translation Technique}
\label{trans_rule}

The translation technique produces a list of small TA, such that the occurrence of each \verb!tock-CSP! event is captured in a small TA with an UPPALL's action,  which records an occurrence of the translated event. The action has the same name as the translated event from the input \verb!tock-CSP! process. The technique composes these small TA into a network of TA, which captures the behaviour of the input \verb!tock-CSP! model. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure} %[H]
\subfigure{\includegraphics [width=0.9\textwidth, height=0.4\textwidth]{EgGenParGray/taGenPar0_0.png}}

\subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix00_1.png}}
 \hspace{0.1\textwidth}
\subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix00_2.png}}

\subfigure{\includegraphics [width=0.55\textwidth]{EgGenParGray/taPrefix00_3.png}}
\subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/SyncTA.png}}

\subfigure{\includegraphics [width=0.55\textwidth]{EgGenParGray/taPrefix01_2.png}}
\subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix01_3.png}}

 \hspace{0.1\textwidth}
% \subfigure{\includegraphics [width=0.3\textwidth]{EgGenParGray/taWait_n01_4.png}}
\subfigure{\includegraphics [width=0.9\textwidth]{EgGenParGray/Env.png}}
\caption{A list of networked TA for the translation of the process ADS}
\label{ta_ads}

\end{figure}



For example, a translation of the process ADS from Example \ref{ads}, which produces a network of small TA in Figure \ref{ta_ads}. Details of the translated TA are as follows. Starting from the top-left corner, the first TA captures the translation of concurrency that starts the two processes \lstinline{Controller} and \lstinline{Lighting} concurrently in two possible orders, either \lstinline{Controller} then \lstinline{Lighting} or vice versa,  depending on the operating environment, and then also waits on state \lstinline{s5} for their termination actions in the two possible orders, either \lstinline{Controller} then \lstinline{Lighting} or vice versa,  depending on the process that terminates first, and then after termination of the other process, the whole system terminates with the action \lstinline{finishID0}.


The second, third and fourth TA capture the translation of the process \lstinline{Controller}. The second TA captures the occurrence of the event \verb!open!. The third TA captures the occurrence of the events \verb!tock?! (with a question mark for synchronising with the environment in recording the progress of time because all processes synchronise with progress of time). Additional details will follow in describing the translation technique.  The fourth TA captures the occurrence of the event \verb!close!, which needs to synchronise with a synchronising controller, that is the fifth TA in the list of the TA.

The sixth and seventh TA capture the translation of the process \lstinline{Lighting}. The sixth TA captures the translation of the event \verb!close!, which also needs to synchronise with the synchronisation controller (fifth TA) on the event \verb!close!. The seventh TA captures the event \verb!offLight!. Finally, the last TA is an environment TA that has co-actions for all the translated events. Also, the environment TA serves the purpose of 'closing' the overall system (in contrast to having an "open system") as required for the model checker. In this last TA, we use the variable $start$ to construct a guard $start==0$ in the environment TA that blocks the environment from restarting the system. This concludes the description of the list of TA for the translated behaviour of the system ADS.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Explanation of TA for ADS
% \paragraph{}
\vspace{0.2cm}


An alternative of using a list of small TA is using a single large TA that captures the behaviour of the translated \verb!tock-CSP! process. However, the main reason for using a list of small TA is coping with the compositional structure of \verb!tock-CSP!, which is not available in TA \cite{DH08}. 

For instance, it can be argued that a linear process constructed with a series of prefix operators can be translated into linear TA. However, the compositional structure of \verb!tock-CSP! is not suitable for this straight forward translation. A network of small TA provides enough flexibility for composing TA in various ways to capture the behaviour of the original \verb!tock-CSP! process.  



In constructing the network of TA, we use additional \textbf{\textit{coordinating actions}} that link the small TA into a network.  For example, in Figure \ref{ta_ads}, the TA communicates over the channels \verb!startIDADS!, \verb!startID00_1!, \verb!startID01_2!. The coordinating actions link the small TA into a network of TA to establish the flow of the translated \verb!tock-CSP! process. For instance, the channel \verb!startIDADS! forms a link that connect the environment TA (last TA in Figure \ref{ads}) with first TA, on performing the actions \verb|startIDADS!| and \verb!startIDADS?!, respectively. Likewise, the channel \verb!startID00_1! connects the first TA with the second TA, on performing the actions \verb|startID00_1!| and \verb!startID00_1?!, respectively.  A precise definition of the coordinating action is in Definition \ref{coordinating_action}, which also describes the types of coordinating actions we use in developing the translation technique.




\begin{definition}

 \textbf{Coordinating Action} is an UPPAAL action, and we use six types of coordinating actions as follows:


\begin{itemize}
\item \textbf{Flow action} coordinates a link between two TA for capturing the flow of the behaviour. 
% of the input \verb!tock-CSP! process. 
    
\item \textbf{Terminating action} records termination information, in addition to coordinating a link between two TA.


\item \textbf{Synchronisation action} coordinates a link between a TA that participate in a multi-synchronisation action and a TA for controlling the multi-synchronisation. 


\item \textbf{External choice action} coordinates external choice, such that choosing one of the TA composed with external choice blocks the other alternative choices TA that participate in the choice.


\item \textbf{Interrupting action} initiates an interrupting transition that enables a TA to interrupt other TA.
% , for the case of translating processes that are composed with an interrupting operator in \verb!tock-CSP!.

\item \textbf{Exception action} coordinates a link between a TA that raises an exception and a control TA that handle the exception. 
\end{itemize}
\label{coordinating_action}
\end{definition}

\vspace{-0.5cm}
The name of each coordinated action is unique for ensuring correct flow of the translated TA. In our implementation, the name of the flow actions are generated in the form \verb!startIDx!, where \verb!x! is either a natural number or the name of the input \verb!tock-CSP! process. This can be seen in Example \ref{ads}, the name of the channel \verb!startID00_1! that connects the first TA with the second TA.

Likewise, the names of the remaining coordinating action follow the same pattern; \verb!keywordIDx!, where  \verb!keyword! is a designated word for each of the coordinating actions: \verb!finish! for terminating action,  \verb!ext! for external choice action, \verb!intrp! for interrupting action, and \verb!excp! for exception action. Similarly, the name of a synchronising action is in the form \verb!eventName___sync!; an event name appended with the keyword \verb!___sync! to differentiate a synchronising action from other actions. 



We provide termination actions for capturing essential termination information from the input \verb!tock-CSP!. This is essential is the cases where a TA needs to communicate a successful termination for another TA to proceed. For example, in the case of translating sequential composition \lstinline{P1;P2} where the process \lstinline{P2} begins only after a successful termination of the process \lstinline{P1}.  



Additionally, for each translated \verb!tock-CSP! specification, we provide an environment TA, like the the last TA in Figure \ref{ads}. Also, the environment TA closes the overall model as part of the requirements for UPPAAL model checker. The environment TA has corresponding co-actions for all the translated events of the input \verb!tock-CSP! model. In addition, the environment TA has two coordinating actions that link the environment TA with the network of the translated TA. First, a flow action that links the environment with the first TA in the list of the translated TA. Also, this first flow action is the starting action that activates the behaviour of the translated TA. Second, a terminating action that links back the final TA in the list of the translated TA to the environment TA, and also records a successful termination of a process and closes the whole system. A precise definition of the structure of environment TA is in Definition \ref{environment_TA}.



% \vspace{0.2cm}

\begin{definition} 
\textbf{Environment TA} models an explicit environment for UPPAAL model. The environment TA has one state and transitions for each co-action of all the events in the original \verb!tock-CSP! process, in addition to two transitions for the first starting flow action and the final termination co-action. 

\label{environment_TA}
\end{definition}



Next, in translating multi-synchronisation, we adopt a centralised approach developed in \cite{O05} and implemented using Java in \cite{F05}. The approach described uses  a separate centralised controller for controlling multi-synchronisation events. Here, we use a separate TA with UPPAAL broadcast channel to communicates synchronising information among synchronising TA and a control TA.
% that control the synchronising action.

% In Example \ref{ads}, 

An example can be seen in Figure \ref{ads}, where we illustrate the strategy in translating synchronising action \verb!close!, which synchronises the two processes \verb!Controller! and \verb!Lighting!. In Figure \ref{ta_ads}, the fifth TA captures the translation of the event \verb!close!, which synchronises the process \lstinline{Controller} and the process \lstinline{Lighting}, that is fourth and sixth TA in the translated TA. In the fifth TA, the broadcast channel \verb!close___sync! synchronises the fourth and sixth TA. A precise definition of the synchronisation TA is provided in Definition \ref{dfn_syncTA}.



\begin{definition} \textbf{Synchronisation TA} coordinates a synchronisation action. The structure of synchronisation TA has an initial state and a committed state for each synchronisation action, such that each committed state is connected to the initial state with two transitions. The first transition from the initial state has a guard and an action. The guard is a conjunction of guards from each process that synchronises on that synchronisation action. The guard is enabled when all the processes are ready for the synchronisation, which also enables the TA to performs the associated action that notifies the environment for the occurrence of the synchronisation action. Then, in the second transition, the TA broadcasts the synchronisation action to all the processes that synchronise on the synchronisation action.


\label{dfn_syncTA}
\end{definition}




To ensure that the synchronisation TA synchronises with the required number of TA that participate in a synchronisation channel, we provide guards that block the broadcast channel until all the required TA are ready for the synchronisation. When the guard become ready, it enables the synchronising TA to broadcast the synchronisation action such that all the participating will synchronise and progress in performing their subsequent actions.






%%%%%%%%%%%%%%%%%% ---  OVERVIEW OF THE TRANSLATION TECHNIQUE
Furthermore, in \verb!tock-CSP!, a process can be interrupted by another process when the two processes are composed with an interrupt operator (\verb!/\!). This is due to the compositional structure of \verb!tock-CSP!. However, in the case of TA, an explicit transition is needed for expressing an interrupting action,  which enables a TA to interrupt another one. Thus, in this translation work, we provide an additional transition for capturing interrupting event using an interrupting action, as defined in Definition \ref{coordinating_action}.


For example, given a process \verb!Pi = P1/\P2!, the process \verb|P1| can be interrupted by process \verb|P2|. Thus, in translating each event of process \verb|P1|, we provide additional transitions for the initials \footnote{Initials are the first visible events of a process.} of the interrupting process \verb|P2|. The additional transitions enable the translated behaviour of process \verb|P2| to interrupt the translated behaviour of process \verb|P1| at any stable state of its behaviour.




Similarly, in translating external choice, we provide additional transitions that enable the behaviour of the chosen process to block the behaviour of the other processes. Initially, in the translated TA, all the initials of the translated processes are available such that choosing one of the processes block the other alternative choices with the provided co-actions for translating external choice, as defined in Definition \ref{coordinating_action}.



For example, given a process \verb!Pe = P1[]P2! that composes \verb!P1! and \verb!P2! with operator external choice; such that \verb!Tp! is a list of TA for translating the process \verb!P!. Similarly, let \verb!Tp1! and \verb!Tp2! be lists of TA for translating the processes \verb!P1! and \verb!P2!, respectively.  In the first TA of the list \verb!Tp1!, we provide additional transitions for the initials of \verb!P2! such that choosing \verb! Tp2! blocks \verb!Tp1!. Similarly, in the first TA  of the list \verb!Tp2!, we provide additional transitions for the initials of \verb!P1! such that choosing \verb!Tp1! blocks the behaviour \verb!Tp2!. Additional examples are also available in an extended report \cite{extendedVersion}.




Also, in \verb!tock-CSP!, an event can be renamed or hidden from the environment. In translating renaming, the translation technique carries a list of renamed events, such that before translating each event, the translation technique checks if the event is  renamed, and then translate the event appropriately with the corresponding new name. In the like manner, if an event is part of the hidden events, the translation technique carries a list of hidden events, such that on translating hidden event the technique uses a special name $itau$ in place of the hidden event. The event $itau$ has similar meaning with the event $tau$, which represents hidden event in FDR. We make them different to differentiate the translated hidden event $itau$ from the event $tau$, mainly for the purpose of analysis.


In \verb!tock-CSP!, the event \verb!tock! records the progress of time. Thus, we translate the event \verb!tock! into a corresponding action \verb!tock! for recording the progress of time in the translated TA with a broadcast channel which enables the translated TA to synchronise in recording the progress of time. The translated action \verb!tock! is guarded with clock $clk<=1$ which trigger the action \verb!tock! and reset the clock $clk=0$. The action \verb!tock! is broadcast by the environment TA, which forces the TA to synchronise and record the progress of time using their corresponding co-actions \verb!tock?! (with question mark), as illustrated in Figure \ref{ta_ads}. In particular, the last TA, which models the environment, has a transition with an action \verb!tock! that is guarded with the expression $ck <= 1$, and resets the clock $ck=0$ to zero on following the transition.
 


In translating non-determinism, TA has a non-determinism facility, using silent transitions that enables a TA to silently takes any of the silent transitions. We translate non-deterministic choice into silent transitions, such that the translated TA follow one of the silent transitions non-deterministically. Also, urgency is translated into the corresponding urgent channel in UPPAAL. However, divergence is not part of the construct that we consider in this translation work,  because divergence is a sign of bad behaviour. This completes an overview for describing the strategy we follow in developing the translation technique.




%----------------------- Sample rule for translation of STOP
\subfile{a4_ruleStopNew}



%  ---------------------------------- EVALUATION 
\section{Evaluation}
\label{evaluation}

To ensure that the translation work is correct, we have to prove soundness. A formal translation ensures that interesting properties of the source model are preserved in the targeted translated models. This is determined by comparing the behaviours of the source model and the behaviours of the translated model \cite{T06, NN07, KM19, B81}. 

In this work, we use traces to compare the behaviour of the input \verb!tock-CSP! models and the traces of the translated TA models. First, we have developed a tool that automates the translation technique. Second, we have developed an evaluation tool, which uses the translation tool to translate \verb!tock-CSP! model into TA, and then uses both FDR and UPPAAL as black boxes in generating a finite set of traces. The structure of the evaluation tool is shown in Figure \ref{trace_analysis_system}. 







\begin{figure}[t!] %[H]
    \centering
%    \includegraphics[width=0.7\textwidth]{C3_figs/traceAnalysis.png}
    \includegraphics[width=\textwidth, height=0.25\textheight]{fig/traceAnalysis.png}
    \caption{Structure of the trace analysis system}
    \label{trace_analysis_system}
\end{figure}






In generating traces, like most of the model-checkers, FDR produces only one trace (counterexample) at a time. So, based on the testing technique developed in \cite{NS08}, we developed a trace generating technique that repeatedly invokes FDR for generating traces until we get all the required traces set of the input \verb!tock-CSP!. Thus, we use the trace generation technique to generate finite traces set of the input \verb!tock-CSP! models with FDR. Similarly, based on the testing technique developed in \cite{LP07}, we developed another trace generation technique, which uses UPPAAL in generating finite discrete traces set for the translated TA models. 

Consequently, these two trace generation techniques serve as component for our trace analysis tool, which has two stages of analysing traces. In the first stage, we generate traces of the input \verb!tock-CSP! and its corresponding translated TA, using both FDR and UPPAAL, respectively. Then, we compare the generated traces, and if they did not match, we move to the second stage for further analysis. In FDR, the trace generation technique is capable of generating and detecting traces with different permutation. Thus, we are able to generate traces with various structure. In contrast,  UPPAAL is not capable of detecting traces with different permutations because UPPAAL uses logical formula in generating traces \cite{LP07, BD06}. 


Basically, UPPAAL was developed for checking if a system satisfies a logical formula for the requirement specifications, irrespective of the behaviour of the system. For example, UPPAAL does not distinguish between the two traces $ \langle e1, e2, e3 \rangle$ and  $\langle e1, e3, e2 \rangle \}$, as long as both of them satisfy the specification formula. The two traces contain the same three actions, but the action $e2$ and $e3$ occur in different order. However, FDR is capable of generating both traces that have different structure. Additional examples together with details implementation of these traces generation techniques are available in an extended report \cite{extendedVersion}. Thus, in the second stage, we use UPPAAL to check if the traces of FDR are acceptable traces of the translated TA. 







% --------- short version begin
We use this evaluation tool in evaluating the translation technique by translating a list of systematically formulated \verb!tock-CSP! processes that pair all the essential constructors of \verb!tock-CSP! within the scope of this translation work, which produces 111 processes of smaller sizes that are not more than five state in size. An archives of the processes and their translations are available in this repository \cite{extendedVersion}




%  Test cases ----------------------------------------
In addition, the translation technique have been tested in various test cases such as an automated barrier to a car park \cite{S10}, thermostat for monitoring ambient temperature \cite{S10}, simple Automated Teller Machine (ATM)  \cite{R05} and  Bookshop Payment system \cite{S10}, and Railway crossing system \cite{R10}. An overview structure of the processes is provided in Table \ref{table_caseStudies}. Traces are not included because the systems have infinite traces. This is the nature of \verb!tock-CSP! models and other timed systems, they are reactive system with non-terminating processes that must allow time to progress \cite{R10}. Even the simple basic process such as $STOP$ have infinite sequence of $tock$ as their traces.




% A reader may like to know the size of these test cases. However, all these test cases are reactive system, which means that, they are non terminating process that have infinite traces. This is the nature of \verb!tock-CSP! models and other time systems, they are non-terminating process that must allow time to progress \cite{R10}. Even the simple basic process such as $STOP$ have infinite sequence of $tock$ as their traces.




\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|}  \hline \hline
System &	States &	Transitions	 &   Events	 \\ \hline
ATM		     &     15  &	33           &  15	     \\ \hline
AutoBarrier	 &     35	&   84	         &  10	    \\  \hline
PaymentSystem & 	7	&   32	        &    9	   \\   \hline
Rail Crossing & 	80	&   361	        &   12	   \\   \hline
Thermostat	  &  	7	&   16	        &   5	   \\   \hline \hline
    \end{tabular}
    \caption{Profiles of the case studies system}
    \label{table_caseStudies}
\end{table}




% Case Studies		Average Timing	States	Transitions	Events	State/Transition
% ATM	FDR	0.0051	15	33	15	0.4545454545
% 	UPPAAL	0.0084				
% AutoBarrier	FDR	0.0059	35	84	10	0.4166666667
% 	UPPAAL	0.0134				
% PaymentSystem	FDR	0.0048	7	32	9	0.21875
% 	UPPAAL	0.0011				
% Rail Crossing	FDR	0.0054	80	361	12	0.2216066482
% 	UPPAAL	0.0072				
% Thermostat	FDR	0.0052	7	16	5	0.4375

%------------------------------------------------------
However, trace analysis is limited to establishing correctness for finite set of traces. Proving correctness considering the complete set of traces involves using mathematical proof to prove that each construct of the input model is translated into an equivalent construct or statements in the target output. This is normally achieved using structural induction in providing proof for infinite behaviour of a system, especially for the case of a non-terminating system \cite{NN07}.  A preliminary proof for the base case of the structural induction is provided in the next section.





\subsection{An Initial Mathematical Proof}
% \subsection{An Initial/Early/Preliminary Mathematical Proof}


%%-------------------------------Math proof
\subfile{mathProof}




%% ----------------------------- RELATED WORK
\section{Related Work}
\label{related_work}



Several researches explore using CSP in verifying temporal specifications, due its potential capability of verifying real-time systems. Timed-CSP \cite{S10} is another popular extension of CSP that provides additional notations for capturing temporal specifications. Unlike \verb!tock-CSP!, Timed-CSP records the progress of time with a series of positive real numbers, which facilitates reasoning that is suitable for verifying real-time systems.



However, the approach of Timed-CSP is lacking in specifying strict progress of time, neither deadline nor urgency. And also traces of Timed-CSP becomes infinite in nature, which is problematic for automatic analysis and verification \cite{R10}. In addition, there is no tool support for verifying Timed-CSP models.



As a result of that, many researchers choose to explore model transformations in supporting Timed-CSP with an automatic verification tool. Thus, Timed-CSP has been translated into \verb!tock-CSP! to enable using FDR for automatic verification \cite{O00}. The work provides a link for utilising the facilities of FDR in verifying Timed-CSP model. 

Also, Timed-CSP has been translated into UPPAAL to facilitates using the facilities of UPPAAL in verifying Timed-CSP. The work was initiated in \cite{DH08} and then subsequently improved in \cite{TS13}. Additionally, Timed-CSP has been translated into Constraint Logic Programming (CLP)  that facilitates reasoning in verifying Timed-CSP, that is supported by constraint solver CLP(R) \cite{DP06}.


However, there is less attention in applying the same transformation techniques in improving \verb!tock-CSP! with a better approach for verifying real-time system. An attempt for transforming TA into \verb!tock-CSP! was proposed in \cite{K11}. Whereas in this work, we consider the opposite direction for translating \verb!tock-CSP! into TA for UPPAAL to be able to utilise the facilities of TA and UPPAAL in verifying \verb!tock-CSP! models.
 


% \begin{cmt}  %---------------------------------------------------
% New addition begins
% \end{cmt}

Furthermore, another approach of reducing the complexity of refusal testing was provided in \cite{DR16}, which introduces a translation technique for using priority operator \cite{R10} to transform a question for refusal testing refinement into trace refinement. The technique is generalised to be applicable to the remaining three observational CSP models, namely acceptances, revivals, and finite linear observations \cite{R05}, all with the same motivation of reducing complexity and providing support for automatic verification for these four behavioural models. 

However, their translation technique \cite{DR16} is limited to finite linear-time. While our translation work targets at using  Timed Computation Tree Logic (TCTL) that is powerful enough to cover branching time. Part of the future work will expand the comparison of our translation work with their approach of translating the refusal testing into trace models. 

% \begin{cmt}  %---------------------------------------------------
% Addition ends
% \end{cmt}

Apart from CSP and TA, model transformations have been used for improving various formal modelling notations. For instance, Circus has been translated into \lstinline{CSP||B} to enable using the tool ProB for automatic verification \cite{KJ17}. Additionally, the language B has been translated into TLA+ for automatic validation with TLC \cite{HL14}. Also, the reverse of translating TLA+ to B has been investigated for automatic validation of TLA+ with ProB \cite{HL12}, such that both B and TLA+ benefit from the resources of each other, specifically their supporting tools ProB and TLC, respectively. 


Model transformation is an established field which has been used for many decades in addressing computational problem. The novelty of this translation work is trace back to early days of model translation works, such as the translation of the timed variants of LOTOS into TA \cite{CO95, HG98}.  A recent survey on model translation provides rich collections of model transformations techniques and their supporting tools \cite{KM19}.



\section{Conclusion}
\label{conclusion}

%-------------  CONCLUSION  --------------------------------------------------

In this work, we presented a technique for translating \verb!tock-CSP! into TA for UPPAAL, which facilitates using the facilities of temporal logic and automatic support with UPPAAL in the verifying \verb!tock-CSP! models. Additionally, this translation would provide an easier alternative of using TCTL in specifying liveness requirements that are difficult to specify and verify in \verb!tock-CSP!. Also, the result of this work sheds additional insight on the complex relationship between \verb!tock-CSP! and TA, as well as the connection between the two popular model checking approaches: refinement model and temporal logic model.

So far, in this work, we used trace analysis in justifying the correctness of the translation work. In the future, we are planning to complete the mathematical proof for the total correctness of the translation technique. Secondly, we are planning to explore using the translation technique in translating extensive case studies that can help us in improving the translation work.
% of \verb!tock-CSP! to UPPAAL.  


Additionally, currently, we translated the event \verb!tock! into an action that is controlled by a timed clock in UPPAAL.  
A recommended next step in this work would be to relate the notion of \verb!tock! to the notion of time in TA and get rid of $tock$ as an action.  This additional extension will help us in exploring additional interesting facilities of UPPAAL for verifying temporal specifications.





==> zz_del/all___.tex <==



\section{Introduction}   %%%-----------------------------------------------------

Communicating Sequential Processes (CSP) is an established process algebra that provides formal notations for both modelling and verification of concurrent systems \cite{R10, S10, H78}. Using CSP for verification has been supported with an automatic model-checker FDR \cite{TP14, R10}. CSP and its modelling approaches have contributed to understanding the complexity of concurrent systems  \cite{S10}. 


%tockCSP------------------------------------------------------------------

Interest in using CSP motivates the introduction of time into its constructs; \verb!tock-CSP! provides an additional event $tock$ to record the progress of time. This addition enables using CSP for modelling temporal specifications in a format that is suitable for formal analysis and verification. The structure of \verb!tock-CSP! retains the original structure of CSP and utilises the existing works and tools for CSP. Thus, automatic verification is supported by FDR. As a result of that,  \verb!tock-CSP! has been used in the verification of real-time systems such as security protocols \cite{NS00} and railways systems \cite{YF12}. Recently, \verb!tock-CSP! has been used for capturing the semantics of RoboChart, a domain-specific language for modelling robotics system \cite{MR16}. Additionally, a recent extension of \verb!tock-CSP! provides notations for specifying budgets and deadlines for effective modelling and verification of temporal specifications \cite{JP19}.



In this work, we add a technique for translating \verb!tock-CSP! into TA that enables using the facilities of UPPAAL \cite{BD06} in verifying \verb!tock-CSP! models. UPPAAL is a tool-suite for modelling and verifying real-time systems using TA and temporal logic. Both temporal logic and refinement are powerful approaches for model checking \cite{G08}. However, each one of these two approaches has a different concept of modelling and verifying system behaviour. 

On one hand, the refinement approach models both the system and its specifications with the same constructs, like in \verb!tock-CSP!, which enables asking a question if the system captures the specification of its requirement \footnote{Generally, a model-checker is used to determine if the system behaviours are subset of the requirement specification, in other words, if the system refines the specification} \cite{R10, S10}. On the other hand,  temporal logic has logical constructs for formulating system specifications, which enables asking a question, if a system is a model for a logical formula of the specification ($system \models formula$) \cite{CE86}. Using both temporal logic and refinement have been supported with automatic verification tools, such as UPPAAL \cite{BD06} and FDR \cite{TP14}, respectively.


Previously, Lowe has investigated the relationship between the refinement oriented approach (with CSP) and the temporal logic-oriented approach. The result shows that, in expressing temporal logic checks using the refinement approach, it is necessary to use the infinite refusal testing model of CSP. The work highlights that the most challenging part is capturing the expressiveness power of temporal logic in specifying the availability of an event (liveness specification). A desirable specification that ensures that a system performs something good.
% or something bad will never happen in the system. 

In addition, due to the difficulty of capturing refusal testing, automatic support becomes problematic. A previous old version of FDR supports refusal testing, but not the recent efficient version of FDR \cite{fdr}.


Additionally, the work \cite{G08} proves that simple refinement checks cannot cope with the expressive power temporal logic, specifically in expressing three operators: $eventually$  ($\diamond p$: $p$ will hold in some subsequent state),  $until$ ($p  \mathcal{U} q$: $p$ holds in every state until $q$ hold)  and $negation$  ($\neg ( \diamond p$): $p$ will never hold in the subsequent states). The problem of capturing the negation operator is mainly due to its connection with the operator $eventually$. All these three operators express behaviour that is captured by infinite traces. 




In the case of TA for UPPAAL, the temporal logic formula is capable of expressing specifications of an infinite trace of a system \cite{ST18}, which can be seen in expressing liveness specifications. Therefore, this translation work will facilitate using the resources of temporal logic (and UPPAAL for automatic support) in checking requirements specifications that are difficult to specify with refinement models, specifically \verb!tock-CSP! models.  This will include liveness specifications, in addition to the three operators that cannot be specified in refinement models. The operators are eventually $(\diamond)$,  $ until (\mathcal{U}$) and  $negation (\neg) $, as illustrated in Example \ref{ads}.



\begin{example} %{A translation of an Automatic Door System (ADS)} \\
\label{ads}
Consider an Automatic Door System (ADS) that opens a door, and then after at least one-time unit, the system closes the door in synchronisation with a lighting controller, which turns-off the light after closing the door. In \verb!tock-CSP!, a description of ADS is as follows:

\begin{lstlisting}
Controller = open -> tock -> close -> Controller

Lighting = close -> offLight -> Lighting

ADS = Controller [|{close}|] Lighting

\end{lstlisting}



\end{example}



The system ADS has two components, \lstinline{Controller} and \lstinline{Lighting}. The component \verb!Controller! opens and closes the door after an interval of at least one unit time. \lstinline{Lighting} turns-off the light after closing the door. The two components synchronise on the event \lstinline{close}, which enables the lighting controller to turn-off the light. 



In particular, in using \verb!tock-CSP!, there is no straightforward way of specifying requirements for checking `if the system will eventually turn-off the light when the environment is ready to switch-of the light'. However, temporal logic provide a direct construct for specifying these kinds of requirements in a simple form. For instance, in temporal logic, using the syntax of UPPAAL \footnote{UPPAAL uses $A\diamond$ for specifying liveness specifications, while the symbol $\diamond$ or $F$ are also commonly use symbols for specifying liveness in the literature of temporal logic} for specifying liveness specification, the requirement is specified as follow.
\begin{itemize}
    \item $A\diamond$ \lstinline{offLight}  \\ 
        - - \textit{Eventually the system turns-off the light if the environment permits.}
    % - - \textit{Can the system always turns-off the light, if the environment permits.}
\end{itemize}
    



In verifying the correctness of the translation technique, we follow a series of steps.  First, we formulate a systematic list of interesting \verb!tock-CSP!  processes, which pair all the constructs of \verb!tock-CSP! within the scope of this translation work. Second, we use the developed translation technique and its tool to translate the formulated processes into TA for UPPAAL.  Third, we developed another tool that assists us in generating and comparing finite traces of the input \verb!tock-CSP! models and the traces of the translated TA models, with the support of both FDR and UPPAAL, respectively. This provides evidence that the translated TA captures the behaviour of the input \verb!tock-CSP! models.

Describing the translation technique is one of the challenging tasks we faced in this work,
So, we take advantage of the concise construct of Haskell \cite{H16} in describing the technical part of the work. Haskell is a functional programming language, which we use for expressing, implementing and evaluating the translation technique. Both concise and expressive power of Haskell helps us in providing a precise description of the translation technique as a list of translation rules.




% Outline of the paper  ----------------------------------------------------------------------
The structure of the paper is as follows. Next, Section \ref{background} provides brief backgrounds that are essential for understanding the translation technique.  In Section \ref{trans_rule}, we describe an overview of the translation technique. In Section \ref{evaluation}, we discuss an evaluation of the translation technique. In Section \ref{related_work}, we highlight relevant related work, and also discuss a brief comparison with this work. Finally, Section \ref{conclusion}, we highlight future work and also provide a conclusion for the paper.





%%  --------------------  BACKGROUND -----------------------
\section{Background}
\label{background}

This section discusses the required background for understanding the translation work. We begin by discussing the notations of \verb!tock-CSP! and then discuss the target outcome of the translation work, that is a list of TA that is suitable for UPPAAL tool. 


%CSP and \verb!tock-CSP!
\subsubsection{tock-CSP} is an extension of CSP that provides notations for modelling processes and their interactions. In \verb!CSP!, there are varieties of constructs, which includes basic processes such as \verb!SKIP! and \verb!STOP!. \verb!SKIP! expresses a successful termination while \verb!STOP! expresses a deadlock behaviour that can no longer perform any communication. Also, there are operators such as \verb!prefix (->)!, which describes an event that leads up to a process. For example, the process \verb!move->SKIP! specifies the behaviour of a system that moves and then terminates. 



Furthermore, there are additional binary operators such as sequential composition (;), which concatenates two processes serially. For instance, a process \verb!P3 = P1;P2!, which expresses a process that behaves as process \verb!P1!, and then after successful termination of the process \verb!P1!, the process \verb!P3! behaves as process \verb!P2!. For example, the process \verb!Ps = (move->SKIP);(turn->SKIP)!, specifies a system that moves, turns and then terminates, successfully.


There are other binary operators for composing processes in different shapes, such as concurrency, choice and interrupt. Also, CSP provides a special event $tau \ ( \tau ) $ that represents invisible actions that are internal to a system, specifically for internal communications of a system that are hidden from the operating environment. The collection of these operators provides a rich set of constructs for modelling untimed systems. Comprehensive detail of CSP constructs, together with examples, are available in these books \cite{R10, S10}. 


Consequently, \verb!tock-CSP! enriches the notations with adding a special event \verb!tock!, which records the progress of time \cite{R10}. Each event \verb!tock! specifies a single unit of time. For example,  a process \verb!Pt= move->tock->tock->turn->SKIP! specifies the behaviour of a system that moves, and then after at least two-time units, the system turns and then terminates. The addition of the special event \verb!tock! enables specifying temporal specification in a format that is suitable for formal analysis of timed system \cite{TP14}. 


In this work, we provide a translation technique that facilitates using the expressive power of temporal logic in verifying real-time system. We provide a BNF for the part of \verb!tock-CSP! we consider in developing the translation technique and its supporting tool. Part of the BNF is presented in Definition \ref{dfn_CSPproc} using the syntax of Haskell. The complete BNF is available in an extended report of this work \cite{extendedVersion}. The BNF forms the basic foundation of this translation work, and provides a good link for other related works and tools that are associated with \verb!tock-CSP!.

\begin{definition} \textbf{Data definition of \lstinline{CSPproc}} 
\label{dfn_CSPproc}


\begin{verbatim}
data CSPproc =   STOP | SKIP | Prefix Event CSPproc 
                | Interleave CSPproc CSPproc 
                | GenPar CSPproc CSPproc [Event] 
                | Interrupt CSPproc CSPproc 
                | ...
\end{verbatim}
\end{definition}




\subsubsection{Timed Automata for UPPAAL}
TA provides graphical notations for modelling hybrid systems. In UPPAAL, systems are modelled as a network of TA with additional variables. Mathematically, a TA is defined as a tuple $(L, l_0, C, A, E, I)$, where $L$ is a set of locations such that $l_0$  is the initial location, $C$ is a set of clocks, $A$ is a set of actions, $E$ is a set of edges that connects the locations $L$, and $I$ is an invariant that is associated with a location $l \in L$. So, an edge $E$ is defined as $E \subseteq (L \times A \times B(C) \times 2^C \times L)$, which describes an edge from location $l \in L$ that is triggered by an action $a \in A$, guarded with a guard $B(C)$, and associated clocks $C$  that are reset on following an edge $e \in E$ to a location $l \in L$. Finally, $I$ is a function that assigns invariant to a location $I:L \longrightarrow B(C)$   \cite{BD06, B11}.


In UPPAAL, a system is modelled as a network of TA that communicate over channels or variables. A sending channel is decorated with exclamation mark $(c!)$ while the corresponding receiving channel is decorated with question $(c?)$. This enables TA to communicate by synchronising over complementary actions  $a!$ and $a?$, for sending and receiving over the channel $a$. For urgency, there are urgent channels that do not allow delay. Also, there is a broadcast channel that communicates with multiple TA, in the form of one-to-many communication simultaneously (one sender with multiple receivers). For instance, in a broadcast channel $b$, a single TA with the action $b!$ synchronises with all the TA that performs $b?$.

In addition, there are other constructs, such as urgent and committed types of location. An urgent location does not allow time to pass. The committed location is an urgent location that must take the next transition before any other transition. The committed location expresses atomicity, specifically for expressing compound action, which spans multiple transitions that must be executed as a unit. An invariant expression is also provided for specifying and enforcing progress in a location. 




%Env TA
Overall, UPPAAL provides graphical notations for modelling system as a network of TA for the components of a system that communicate with one another and the operating environment, which is also modelled as a TA. For instance, the collection of TA in Figure \ref{ta_ads}, which will be explained later in more details. For specifications, UPPAAL uses a subset of Timed Computational Tree Logic (TCTL) \cite{B09}  for specifying system properties that can be verified automatically  \cite{LP07, LP97, BD06}.  


\section{An Overview of the Translation Technique}
\label{trans_rule}

The translation technique produces a list of small TA, such that the occurrence of each \verb!tock-CSP! event is captured in a small TA with an UPPALL action,  which records an occurrence of the translated event. The action has the same name as the translated event from the input \verb!tock-CSP! process. The technique composes these small TA into a network of TA, which captures the behaviour of the input \verb!tock-CSP! model. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure} %[H]
\subfigure{\includegraphics [width=0.9\textwidth, height=0.4\textwidth]{EgGenParGray/taGenPar0_0.png}}

\subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix00_1.png}}
 \hspace{0.1\textwidth}
\subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix00_2.png}}

\subfigure{\includegraphics [width=0.55\textwidth]{EgGenParGray/taPrefix00_3.png}}
\subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/SyncTA.png}}

\subfigure{\includegraphics [width=0.55\textwidth]{EgGenParGray/taPrefix01_2.png}}
\subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix01_3.png}}

 \hspace{0.1\textwidth}
% \subfigure{\includegraphics [width=0.3\textwidth]{EgGenParGray/taWait_n01_4.png}}
\subfigure{\includegraphics [width=0.9\textwidth]{EgGenParGray/Env.png}}
\caption{A list of networked TA for the translation of the process ADS}
\label{ta_ads}

\end{figure}



For example, a translation of the process ADS from Example \ref{ads}, which produces a network of small TA in Figure \ref{ta_ads}. Details of the translated TA are as follows. Starting from the top-left corner, the first TA captures the translation of concurrency that starts the two processes \lstinline{Controller} and \lstinline{Lighting} concurrently in two possible orders, either \lstinline{Controller} then \lstinline{Lighting} or vice versa,  depending on the operating environment, and then also waits on state \lstinline{s5} for their termination actions in the two possible orders, either \lstinline{Controller} then \lstinline{Lighting} or vice versa,  depending on the process that terminates first, and then after the termination of the other process, the whole system terminates with the action \lstinline{finishID0}.


The second, third and fourth TA capture the translation of the process \lstinline{Controller}. The second TA captures the occurrence of the event \verb!open!. The third TA captures the occurrence of the events \verb!tock?! (with a question mark for synchronising with the environment in recording the progress of time because all processes synchronise with the progress of time). Additional details will follow in describing the translation technique.  The fourth TA captures the occurrence of the event \verb!close!, which needs to synchronise with a synchronising controller, that is the fifth TA in the list of the TA.

The sixth and seventh TA capture the translation of the process \lstinline{Lighting}. The sixth TA captures the translation of the event \verb!close!, which also needs to synchronise with the synchronisation controller (fifth TA) on the event \verb!close!. The seventh TA captures the event \verb!offLight!. Finally, the last TA is an environment TA that has co-actions for all the translated events. Also, the environment TA serves the purpose of 'closing' the overall system (in contrast to having an "open system") as required for the model checker. In this last TA, we use the variable $start$ to construct a guard $start==0$ in the environment TA that blocks the environment from restarting the system. This concludes the description of the list of TA for the translated behaviour of the system ADS.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Explanation of TA for ADS
% \paragraph{}
\vspace{0.2cm}


An alternative of using a list of small TA is using a single large TA that captures the behaviour of the translated \verb!tock-CSP! process. However, the main reason for using a list of small TA is coping with the compositional structure of \verb!tock-CSP!, which is not available in TA \cite{DH08}. 

For instance, it can be argued that a linear process constructed with a series of prefix operators can be translated into linear TA. However, the compositional structure of \verb!tock-CSP! is not suitable for this straight forward translation. A network of small TA provides enough flexibility for composing TA in various ways to capture the behaviour of the original \verb!tock-CSP! process.  



In constructing the network of TA, we use additional \textbf{\textit{coordinating actions}} that link the small TA into a network.  For example, in Figure \ref{ta_ads}, the TA communicates over the channels \verb!startIDADS!, \verb!startID00_1!, \verb!startID01_2!. The coordinating actions link the small TA into a network of TA to establish the flow of the translated \verb!tock-CSP! process. For instance, the channel \verb!startIDADS! forms a link that connect the environment TA (last TA in Figure \ref{ads}) with first TA, on performing the actions \verb|startIDADS!| and \verb!startIDADS?!, respectively. Likewise, the channel \verb!startID00_1! connects the first TA with the second TA, on performing the actions \verb|startID00_1!| and \verb!startID00_1?!, respectively.  A precise definition of the coordinating action is in Definition \ref{coordinating_action}, which also describes the types of coordinating actions we use in developing the translation technique.




\begin{definition}

 \textbf{Coordinating Action} is an UPPAAL action, and we use six types of coordinating actions as follows:


\begin{itemize}
\item \textbf{Flow action} coordinates a link between two TA for capturing the flow of the behaviour. 
% of the input \verb!tock-CSP! process. 
    
\item \textbf{Terminating action} records termination information, in addition to coordinating a link between two TA.


\item \textbf{Synchronisation action} coordinates a link between a TA that participate in a multi-synchronisation action and a TA for controlling the multi-synchronisation. 


\item \textbf{External choice action} coordinates external choice, such that choosing one of the TA composed with external choice blocks the other alternative choices TA that participate in the choice.


\item \textbf{Interrupting action} initiates an interrupting transition that enables a TA to interrupt other TA.
% , for the case of translating processes that are composed with an interrupting operator in \verb!tock-CSP!.

\item \textbf{Exception action} coordinates a link between a TA that raises an exception and a control TA that handle the exception. 
\end{itemize}
\label{coordinating_action}
\end{definition}

\vspace{-0.5cm}
The name of each coordinated action is unique for ensuring the correct flow of the translated TA. In our implementation, the name of the flow actions are generated in the form \verb!startIDx!, where \verb!x! is either a natural number or the name of the input \verb!tock-CSP! process. This can be seen in Example \ref{ads}, the name of the channel \verb!startID00_1! that connects the first TA with the second TA.

Likewise, the names of the remaining coordinating action follow the same pattern; \verb!keywordIDx!, where  \verb!keyword! is a designated word for each of the coordinating actions: \verb!finish! for terminating action,  \verb!ext! for external choice action, \verb!intrp! for interrupting action, and \verb!excp! for exception action. Similarly, the name of a synchronising action is in the form \verb!eventName___sync!; an event name appended with the keyword \verb!___sync! to differentiate a synchronising action from other actions. 



We provide termination actions for capturing essential termination information from the input \verb!tock-CSP!. This is essential is the cases where a TA needs to communicate a successful termination for another TA to proceed. For example, in the case of translating sequential composition \lstinline{P1;P2} where the process \lstinline{P2} begins only after successful termination of the process \lstinline{P1}.  



Additionally, for each translated \verb!tock-CSP! specification, we provide an environment TA, like the last TA in Figure \ref{ads}. Also, the environment TA closes the overall model as part of the requirements for UPPAAL model checker. The environment TA has corresponding co-actions for all the translated events of the input \verb!tock-CSP! model. In addition, the environment TA has two coordinating actions that link the environment TA with the network of the translated TA. First, a flow action that links the environment with the first TA in the list of the translated TA. Also, this first flow action is the starting action that activates the behaviour of the translated TA. Second, a terminating action that links back the final TA in the list of the translated TA to the environment TA, and also records a successful termination of a process and closes the whole system. A precise definition of the structure of environment TA is in Definition \ref{environment_TA}.



% \vspace{0.2cm}

\begin{definition} 
\textbf{Environment TA} models an explicit environment for UPPAAL model. The environment TA has one state and transitions for each co-action of all the events in the original \verb!tock-CSP! process, in addition to two transitions for the first starting flow action and the final termination co-action. 

\label{environment_TA}
\end{definition}



Next, in translating multi-synchronisation, we adopt a centralised approach developed in \cite{O05} and implemented using Java in \cite{F05}. The approach described uses a separate centralised controller for controlling multi-synchronisation events. Here, we use a separate TA with UPPAAL broadcast channel to communicates synchronising information among synchronising TA and a control TA.
% that control the synchronising action.

% In Example \ref{ads}, 

An example can be seen in Figure \ref{ads}, where we illustrate the strategy in translating synchronising action \verb!close!, which synchronises the two processes \verb!Controller! and \verb!Lighting!. In Figure \ref{ta_ads}, the fifth TA captures the translation of the event \verb!close!, which synchronises the process \lstinline{Controller} and the process \lstinline{Lighting}, that is fourth and sixth TA in the translated TA. In the fifth TA, the broadcast channel \verb!close___sync! synchronises the fourth and sixth TA. A precise definition of the synchronisation TA is provided in Definition \ref{dfn_syncTA}.



\begin{definition} \textbf{Synchronisation TA} coordinates a synchronisation action. The structure of synchronisation TA has an initial state and a committed state for each synchronisation action, such that each committed state is connected to the initial state with two transitions. The first transition from the initial state has a guard and an action. The guard is a conjunction of guards from each process that synchronises on that synchronisation action. The guard is enabled when all the processes are ready for the synchronisation, which also enables the TA to performs the associated action that notifies the environment for the occurrence of the synchronisation action. Then, in the second transition, the TA broadcasts the synchronisation action to all the processes that synchronise on the synchronisation action.


\label{dfn_syncTA}
\end{definition}




To ensure that the synchronisation TA synchronises with the required number of TA that participate in a synchronisation channel, we provide guards that block the broadcast channel until all the required TA are ready for the synchronisation. When the guard becomes ready, it enables the synchronising TA to broadcast the synchronisation action such that all the participating will synchronise and progress in performing their subsequent actions.






%%%%%%%%%%%%%%%%%% ---  OVERVIEW OF THE TRANSLATION TECHNIQUE
Furthermore, in \verb!tock-CSP!, a process can be interrupted by another process when the two processes are composed with an interrupt operator (\verb!/\!). This is due to the compositional structure of \verb!tock-CSP!. However, in the case of TA, an explicit transition is needed for expressing an interrupting action,  which enables a TA to interrupt another one. Thus, in this translation work, we provide an additional transition for capturing interrupting event using an interrupting action, as defined in Definition \ref{coordinating_action}.


For example, given a process \verb!Pi = P1/\P2!, the process \verb|P1| can be interrupted by process \verb|P2|. Thus, in translating each event of process \verb|P1|, we provide additional transitions for the initials \footnote{Initials are the first visible events of a process.} of the interrupting process \verb|P2|. The additional transitions enable the translated behaviour of process \verb|P2| to interrupt the translated behaviour of process \verb|P1| at any stable state of its behaviour.




Similarly, in translating external choice, we provide additional transitions that enable the behaviour of the chosen process to block the behaviour of the other processes. Initially, in the translated TA, all the initials of the translated processes are available such that choosing one of the processes to block the other alternative choices with the provided co-actions for translating external choice, as defined in Definition \ref{coordinating_action}.



For example, given a process \verb!Pe = P1[]P2! that composes \verb!P1! and \verb!P2! with operator external choice; such that \verb!Tp! is a list of TA for translating the process \verb!P!. Similarly, let \verb!Tp1! and \verb!Tp2! be lists of TA for translating the processes \verb!P1! and \verb!P2!, respectively.  In the first TA of the list \verb!Tp1!, we provide additional transitions for the initials of \verb!P2! such that choosing \verb! Tp2! blocks \verb!Tp1!. Similarly, in the first TA  of the list \verb!Tp2!, we provide additional transitions for the initials of \verb!P1! such that choosing \verb!Tp1! blocks the behaviour \verb!Tp2!. Additional examples are also available in an extended report \cite{extendedVersion}.




Also, in \verb!tock-CSP!, an event can be renamed or hidden from the environment. In translating renaming, the translation technique carries a list of renamed events, such that before translating each event, the translation technique checks if the event is renamed, and then translate the event appropriately with the corresponding new name. In the like manner, if an event is part of the hidden events, the translation technique carries a list of hidden events, such that on translating hidden event the technique uses a special name $itau$ in place of the hidden event. The event $itau$ has similar meaning with the event $tau$, which represents a hidden event in FDR. We make them different to differentiate the translated hidden event $itau$ from the event $tau$, mainly for the purpose of analysis.


In \verb!tock-CSP!, the event \verb!tock! records the progress of time. Thus, we translate the event \verb!tock! into a corresponding action \verb!tock! for recording the progress of time in the translated TA with a broadcast channel which enables the translated TA to synchronise in recording the progress of time. The translated action \verb!tock! is guarded with clock $clk<=1$ which trigger the action \verb!tock! and reset the clock $clk=0$. The action \verb!tock! is broadcast by the environment TA, which forces the TA to synchronise and record the progress of time using their corresponding co-actions \verb!tock?! (with a question mark), as illustrated in Figure \ref{ta_ads}. In particular, the last TA, which models the environment, has a transition with an action \verb!tock! that is guarded with the expression $ck <= 1$, and resets the clock $ck=0$ to zero on following the transition.
 


In translating non-determinism, TA has a non-determinism facility, using silent transitions that enable a TA to silently takes any of the silent transitions. We translate non-deterministic choice into silent transitions, such that the translated TA follow one of the silent transitions non-deterministically. Also, urgency is translated into the corresponding urgent channel in UPPAAL. Nevertheless, divergence is not part of the construct that we consider in this translation work because divergence is a sign of bad behaviour. This completes an overview for describing the strategy we follow in developing the translation technique.




%----------------------- Sample rule for translation of STOP
\subfile{a4_ruleStopNew}



%  ---------------------------------- EVALUATION 
\section{Evaluation}
\label{evaluation}

To ensure that the translation work is correct, we have to prove soundness. A formal translation ensures that interesting properties of the source model are preserved in the targeted translated models. This is determined by comparing the behaviours of the source model and the behaviours of the translated model \cite{T06, NN07, KM19, B81}. 

In this work, we use traces to compare the behaviour of the input \verb!tock-CSP! models and the traces of the translated TA models. First, we have developed a tool that automates the translation technique. Second, we have developed an evaluation tool, which uses the translation tool to translate \verb!tock-CSP! model into TA, and then uses both FDR and UPPAAL as black boxes in generating a finite set of traces. The structure of the evaluation tool is shown in Figure \ref{trace_analysis_system}. 







\begin{figure}[t!] %[H]
    \centering
%    \includegraphics[width=0.7\textwidth]{C3_figs/traceAnalysis.png}
    \includegraphics[width=\textwidth, height=0.25\textheight]{fig/traceAnalysis.png}
    \caption{Structure of the trace analysis system}
    \label{trace_analysis_system}
\end{figure}






In generating traces, like most of the model-checkers, FDR produces only one trace (counterexample) at a time. So, based on the testing technique developed in \cite{NS08}, we developed a trace generating technique that repeatedly invokes FDR for generating traces until we get all the required traces set of the input \verb!tock-CSP!. Thus, we use the trace generation technique to generate finite traces set of the input \verb!tock-CSP! models with FDR. Similarly, based on the testing technique developed in \cite{LP07}, we developed another trace generation technique, which uses UPPAAL in generating finite discrete traces set for the translated TA models. 

Consequently, these two trace generation techniques serve as components for our trace analysis tool, which has two stages of analysing traces. In the first stage, we generate traces of the input \verb!tock-CSP! and its corresponding translated TA, using both FDR and UPPAAL, respectively. Then, we compare the generated traces, and if they did not match, we move to the second stage for further analysis. In FDR, the trace generation technique is capable of generating and detecting traces with different permutation. Thus, we are able to generate traces with various structure. In contrast,  UPPAAL is not capable of detecting traces with different permutations because UPPAAL uses a logical formula in generating traces \cite{LP07, BD06}. 


Basically, UPPAAL was developed for checking if a system satisfies a logical formula for the requirement specifications, irrespective of the behaviour of the system. For example, UPPAAL does not distinguish between the two traces $ \langle e1, e2, e3 \rangle$ and  $\langle e1, e3, e2 \rangle \}$, as long as both of them satisfy the specification formula. The two traces contain the same three actions, but the action $e2$ and $e3$ occur in a different order. However, FDR is capable of generating both traces that have different structure. Additional examples, together with details implementation of the trace generation techniques, are available in an extended report \cite{extendedVersion}. Thus, in the second stage, we use UPPAAL to check if the traces of FDR are acceptable traces of the translated TA. 







% --------- short version begin
We use this evaluation tool in evaluating the translation technique by translating a list of systematically formulated \verb!tock-CSP! processes that pair all the essential constructors of \verb!tock-CSP! within the scope of this translation work, which produces 111 processes of smaller sizes that are not more than five states in size. Archives of the processes and their translations are available in this repository \cite{extendedVersion}




%  Test cases ----------------------------------------
In addition, the translation technique has been tested in various test cases such as an automated barrier to a car park \cite{S10}, thermostat for monitoring ambient temperature \cite{S10}, simple Automated Teller Machine (ATM)  \cite{R05} and  Bookshop Payment system \cite{S10}, and Railway crossing system \cite{R10}. An overview structure of the processes is provided in Table \ref{table_caseStudies}. Traces are not included because the systems have infinite traces. This is the nature of \verb!tock-CSP! models and other timed systems, they are reactive system with non-terminating processes that must allow time to progress \cite{R10}. Even the simple basic process such as $STOP$ have an infinite sequence of $tock$ as their traces.




% A reader may like to know the size of these test cases. However, all these test cases are reactive system, which means that they are non terminating process that has infinite traces. This is the nature of \verb!tock-CSP! models and other time systems, they are non-terminating process that must allow time to progress \cite{R10}. Even the simple basic process such as $STOP$ have an infinite sequence of $tock$ as their traces.




\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|}  \hline \hline
System &    States &    Transitions     &   Events     \\ \hline
ATM             &     15  &    33           &  15         \\ \hline
AutoBarrier     &     35    &   84             &  10        \\  \hline
PaymentSystem &     7    &   32            &    9       \\   \hline
Rail Crossing &     80    &   361            &   12       \\   \hline
Thermostat      &      7    &   16            &   5       \\   \hline \hline
    \end{tabular}
    \caption{Profiles of the case studies system}
    \label{table_caseStudies}
\end{table}




% Case Studies        Average Timing    States    Transitions    Events    State/Transition
% ATM    FDR    0.0051    15    33    15    0.4545454545
%     UPPAAL    0.0084                
% AutoBarrier    FDR    0.0059    35    84    10    0.4166666667
%     UPPAAL    0.0134                
% PaymentSystem    FDR    0.0048    7    32    9    0.21875
%     UPPAAL    0.0011                
% Rail Crossing    FDR    0.0054    80    361    12    0.2216066482
%     UPPAAL    0.0072                
% Thermostat    FDR    0.0052    7    16    5    0.4375

%------------------------------------------------------
However, trace analysis is limited to establishing correctness for a finite set of traces. Proving correctness considering the complete set of traces involves using mathematical proof to prove that each construct of the input model is translated into an equivalent construct or statements in the target output. This is normally achieved using structural induction in providing proof for infinite behaviour of a system, especially for the case of a non-terminating system \cite{NN07}.  A preliminary proof for the base case of the structural induction is provided in the next section.





\subsection{An Initial Mathematical Proof}
% \subsection{An Initial/Early/Preliminary Mathematical Proof}


%%-------------------------------Math proof
\subfile{mathProof}




%% ----------------------------- RELATED WORK
\section{Related Work}
\label{related_work}



Several types of research explore using CSP in verifying temporal specifications, due to its potential capability of verifying real-time systems. Timed-CSP \cite{S10} is another popular extension of CSP that provides additional notations for capturing temporal specifications. Unlike \verb!tock-CSP!, Timed-CSP records the progress of time with a series of positive real numbers, which facilitates reasoning that is suitable for verifying real-time systems.



However, the approach of Timed-CSP is lacking in specifying strict progress of time, neither deadline nor urgency. And also traces of Timed-CSP becomes infinite in nature, which is problematic for automatic analysis and verification \cite{R10}. In addition, there is no tool support for verifying Timed-CSP models.



As a result of that, many researchers choose to explore model transformations in supporting Timed-CSP with an automatic verification tool. Thus, Timed-CSP has been translated into \verb!tock-CSP! to enable using FDR for automatic verification \cite{O00}. The work provides a link for utilising the facilities of FDR in verifying Timed-CSP model. 

Also, Timed-CSP has been translated into UPPAAL to facilitates using the facilities of UPPAAL in verifying Timed-CSP. The work was initiated in \cite{DH08} and then subsequently improved in \cite{TS13}. Additionally, Timed-CSP has been translated into Constraint Logic Programming (CLP)  that facilitates reasoning in verifying Timed-CSP, that is supported by constraint solver CLP(R) \cite{DP06}.


However, there is less attention in applying the same transformation techniques in improving \verb!tock-CSP! with a better approach for verifying real-time system. An attempt for transforming TA into \verb!tock-CSP! was proposed in \cite{K11}. Whereas in this work, we consider the opposite direction for translating \verb!tock-CSP! into TA for UPPAAL to be able to utilise the facilities of TA and UPPAAL in verifying \verb!tock-CSP! models.
 


% \begin{cmt}  %---------------------------------------------------
% New addition begins
% \end{cmt}

Furthermore, another approach of reducing the complexity of refusal testing was provided in \cite{DR16}, which introduces a translation technique for using priority operator \cite{R10} to transform a question for refusal testing refinement into trace refinement. The technique is generalised to be applicable to the remaining three observational CSP models, namely acceptances, revivals, and finite linear observations \cite{R05}, all with the same motivation of reducing complexity and providing support for automatic verification for these four behavioural models. 

However, their translation technique \cite{DR16} is limited to finite linear-time. While our translation work targets at using  Timed Computation Tree Logic (TCTL) that is powerful enough to cover branching time. Part of the future work will expand the comparison of our translation work with their approach of translating the refusal testing into trace models. 

% \begin{cmt}  %---------------------------------------------------
% Addition ends
% \end{cmt}

Apart from CSP and TA, model transformations have been used for improving various formal modelling notations. For instance, Circus has been translated into \lstinline{CSP||B} to enable using the tool ProB for automatic verification \cite{KJ17}. Additionally, B has been translated into TLA+ for automatic validation with TLC \cite{HL14}. Also, the reverse of translating TLA+ to B has been investigated for automatic validation of TLA+ with ProB \cite{HL12}, such that both B and TLA+ benefit from the resources of each other, specifically their supporting tools ProB and TLC, respectively. 


Model transformation is an established field which has been used for many decades in addressing computational problems. The novelty of this translation work is trace back to early days of model translation works, such as the translation of the timed variants of LOTOS into TA \cite{CO95, HG98}.  A recent survey on model translation provides rich collections of model transformations techniques and their supporting tools \cite{KM19}.



\section{Conclusion}
\label{conclusion}

%-------------  CONCLUSION  --------------------------------------------------

In this work, we presented a technique for translating \verb!tock-CSP! into TA for UPPAAL, which facilitates using the facilities of temporal logic and automatic support with UPPAAL in the verifying \verb!tock-CSP! models. Additionally, this translation would provide an easier alternative of using TCTL in specifying liveness requirements that are difficult to specify and verify in \verb!tock-CSP!. Also, the result of this work sheds additional insight into the complex relationship between \verb!tock-CSP! and TA, as well as the connection between the two popular model checking approaches; refinement model and temporal logic model.

So far, in this work, we used trace analysis in justifying the correctness of the translation work. In the future, we are planning to complete the mathematical proof for the total correctness of the translation technique. Secondly, we are planning to explore using the translation technique in translating extensive case studies that can help us in improving the translation work.
% of \verb!tock-CSP! to UPPAAL.  


Additionally, currently, we translated the event \verb!tock! into an action that is controlled by a timed clock in UPPAAL.  
A recommended next step in this work would be to relate the notion of \verb!tock! to the notion of time in TA and get rid of $tock$ as an action.  This additional extension will help us in exploring additional interesting facilities of UPPAAL for verifying temporal specifications.





==> zz_del/all_____.tex <==





\section{Introduction}   %%%-----------------------------------------------------

Communicating Sequential Processes (CSP) is an established process algebra that provides a formal notation for both modelling and verification of concurrent systems \cite{R10, S10, H78}. Use of CSP for verification has been supported by several tools including powerful model-checkers \cite{TP14, R10, SL09}. 
% CSP and its modelling approaches have contributed to understanding the complexity of concurrent systems  \cite{S10}. 


%tockCSP------------------------------------------------------------------

Interest in using CSP has motivated the introduction of support to model time into its constructs; \verb!tock-CSP! provides an additional event $tock$ to record the progress of time. This enables using CSP for modelling temporal specifications in a format suitable for formal verification. The notation of \verb!tock-CSP! retains of CSP, thus, automatic verification is supported by existing tools. As a result,  \verb!tock-CSP! has been used in the verification of real-time systems such as security protocols \cite{NS00} and railways systems \cite{YF12}. Recently, \verb!tock-CSP! has been used for capturing the semantics of RoboChart, a domain-specific language for modelling robotics system \cite{MR16}. Additionally, a recent extension of \verb!tock-CSP! provides notations for specifying budgets and deadlines for effective modelling and verification of temporal specifications \cite{JP19}.



In this work, we add a technique for translating \verb!tock-CSP! into TA that enables using the facilities of UPPAAL \cite{BD06} in verifying \verb!tock-CSP! models. UPPAAL is a tool-suite for modelling and verifying real-time systems using TA and temporal logic. Both temporal logic and refinement are powerful approaches for model checking \cite{G08}. However, each one of these two approaches have a different concept of modelling and verifying system behaviour. 

On one hand, the refinement approach models both the system and its specifications with the same constructs, like in \verb!tock-CSP!, which enables asking a question if the system captures the specification of its requirement \footnote{Generally, a model-checker is used to determine if the system behaviours are subset of the requirement specification, in other words, if the system refines the specification} \cite{R10, S10}. On the other hand,  temporal logic has logical constructs for formulating system specifications, which enables asking a question, if a system is a model for a logical formula of the specification ($system \models formula$) \cite{CE86}. Using both temporal logic and refinement have been supported with automatic verification tools, such as UPPAAL \cite{BD06} and FDR \cite{TP14}, respectively.


Previously, Lowe has investigated the relationship between the refinement oriented approach (with CSP) and the temporal logic-oriented approach. The result shows that, in expressing temporal logic checks using the refinement approach, it is necessary to use the infinite refusal testing model of CSP. The work highlights that the most challenging part is capturing the expressiveness power of temporal logic in specifying the availability of an event (liveness specification). A desirable specification that ensures that a system performs something good.
% or something bad will never happen in the system. 

Also, due to the difficulty of capturing refusal testing, automatic support becomes problematic. A previous old version of FDR supports refusal testing, but not the recent efficient version of FDR \cite{fdr}.


Additionally, the work \cite{G08} proves that simple refinement checks cannot cope with the expressive power temporal logic, specifically in expressing three operators: $eventually$  ($\diamond p$: $p$ will hold in some subsequent state),  $until$ ($p  \mathcal{U} q$: $p$ holds in every state until $q$ hold)  and $negation$  ($\neg ( \diamond p$): $p$ will never hold in the subsequent states). The problem of capturing the negation operator is mainly due to its connection with the operator $eventually$. All these three operators express behaviour that is captured by infinite traces. 




In the case of TA for UPPAAL, the temporal logic formula is capable of expressing specifications of an infinite trace of a system \cite{ST18}, which can be seen in expressing liveness specifications. Therefore, this translation work will facilitate using the resources of temporal logic (and UPPAAL for automatic support) in checking requirements specifications that are difficult to specify with refinement models, specifically \verb!tock-CSP! models.  This will include liveness specifications, in addition to the three operators that cannot be specified in refinement models: eventually $(\diamond)$,  $ until (\mathcal{U}$) and  $negation (\neg) $, as illustrated in Example \ref{ads}.



\begin{example} %{A translation of an Automatic Door System (ADS)} \\
\label{ads}
Consider an Automatic Door System (ADS) that opens a door, and then after at least one-time unit, the system closes the door in synchronisation with a lighting controller, which turns-off the light after closing the door. In \verb!tock-CSP!, a description of ADS is as follows:

\begin{lstlisting}
Controller = open -> tock -> close -> Controller

Lighting = close -> offLight -> Lighting

ADS = Controller [|{close}|] Lighting

\end{lstlisting}



\end{example}



The system ADS have two components, \lstinline{Controller} and \lstinline{Lighting}. The component \verb!Controller! opens and closes the door after an interval of at least one unit time. \lstinline{Lighting} turns-off the light after closing the door. The two components synchronise on the event \lstinline{close}, which enables the lighting controller to turn-off the light after closing the door. 



For instance, in using \verb!tock-CSP!, there is no uncomplicated way of specifying requirements for checking `if the system will eventually turn-off the light when the environment is ready to switch-of the light'. However, temporal logic provide a direct construct for specifying these kinds of requirements in a simple form. For instance, in temporal logic, using the syntax of UPPAAL \footnote{UPPAAL uses $A\diamond$ for specifying liveness specifications, while the symbol $\diamond$ or $F$ are also commonly use symbols for specifying liveness in the literature of temporal logic} for specifying liveness specification, the requirement is specified as follow.
\begin{itemize}
    \item $A\diamond$ \lstinline{offLight}  \\ 
        - - \textit{ The system eventually turns-off the light, if the environment permits.}
    % - - \textit{Can the system always turns-off the light, if the environment permits.}
\end{itemize}
    



In verifying the correctness of the translation technique, we follow a series of steps.  First, we formulate a systematic list of interesting \verb!tock-CSP!  processes, which pair all the constructs of \verb!tock-CSP! within the scope of this translation work. Second, we use the developed translation technique and its tool to translate the formulated processes into TA for UPPAAL.  Third, we developed another tool that assists us in generating and comparing finite traces of the input \verb!tock-CSP! models and the traces of the translated TA models, with the support of both FDR and UPPAAL, respectively. This provides evidence that the translated TA captures the behaviour of the input \verb!tock-CSP! models.

Describing the translation technique is one of the challenging tasks we faced in this work,
So, we take advantage of the concise construct of Haskell \cite{H16} in describing the technical part of the work. Haskell is a functional programming language, which we use for expressing, implementing and evaluating the translation technique. Both concise and expressive power of Haskell helps us in providing a precise description of the translation technique as a list of translation rules.




% Outline of the paper  ----------------------------------------------------------------------
The structure of the paper is as follows. Next, Section \ref{background} provides brief backgrounds that are essential for understanding the translation technique.  In Section \ref{trans_rule}, we describe an overview of the translation technique. In Section \ref{evaluation}, we discuss an evaluation of the translation technique. In Section \ref{related_work}, we highlight relevant related works, and also present a brief comparison with this work. Finally, Section \ref{conclusion}, we highlight future work and also provide a conclusion for the paper.





%%  --------------------  BACKGROUND -----------------------
\section{Background}
\label{background}

This section discusses the required background for understanding the translation work. We begin by discussing the notations of \verb!tock-CSP! and then discuss the target outcome of the translation work, a network of suitable TA for UPPAAL. 


%CSP and \verb!tock-CSP!
\subsubsection{tock-CSP} is an extension of CSP that provides notations for modelling processes and their interactions. In \verb!CSP!, there are varieties of constructs, which includes basic processes such as \verb!SKIP! and \verb!STOP!. \verb!SKIP! expresses a successful termination while \verb!STOP! expresses a deadlock behaviour that can no longer perform any communication. Also, there are operators such as \verb!prefix (->)!, which describes an event that leads up to a process. For example, the process \verb!move->SKIP! describes a system that moves and then terminates. 



Furthermore, there are additional binary operators such as sequential composition (;), which concatenates two processes serially. For instance, a process \verb!P3 = P1;P2!, which expresses a process that behaves as process \verb!P1!, and then after successful termination of the process \verb!P1!, the process \verb!P3! behaves as process \verb!P2!. For example, the process \verb!Ps = (move->SKIP);(turn->SKIP)!, specifies a system that moves, turns and then terminates, successfully.


There are other binary operators for composing processes in different shapes, such as concurrency, choice and interrupt. Also, CSP provides a special event $tau \ ( \tau ) $ that represents invisible actions that are internal to a system, specifically for internal communications of a system that are hidden from the operating environment. The collection of these operators provides a rich set of constructs for modelling untimed systems. Comprehensive full detail of CSP constructs, together with examples, are available in these books \cite{R10, S10}. 


Consequently, \verb!tock-CSP! enriches the notations with adding a special event \verb!tock!, which records the progress of time \cite{R10}. Each event \verb!tock! specifies a single unit of time. For example,  a process \verb!Pt= move->tock->tock->turn->SKIP! specifies the behaviour of a system that moves, and then after at least two-time units, the system turns and then terminates. The addition of the special event \verb!tock! enables specifying temporal specification in a format that is suitable for formal analysis of timed system \cite{TP14}. 


In this work, we provide a translation technique that facilitates using the expressive power of temporal logic in verifying temporal specifications of real-time systems. We provide a BNF for the part of \verb!tock-CSP! we consider in developing this translation technique and its supporting tool. Part of the BNF is presented in Definition \ref{dfn_CSPproc} using the syntax of Haskell. The complete BNF is available in an extended report of this work \cite{extendedVersion}. The BNF forms the basic foundation of this translation work, and provides a good link for other related works and tools that are associated with \verb!tock-CSP!.

\begin{definition} \textbf{Data definition of \lstinline{CSPproc}} 
\label{dfn_CSPproc}


\begin{verbatim}
data CSPproc =   STOP | SKIP | Prefix Event CSPproc 
                | Interleave CSPproc CSPproc 
                | GenPar CSPproc CSPproc [Event] 
                | Interrupt CSPproc CSPproc 
                | ...
\end{verbatim}
\end{definition}




\subsubsection{Timed Automata for UPPAAL}
TA provides graphical notations for modelling hybrid systems. In UPPAAL, systems are modelled as a network of TA with additional variables. Mathematically, a TA is defined as a tuple $(L, l_0, C, A, E, I)$, where $L$ is a set of locations such that $l_0$  is the initial location, $C$ is a set of clocks, $A$ is a set of actions, $E$ is a set of edges that connects the locations $L$, and $I$ is an invariant that is associated with a location $l \in L$. So, an edge $E$ is defined as $E \subseteq (L \times A \times B(C) \times 2^C \times L)$, which describes an edge from location $l \in L$ that is triggered by an action $a \in A$, guarded with a guard $B(C)$, and associated clocks $C$  that are reset on following an edge $e \in E$ to a location $l \in L$. Finally, $I$ is a function that assigns invariant to a location $I:L \longrightarrow B(C)$   \cite{BD06, B11}.


In UPPAAL, a system is modelled as a network of TA that communicate over channels or variables. A sending channel is decorated with exclamation mark $(c!)$ while the corresponding receiving channel is decorated with question $(c?)$. This enables TA to communicate by synchronising channel over complementary actions  $a!$ and $a?$, for sending and receiving, respectively. For urgency, there are urgent channels that do not allow delay. Also, there is a broadcast channel that communicates with multiple TA, in the form of one-to-many communication simultaneously (one sender with multiple receivers). For instance, in a broadcast channel $b$, a single TA with the action $b!$ synchronises with all the TA that performs the corresponding co-action $b?$.

Furthermore, there are other important such as urgent and committed types of location. An urgent location is a type of location that does not allow time to pass. And a committed location is an urgent location that must participate in the next transition before any other transition. The committed location is useful in expressing atomicity, specifically for expressing compound action, which spans multiple transitions that must be executed as a unit. There is also invariant for specifying and enforcing progress in a location. 




%Env TA
Overall, UPPAAL provides graphical notations for modelling system as a network of TA for the components of a system that communicate with one another and the operating environment, which is also modelled as a TA. For instance, the collection of TA in Figure \ref{ta_ads}, which will be explained later in more details. For specifications, UPPAAL uses a subset of Timed Computational Tree Logic (TCTL) \cite{B09}  for specifying system properties that can be verified automatically  \cite{LP07, LP97, BD06}.  


\section{An Overview of the Translation Technique}
\label{trans_rule}

We developed the translation technique to produce a list of small TA, such that the occurrence of each \verb!tock-CSP! event is captured in a small TA with an UPPALL action,  which records an occurrence of the translated event. The action has the same name as the translated event from the input \verb!tock-CSP! process. The technique composes these small TA into a network of TA, which captures the behaviour of the input \verb!tock-CSP! model. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure} %[H]
\subfigure{\includegraphics [width=0.9\textwidth, height=0.4\textwidth]{EgGenParGray/taGenPar0_0.png}}

\subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix00_1.png}}
 \hspace{0.1\textwidth}
\subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix00_2.png}}

\subfigure{\includegraphics [width=0.55\textwidth]{EgGenParGray/taPrefix00_3.png}}
\subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/SyncTA.png}}

\subfigure{\includegraphics [width=0.55\textwidth]{EgGenParGray/taPrefix01_2.png}}
\subfigure{\includegraphics [width=0.4\textwidth]{EgGenParGray/taPrefix01_3.png}}

 \hspace{0.1\textwidth}
% \subfigure{\includegraphics [width=0.3\textwidth]{EgGenParGray/taWait_n01_4.png}}
\subfigure{\includegraphics [width=0.9\textwidth]{EgGenParGray/Env.png}}
\caption{A list of networked TA for the translation of the process ADS}
\label{ta_ads}

\end{figure}



For example, a translation of the process ADS, from Example \ref{ads}, produces a network of small TA in Figure \ref{ta_ads}. Details of the translated TA are as follows. Starting from the top-left corner, the first TA captures the translation of a concurrency that starts the two concurrent processes \lstinline{Controller} and \lstinline{Lighting} concurrently in two possible orders, either \lstinline{Controller} then \lstinline{Lighting} or vice versa,  depending on the choice of the operating environment, and then also waits on state \lstinline{s5} for their termination actions in the two possible orders, either \lstinline{Controller} then \lstinline{Lighting} or vice versa,  depending on the process that terminates first. Then after the termination of the other process, the whole system terminates with the action \lstinline{finishID0}.


The second, third and fourth TA capture the translation of the process \lstinline{Controller}. The second TA captures the occurrence of the event \verb!open!. The third TA captures the occurrence of the event \verb!tock?! (with a question mark for synchronising with the environment in recording the progress of time because all processes synchronise with the progress of time). Additional details will follow in describing the translation technique.  The fourth TA captures the occurrence of the event \verb!close!, which needs to synchronise with a synchronising controller, that is the fifth TA in the list of the TA.

The sixth and seventh TA capture the translation of the process \lstinline{Lighting}. The sixth TA captures the translation of the event \verb!close!, which also needs to synchronise with the synchronisation controller (fifth TA) on the event \verb!close!. The seventh TA captures the event \verb!offLight!. Finally, the last TA is an environment TA that has co-actions for all the translated events. Also, the environment TA serves the purpose of 'closing' the overall system (in contrast to having an "open system") as required for the model checker. In this last TA, we use the variable $start$ to construct a guard $start==0$ in the environment TA that blocks the environment from restarting the system. This concludes the description of the list of TA for the translated behaviour of the system ADS.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Explanation of TA for ADS
% \paragraph{}
\vspace{0.2cm}


An alternative of using a list of small TA is using a single large TA that captures the behaviour of the translated \verb!tock-CSP! process. However, the main reason for using a list of small TA is coping with the compositional structure of \verb!tock-CSP!, which is not available in TA \cite{DH08}. 

For instance, it can be argued that a linear process constructed with a series of prefix operators can be translated into linear TA. However, the compositional structure of \verb!tock-CSP! is not suitable for this straightforward translation. A network of small TA provides enough flexibility for composing TA in various ways to capture the behaviour of the original \verb!tock-CSP! process.  



In constructing the network of TA, we use additional \textbf{\textit{coordinating actions}} that link the small TA into a network.  For example, in Figure \ref{ta_ads}, the TA communicates over the channels \verb!startIDADS!, \verb!startID00_1!, \verb!startID01_2!. The coordinating actions link the small TA into a network of TA to establish the flow of the translated \verb!tock-CSP! process. For instance, the channel \verb!startIDADS! forms a link that connect the environment TA (last TA in Figure \ref{ads}) with first TA, on performing the actions \verb|startIDADS!| and \verb!startIDADS?!, respectively. Likewise, the channel \verb!startID00_1! connects the first TA with the second TA, on performing the actions \verb|startID00_1!| and \verb!startID00_1?!, respectively.  A precise definition of the coordinating action is in Definition \ref{coordinating_action}, which also describes the types of coordinating actions we use in developing the translation technique.




\begin{definition}

 \textbf{Coordinating Action} is an UPPAAL action, and we use six types of coordinating actions as follows:


\begin{itemize}
\item \textbf{Flow action} coordinates a link between two TA for capturing the flow of the behaviour. 
% of the input \verb!tock-CSP! process. 
    
\item \textbf{Terminating action} records termination information, in addition to coordinating a link between two TA.


\item \textbf{Synchronisation action} coordinates a link between a TA that participate in a synchronisation action and a TA for controlling the multi-synchronisation. 


\item \textbf{External choice action} coordinates external choice, such that choosing one of the TA that is part of the external choice should block the other alternative choices TA that participate in the external choice.


\item \textbf{Interrupting action} initiates an interrupting transition that enables a TA to interrupt other TA.
% , for the case of translating processes that are composed with an interrupting operator in \verb!tock-CSP!.

\item \textbf{Exception action} coordinates a link between a TA that raises an exception and a control TA that handle the exception. 
\end{itemize}
\label{coordinating_action}
\end{definition}

\vspace{-0.5cm}
The names of each coordinated action is unique for ensuring the correct flow of the translated TA. In our implementation, the name of the flow actions are generated in the form \verb!startIDx!, where \verb!x! is either a natural number or the name of the input \verb!tock-CSP! process. This can be seen in Example \ref{ads}, the name of the channel \verb!startID00_1! that connects the first TA with the second TA.

Likewise, the names of the remaining coordinating action follow the same pattern: \verb!keywordIDx!, where  \verb!keyword! is a designated word for each of the coordinating actions: \verb!finish! for terminating action,  \verb!ext! for external choice action, \verb!intrp! for interrupting action, and \verb!excp! for exception action. Similarly, the name of a synchronising action is in the form \verb!eventName___sync!; an event name appended with the keyword \verb!___sync! to differentiate a synchronising action from other actions, especially for analysis. 



We provide termination actions for capturing essential termination information from the input \verb!tock-CSP!. This is essential is the cases where a TA needs to communicate a successful termination for another TA to proceed. For example, in the case of translating sequential composition \lstinline{P1;P2} where the process \lstinline{P2} begins only after successful termination of the process \lstinline{P1}.  



Additionally, for each translated \verb!tock-CSP! specification, we provide an environment TA, like the last TA in Figure \ref{ads}. Also, the environment TA closes the overall model as part of the requirements for UPPAAL model checker. The environment TA has corresponding co-actions for all the translated events of the input \verb!tock-CSP! model. Also, the environment TA has two coordinating actions that link the environment TA with the network of the translated TA. First, a flow action that links the environment with the first TA in the list of the translated TA. Also, this first flow action is the starting action that activates the behaviour of the translated TA. Second, a terminating action that links back the final TA in the list of the translated TA to the environment TA, and records a successful termination of a process. Moreover, the environment TA serves the purpose of closing the overall network of TA.  A precise definition of the structure of environment TA is in Definition \ref{environment_TA}.



% \vspace{0.2cm}

\begin{definition} 
\textbf{Environment TA} models an explicit environment for UPPAAL model. The environment TA has one state and transitions for each co-action of all the events in the original \verb!tock-CSP! process, in addition to two transitions for the first starting flow action and the final termination co-action. 

\label{environment_TA}
\end{definition}



Next, in translating multi-synchronisation, we adopt a centralised approach developed in \cite{O05} and implemented using Java in \cite{F05}. The approach described uses a separate centralised controller for controlling multi-synchronisation events. Here, we use a separate TA with UPPAAL broadcast channel to communicates synchronising information among synchronising TA and a control TA.
% that control the synchronising action.

% In Example \ref{ads}, 

An example can be seen in Figure \ref{ads}, where we illustrate the strategy in translating synchronising action \verb!close!, which synchronises the two processes \verb!Controller! and \verb!Lighting!. In Figure \ref{ta_ads}, the fifth TA captures the translation of the event \verb!close!, which synchronises the process \lstinline{Controller} and the process \lstinline{Lighting}, that is fourth and sixth TA in the translated TA. In the fifth TA, the broadcast channel \verb!close___sync! synchronises the fourth and sixth TA. A precise definition of the synchronisation TA is provided in Definition \ref{dfn_syncTA}.



\begin{definition} \textbf{Synchronisation TA} coordinates a synchronisation action. The structure of synchronisation TA has an initial state and a committed state for each synchronisation action, such that each committed state is connected to the initial state with two transitions. The first transition from the initial state has a guard and an action. The guard is a conjunction of guards from each process that synchronises on that synchronisation action. The guard is enabled when all the processes are ready for the synchronisation, which also enables the TA to performs the associated action that notifies the environment for the occurrence of the synchronisation action. Then, in the second transition, the TA broadcasts the synchronisation action to all the processes that synchronise on the synchronisation action.


\label{dfn_syncTA}
\end{definition}




To ensure that the synchronisation TA synchronises with the required number of TA that participate in a synchronisation channel, we provide guards that block the broadcast channel until all the required TA are ready for the synchronisation. When the guard becomes ready, it enables the synchronising TA to broadcast the synchronisation action such that all the participating will synchronise and progress with their behaviour, as well as the behaviour of the whole system.






%%%%%%%%%%%%%%%%%% ---  OVERVIEW OF THE TRANSLATION TECHNIQUE
Furthermore, in \verb!tock-CSP!, a process can be interrupted by another process when the two processes are composed with an interrupt operator (\verb!/\!). This is due to the compositional structure of \verb!tock-CSP!. However, in the case of TA, an explicit transition is needed for expressing an interrupting action,  which enables a TA to interrupt another one. Thus, in this translation work, we provide an additional transition for capturing interrupting event using an interrupting action, as defined in Definition \ref{coordinating_action}.


For example, given a process \verb!Pi = P1/\P2!, the process \verb|P1| can be interrupted by process \verb|P2|. Thus, in translating each event of process \verb|P1|, we provide additional transitions for the initials \footnote{Initials are the first visible events of a process.} of the interrupting process \verb|P2|. The additional transitions enable the translated behaviour of process \verb|P2| to interrupt the translated behaviour of process \verb|P1| at any stable state of its behaviour.




Similarly, in translating external choice, we provide additional transitions that enable the behaviour of the chosen process to block the behaviour of the other processes. Initially, in the translated TA, all the initials of the translated processes are available such that choosing one of the processes to block the other alternative choices with the provided co-actions for translating external choice, as defined in Definition \ref{coordinating_action}.



For example, given a process \verb!Pe = P1[]P2! that composes \verb!P1! and \verb!P2! with operator external choice; such that \verb!Tp! is a list of TA for translating the process \verb!P!. Similarly, let \verb!Tp1! and \verb!Tp2! be lists of TA for translating the processes \verb!P1! and \verb!P2!, respectively.  In the first TA of the list \verb!Tp1!, we provide additional transitions for the initials of \verb!P2! such that choosing \verb! Tp2! blocks \verb!Tp1!. Similarly, in the first TA  of the list \verb!Tp2!, we provide additional transitions for the initials of \verb!P1! such that choosing \verb!Tp1! blocks the behaviour \verb!Tp2!. Additional examples are also available in an extended report \cite{extendedVersion}.




Also, in \verb!tock-CSP!, an event can be renamed or hidden from the environment. In translating renaming, the translation technique carries a list of renamed events, such that before translating each event, the translation technique checks if the event is renamed, and then translate the event appropriately with the corresponding new name. In the like manner, if an event is part of the hidden events, the translation technique carries a list of hidden events, such that on translating hidden event the technique uses a special name $itau$ in place of the hidden event. The event $itau$ has similar meaning with the event $tau$, which represents a hidden event in FDR. We make them different to differentiate the translated hidden event $itau$ from the event $tau$, mainly for the purpose of analysis.


In \verb!tock-CSP!, the event \verb!tock! records the progress of time. Thus, we translate the event \verb!tock! into a corresponding action \verb!tock! for recording the progress of time in the translated TA with a broadcast channel which enables the translated TA to synchronise in recording the progress of time. The translated action \verb!tock! is guarded with clock $clk<=1$ which trigger the action \verb!tock! and reset the clock $clk=0$. The action \verb!tock! is broadcast by the environment TA, which forces the TA to synchronise and record the progress of time using their corresponding co-actions \verb!tock?! (with a question mark), as illustrated in Figure \ref{ta_ads}. In particular, the last TA, which models the environment, has a transition with an action \verb!tock! that is guarded with the expression $ck <= 1$, and resets the clock $ck=0$ to zero on following the transition.
 


In translating non-determinism, TA has a non-determinism facility, using silent transitions that enable a TA to silently takes any of the silent transitions. We translate non-deterministic choice into silent transitions, such that the translated TA follow one of the silent transitions non-deterministically. Also, urgency is translated into the corresponding urgent channel in UPPAAL. Nevertheless, divergence is not part of the construct that we consider in this translation work because divergence is a sign of bad behaviour. This completes an overview for describing the strategy we follow in developing the translation technique.




%----------------------- Sample rule for translation of STOP
\subfile{a4_ruleStopNew}



%  ---------------------------------- EVALUATION 
\section{Evaluation}
\label{evaluation}

To ensure that the translation work is correct, we have to prove soundness. A formal translation ensures that interesting properties of the source model are preserved in the targeted translated models. This is determined by comparing the behaviours of the source model and the behaviours of the translated model \cite{T06, NN07, KM19, B81}. 

In this work, we use traces to compare the behaviour of the input \verb!tock-CSP! models and the traces of the translated TA models. First, we have developed a tool that automates the translation technique. Second, we have developed an evaluation tool, which uses the translation tool to translate \verb!tock-CSP! model into TA, and then uses both FDR and UPPAAL as black boxes in generating a finite set of traces. The structure of the evaluation tool is shown in Figure \ref{trace_analysis_system}. 







\begin{figure}[t!] %[H]
    \centering
%    \includegraphics[width=0.7\textwidth]{C3_figs/traceAnalysis.png}
    \includegraphics[width=\textwidth, height=0.25\textheight]{fig/traceAnalysis.png}
    \caption{Structure of the trace analysis system}
    \label{trace_analysis_system}
\end{figure}






In generating traces, like most of the model-checkers, FDR produces only one trace (counterexample) at a time. So, based on the testing technique developed in \cite{NS08}, we developed a trace generating technique that repeatedly invokes FDR for generating traces until we get all the required traces set of the input \verb!tock-CSP!. Thus, we use the trace generation technique to generate finite traces set of the input \verb!tock-CSP! models with FDR. Similarly, based on the testing technique developed in \cite{LP07}, we developed another trace generation technique, which uses UPPAAL in generating finite discrete traces set for the translated TA models. 

Consequently, these two trace generation techniques serve as components for our trace analysis tool, which has two stages of analysing traces. In the first stage, we generate traces of the input \verb!tock-CSP! and its corresponding translated TA, using both FDR and UPPAAL, respectively. Then, we compare the generated traces, and if they did not match, we move to the second stage for further analysis. In FDR, the trace generation technique is capable of generating and detecting traces with different permutation. Thus, we generate the required traces with various structure. In contrast,  UPPAAL is not capable of detecting traces with different permutations because UPPAAL uses a logical formula in generating traces \cite{LP07, BD06}. Thus, we use the power of FDR to complement UPPAAL in generating and comparing traces of \verb!tock-CSP! and TA.


Basically, UPPAAL was developed for checking if a system satisfies a logical formula for the requirement specifications, irrespective of the behaviour of the system. For example, UPPAAL does not distinguish between the two traces $ \langle e1, e2, e3 \rangle$ and  $\langle e1, e3, e2 \rangle \}$, if both of them satisfy the specification formula. The two traces contain the same three actions, but the action $e2$ and $e3$ occur in a different order. However, FDR is capable of generating both traces that have similar and different structures. Additional examples, together with details implementation of the trace generation techniques, are available in an extended report \cite{extendedVersion}. Thus, in the second stage, we use UPPAAL to check if the traces of FDR are acceptable traces of the translated TA. 







% --------- short version begin
We use this evaluation tool in evaluating the translation technique by translating a list of systematically formulated \verb!tock-CSP! processes that pair the constructs of \verb!tock-CSP!, within the scope of this translation work, which produces 111 processes of smaller sizes that are not more than five states in size. Archives of the processes and their translations are available in this repository \cite{extendedVersion}




%  Test cases ----------------------------------------
In addition, the translation technique has been tested in various test cases such as an automated barrier to a car park \cite{S10}, thermostat for monitoring ambient temperature \cite{S10}, simple Automated Teller Machine (ATM)  \cite{R05} and  Bookshop Payment system \cite{S10}, and Railway crossing system \cite{R10}. An overview structure of the processes is provided in Table \ref{table_caseStudies}. Traces are not included because the systems have infinite traces. This is due to the nature of \verb!tock-CSP! models and other timed systems, they are reactive system with non-terminating processes that must allow time to progress \cite{R10}. Even a simple process such as $STOP$ have an infinite sequence of $tock$ as their traces.




% A reader may like to know the size of these test cases. However, all these test cases are reactive system, which means that they are non terminating process that has infinite traces. This is the nature of \verb!tock-CSP! models and other time systems, they are non-terminating process that must allow time to progress \cite{R10}. Even the simple basic process such as $STOP$ have an infinite sequence of $tock$ as their traces.




\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|}  \hline \hline
System &    States &    Transitions     &   Events     \\ \hline
Simple ATM             &     15  &    33           &  15         \\ \hline
AutoBarrier     &     35    &   84             &  10        \\  \hline
PaymentSystem &     7    &   32            &    9       \\   \hline
Rail Crossing &     80    &   361            &   12       \\   \hline
Thermostat      &      7    &   16            &   5       \\   \hline \hline
    \end{tabular}
    \caption{Profiles of the case studies system}
    \label{table_caseStudies}
\end{table}




% Case Studies        Average Timing    States    Transitions    Events    State/Transition
% ATM    FDR    0.0051    15    33    15    0.4545454545
%     UPPAAL    0.0084                
% AutoBarrier    FDR    0.0059    35    84    10    0.4166666667
%     UPPAAL    0.0134                
% PaymentSystem    FDR    0.0048    7    32    9    0.21875
%     UPPAAL    0.0011                
% Rail Crossing    FDR    0.0054    80    361    12    0.2216066482
%     UPPAAL    0.0072                
% Thermostat    FDR    0.0052    7    16    5    0.4375

%------------------------------------------------------
However, trace analysis is only approximation to establishing correctness with a finite set of traces. Proving correctness for the complete set of traces involves using mathematical proof to prove that each construct of the input model is translated into an equivalent construct or statements in the target output. This is usually achieved using structural induction in providing proof for infinite behaviour of a system, especially for the case of a non-terminating system \cite{NN07}.  An initial proof for the structural induction is provided in the next section.





\subsection{An Initial Mathematical Proof}
% \subsection{An Initial/Early/Preliminary Mathematical Proof}


%%-------------------------------Math proof
\subfile{mathProof}




%% ----------------------------- RELATED WORK
\section{Related Work}
\label{related_work}



Several types of research explore using CSP in verifying temporal specifications, due to its potential capability of verifying real-time systems. Timed-CSP \cite{S10} is another popular extension of CSP that provides additional notations for capturing temporal specifications. Unlike \verb!tock-CSP!, Timed-CSP records the progress of time with a series of positive real numbers, which facilitates reasoning that is suitable for verifying real-time systems.



However, the approach of Timed-CSP is lacking in specifying strict progress of time, neither deadline nor urgency. Additionally, traces of Timed-CSP becomes infinite, which is problematic for automatic analysis and verification \cite{R10}. Besides, there is no tool support for verifying Timed-CSP models.



As a result of that, many researchers choose to explore model transformations in supporting Timed-CSP with an automated verification tool. Thus, Timed-CSP has been translated into \verb!tock-CSP! to enable using FDR for automatic verification \cite{O00}. The work provides a link for utilising the facilities \verb!tock-CSP! and its supporting tool FDR in verifying Timed-CSP model. 

Also, Timed-CSP has been translated into UPPAAL to facilitates using the facilities of UPPAAL in verifying Timed-CSP. The work was initiated in \cite{DH08} and then subsequently improved in \cite{TS13}. Additionally, Timed-CSP has been translated into Constraint Logic Programming (CLP)  that facilitates reasoning in verifying Timed-CSP, that is supported by constraint solver CLP(R) \cite{DP06}.


However, there is less attention in applying the same transformation techniques in improving \verb!tock-CSP! with a better approach for verifying real-time system. An attempt for transforming TA into \verb!tock-CSP! was proposed in \cite{K11}. Whereas in this work, we consider the opposite direction for translating \verb!tock-CSP! into TA for UPPAAL to be able to utilise the facilities of TA and UPPAAL in verifying \verb!tock-CSP! models.
 


% \begin{cmt}  %---------------------------------------------------
% New addition begins
% \end{cmt}

Furthermore, another approach of reducing the complexity of refusal testing was provided in \cite{DR16}, which introduces a translation technique for using priority operator \cite{R10} to transform a question for refusal testing refinement into trace refinement. The technique is generalised to be applicable to the remaining three observational CSP models, namely acceptances, revivals, and finite linear observations \cite{R05}, all with the same motivation of reducing complexity and providing support for automatic verification for these four behavioural models. 

However, their translation technique \cite{DR16} is limited to finite linear-time. While our translation work targets at using  Timed Computation Tree Logic (TCTL) that is powerful enough to cover branching time. Part of the future work will expand the comparison of our translation work with their approach of translating the refusal testing into trace models. 

% \begin{cmt}  %---------------------------------------------------
% Addition ends
% \end{cmt}

Apart from CSP and TA, model transformations have been used for improving various formal modelling notations. For instance, Circus has been translated into \lstinline{CSP||B} to enable using the tool ProB for automatic verification \cite{KJ17}. Additionally, B has been translated into TLA+ for automatic validation with TLC \cite{HL14}. Also, the reverse of translating TLA+ to B has been investigated for automated validation of TLA+ with ProB \cite{HL12}, such that both B and TLA+ benefit from the resources of each other, specifically their supporting tools ProB and TLC, respectively, for automated verification. 


Model transformation is an established field which has been used for many decades in addressing computational problems. The novelty of this translation work is trace back to early days of model translation works, such as the translation of the timed variants of LOTOS into TA \cite{CO95, HG98}. Recently, there is systematic survey model translation, which provides a rich collection of model transformations techniques and their supporting tools \cite{KM19}.

% A recent survey on model translation provides rich collections of model transformations techniques and their supporting tools \cite{KM19}.









\section{Conclusion}
\label{conclusion}

%-------------  CONCLUSION  --------------------------------------------------

In this work, we presented a technique for translating \verb!tock-CSP! into TA for UPPAAL, which facilitates using the facilities of temporal logic and automatic support with UPPAAL in the verifying \verb!tock-CSP! models. Additionally, this translation would provide an easier alternative of using TCTL in specifying liveness requirements that are difficult to specify and verify in \verb!tock-CSP!. Also, the result of this work sheds additional insight into the complex relationship between \verb!tock-CSP! and TA, as well as the connection between the two popular model checking approaches; refinement model and temporal logic model.

So far, in this work, we used trace analysis in justifying the correctness of the translation work. In the future, we are planning to complete the mathematical proof for the total correctness of the translation technique. Secondly, we are planning to explore using the translation technique in translating extensive case studies that can help us in improving the translation work.
% of \verb!tock-CSP! to UPPAAL.  


Additionally, currently, we translated the event \verb!tock! into an action that is controlled by a timed clock in UPPAAL.  
A recommended next step in this work would be to relate the notion of \verb!tock! to the notion of time in TA and get rid of $tock$ as an action.  This additional extension will help us in exploring additional interesting facilities of UPPAAL for verifying temporal specifications.





==> zz_del/background.tex <==
CSP
tock-CSP
tick-tock-CSP
BNF
TA 
UPPAAL
Haskell
??Bashscript???

Automatic Validation of Infinite Real-Time Systems
Model checking Timed CSP



Advantage of UPPAAL
Facilities for verifying temporal specifications
Gavin paper for specifying temporal specs


Background

This section discusses the required background for understanding the translation work. We begins with discussing tock-CSP and then discuss the target outcome of the translation work, TA for UPPAAL tool, and then subsequently discusses Haskell, which is the language we used for both presenting the translation technique and also both implementing and evaluating the translation technique.


CSP and tock-CSP
tock-CSP is an extension of CSP, which provides notations for modelling process and their interactions. The basic constant process are SKIP and STOP that express processes that terminates successful and deadlock respectively. A prefix operator (->) for prefixing an event to a process. So e -> P1 is process that performs the event e and then behave as P1.  For example move -> SKIP, is a process that specifies the behaviour of a system that moves and then terminate. 

Additional binary operators include sequential composition (;), which composes two processes one after the other. So a process P1;P2 is a process that behaves as P1 and then after P1 terminates, the process behaves as P2. For example (move -> SKIP; turn-> SKIP), is a process that moves, turns and then terminates.


There are other binary operators for composing processes in different shapes, such as concurrency, choice, interrupt. This provided a rich set of constructs for specifying complex behaviour of a system. Details of the CSP operators is available in these books \cire{R10, C10}. Automatic verifications with CSP is supported with a verification tool FDR \ref{}


%However the notations of CSP did not specify time, which means that the process can not specify timing and temporal specifications. This means that there is no possible way for expressing a specification of budget and deadline.  essential specifications for modelling cyber-physical systems.

%tock
tock-CSP builds on that with providing additional event tock for recording a progress of time \ref{}. Each event tock is a timeframe which indicates a passage of a single time unit. For example, move -> tock -> tock -> SKIP, is a process that moves and then after at least 2 time unit and then terminates. This enables specifying timing information between events. 

Support for automatic verification has been provided in the newer versions of the FDR, specifically FDR4, which provides a separate section, timed section, specifically designed for writing tock-CSP specifications.

tock-CSP retains the original structure of CSP which enable using the established tool of CSP, FDR for the verification of tock-CSP specifications. And utilises the existing works and theories and tools developed for CSP.  
%is supported in the automatic verification tool FDR. This is provided in a time-section of a CSP file. 



%We  provide a good foundation for the translation work, with providing BNF base on the tock-CSP extension \ref{JP19}. The BNF describes the selected operators we chose for this translation work.

%Based on this series we develop a translation techniques that translates tock-CSP into UPPAAL that enable using the facilities UPPAAL for the verification.

%Put the BNF here
BNF 





%Alur, Courcoubetis, and Dill’s seminal work on region graphs [ACD90,
ACD93] provided the first algorithm to model check (continuous-time) timed
graphs with respect to satisfiability of formulas expressed in the temporal
logic TCTL. Timed graphs consist of a finite set of nodes together with a
finite set of real-valued clocks, giving rise to an uncountable number of states.
However, Alur et al. showed that it was possible to construct an equivalence
relation on the state space, partitioning it into a finite number of regions,
in such a way that no TCTL formula can distinguish states belonging to
the same region. This led naturally to a model checking algorithm. The
technique is however computationally expensive—deciding satisfiability of
TCTL formulas by timed graphs can be shown to be PSPACE-complete—
and much subsequent research has concentrated on finding ways to curb the
resulting complexity [HNSY94, LL95, SS95, HKV96, HK97].


Brief about Timed Automata and  UPPAAL
% summary of UPPAAL section



In UPPAAL, systems are modelled as a network of TA, in which TA modelled a process. Mathematically, a TA is defined as a tuple $(L, l_0, C, A E, I)$, where L describes the set of possible locations, $l_0$  is the initial location, C is the set of clocks, A is the set of actions, E is the set of possible edges that connects the locations of the TA, which is defined as $E \subset L \times A \times B(C) \times 2^C \times L$.  This describes an edge from location L that is triggered by an action A associated with set of clocks B(C), which is a set of clocks that are reset on following the edge E to a location L  \ref{BD04, B12}.

  
The semantics of each TA is defined as a labelled transition system (LTS), which is a tuple $(S, s_0, \rightarrow)$, where $S  \subset L  \times R^C$, combination of location and an associated clocks value, $s_0$ is the initial state, transition $(\rightarrow)$ in the form of $S \times  A \times S$. There are two forms of transitions. A transition from a state to state over either time delay (t) or an action ($\sigma$) or combination of both.
% This defines the two possible transitions with action or delay.

%NOT CLEAR
% The operational semantics is defined as follows, given a $TA = (L, l_0, C, A, E, I)$ with a LTS as $(S, s_0, \rightarrow)$, the two possible transitions are

\paragraph{1. Delay transition}  is a transition from state to state over time delay.
\[  (l,u) \xrightarrow{\text{d}}  (l, u+d) \iff (\forall d : 0 \le d' \le d \implies u+d' \in I(l)  \]
%\item 
\paragraph{2. Action transition:} is a transition triggered by an action.
\[ (l, u)  \xrightarrow{ \text{a}}  (l', u') \iff  \exists  e = (l, a, g, r, l') \in E \]
\vspace{- 0.9cm}
\[  such \  that \ u \in g, \ u' =[r \rightarrow 0] u \ and \ also \ u' \in I(l) \]

% \begin{cmt}
% \textit{
% %The Z specification for the above transition is incomplete yet. The above mathematical expressions will be replaced with Z specification
% %After completing the Z specification, it will replace t
% The above mathematical expressions will be replace with Z specifications. At the moment the specifications are incomplete.}
% \end{cmt}
% \textit{Suggestion: They do not necessarily need to be replace with Z *specifications*, but they do need to be in Z syntax. In particular, consider the syntax of the quantified predicates. \\ \\
% I did not understand the above suggestion.}
% \vspace{0.3cm}

In UPPAAL, a TA performs an action over an edge, synchronously with the environment and possibly with some other TA. An action triggered a transition from one location to another or possibly return to the same location. A state of a system comprises the locations of all the network TA together with their associated clock values and value of the discrete variable. So performing an action changes the state of the whole system.  
  

%%%%%%%%%%  Example





Haskell
Here, we briefly introduce Haskell \cite{H16} as a functional programming language, which we use for expressing, implementing and evaluating the translation technique. We discuss both the style of functional programming approach and highlights some of the provided constructs of Haskell that will help in understanding the work.


% Why Haskell
We choose to use Haskell for 3 reasons.  First, the concise structure of Haskell helps us in providing a concise description of all the translation techniques in the form of translation rules, which is in an executable format that maintain consistency of the translation technique. Secondly, Haskell provides an easier way of representing an abstract syntax tree (AST)\cite{R12}, which plays a major role in providing a solid foundation of the translation work. Thirdly, in the future, the reasoning facilities in Haskell is another important features, which will enable us to reason about the translation rules.


%makes the translation rule to remain consistent with one another. Secondly, Haskell provides an easier way of representing an abstract syntax tree (AST)\cite{R12}. This plays a major role in the foundation of this translation work. Thirdly, the provision of reasoning facilities in Haskell is another important features, which will enable us to reason about the translation rules.



% Description of function
In a nutshell, in Haskell, computation is evaluation of expression and application of a function to its argument, which produces a result. A function has parameters and a body. The parameters describe the input of the function, while the body describes the evaluation of the input to get an output. Normally, a function has a name for identification. However, an anonymous function is also possible using $Lambda\ expression$. \footnote{ For example, \verb!\x -> x*x!, is an anonymous function that takes input $x$ and computes the square of the input number x.}  Also, both the argument and output can be a function, a concept known as higher-order functions.  This concept provides an interesting concept for composing a chain of function for expressing complex computation \cite{H89, H16}.

%Example 1
\begin{exl}  A simple Haskell program for computing a Fibonacci number.
\label{fib}
%todo: change to lstlisten
\begin{Verbatim}

1.   fibonacci :: Int -> Int
2.   fibonacci    0   =  0
3.   fibonacci    1   =  1
4.   fibonacci    n   =  fibonacci (n-1) + fibonacci (n-2)

\end{Verbatim}
\end{exl}


% Explanation of the example
Example  \ref{fib} demonstrates basic Haskell’s constructs, such as type, pattern matching, and recursive call.  Details of Example \ref{fib} is as follows. Line 1 specifies a type for the function. The function \lstinline{fibonacci} takes an argument of type integer and returns an output of type integer. Line 2 and 3 specify the base cases of the function. For the input values 0 and 1, the function returns the same input value 0 and 1 respectively. While for any other value the function returns the sum of two previous terms. This illustrates using the concept of pattern matching to determine the appropriate evaluation of each input. While Line 4 illustrates using recursive calls in evaluating the input. Altogether, this example illustrates a complete Haskell program, which is a function \lstinline{fibonacci}.


In summary, this section provides a brief background for understanding the work. The section briefly discusses the main components of the translation technique, which takes input tock-CSP and translates it into TA for UPPAAL. And also Haskell, which we used for developing the translation technique. In the next section we will discuss the details of the translation technique.



---------------------------------------------------------------------------------------------
%Each of the TA is used to model a process in the system.
%UPPAAL is an automatic verification tool for Automata. The tool is developed for modelling real-time system. 

%UPPAAL is a tool for modelling real-time systems. Systems are model as a parallel composition of timed automata (TA) that have an external clock.  The clock modelled the progress of time with a continuous time model, in which time progresses synchronously with the global clock. Time is quantified with a real number value.  Each of the TA is used to model a single process in the system.

%Verification with TA has been supported with an automatic tool, UPPAAL, which is developed for modelling and verification of RTS. In

%UPPAAL is an automatic verification tool for Automata. The tool is developed for modelling real-time system. 

%UPPAAL is a tool for modelling real-time systems. Systems are model as a parallel composition of timed automata (TA) that have an external clock.  The clock is modelled with a  continuous time model, in which time progresses synchronously with the global clock. Time is quantified with a real number value.  Each of the TA is used to model a single process in the system.







==> zz_del/mathProof.tex <==
% ????? "You should say that the proof technique is structural induction over the syntax of your fragment of Tock-CSP, and your example is of the simplest base case."

%ToReturn
% This is an overview of our initial proof of the translation rules. We plan to use structural induction over the constructs of the input \verb!tock-CSP!, within the scope of this translation work. 

Here, we illustrate an early part of the proof using a translation of the construct $STOP$, which is one of the base cases of the structural induction.

% Our plan is to use mathematical induction in proving the translation rules.
% One of the base case is the translation of the construct $STOP$. The proof of the base case is as follow.



% \vspace{0.3cm}
% From Section \ref{background}, Mathematically, a TA is tuple, 

% % \[ TA = (L, l_0, C, A, E, I)  \]
% \begin{equation} \label{ta}
%     TA = (L, l_0, C, A, E, I)
% \end{equation}

Consider \lstinline{TA1} as the left TA of Figure \ref{stop_ta1}; (from Section \ref{background})  mathematically TA1 is defined as the following tuple.

\vspace{-0.4cm}
\begin{multline}
    TA1 =   ( \{s0, s1\}, s0,  \{ck\}, \{startID00, tock\}, \\
    \{(s0, startID, \emptyset, \emptyset, s1), (s1, tock, ck\le1, ck, s1) \}, \{\} )
\end{multline}


% \[ TA1 =   ( \{s0, s1\}, \ s0, \  \{ck\},  \ \{startID, tock\}, \  \{(s0, startID, , , s1), (s1, ck, tock, ck\le1, s1) \}, \ \{\} ) \]


% According to Alur \cite{AD94} and Bouyer \cite{B11}, in


% ?? Check path and trace again ??

%------------------------------------
% \noindent
% In TA, a path \cite{AD94, B11} is a sequence of consecutive transitions that begins from the initial state. There is only one path in TA1, as follows. 

% \begin{equation}
%  path =  \{ \langle (s0, startID, \emptyset, \emptyset, s1), (s1, tock, ck\le1, ck, s1) \rangle   \}   
% \end{equation}

% \noindent
% Also, a trace \cite{AD94, B11} (or word in the language of TA) is a sequence of actions in a given path. Therefore, a trace of TA1 is as follows.
%------------------------------------



\noindent
A path \cite{AD94, B11} is a sequence of consecutive transitions that begins from the initial state. A trace \cite{AD94, B11} (or word in the language of TA) is a sequence of actions in a given path. There is only one path in TA1, and the traces on the path are as follows.

% Similarly, according to Alur \cite{AD94} and Bouyer \cite{B12}, a trace (or word in the language of TA) is a sequence of action in a given path.

\begin{equation}
traces'_{\lstinline{TA}}(TA1) =  \{  \langle \rangle,  \langle startID00 \rangle  \cat \langle tock \rangle^n  \} \ \ \ \ \ \ n = 0,1,2 \dots     
\end{equation}

\noindent
The function $trace'_{TA}(TA)$ describes the traces of TA1 as follow. The first empty sequence happens before taking any transition. The action \verb!startID00! happens on the second transition. The action \verb!tock! happens on the third transition, which is repeated infinitely to produce the infinite traces $\langle tock \rangle ^ n $.

% Thus, the function $traces'_{\lstinline{TA}}(TA)$ starts from the initial location \lstinline{(l0)} of the first TA in the list of input TA, and traverse the network of TA to return a list of associated actions of the transitions on the path.



% \[ traces_{TA}(TA) =  \{ [ \langle \rangle] ], \ [ \langle startID \rangle], \ [ \langle startID, tock^n \rangle]]  \} \]

% \noindent
% The function $traces'_{\lstinline{TA}}(TA)$ starts from the initial location \lstinline{(l0)} of the first TA in the list of input TA, and traverse the network of TA to return a list of associated actions of the transitions on the path.

%, as described in the definition of traces above.

% For example, let \lstinline{TA1} be the first TA in Figure \ref{stop_ta1} then
% \[ traceTA(TA1) =  \{ \langle startID, tock \rangle  \} \]


%ToReturn
% For example, in Figure \ref{stop_ta1}, starting from the left TA that has an initial location \lstinline{s0}, the first transition connects the two locations \lstinline{s0} and \lstinline{s1} with the action \lstinline{startID01}, and the trace becomes $ \{ \langle startID01 \rangle \}$. After that, the second transition from location \lstinline{s1} to itself \lstinline{s1} for the action \lstinline{tock}, and the trace becomes $ \{ \langle startID01, tock \rangle \}$. This second transition is repeated infinitely to create infinite series of the actions  $\lstinline{tock}^n$, and the trace becomes $ \{ \langle startID01,\ tock^n \rangle \}$.


Another function $trace_{TA}(TA)$ is similar to $traces'_{\lstinline{TA}}(TA)$ but removes all the coordinating actions (Definition \ref{coordinating_action}), which we use in this work.

\vspace{-0.3cm}
\begin{equation}
traces_{\lstinline{TA}}(TA1) =  traces'_{\lstinline{TA}}(TA1) \ \backslash  \ CoordinatingActions
\end{equation}

\noindent
So, the function $trace'_{TA}(TA)$ takes a list of TA and returns set of traces without the coordinating actions. For instance, without the coordinating actions the traces of TA1 becomes.

 \vspace{-0.3cm}
\begin{equation}
traces_{\lstinline{TA}}(TA1) =  \{  \langle tock \rangle ^n  \}    
\end{equation}


% \[ trace_{TA}(TA)  = traces(TA) \backslash CoordinatingActions   \]


% This sections discusses the mathematical proofs  to setup a path for proving total correctness of the translation technique, which we developed in this work. The mathematical proof will establish that the traces of tock-CSP are similar to the traces of the translated TA in the following steps.

% We plan to use Mathematical proof to establish that the traces of tock-CSP are similar to the traces of the translated TA in the following steps.

%We plan to use this mathematical proof to establish that  

\vspace{0.2cm}

% \noindent
% For this proof, our goal is establishing that the traces of \verb!tock-CSP! models are the same as those of the translated TA models.
%This is describe in the following steps.

% \vspace{-0.5cm}
% \begin{equation}
%  traces_{tock-CSP}( \lstinline{tock-CSP}) \equiv traces_{\lstinline{TA}}(transTA(\lstinline{tock-CSP}))    
% \end{equation} 

\noindent
\noindent
For this proof, our goal is establishing that the traces of \verb!tock-CSP! models are the same as those of the translated TA models. Here, \lstinline{transTA} is the translation function we have formalised (See Section \ref{trans_rule} ) for translating \verb!tock-CSP! models into TA models.  Thus, we need to establish that, for each valid \verb!tock-CSP! process \lstinline{P}, within the scope of this work

 \vspace{-0.1cm}
\begin{equation}
traces_{\lstinline{tock-CSP}}(P)  \equiv  traces_{\lstinline{TA}}(transTA(P)) 
\end{equation}

% \[ traces_{\lstinline{tock-CSP}}(P) == traces_{\lstinline{TA}}(transTA(P))   \]

\vspace{0.2cm}
% In this case, for each translation rule we need to proof that the translated TA captures the behaviour of the translated construct of the \verb!tock-CSP!. Thus, starting with Rule \ref{rule_STOP} for the construct of a constant process \lstinline{STOP}:

\noindent
In this case, for each translation rule we need to prove that the translated TA captures the behaviour of its translated construct from \verb!tock-CSP!. Thus, starting with the first rule for translating the construct of a basic process \lstinline{STOP}:

% In this case, we need to establish that, each construct of the tock-CSP has similar behaviour with the equivalent translated TA. This means that we have to use mathematical proof to establish the correctness of translating each construct, that is the list of the translation rules. Thus, starting with Rule \ref{rule_STOP} for the construct of a constant process \lstinline{STOP}:

% \vspace{-0.3cm} 

\begin{equation}
     traces_{\lstinline{tock-CSP}}(STOP) \equiv traces_{\lstinline{TA}}(transTA(STOP)) 
\end{equation}
% \[ traces_{\lstinline{tock-CSP}}(STOP) == traces_{\lstinline{TA}}(transTA(STOP))   \]


\vspace{0.3cm}
\noindent
For the LHS, in \verb!tock-CSP! \cite{R10}, the traces of the constant process \lstinline{STOP} are:
\begin{equation} \label{lhs}
  traces_{\lstinline{tock-CSP}}(STOP) = \{ \langle tock ^n \rangle \} 
 \end{equation}

% \begin{equation}
% traces_{\lstinline{tock-CSP}}(STOP) = \{\langle\rangle, \langle tock ^n \rangle \}     
% \end{equation}

% \[ traces_{\lstinline{tock-CSP}}(STOP) = \{\langle\rangle, \langle tock \rangle \}  \]

% \vspace{0.3cm}
% \noindent
% For the RHS, the traces of the translated TA are as follows.
% \[ traces_{\lstinline{TA}}(transTA(STOP))  \] 
%--------------------


\vspace{0.2cm}
\noindent
For the RHS, Example \ref{ex_STOP} produces a TA that captures the translation of construct $STOP$, then the traces of the TA are as follows.
% For the RHS, Example \ref{ex_STOP}, describes the translation of the construct $STOP$. Let TA1 be the first TA, which captures the translation of construct $STOP$, then the traces of TA1 are as follows.


\begin{equation}
traces'_{\lstinline{TA}}(TA1) =  \{ \langle \rangle, \ \langle startID00 \rangle \cat \langle tock \rangle ^n    \}    
\end{equation}
% \[ traceTA(TA1) =  \{ [<>], \ [<startID>], \ [<startID, tock>^n]]  \} \]


% \[ traces_{\lstinline{TA}} \{ \]

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.3\textwidth]{C4_figs/stopTrace.jpg}
%     % \caption{Caption}
%     % \label{fig:my_label}
% \end{figure}

% \Verb!                      } !


\vspace{0.2cm} 
\noindent
After dropping the flow actions, the traces become:
\vspace{-0.1cm}
\begin{equation} \label{rhs}
traces_{\lstinline{TA}}(TA1) =  \{ \langle tock \rangle^n \}    
\end{equation}

% \[  traceTA(TA1) =  \{ [\langle \rangle], [\langle tock \rangle ^n]]  \} \]



\vspace{0.2cm}
\noindent
Therefore, from Equations (\ref{lhs}) and (\ref{rhs}), 
\[ traces_{\lstinline{tock-CSP}}(STOP) \equiv traces_{\lstinline{TA}}(transTA(STOP))  \]
% \[ \ \ traces( \lstinline{tock-CSP}) == traces(transTA(\lstinline{tock-CSP}))  \]

% \[ That \ is \ \ \{ [\langle \rangle], [\langle tock \rangle ^n]] \} == \{ [\langle \rangle], [\langle tock \rangle^n] \}  \]


\noindent
This proves that the traces of the translated TA for $STOP$ captures its traces correctly. We plan to follow the same pattern in completing the proof.

% We plan to proof all the remaining rules to establish the correctness of the translation rules that will cover infinite traces.

% This proves that the traces of the translated TA for the construct STOP captures its traces. We plan to proof all the remaining rules to establish the correctness of the translation rules that will cover infinite traces.



==> zz_del/mathProof_.tex <==
This sections discusses the mathematical proofs  to setup a path for proving total correctness of the translation technique, which we developed in this work. The methematical proof will establish that the traces of tock-CSP are similar to the traces of the translated TA in the following steps.

\vspace{0.3cm}
We plan to use this mathematical proof to establish that  \vspace{-0.3cm}
\[ traces( \lstinline{tock-CSP}) == traces(transTA(\lstinline{tock-CSP}))  \]
Where, \lstinline{transTA} is the function we developed for translating tock-CSP models into TA models.

% So we need to established that 
So, for each valid tock-CSP process \lstinline{P}, within the scope of this work

\[ traces_{\lstinline{tock-CSP}}(P) == traces_{\lstinline{TA}}(transTA(P))   \]

We need to establish that, each construct of the tock-CSP has similar behaviour with the equivalent translation in TA. 

Starting with the construct of a constant process \lstinline{STOP}:

\[ traces_{\lstinline{tock-CSP}}(STOP) == traces_{\lstinline{TA}}(transTA(STOP))   \]

For the LHS, traces of the constant process \lstinline{STOP}
\[ traces_{\lstinline{tock-CSP}}(STOP) = \{<>, <tock>\}  \]

For the RHS, traces of the translated TA:
\[ traces_{\lstinline{TA}}(transTA(STOP)) =  \] 

\[ traces_{\lstinline{TA}} \{ \]

\begin{figure}[H]
    \centering
    \includegraphics[width=0.3\textwidth]{C4_figs/stopTrace.jpg}
    % \caption{Caption}
    % \label{fig:my_label}
\end{figure}

\Verb!                      } !


Mathematically, a TA is tuple, as discussed in Section \ref{ch02UppalTA}. 
\[ TA = (L, l_0, C, A, E, I)  \]


Therefore, the above TA is express in the following tuple.
\vspace{0.3cm}

 $transTA(STOP)$ = \vspace{-0.3cm}
 \[ ( \{s0, s1\}, \ s0, \  \{ck\},  \ \{startID, tock\}, \  \{(s0, startID, , , s1), (s1, ck, tock, ck\le1, s1) \}, \ \{\} ) \]


According to Alur \cite{AD94} and Bouyer \cite{B12}, in TA, a path is a sequence of consecutive transitions that begins from initial state. Therefore, the possible paths in the above TA are as follow. 
\[ paths =  \{ [<>], \ [<(s0, startID, , , s1)>], \ [<(s0, startID, , , s1),\ (s1, ck, tock, ck\le1, s1)>]   \} \]

% \[ \{ [<>], [<s0, s1, startID>], [<s0, s1, startID> <s1, s1, tock>^n ]  \}   \]


Similarly, according to Alur \cite{AD94} and Bouyer \cite{B12}, a trace (or word in the language of TA) is a sequence of action in a give path.

\[ trace =  \{ [<>], \ [<startID>], \ [<startID, tock>^n]]  \} \]
 
Dropping the added flow actions in the TA, the set of traces becomes:

\[  trace =  \{ [<>], [<tock>^n]]  \} \]


% Therefore, 
\[ Therefore, \ \ traces( \lstinline{tock-CSP}) == traces(transTA(\lstinline{tock-CSP}))  \]

\[ That \ is, \ \ \{ [<>], [<tock>^n]] \} == \{ [<>], [<tock>^n]] \}  \]

% \begin{align*}
%     transTA(STOP) &= ( \{s0, s1\}, s0, \{ck\},  \{startID, tock\} \\
%     &= 2\cdot(t^2+u^2) \\
%     4xyzw &= 2\cdot2tu \\
%     &\le 2\cdot(t^2+u^2) \\
%     &= 2\cdot((xy)^2+(zw)^2) &&\text{(substituting variables)} \\
%     &= 2\cdot(x^2y^2+z^2w^2) \\ 
%     &= 2x^2y^2+2z^2w^2 \\
%     &\le ((x^2)^2+(y^2)^2)+((z^2)^2)+(w^2)^2) \\
%     &= x^4+y^4+z^4+w^4  &&\qedhere
%   \end{align*}
